Upgrade the Retriever First: What an LLM Call per Chunk Buys in RAG

Many RAG pipelines pay one LLM call per chunk at indexing time to add titles, summaries, keywords and questions (enrichment) or document context (contextual retrieval, CR). We ask what that call buys over free structure and a better retriever. Our advice: upgrade the retriever first, chunk at headers, and enrich mainly for lexical retrieval. Under a plan made public before any index was built, 7B enrichment beats a free section-path prefix under a hybrid retriever by +5.5 recall points on Qasper; on FreshStack its gain (+2.7) does not survive Holm adjustment. It is equivalent to CR, which sends 5.8-8.7 times the input tokens, and Qasper answer F1 (7B reader) is equivalent for both contrasts. Header-led chunks beat 512-character windows; on FreshStack they lose to overlapping 256-token windows. Under qwen3-embedding and a reranker, the two strongest of eight retrievers (named as secondary before any outcome was computed), the CIs of 7B enrichment against the free prefix fall within the equivalence margins; under BM25 it gains +8.7. Exploratory analyses attribute the hybrid gain to document expansion and to repairing an untuned rank fusion; the free prefix under either strong retriever beats hybrid enrichment by +3.4 to +6.3 points, though the best 120B-indexed configuration leads the best free one by +2.5 on Qasper. Add-ons built on the call do no better than LLM-free controls, and late chunking lowers Qasper recall. We release the plan, harness and per-question results.

==> numbers.tex <==
% Generated by MDKeyChunker-eval/paper_numbers.py; do not edit by hand.
\makeatletter
\providecommand{\R}[1]{\@ifundefined{r@#1}{\textbf{??#1}}{\csname r@#1\endcsname}}
\expandafter\def\csname r@CRST-fs\endcsname{+1.0 [$-$0.8, +2.8]}
\expandafter\def\csname r@CRST-fs-ci\endcsname{[$-$0.8, +2.8]}
\expandafter\def\csname r@CRST-fs-ci95\endcsname{[$-$0.8, +2.8]}
\expandafter\def\csname r@CRST-fs-d\endcsname{+1.0}
\expandafter\def\csname r@CRST-fs-p\endcsname{--}
\expandafter\def\csname r@CRST-fs-v\endcsname{n.d.}
\expandafter\def\csname r@CRST-qasper\endcsname{+3.4 [+1.3, +5.6]}
\expandafter\def\csname r@CRST-qasper-ci\endcsname{[+1.3, +5.6]}
\expandafter\def\csname r@CRST-qasper-ci95\endcsname{[+1.3, +5.6]}
\expandafter\def\csname r@CRST-qasper-d\endcsname{+3.4}
\expandafter\def\csname r@CRST-qasper-p\endcsname{--}
\expandafter\def\csname r@CRST-qasper-v\endcsname{diff.}
\expandafter\def\csname r@EAX-E-fs\endcsname{+2.8 [+0.2, +5.5]}
\expandafter\def\csname r@EAX-E-fs-ci\endcsname{[+0.2, +5.5]}
\expandafter\def\csname r@EAX-E-fs-ci95\endcsname{[+0.2, +5.5]}
\expandafter\def\csname r@EAX-E-fs-d\endcsname{+2.8}
\expandafter\def\csname r@EAX-E-fs-p\endcsname{--}
\expandafter\def\csname r@EAX-E-fs-v\endcsname{diff.}
\expandafter\def\csname r@EAX-E-qasper\endcsname{$-$7.8 [$-$10.3, $-$5.3]}
\expandafter\def\csname r@EAX-E-qasper-ci\endcsname{[$-$10.3, $-$5.3]}
\expandafter\def\csname r@EAX-E-qasper-ci95\endcsname{[$-$10.3, $-$5.3]}
\expandafter\def\csname r@EAX-E-qasper-d\endcsname{$-$7.8}
\expandafter\def\csname r@EAX-E-qasper-p\endcsname{--}
\expandafter\def\csname r@EAX-E-qasper-v\endcsname{diff.}
\expandafter\def\csname r@EKX-ESX-fs\endcsname{+0.4 [$-$2.2, +3.1]}
\expandafter\def\csname r@EKX-ESX-fs-ci\endcsname{[$-$2.2, +3.1]}
\expandafter\def\csname r@EKX-ESX-fs-ci95\endcsname{[$-$2.2, +3.1]}
\expandafter\def\csname r@EKX-ESX-fs-d\endcsname{+0.4}
\expandafter\def\csname r@EKX-ESX-fs-p\endcsname{--}
\expandafter\def\csname r@EKX-ESX-fs-v\endcsname{n.d.}
\expandafter\def\csname r@EKX-ESX-qasper\endcsname{$-$6.2 [$-$8.4, $-$4.0]}
\expandafter\def\csname r@EKX-ESX-qasper-ci\endcsname{[$-$8.4, $-$4.0]}
\expandafter\def\csname r@EKX-ESX-qasper-ci95\endcsname{[$-$8.4, $-$4.0]}
\expandafter\def\csname r@EKX-ESX-qasper-d\endcsname{$-$6.2}
\expandafter\def\csname r@EKX-ESX-qasper-p\endcsname{--}
\expandafter\def\csname r@EKX-ESX-qasper-v\endcsname{diff.}
\expandafter\def\csname r@ESX-E-fs\endcsname{+0.8 [$-$0.6, +2.3]}
\expandafter\def\csname r@ESX-E-fs-ci\endcsname{[$-$0.6, +2.3]}
\expandafter\def\csname r@ESX-E-fs-ci95\endcsname{[$-$0.6, +2.3]}
\expandafter\def\csname r@ESX-E-fs-d\endcsname{+0.8}
\expandafter\def\csname r@ESX-E-fs-p\endcsname{--}
\expandafter\def\csname r@ESX-E-fs-v\endcsname{n.d.}
\expandafter\def\csname r@ESX-E-qasper\endcsname{$-$3.8 [$-$5.8, $-$2.0]}
\expandafter\def\csname r@ESX-E-qasper-ci\endcsname{[$-$5.8, $-$2.0]}
\expandafter\def\csname r@ESX-E-qasper-ci95\endcsname{[$-$5.8, $-$2.0]}
\expandafter\def\csname r@ESX-E-qasper-d\endcsname{$-$3.8}
\expandafter\def\csname r@ESX-E-qasper-p\endcsname{--}
\expandafter\def\csname r@ESX-E-qasper-v\endcsname{diff.}
\expandafter\def\csname r@Emetakey-E-fs\endcsname{$-$0.4 [$-$1.1, +0.2]}
\expandafter\def\csname r@Emetakey-E-fs-ci\endcsname{[$-$1.1, +0.2]}
\expandafter\def\csname r@Emetakey-E-fs-ci95\endcsname{[$-$1.1, +0.2]}
\expandafter\def\csname r@Emetakey-E-fs-d\endcsname{$-$0.4}
\expandafter\def\csname r@Emetakey-E-fs-p\endcsname{--}
\expandafter\def\csname r@Emetakey-E-fs-v\endcsname{n.d.}
\expandafter\def\csname r@Emetakey-E-qasper\endcsname{+0.0 [$-$0.9, +1.0]}
\expandafter\def\csname r@Emetakey-E-qasper-ci\endcsname{[$-$0.9, +1.0]}
\expandafter\def\csname r@Emetakey-E-qasper-ci95\endcsname{[$-$0.9, +1.0]}
\expandafter\def\csname r@Emetakey-E-qasper-d\endcsname{+0.0}
\expandafter\def\csname r@Emetakey-E-qasper-p\endcsname{--}
\expandafter\def\csname r@Emetakey-E-qasper-v\endcsname{n.d.}
\expandafter\def\csname r@EsE-fs\endcsname{$-$1.0 [$-$2.9, +0.9]}
\expandafter\def\csname r@EsE-fs-ci\endcsname{[$-$2.9, +0.9]}
\expandafter\def\csname r@EsE-fs-ci95\endcsname{[$-$2.9, +0.9]}
\expandafter\def\csname r@EsE-fs-d\endcsname{$-$1.0}
\expandafter\def\csname r@EsE-fs-p\endcsname{--}
\expandafter\def\csname r@EsE-fs-v\endcsname{n.d.}
\expandafter\def\csname r@EsE-qasper\endcsname{+1.2 [$-$1.3, +3.7]}
\expandafter\def\csname r@EsE-qasper-ci\endcsname{[$-$1.3, +3.7]}
\expandafter\def\csname r@EsE-qasper-ci95\endcsname{[$-$1.3, +3.7]}
\expandafter\def\csname r@EsE-qasper-d\endcsname{+1.2}
\expandafter\def\csname r@EsE-qasper-p\endcsname{--}
\expandafter\def\csname r@EsE-qasper-v\endcsname{n.d.}
\expandafter\def\csname r@F1-H1\endcsname{+1.4 [$-$0.3, +2.9]}
\expandafter\def\csname r@F1-H1-ci\endcsname{[$-$0.3, +2.9]}
\expandafter\def\csname r@F1-H1-ci95\endcsname{[$-$0.6, +3.2]}
\expandafter\def\csname r@F1-H1-d\endcsname{+1.4}
\expandafter\def\csname r@F1-H1-p\endcsname{0.001}
\expandafter\def\csname r@F1-H1-pperm\endcsname{0.637}
\expandafter\def\csname r@F1-H1-v\endcsname{equiv.}
\expandafter\def\csname r@F1-H1s\endcsname{+1.4 [$-$0.7, +3.6]}
\expandafter\def\csname r@F1-H1s-ci\endcsname{[$-$0.7, +3.6]}
\expandafter\def\csname r@F1-H1s-ci95\endcsname{[$-$0.7, +3.6]}
\expandafter\def\csname r@F1-H1s-d\endcsname{+1.4}
\expandafter\def\csname r@F1-H1s-p\endcsname{--}
\expandafter\def\csname r@F1-H1s-v\endcsname{n.d.}
\expandafter\def\csname r@F1-H2\endcsname{+0.2 [$-$1.4, +1.9]}
\expandafter\def\csname r@F1-H2-ci\endcsname{[$-$1.4, +1.9]}
\expandafter\def\csname r@F1-H2-ci95\endcsname{[$-$1.7, +2.2]}
\expandafter\def\csname r@F1-H2-d\endcsname{+0.2}
\expandafter\def\csname r@F1-H2-p\endcsname{0.001}
\expandafter\def\csname r@F1-H2-pperm\endcsname{0.818}
\expandafter\def\csname r@F1-H2-v\endcsname{equiv.}
\expandafter\def\csname r@F1-H2s\endcsname{+0.0 [$-$1.9, +2.1]}
\expandafter\def\csname r@F1-H2s-ci\endcsname{[$-$1.9, +2.1]}
\expandafter\def\csname r@F1-H2s-ci95\endcsname{[$-$1.9, +2.1]}
\expandafter\def\csname r@F1-H2s-d\endcsname{+0.0}
\expandafter\def\csname r@F1-H2s-p\endcsname{--}
\expandafter\def\csname r@F1-H2s-v\endcsname{n.d.}
\expandafter\def\csname r@H1-angular\endcsname{+2.6 [$-$0.7, +6.3]}
\expandafter\def\csname r@H1-angular-ci\endcsname{[$-$0.7, +6.3]}
\expandafter\def\csname r@H1-angular-ci95\endcsname{[$-$0.7, +6.3]}
\expandafter\def\csname r@H1-angular-d\endcsname{+2.6}
\expandafter\def\csname r@H1-angular-p\endcsname{--}
\expandafter\def\csname r@H1-angular-v\endcsname{incon.}
\expandafter\def\csname r@H1-fs-bm25\endcsname{+2.4}
\expandafter\def\csname r@H1-fs-bm25ci\endcsname{[+0.9, +4.3]}
\expandafter\def\csname r@H1-fs-hyb\endcsname{+2.7 [+0.9, +4.7]}
\expandafter\def\csname r@H1-fs-hyb-ci\endcsname{[+0.9, +4.7]}
\expandafter\def\csname r@H1-fs-hyb-ci95\endcsname{[+0.5, +5.1]}
\expandafter\def\csname r@H1-fs-hyb-d\endcsname{+2.7}
\expandafter\def\csname r@H1-fs-hyb-p\endcsname{0.289}
\expandafter\def\csname r@H1-fs-hyb-pperm\endcsname{0.057}
\expandafter\def\csname r@H1-fs-hyb-v\endcsname{diff.}
\expandafter\def\csname r@H1-fs-mxbai\endcsname{+0.0 [$-$2.3, +2.3]}
\expandafter\def\csname r@H1-fs-mxbai-ci\endcsname{[$-$2.3, +2.3]}
\expandafter\def\csname r@H1-fs-mxbai-ci95\endcsname{[$-$2.3, +2.3]}
\expandafter\def\csname r@H1-fs-mxbai-d\endcsname{+0.0}
\expandafter\def\csname r@H1-fs-mxbai-p\endcsname{--}
\expandafter\def\csname r@H1-fs-mxbai-v\endcsname{equiv.}
\expandafter\def\csname r@H1-fs-nomic\endcsname{+2.6 [+0.3, +5.0]}
\expandafter\def\csname r@H1-fs-nomic-ci\endcsname{[+0.3, +5.0]}
\expandafter\def\csname r@H1-fs-nomic-ci95\endcsname{[+0.3, +5.0]}
\expandafter\def\csname r@H1-fs-nomic-d\endcsname{+2.6}
\expandafter\def\csname r@H1-fs-nomic-p\endcsname{--}
\expandafter\def\csname r@H1-fs-nomic-v\endcsname{diff.}
\expandafter\def\csname r@H1-laravel\endcsname{+4.6 [+1.7, +8.1]}
\expandafter\def\csname r@H1-laravel-ci\endcsname{[+1.7, +8.1]}
\expandafter\def\csname r@H1-laravel-ci95\endcsname{[+1.7, +8.1]}
\expandafter\def\csname r@H1-laravel-d\endcsname{+4.6}
\expandafter\def\csname r@H1-laravel-p\endcsname{--}
\expandafter\def\csname r@H1-laravel-v\endcsname{diff.}
\expandafter\def\csname r@H1-qasper-bm25\endcsname{+8.7}
\expandafter\def\csname r@H1-qasper-bm25ci\endcsname{[+6.6, +10.8]}
\expandafter\def\csname r@H1-qasper-hyb\endcsname{+5.5 [+3.3, +7.7]}
\expandafter\def\csname r@H1-qasper-hyb-ci\endcsname{[+3.3, +7.7]}
\expandafter\def\csname r@H1-qasper-hyb-ci95\endcsname{[+2.9, +8.1]}
\expandafter\def\csname r@H1-qasper-hyb-d\endcsname{+5.5}
\expandafter\def\csname r@H1-qasper-hyb-p\endcsname{0.639}
\expandafter\def\csname r@H1-qasper-hyb-pperm\endcsname{0.000}
\expandafter\def\csname r@H1-qasper-hyb-v\endcsname{diff.}
\expandafter\def\csname r@H1-qasper-mxbai\endcsname{+0.7 [$-$1.8, +3.3]}
\expandafter\def\csname r@H1-qasper-mxbai-ci\endcsname{[$-$1.8, +3.3]}
\expandafter\def\csname r@H1-qasper-mxbai-ci95\endcsname{[$-$1.8, +3.3]}
\expandafter\def\csname r@H1-qasper-mxbai-d\endcsname{+0.7}
\expandafter\def\csname r@H1-qasper-mxbai-p\endcsname{--}
\expandafter\def\csname r@H1-qasper-mxbai-v\endcsname{equiv.}
\expandafter\def\csname r@H1-qasper-nomic\endcsname{+0.9 [$-$1.7, +3.3]}
\expandafter\def\csname r@H1-qasper-nomic-ci\endcsname{[$-$1.7, +3.3]}
\expandafter\def\csname r@H1-qasper-nomic-ci95\endcsname{[$-$1.7, +3.3]}
\expandafter\def\csname r@H1-qasper-nomic-d\endcsname{+0.9}
\expandafter\def\csname r@H1-qasper-nomic-p\endcsname{--}
\expandafter\def\csname r@H1-qasper-nomic-v\endcsname{equiv.}
\expandafter\def\csname r@H1-yolo\endcsname{$-$0.7 [$-$7.0, +5.3]}
\expandafter\def\csname r@H1-yolo-ci\endcsname{[$-$7.0, +5.3]}
\expandafter\def\csname r@H1-yolo-ci95\endcsname{[$-$7.0, +5.3]}
\expandafter\def\csname r@H1-yolo-d\endcsname{$-$0.7}
\expandafter\def\csname r@H1-yolo-p\endcsname{--}
\expandafter\def\csname r@H1-yolo-v\endcsname{incon.}
\expandafter\def\csname r@H1s-fs-bm25\endcsname{+2.1}
\expandafter\def\csname r@H1s-fs-bm25ci\endcsname{[+0.2, +4.1]}
\expandafter\def\csname r@H1s-fs-hyb\endcsname{+1.8 [$-$0.3, +3.9]}
\expandafter\def\csname r@H1s-fs-hyb-ci\endcsname{[$-$0.3, +3.9]}
\expandafter\def\csname r@H1s-fs-hyb-ci95\endcsname{[$-$0.7, +4.3]}
\expandafter\def\csname r@H1s-fs-hyb-d\endcsname{+1.8}
\expandafter\def\csname r@H1s-fs-hyb-p\endcsname{0.081}
\expandafter\def\csname r@H1s-fs-hyb-pperm\endcsname{0.637}
\expandafter\def\csname r@H1s-fs-hyb-v\endcsname{incon.}
\expandafter\def\csname r@H1s-fs-mxbai\endcsname{$-$0.7 [$-$3.1, +1.6]}
\expandafter\def\csname r@H1s-fs-mxbai-ci\endcsname{[$-$3.1, +1.6]}
\expandafter\def\csname r@H1s-fs-mxbai-ci95\endcsname{[$-$3.1, +1.6]}
\expandafter\def\csname r@H1s-fs-mxbai-d\endcsname{$-$0.7}
\expandafter\def\csname r@H1s-fs-mxbai-p\endcsname{--}
\expandafter\def\csname r@H1s-fs-mxbai-v\endcsname{equiv.}
\expandafter\def\csname r@H1s-fs-nomic\endcsname{+2.2 [$-$0.3, +4.7]}
\expandafter\def\csname r@H1s-fs-nomic-ci\endcsname{[$-$0.3, +4.7]}
\expandafter\def\csname r@H1s-fs-nomic-ci95\endcsname{[$-$0.3, +4.7]}
\expandafter\def\csname r@H1s-fs-nomic-d\endcsname{+2.2}
\expandafter\def\csname r@H1s-fs-nomic-p\endcsname{--}
\expandafter\def\csname r@H1s-fs-nomic-v\endcsname{incon.}
\expandafter\def\csname r@H1s-qasper-bm25\endcsname{+10.0}
\expandafter\def\csname r@H1s-qasper-bm25ci\endcsname{[+7.6, +12.7]}
\expandafter\def\csname r@H1s-qasper-hyb\endcsname{+6.7 [+4.3, +9.0]}
\expandafter\def\csname r@H1s-qasper-hyb-ci\endcsname{[+4.3, +9.0]}
\expandafter\def\csname r@H1s-qasper-hyb-ci95\endcsname{[+3.9, +9.5]}
\expandafter\def\csname r@H1s-qasper-hyb-d\endcsname{+6.7}
\expandafter\def\csname r@H1s-qasper-hyb-p\endcsname{0.878}
\expandafter\def\csname r@H1s-qasper-hyb-pperm\endcsname{0.000}
\expandafter\def\csname r@H1s-qasper-hyb-v\endcsname{diff.}
\expandafter\def\csname r@H1s-qasper-mxbai\endcsname{+2.2 [$-$0.3, +4.7]}
\expandafter\def\csname r@H1s-qasper-mxbai-ci\endcsname{[$-$0.3, +4.7]}
\expandafter\def\csname r@H1s-qasper-mxbai-ci95\endcsname{[$-$0.3, +4.7]}
\expandafter\def\csname r@H1s-qasper-mxbai-d\endcsname{+2.2}
\expandafter\def\csname r@H1s-qasper-mxbai-p\endcsname{--}
\expandafter\def\csname r@H1s-qasper-mxbai-v\endcsname{equiv.}
\expandafter\def\csname r@H1s-qasper-nomic\endcsname{+3.6 [+1.0, +6.1]}
\expandafter\def\csname r@H1s-qasper-nomic-ci\endcsname{[+1.0, +6.1]}
\expandafter\def\csname r@H1s-qasper-nomic-ci95\endcsname{[+1.0, +6.1]}
\expandafter\def\csname r@H1s-qasper-nomic-d\endcsname{+3.6}
\expandafter\def\csname r@H1s-qasper-nomic-p\endcsname{--}
\expandafter\def\csname r@H1s-qasper-nomic-v\endcsname{diff.}
\expandafter\def\csname r@H2-angular\endcsname{+0.5 [$-$2.7, +3.6]}
\expandafter\def\csname r@H2-angular-ci\endcsname{[$-$2.7, +3.6]}
\expandafter\def\csname r@H2-angular-ci95\endcsname{[$-$2.7, +3.6]}
\expandafter\def\csname r@H2-angular-d\endcsname{+0.5}
\expandafter\def\csname r@H2-angular-p\endcsname{--}
\expandafter\def\csname r@H2-angular-v\endcsname{equiv.}
\expandafter\def\csname r@H2-fs-bm25\endcsname{+2.1}
\expandafter\def\csname r@H2-fs-bm25ci\endcsname{[+0.5, +3.9]}
\expandafter\def\csname r@H2-fs-hyb\endcsname{+1.8 [+0.2, +3.4]}
\expandafter\def\csname r@H2-fs-hyb-ci\endcsname{[+0.2, +3.4]}
\expandafter\def\csname r@H2-fs-hyb-ci95\endcsname{[$-$0.1, +3.7]}
\expandafter\def\csname r@H2-fs-hyb-d\endcsname{+1.8}
\expandafter\def\csname r@H2-fs-hyb-p\endcsname{0.033}
\expandafter\def\csname r@H2-fs-hyb-pperm\endcsname{0.142}
\expandafter\def\csname r@H2-fs-hyb-v\endcsname{equiv.}
\expandafter\def\csname r@H2-fs-mxbai\endcsname{+0.6 [$-$1.5, +2.6]}
\expandafter\def\csname r@H2-fs-mxbai-ci\endcsname{[$-$1.5, +2.6]}
\expandafter\def\csname r@H2-fs-mxbai-ci95\endcsname{[$-$1.5, +2.6]}
\expandafter\def\csname r@H2-fs-mxbai-d\endcsname{+0.6}
\expandafter\def\csname r@H2-fs-mxbai-p\endcsname{--}
\expandafter\def\csname r@H2-fs-mxbai-v\endcsname{equiv.}
\expandafter\def\csname r@H2-fs-nomic\endcsname{+2.2 [+0.3, +4.3]}
\expandafter\def\csname r@H2-fs-nomic-ci\endcsname{[+0.3, +4.3]}
\expandafter\def\csname r@H2-fs-nomic-ci95\endcsname{[+0.3, +4.3]}
\expandafter\def\csname r@H2-fs-nomic-d\endcsname{+2.2}
\expandafter\def\csname r@H2-fs-nomic-p\endcsname{--}
\expandafter\def\csname r@H2-fs-nomic-v\endcsname{diff., equiv.}
\expandafter\def\csname r@H2-laravel\endcsname{+2.5 [+0.2, +5.2]}
\expandafter\def\csname r@H2-laravel-ci\endcsname{[+0.2, +5.2]}
\expandafter\def\csname r@H2-laravel-ci95\endcsname{[+0.2, +5.2]}
\expandafter\def\csname r@H2-laravel-d\endcsname{+2.5}
\expandafter\def\csname r@H2-laravel-p\endcsname{--}
\expandafter\def\csname r@H2-laravel-v\endcsname{diff.}
\expandafter\def\csname r@H2-qasper-bm25\endcsname{+5.0}
\expandafter\def\csname r@H2-qasper-bm25ci\endcsname{[+2.7, +7.4]}
\expandafter\def\csname r@H2-qasper-hyb\endcsname{+2.1 [+0.1, +4.0]}
\expandafter\def\csname r@H2-qasper-hyb-ci\endcsname{[+0.1, +4.0]}
\expandafter\def\csname r@H2-qasper-hyb-ci95\endcsname{[$-$0.3, +4.4]}
\expandafter\def\csname r@H2-qasper-hyb-d\endcsname{+2.1}
\expandafter\def\csname r@H2-qasper-hyb-p\endcsname{0.033}
\expandafter\def\csname r@H2-qasper-hyb-pperm\endcsname{0.142}
\expandafter\def\csname r@H2-qasper-hyb-v\endcsname{equiv.}
\expandafter\def\csname r@H2-qasper-mxbai\endcsname{+1.5 [$-$1.0, +4.0]}
\expandafter\def\csname r@H2-qasper-mxbai-ci\endcsname{[$-$1.0, +4.0]}
\expandafter\def\csname r@H2-qasper-mxbai-ci95\endcsname{[$-$1.0, +4.0]}
\expandafter\def\csname r@H2-qasper-mxbai-d\endcsname{+1.5}
\expandafter\def\csname r@H2-qasper-mxbai-p\endcsname{--}
\expandafter\def\csname r@H2-qasper-mxbai-v\endcsname{equiv.}
\expandafter\def\csname r@H2-qasper-nomic\endcsname{$-$1.2 [$-$3.7, +1.2]}
\expandafter\def\csname r@H2-qasper-nomic-ci\endcsname{[$-$3.7, +1.2]}
\expandafter\def\csname r@H2-qasper-nomic-ci95\endcsname{[$-$3.7, +1.2]}
\expandafter\def\csname r@H2-qasper-nomic-d\endcsname{$-$1.2}
\expandafter\def\csname r@H2-qasper-nomic-p\endcsname{--}
\expandafter\def\csname r@H2-qasper-nomic-v\endcsname{equiv.}
\expandafter\def\csname r@H2-yolo\endcsname{+2.8 [$-$1.9, +7.9]}
\expandafter\def\csname r@H2-yolo-ci\endcsname{[$-$1.9, +7.9]}
\expandafter\def\csname r@H2-yolo-ci95\endcsname{[$-$1.9, +7.9]}
\expandafter\def\csname r@H2-yolo-d\endcsname{+2.8}
\expandafter\def\csname r@H2-yolo-p\endcsname{--}
\expandafter\def\csname r@H2-yolo-v\endcsname{incon.}
\expandafter\def\csname r@H2s-fs-bm25\endcsname{--}
\expandafter\def\csname r@H2s-fs-hyb\endcsname{--}
\expandafter\def\csname r@H2s-fs-hyb-ci\endcsname{--}
\expandafter\def\csname r@H2s-fs-hyb-d\endcsname{--}
\expandafter\def\csname r@H2s-fs-hyb-p\endcsname{--}
\expandafter\def\csname r@H2s-fs-hyb-v\endcsname{--}
\expandafter\def\csname r@H2s-fs-mxbai\endcsname{--}
\expandafter\def\csname r@H2s-fs-mxbai-ci\endcsname{--}
\expandafter\def\csname r@H2s-fs-mxbai-d\endcsname{--}
\expandafter\def\csname r@H2s-fs-mxbai-p\endcsname{--}
\expandafter\def\csname r@H2s-fs-mxbai-v\endcsname{--}
\expandafter\def\csname r@H2s-fs-nomic\endcsname{--}
\expandafter\def\csname r@H2s-fs-nomic-ci\endcsname{--}
\expandafter\def\csname r@H2s-fs-nomic-d\endcsname{--}
\expandafter\def\csname r@H2s-fs-nomic-p\endcsname{--}
\expandafter\def\csname r@H2s-fs-nomic-v\endcsname{--}
\expandafter\def\csname r@H2s-qasper-bm25\endcsname{+6.2}
\expandafter\def\csname r@H2s-qasper-bm25ci\endcsname{[+3.7, +8.7]}
\expandafter\def\csname r@H2s-qasper-hyb\endcsname{+1.6 [$-$0.7, +3.8]}
\expandafter\def\csname r@H2s-qasper-hyb-ci\endcsname{[$-$0.7, +3.8]}
\expandafter\def\csname r@H2s-qasper-hyb-ci95\endcsname{[$-$1.1, +4.2]}
\expandafter\def\csname r@H2s-qasper-hyb-d\endcsname{+1.6}
\expandafter\def\csname r@H2s-qasper-hyb-p\endcsname{0.017}
\expandafter\def\csname r@H2s-qasper-hyb-pperm\endcsname{0.637}
\expandafter\def\csname r@H2s-qasper-hyb-v\endcsname{equiv.}
\expandafter\def\csname r@H2s-qasper-mxbai\endcsname{+3.7 [+1.0, +6.2]}
\expandafter\def\csname r@H2s-qasper-mxbai-ci\endcsname{[+1.0, +6.2]}
\expandafter\def\csname r@H2s-qasper-mxbai-ci95\endcsname{[+1.0, +6.2]}
\expandafter\def\csname r@H2s-qasper-mxbai-d\endcsname{+3.7}
\expandafter\def\csname r@H2s-qasper-mxbai-p\endcsname{--}
\expandafter\def\csname r@H2s-qasper-mxbai-v\endcsname{diff.}
\expandafter\def\csname r@H2s-qasper-nomic\endcsname{+0.2 [$-$2.3, +2.6]}
\expandafter\def\csname r@H2s-qasper-nomic-ci\endcsname{[$-$2.3, +2.6]}
\expandafter\def\csname r@H2s-qasper-nomic-ci95\endcsname{[$-$2.3, +2.6]}
\expandafter\def\csname r@H2s-qasper-nomic-d\endcsname{+0.2}
\expandafter\def\csname r@H2s-qasper-nomic-p\endcsname{--}
\expandafter\def\csname r@H2s-qasper-nomic-v\endcsname{equiv.}
\expandafter\def\csname r@H3a-fs-bm25\endcsname{+3.2}
\expandafter\def\csname r@H3a-fs-bm25ci\endcsname{[+1.3, +5.4]}
\expandafter\def\csname r@H3a-fs-hyb\endcsname{+3.1 [+0.9, +5.5]}
\expandafter\def\csname r@H3a-fs-hyb-ci\endcsname{[+0.9, +5.5]}
\expandafter\def\csname r@H3a-fs-hyb-ci95\endcsname{[+0.9, +5.5]}
\expandafter\def\csname r@H3a-fs-hyb-d\endcsname{+3.1}
\expandafter\def\csname r@H3a-fs-hyb-p\endcsname{0.024}
\expandafter\def\csname r@H3a-fs-hyb-pperm\endcsname{0.024}
\expandafter\def\csname r@H3a-fs-hyb-v\endcsname{diff.}
\expandafter\def\csname r@H3a-fs-mxbai\endcsname{+3.1 [+1.0, +5.3]}
\expandafter\def\csname r@H3a-fs-mxbai-ci\endcsname{[+1.0, +5.3]}
\expandafter\def\csname r@H3a-fs-mxbai-ci95\endcsname{[+1.0, +5.3]}
\expandafter\def\csname r@H3a-fs-mxbai-d\endcsname{+3.1}
\expandafter\def\csname r@H3a-fs-mxbai-p\endcsname{--}
\expandafter\def\csname r@H3a-fs-mxbai-v\endcsname{diff.}
\expandafter\def\csname r@H3a-fs-nomic\endcsname{+1.8 [+0.0, +3.8]}
\expandafter\def\csname r@H3a-fs-nomic-ci\endcsname{[+0.0, +3.8]}
\expandafter\def\csname r@H3a-fs-nomic-ci95\endcsname{[+0.0, +3.8]}
\expandafter\def\csname r@H3a-fs-nomic-d\endcsname{+1.8}
\expandafter\def\csname r@H3a-fs-nomic-p\endcsname{--}
\expandafter\def\csname r@H3a-fs-nomic-v\endcsname{diff.}
\expandafter\def\csname r@H3a-qasper-bm25\endcsname{+3.0}
\expandafter\def\csname r@H3a-qasper-bm25ci\endcsname{[+0.5, +5.4]}
\expandafter\def\csname r@H3a-qasper-hyb\endcsname{+7.5 [+4.8, +10.1]}
\expandafter\def\csname r@H3a-qasper-hyb-ci\endcsname{[+4.8, +10.1]}
\expandafter\def\csname r@H3a-qasper-hyb-ci95\endcsname{[+4.8, +10.1]}
\expandafter\def\csname r@H3a-qasper-hyb-d\endcsname{+7.5}
\expandafter\def\csname r@H3a-qasper-hyb-p\endcsname{0.000}
\expandafter\def\csname r@H3a-qasper-hyb-pperm\endcsname{0.000}
\expandafter\def\csname r@H3a-qasper-hyb-v\endcsname{diff.}
\expandafter\def\csname r@H3a-qasper-mxbai\endcsname{+8.0 [+5.2, +10.7]}
\expandafter\def\csname r@H3a-qasper-mxbai-ci\endcsname{[+5.2, +10.7]}
\expandafter\def\csname r@H3a-qasper-mxbai-ci95\endcsname{[+5.2, +10.7]}
\expandafter\def\csname r@H3a-qasper-mxbai-d\endcsname{+8.0}
\expandafter\def\csname r@H3a-qasper-mxbai-p\endcsname{--}
\expandafter\def\csname r@H3a-qasper-mxbai-v\endcsname{diff.}
\expandafter\def\csname r@H3a-qasper-nomic\endcsname{+9.8 [+7.2, +12.5]}
\expandafter\def\csname r@H3a-qasper-nomic-ci\endcsname{[+7.2, +12.5]}
\expandafter\def\csname r@H3a-qasper-nomic-ci95\endcsname{[+7.2, +12.5]}
\expandafter\def\csname r@H3a-qasper-nomic-d\endcsname{+9.8}
\expandafter\def\csname r@H3a-qasper-nomic-p\endcsname{--}
\expandafter\def\csname r@H3a-qasper-nomic-v\endcsname{diff.}
\expandafter\def\csname r@H3b-angular\endcsname{$-$2.9 [$-$6.6, +0.5]}
\expandafter\def\csname r@H3b-angular-ci\endcsname{[$-$6.6, +0.5]}
\expandafter\def\csname r@H3b-angular-ci95\endcsname{[$-$6.6, +0.5]}
\expandafter\def\csname r@H3b-angular-d\endcsname{$-$2.9}
\expandafter\def\csname r@H3b-angular-p\endcsname{--}
\expandafter\def\csname r@H3b-angular-v\endcsname{n.d.}
\expandafter\def\csname r@H3b-fs-bm25\endcsname{$-$1.8}
\expandafter\def\csname r@H3b-fs-bm25ci\endcsname{[$-$4.1, +0.5]}
\expandafter\def\csname r@H3b-fs-hyb\endcsname{$-$2.9 [$-$5.4, $-$0.3]}
\expandafter\def\csname r@H3b-fs-hyb-ci\endcsname{[$-$5.4, $-$0.3]}
\expandafter\def\csname r@H3b-fs-hyb-ci95\endcsname{[$-$5.4, $-$0.3]}
\expandafter\def\csname r@H3b-fs-hyb-d\endcsname{$-$2.9}
\expandafter\def\csname r@H3b-fs-hyb-p\endcsname{0.028}
\expandafter\def\csname r@H3b-fs-hyb-pperm\endcsname{0.028}
\expandafter\def\csname r@H3b-fs-hyb-v\endcsname{diff.}
\expandafter\def\csname r@H3b-fs-mxbai\endcsname{$-$0.5 [$-$3.1, +2.0]}
\expandafter\def\csname r@H3b-fs-mxbai-ci\endcsname{[$-$3.1, +2.0]}
\expandafter\def\csname r@H3b-fs-mxbai-ci95\endcsname{[$-$3.1, +2.0]}
\expandafter\def\csname r@H3b-fs-mxbai-d\endcsname{$-$0.5}
\expandafter\def\csname r@H3b-fs-mxbai-p\endcsname{--}
\expandafter\def\csname r@H3b-fs-mxbai-v\endcsname{n.d.}
\expandafter\def\csname r@H3b-fs-nomic\endcsname{$-$3.5 [$-$5.9, $-$1.2]}
\expandafter\def\csname r@H3b-fs-nomic-ci\endcsname{[$-$5.9, $-$1.2]}
\expandafter\def\csname r@H3b-fs-nomic-ci95\endcsname{[$-$5.9, $-$1.2]}
\expandafter\def\csname r@H3b-fs-nomic-d\endcsname{$-$3.5}
\expandafter\def\csname r@H3b-fs-nomic-p\endcsname{--}
\expandafter\def\csname r@H3b-fs-nomic-v\endcsname{diff.}
\expandafter\def\csname r@H3b-laravel\endcsname{$-$2.7 [$-$6.7, +1.0]}
\expandafter\def\csname r@H3b-laravel-ci\endcsname{[$-$6.7, +1.0]}
\expandafter\def\csname r@H3b-laravel-ci95\endcsname{[$-$6.7, +1.0]}
\expandafter\def\csname r@H3b-laravel-d\endcsname{$-$2.7}
\expandafter\def\csname r@H3b-laravel-p\endcsname{--}
\expandafter\def\csname r@H3b-laravel-v\endcsname{n.d.}
\expandafter\def\csname r@H3b-qasper-bm25\endcsname{+5.7}
\expandafter\def\csname r@H3b-qasper-bm25ci\endcsname{[+3.5, +7.8]}
\expandafter\def\csname r@H3b-qasper-hyb\endcsname{+7.5 [+5.0, +10.1]}
\expandafter\def\csname r@H3b-qasper-hyb-ci\endcsname{[+5.0, +10.1]}
\expandafter\def\csname r@H3b-qasper-hyb-ci95\endcsname{[+5.0, +10.1]}
\expandafter\def\csname r@H3b-qasper-hyb-d\endcsname{+7.5}
\expandafter\def\csname r@H3b-qasper-hyb-p\endcsname{0.000}
\expandafter\def\csname r@H3b-qasper-hyb-pperm\endcsname{0.000}
\expandafter\def\csname r@H3b-qasper-hyb-v\endcsname{diff.}
\expandafter\def\csname r@H3b-qasper-mxbai\endcsname{+8.9 [+6.1, +11.7]}
\expandafter\def\csname r@H3b-qasper-mxbai-ci\endcsname{[+6.1, +11.7]}
\expandafter\def\csname r@H3b-qasper-mxbai-ci95\endcsname{[+6.1, +11.7]}
\expandafter\def\csname r@H3b-qasper-mxbai-d\endcsname{+8.9}
\expandafter\def\csname r@H3b-qasper-mxbai-p\endcsname{--}
\expandafter\def\csname r@H3b-qasper-mxbai-v\endcsname{diff.}
\expandafter\def\csname r@H3b-qasper-nomic\endcsname{+10.4 [+7.7, +13.4]}
\expandafter\def\csname r@H3b-qasper-nomic-ci\endcsname{[+7.7, +13.4]}
\expandafter\def\csname r@H3b-qasper-nomic-ci95\endcsname{[+7.7, +13.4]}
\expandafter\def\csname r@H3b-qasper-nomic-d\endcsname{+10.4}
\expandafter\def\csname r@H3b-qasper-nomic-p\endcsname{--}
\expandafter\def\csname r@H3b-qasper-nomic-v\endcsname{diff.}
\expandafter\def\csname r@H3b-yolo\endcsname{$-$3.0 [$-$9.7, +4.4]}
\expandafter\def\csname r@H3b-yolo-ci\endcsname{[$-$9.7, +4.4]}
\expandafter\def\csname r@H3b-yolo-ci95\endcsname{[$-$9.7, +4.4]}
\expandafter\def\csname r@H3b-yolo-d\endcsname{$-$3.0}
\expandafter\def\csname r@H3b-yolo-p\endcsname{--}
\expandafter\def\csname r@H3b-yolo-v\endcsname{n.d.}
\expandafter\def\csname r@H4a-fs\endcsname{+0.4 [$-$0.7, +1.6]}
\expandafter\def\csname r@H4a-fs-ci\endcsname{[$-$0.7, +1.6]}
\expandafter\def\csname r@H4a-fs-ci95\endcsname{[$-$0.7, +1.6]}
\expandafter\def\csname r@H4a-fs-d\endcsname{+0.4}
\expandafter\def\csname r@H4a-fs-p\endcsname{1.000}
\expandafter\def\csname r@H4a-fs-pperm\endcsname{1.000}
\expandafter\def\csname r@H4a-fs-v\endcsname{n.d.}
\expandafter\def\csname r@H4a-qasper\endcsname{+1.9 [+0.3, +3.5]}
\expandafter\def\csname r@H4a-qasper-ci\endcsname{[+0.3, +3.5]}
\expandafter\def\csname r@H4a-qasper-ci95\endcsname{[+0.3, +3.5]}
\expandafter\def\csname r@H4a-qasper-d\endcsname{+1.9}
\expandafter\def\csname r@H4a-qasper-p\endcsname{0.078}
\expandafter\def\csname r@H4a-qasper-pperm\endcsname{0.136}
\expandafter\def\csname r@H4a-qasper-v\endcsname{n.d.}
\expandafter\def\csname r@H4b-fs\endcsname{+0.4 [$-$1.0, +1.8]}
\expandafter\def\csname r@H4b-fs-ci\endcsname{[$-$1.0, +1.8]}
\expandafter\def\csname r@H4b-fs-ci95\endcsname{[$-$1.0, +1.8]}
\expandafter\def\csname r@H4b-fs-d\endcsname{+0.4}
\expandafter\def\csname r@H4b-fs-p\endcsname{1.000}
\expandafter\def\csname r@H4b-fs-pperm\endcsname{1.000}
\expandafter\def\csname r@H4b-fs-v\endcsname{n.d.}
\expandafter\def\csname r@H4b-qasper\endcsname{$-$0.1 [$-$1.9, +1.8]}
\expandafter\def\csname r@H4b-qasper-ci\endcsname{[$-$1.9, +1.8]}
\expandafter\def\csname r@H4b-qasper-ci95\endcsname{[$-$1.9, +1.8]}
\expandafter\def\csname r@H4b-qasper-d\endcsname{$-$0.1}
\expandafter\def\csname r@H4b-qasper-p\endcsname{1.000}
\expandafter\def\csname r@H4b-qasper-pperm\endcsname{1.000}
\expandafter\def\csname r@H4b-qasper-v\endcsname{n.d.}
\expandafter\def\csname r@H4c-fs\endcsname{+0.3 [$-$0.8, +1.4]}
\expandafter\def\csname r@H4c-fs-ci\endcsname{[$-$0.8, +1.4]}
\expandafter\def\csname r@H4c-fs-ci95\endcsname{[$-$1.0, +1.6]}
\expandafter\def\csname r@H4c-fs-d\endcsname{+0.3}
\expandafter\def\csname r@H4c-fs-p\endcsname{0.001}
\expandafter\def\csname r@H4c-fs-pperm\endcsname{1.000}
\expandafter\def\csname r@H4c-fs-v\endcsname{equiv.}
\expandafter\def\csname r@H4c-qasper\endcsname{$-$2.2 [$-$3.6, $-$0.9]}
\expandafter\def\csname r@H4c-qasper-ci\endcsname{[$-$3.6, $-$0.9]}
\expandafter\def\csname r@H4c-qasper-ci95\endcsname{[$-$3.8, $-$0.7]}
\expandafter\def\csname r@H4c-qasper-d\endcsname{$-$2.2}
\expandafter\def\csname r@H4c-qasper-p\endcsname{0.006}
\expandafter\def\csname r@H4c-qasper-pperm\endcsname{0.054}
\expandafter\def\csname r@H4c-qasper-v\endcsname{equiv.}
\expandafter\def\csname r@H4d-fs\endcsname{+1.4 [+0.1, +2.7]}
\expandafter\def\csname r@H4d-fs-ci\endcsname{[+0.1, +2.7]}
\expandafter\def\csname r@H4d-fs-ci95\endcsname{[$-$0.1, +2.9]}
\expandafter\def\csname r@H4d-fs-d\endcsname{+1.4}
\expandafter\def\csname r@H4d-fs-p\endcsname{0.002}
\expandafter\def\csname r@H4d-fs-pperm\endcsname{0.500}
\expandafter\def\csname r@H4d-fs-v\endcsname{equiv.}
\expandafter\def\csname r@H4d-qasper\endcsname{+0.7 [$-$1.0, +2.4]}
\expandafter\def\csname r@H4d-qasper-ci\endcsname{[$-$1.0, +2.4]}
\expandafter\def\csname r@H4d-qasper-ci95\endcsname{[$-$1.3, +2.7]}
\expandafter\def\csname r@H4d-qasper-d\endcsname{+0.7}
\expandafter\def\csname r@H4d-qasper-p\endcsname{0.001}
\expandafter\def\csname r@H4d-qasper-pperm\endcsname{1.000}
\expandafter\def\csname r@H4d-qasper-v\endcsname{equiv.}
\expandafter\def\csname r@H5a-fs\endcsname{+1.2 [$-$1.5, +4.2]}
\expandafter\def\csname r@H5a-fs-ci\endcsname{[$-$1.5, +4.2]}
\expandafter\def\csname r@H5a-fs-ci95\endcsname{[$-$1.5, +4.2]}
\expandafter\def\csname r@H5a-fs-d\endcsname{+1.2}
\expandafter\def\csname r@H5a-fs-p\endcsname{0.399}
\expandafter\def\csname r@H5a-fs-pperm\endcsname{0.399}
\expandafter\def\csname r@H5a-fs-v\endcsname{n.d.}
\expandafter\def\csname r@H5a-qasper\endcsname{$-$10.0 [$-$12.3, $-$7.6]}
\expandafter\def\csname r@H5a-qasper-ci\endcsname{[$-$12.3, $-$7.6]}
\expandafter\def\csname r@H5a-qasper-ci95\endcsname{[$-$12.3, $-$7.6]}
\expandafter\def\csname r@H5a-qasper-d\endcsname{$-$10.0}
\expandafter\def\csname r@H5a-qasper-p\endcsname{0.000}
\expandafter\def\csname r@H5a-qasper-pperm\endcsname{0.000}
\expandafter\def\csname r@H5a-qasper-v\endcsname{diff.}
\expandafter\def\csname r@H5b-fs\endcsname{$-$1.6 [$-$3.1, +0.1]}
\expandafter\def\csname r@H5b-fs-ci\endcsname{[$-$3.1, +0.1]}
\expandafter\def\csname r@H5b-fs-ci95\endcsname{[$-$3.1, +0.1]}
\expandafter\def\csname r@H5b-fs-d\endcsname{$-$1.6}
\expandafter\def\csname r@H5b-fs-p\endcsname{0.136}
\expandafter\def\csname r@H5b-fs-pperm\endcsname{0.136}
\expandafter\def\csname r@H5b-fs-v\endcsname{n.d.}
\expandafter\def\csname r@H5b-qasper\endcsname{$-$2.2 [$-$4.3, $-$0.2]}
\expandafter\def\csname r@H5b-qasper-ci\endcsname{[$-$4.3, $-$0.2]}
\expandafter\def\csname r@H5b-qasper-ci95\endcsname{[$-$4.3, $-$0.2]}
\expandafter\def\csname r@H5b-qasper-d\endcsname{$-$2.2}
\expandafter\def\csname r@H5b-qasper-p\endcsname{0.136}
\expandafter\def\csname r@H5b-qasper-pperm\endcsname{0.136}
\expandafter\def\csname r@H5b-qasper-v\endcsname{n.d.}
\expandafter\def\csname r@H6\endcsname{+1.6 [$-$1.5, +4.6]}
\expandafter\def\csname r@H6-ci\endcsname{[$-$1.5, +4.6]}
\expandafter\def\csname r@H6-ci95\endcsname{[$-$2.1, +5.1]}
\expandafter\def\csname r@H6-d\endcsname{+1.6}
\expandafter\def\csname r@H6-p\endcsname{0.029}
\expandafter\def\csname r@H6-pperm\endcsname{0.382}
\expandafter\def\csname r@H6-v\endcsname{equiv.}
\expandafter\def\csname r@H7-fs\endcsname{$-$2.8 [$-$4.9, $-$0.8]}
\expandafter\def\csname r@H7-fs-ci\endcsname{[$-$4.9, $-$0.8]}
\expandafter\def\csname r@H7-fs-ci95\endcsname{[$-$4.9, $-$0.8]}
\expandafter\def\csname r@H7-fs-d\endcsname{$-$2.8}
\expandafter\def\csname r@H7-fs-p\endcsname{0.008}
\expandafter\def\csname r@H7-fs-pperm\endcsname{0.008}
\expandafter\def\csname r@H7-fs-v\endcsname{diff.}
\expandafter\def\csname r@H7-qasper\endcsname{+4.1 [+1.7, +6.6]}
\expandafter\def\csname r@H7-qasper-ci\endcsname{[+1.7, +6.6]}
\expandafter\def\csname r@H7-qasper-ci95\endcsname{[+1.7, +6.6]}
\expandafter\def\csname r@H7-qasper-d\endcsname{+4.1}
\expandafter\def\csname r@H7-qasper-p\endcsname{0.002}
\expandafter\def\csname r@H7-qasper-pperm\endcsname{0.002}
\expandafter\def\csname r@H7-qasper-v\endcsname{diff.}
\expandafter\def\csname r@SFL-fs\endcsname{+1.6 [$-$0.6, +3.9]}
\expandafter\def\csname r@SFL-fs-ci\endcsname{[$-$0.6, +3.9]}
\expandafter\def\csname r@SFL-fs-ci95\endcsname{[$-$0.6, +3.9]}
\expandafter\def\csname r@SFL-fs-d\endcsname{+1.6}
\expandafter\def\csname r@SFL-fs-p\endcsname{--}
\expandafter\def\csname r@SFL-fs-v\endcsname{n.d.}
\expandafter\def\csname r@SFL-qasper\endcsname{+8.2 [+5.3, +11.1]}
\expandafter\def\csname r@SFL-qasper-ci\endcsname{[+5.3, +11.1]}
\expandafter\def\csname r@SFL-qasper-ci95\endcsname{[+5.3, +11.1]}
\expandafter\def\csname r@SFL-qasper-d\endcsname{+8.2}
\expandafter\def\csname r@SFL-qasper-p\endcsname{--}
\expandafter\def\csname r@SFL-qasper-v\endcsname{diff.}
\expandafter\def\csname r@SP-fs\endcsname{$-$2.0 [$-$4.5, +0.5]}
\expandafter\def\csname r@SP-fs-ci\endcsname{[$-$4.5, +0.5]}
\expandafter\def\csname r@SP-fs-ci95\endcsname{[$-$4.5, +0.5]}
\expandafter\def\csname r@SP-fs-d\endcsname{$-$2.0}
\expandafter\def\csname r@SP-fs-p\endcsname{--}
\expandafter\def\csname r@SP-fs-v\endcsname{n.d.}
\expandafter\def\csname r@SP-qasper\endcsname{+5.2 [+2.7, +7.8]}
\expandafter\def\csname r@SP-qasper-ci\endcsname{[+2.7, +7.8]}
\expandafter\def\csname r@SP-qasper-ci95\endcsname{[+2.7, +7.8]}
\expandafter\def\csname r@SP-qasper-d\endcsname{+5.2}
\expandafter\def\csname r@SP-qasper-p\endcsname{--}
\expandafter\def\csname r@SP-qasper-v\endcsname{diff.}
\expandafter\def\csname r@STS-fs\endcsname{+1.3 [$-$0.4, +3.2]}
\expandafter\def\csname r@STS-fs-ci\endcsname{[$-$0.4, +3.2]}
\expandafter\def\csname r@STS-fs-ci95\endcsname{[$-$0.4, +3.2]}
\expandafter\def\csname r@STS-fs-d\endcsname{+1.3}
\expandafter\def\csname r@STS-fs-p\endcsname{--}
\expandafter\def\csname r@STS-fs-v\endcsname{n.d.}
\expandafter\def\csname r@STS-qasper\endcsname{+0.2 [$-$1.6, +2.1]}
\expandafter\def\csname r@STS-qasper-ci\endcsname{[$-$1.6, +2.1]}
\expandafter\def\csname r@STS-qasper-ci95\endcsname{[$-$1.6, +2.1]}
\expandafter\def\csname r@STS-qasper-d\endcsname{+0.2}
\expandafter\def\csname r@STS-qasper-p\endcsname{--}
\expandafter\def\csname r@STS-qasper-v\endcsname{n.d.}
\expandafter\def\csname r@ax-add-fs-CR-new\endcsname{17.4}
\expandafter\def\csname r@ax-add-fs-CR-newc\endcsname{11.3}
\expandafter\def\csname r@ax-add-fs-CR-text\endcsname{58}
\expandafter\def\csname r@ax-add-fs-E-new\endcsname{15.9}
\expandafter\def\csname r@ax-add-fs-E-newc\endcsname{9.2}
\expandafter\def\csname r@ax-add-fs-E-strong-new\endcsname{29.5}
\expandafter\def\csname r@ax-add-fs-E-strong-newc\endcsname{18.6}
\expandafter\def\csname r@ax-add-fs-E-strong-text\endcsname{58}
\expandafter\def\csname r@ax-add-fs-E-text\endcsname{58}
\expandafter\def\csname r@ax-add-fs-S+T-new\endcsname{2.4}
\expandafter\def\csname r@ax-add-fs-S+T-newc\endcsname{2.2}
\expandafter\def\csname r@ax-add-fs-S+T-text\endcsname{58}
\expandafter\def\csname r@ax-add-qasper-CR-new\endcsname{18.5}
\expandafter\def\csname r@ax-add-qasper-CR-newc\endcsname{14.1}
\expandafter\def\csname r@ax-add-qasper-CR-text\endcsname{91}
\expandafter\def\csname r@ax-add-qasper-E-new\endcsname{15.8}
\expandafter\def\csname r@ax-add-qasper-E-newc\endcsname{11.1}
\expandafter\def\csname r@ax-add-qasper-E-strong-new\endcsname{28.7}
\expandafter\def\csname r@ax-add-qasper-E-strong-newc\endcsname{21.4}
\expandafter\def\csname r@ax-add-qasper-E-strong-text\endcsname{91}
\expandafter\def\csname r@ax-add-qasper-E-text\endcsname{91}
\expandafter\def\csname r@ax-add-qasper-S+T-new\endcsname{6.3}
\expandafter\def\csname r@ax-add-qasper-S+T-newc\endcsname{5.6}
\expandafter\def\csname r@ax-add-qasper-S+T-text\endcsname{91}
\expandafter\def\csname r@ax-br-fs-bm25-c\endcsname{+1.2 [$-$2.9, +4.6]}
\expandafter\def\csname r@ax-br-fs-bm25-c-ci\endcsname{[$-$2.9, +4.6]}
\expandafter\def\csname r@ax-br-fs-bm25-c-ci95\endcsname{[$-$2.9, +4.6]}
\expandafter\def\csname r@ax-br-fs-bm25-c-d\endcsname{+1.2}
\expandafter\def\csname r@ax-br-fs-bm25-c-p\endcsname{--}
\expandafter\def\csname r@ax-br-fs-bm25-c-v\endcsname{n.d.}
\expandafter\def\csname r@ax-br-fs-bm25-gainshare\endcsname{73}
\expandafter\def\csname r@ax-br-fs-bm25-lossn\endcsname{78}
\expandafter\def\csname r@ax-br-fs-bm25-lossshare\endcsname{55}
\expandafter\def\csname r@ax-br-fs-bm25-miss\endcsname{+1.6 [$-$0.8, +5.5]}
\expandafter\def\csname r@ax-br-fs-bm25-miss-ci\endcsname{[$-$0.8, +5.5]}
\expandafter\def\csname r@ax-br-fs-bm25-miss-ci95\endcsname{[$-$0.8, +5.5]}
\expandafter\def\csname r@ax-br-fs-bm25-miss-d\endcsname{+1.6}
\expandafter\def\csname r@ax-br-fs-bm25-miss-p\endcsname{--}
\expandafter\def\csname r@ax-br-fs-bm25-miss-v\endcsname{n.d.}
\expandafter\def\csname r@ax-br-fs-bm25-none\endcsname{--}
\expandafter\def\csname r@ax-br-fs-bm25-none-ci\endcsname{--}
\expandafter\def\csname r@ax-br-fs-bm25-none-d\endcsname{--}
\expandafter\def\csname r@ax-br-fs-bm25-none-p\endcsname{--}
\expandafter\def\csname r@ax-br-fs-bm25-none-v\endcsname{--}
\expandafter\def\csname r@ax-br-fs-bm25-tien\endcsname{57}
\expandafter\def\csname r@ax-br-fs-bm25-tieshare\endcsname{67}
\expandafter\def\csname r@ax-br-fs-bm25-winn\endcsname{100}
\expandafter\def\csname r@ax-br-fs-bm25-winshare\endcsname{62}
\expandafter\def\csname r@ax-br-fs-bm25-yes\endcsname{+2.9 [+1.0, +5.0]}
\expandafter\def\csname r@ax-br-fs-bm25-yes-ci\endcsname{[+1.0, +5.0]}
\expandafter\def\csname r@ax-br-fs-bm25-yes-ci95\endcsname{[+1.0, +5.0]}
\expandafter\def\csname r@ax-br-fs-bm25-yes-d\endcsname{+2.9}
\expandafter\def\csname r@ax-br-fs-bm25-yes-p\endcsname{--}
\expandafter\def\csname r@ax-br-fs-bm25-yes-v\endcsname{diff.}
\expandafter\def\csname r@ax-br-fs-hq3-c\endcsname{+0.4 [$-$3.5, +4.3]}
\expandafter\def\csname r@ax-br-fs-hq3-c-ci\endcsname{[$-$3.5, +4.3]}
\expandafter\def\csname r@ax-br-fs-hq3-c-ci95\endcsname{[$-$3.5, +4.3]}
\expandafter\def\csname r@ax-br-fs-hq3-c-d\endcsname{+0.4}
\expandafter\def\csname r@ax-br-fs-hq3-c-p\endcsname{--}
\expandafter\def\csname r@ax-br-fs-hq3-c-v\endcsname{n.d.}
\expandafter\def\csname r@ax-br-fs-hq3-gainshare\endcsname{69}
\expandafter\def\csname r@ax-br-fs-hq3-miss\endcsname{+0.8 [$-$2.1, +3.4]}
\expandafter\def\csname r@ax-br-fs-hq3-miss-ci\endcsname{[$-$2.1, +3.4]}
\expandafter\def\csname r@ax-br-fs-hq3-miss-ci95\endcsname{[$-$2.1, +3.4]}
\expandafter\def\csname r@ax-br-fs-hq3-miss-d\endcsname{+0.8}
\expandafter\def\csname r@ax-br-fs-hq3-miss-p\endcsname{--}
\expandafter\def\csname r@ax-br-fs-hq3-miss-v\endcsname{n.d.}
\expandafter\def\csname r@ax-br-fs-hq3-none\endcsname{--}
\expandafter\def\csname r@ax-br-fs-hq3-none-ci\endcsname{--}
\expandafter\def\csname r@ax-br-fs-hq3-none-d\endcsname{--}
\expandafter\def\csname r@ax-br-fs-hq3-none-p\endcsname{--}
\expandafter\def\csname r@ax-br-fs-hq3-none-v\endcsname{--}
\expandafter\def\csname r@ax-br-fs-hq3-yes\endcsname{+1.2 [$-$1.5, +3.8]}
\expandafter\def\csname r@ax-br-fs-hq3-yes-ci\endcsname{[$-$1.5, +3.8]}
\expandafter\def\csname r@ax-br-fs-hq3-yes-ci95\endcsname{[$-$1.5, +3.8]}
\expandafter\def\csname r@ax-br-fs-hq3-yes-d\endcsname{+1.2}
\expandafter\def\csname r@ax-br-fs-hq3-yes-p\endcsname{--}
\expandafter\def\csname r@ax-br-fs-hq3-yes-v\endcsname{n.d.}
\expandafter\def\csname r@ax-br-fs-hyb-c\endcsname{$-$0.5 [$-$5.3, +4.2]}
\expandafter\def\csname r@ax-br-fs-hyb-c-ci\endcsname{[$-$5.3, +4.2]}
\expandafter\def\csname r@ax-br-fs-hyb-c-ci95\endcsname{[$-$5.3, +4.2]}
\expandafter\def\csname r@ax-br-fs-hyb-c-d\endcsname{$-$0.5}
\expandafter\def\csname r@ax-br-fs-hyb-c-p\endcsname{--}
\expandafter\def\csname r@ax-br-fs-hyb-c-v\endcsname{n.d.}
\expandafter\def\csname r@ax-br-fs-hyb-gainshare\endcsname{56}
\expandafter\def\csname r@ax-br-fs-hyb-miss\endcsname{+3.1 [$-$0.6, +7.1]}
\expandafter\def\csname r@ax-br-fs-hyb-miss-ci\endcsname{[$-$0.6, +7.1]}
\expandafter\def\csname r@ax-br-fs-hyb-miss-ci95\endcsname{[$-$0.6, +7.1]}
\expandafter\def\csname r@ax-br-fs-hyb-miss-d\endcsname{+3.1}
\expandafter\def\csname r@ax-br-fs-hyb-miss-p\endcsname{--}
\expandafter\def\csname r@ax-br-fs-hyb-miss-v\endcsname{n.d.}
\expandafter\def\csname r@ax-br-fs-hyb-none\endcsname{--}
\expandafter\def\csname r@ax-br-fs-hyb-none-ci\endcsname{--}
\expandafter\def\csname r@ax-br-fs-hyb-none-d\endcsname{--}
\expandafter\def\csname r@ax-br-fs-hyb-none-p\endcsname{--}
\expandafter\def\csname r@ax-br-fs-hyb-none-v\endcsname{--}
\expandafter\def\csname r@ax-br-fs-hyb-yes\endcsname{+2.5 [$-$0.3, +5.2]}
\expandafter\def\csname r@ax-br-fs-hyb-yes-ci\endcsname{[$-$0.3, +5.2]}
\expandafter\def\csname r@ax-br-fs-hyb-yes-ci95\endcsname{[$-$0.3, +5.2]}
\expandafter\def\csname r@ax-br-fs-hyb-yes-d\endcsname{+2.5}
\expandafter\def\csname r@ax-br-fs-hyb-yes-p\endcsname{--}
\expandafter\def\csname r@ax-br-fs-hyb-yes-v\endcsname{n.d.}
\expandafter\def\csname r@ax-br-fs-missbridged\endcsname{3}
\expandafter\def\csname r@ax-br-fs-missing\endcsname{43.0}
\expandafter\def\csname r@ax-br-fs-mxbai-c\endcsname{$-$1.4 [$-$6.0, +3.2]}
\expandafter\def\csname r@ax-br-fs-mxbai-c-ci\endcsname{[$-$6.0, +3.2]}
\expandafter\def\csname r@ax-br-fs-mxbai-c-ci95\endcsname{[$-$6.0, +3.2]}
\expandafter\def\csname r@ax-br-fs-mxbai-c-d\endcsname{$-$1.4}
\expandafter\def\csname r@ax-br-fs-mxbai-c-p\endcsname{--}
\expandafter\def\csname r@ax-br-fs-mxbai-c-v\endcsname{n.d.}
\expandafter\def\csname r@ax-br-fs-mxbai-gainshare\endcsname{-3743}
\expandafter\def\csname r@ax-br-fs-mxbai-miss\endcsname{+0.9 [$-$2.7, +4.4]}
\expandafter\def\csname r@ax-br-fs-mxbai-miss-ci\endcsname{[$-$2.7, +4.4]}
\expandafter\def\csname r@ax-br-fs-mxbai-miss-ci95\endcsname{[$-$2.7, +4.4]}
\expandafter\def\csname r@ax-br-fs-mxbai-miss-d\endcsname{+0.9}
\expandafter\def\csname r@ax-br-fs-mxbai-miss-p\endcsname{--}
\expandafter\def\csname r@ax-br-fs-mxbai-miss-v\endcsname{n.d.}
\expandafter\def\csname r@ax-br-fs-mxbai-none\endcsname{--}
\expandafter\def\csname r@ax-br-fs-mxbai-none-ci\endcsname{--}
\expandafter\def\csname r@ax-br-fs-mxbai-none-d\endcsname{--}
\expandafter\def\csname r@ax-br-fs-mxbai-none-p\endcsname{--}
\expandafter\def\csname r@ax-br-fs-mxbai-none-v\endcsname{--}
\expandafter\def\csname r@ax-br-fs-mxbai-yes\endcsname{$-$0.5 [$-$3.3, +2.4]}
\expandafter\def\csname r@ax-br-fs-mxbai-yes-ci\endcsname{[$-$3.3, +2.4]}
\expandafter\def\csname r@ax-br-fs-mxbai-yes-ci95\endcsname{[$-$3.3, +2.4]}
\expandafter\def\csname r@ax-br-fs-mxbai-yes-d\endcsname{$-$0.5}
\expandafter\def\csname r@ax-br-fs-mxbai-yes-p\endcsname{--}
\expandafter\def\csname r@ax-br-fs-mxbai-yes-v\endcsname{n.d.}
\expandafter\def\csname r@ax-br-fs-n\endcsname{143}
\expandafter\def\csname r@ax-br-fs-nmiss\endcsname{92}
\expandafter\def\csname r@ax-br-fs-nnone\endcsname{0}
\expandafter\def\csname r@ax-br-fs-nomic-c\endcsname{+3.5 [$-$1.5, +8.2]}
\expandafter\def\csname r@ax-br-fs-nomic-c-ci\endcsname{[$-$1.5, +8.2]}
\expandafter\def\csname r@ax-br-fs-nomic-c-ci95\endcsname{[$-$1.5, +8.2]}
\expandafter\def\csname r@ax-br-fs-nomic-c-d\endcsname{+3.5}
\expandafter\def\csname r@ax-br-fs-nomic-c-p\endcsname{--}
\expandafter\def\csname r@ax-br-fs-nomic-c-v\endcsname{n.d.}
\expandafter\def\csname r@ax-br-fs-nomic-gainshare\endcsname{92}
\expandafter\def\csname r@ax-br-fs-nomic-miss\endcsname{+0.5 [$-$3.1, +4.2]}
\expandafter\def\csname r@ax-br-fs-nomic-miss-ci\endcsname{[$-$3.1, +4.2]}
\expandafter\def\csname r@ax-br-fs-nomic-miss-ci95\endcsname{[$-$3.1, +4.2]}
\expandafter\def\csname r@ax-br-fs-nomic-miss-d\endcsname{+0.5}
\expandafter\def\csname r@ax-br-fs-nomic-miss-p\endcsname{--}
\expandafter\def\csname r@ax-br-fs-nomic-miss-v\endcsname{n.d.}
\expandafter\def\csname r@ax-br-fs-nomic-none\endcsname{--}
\expandafter\def\csname r@ax-br-fs-nomic-none-ci\endcsname{--}
\expandafter\def\csname r@ax-br-fs-nomic-none-d\endcsname{--}
\expandafter\def\csname r@ax-br-fs-nomic-none-p\endcsname{--}
\expandafter\def\csname r@ax-br-fs-nomic-none-v\endcsname{--}
\expandafter\def\csname r@ax-br-fs-nomic-yes\endcsname{+4.0 [+0.9, +7.4]}
\expandafter\def\csname r@ax-br-fs-nomic-yes-ci\endcsname{[+0.9, +7.4]}
\expandafter\def\csname r@ax-br-fs-nomic-yes-ci95\endcsname{[+0.9, +7.4]}
\expandafter\def\csname r@ax-br-fs-nomic-yes-d\endcsname{+4.0}
\expandafter\def\csname r@ax-br-fs-nomic-yes-p\endcsname{--}
\expandafter\def\csname r@ax-br-fs-nomic-yes-v\endcsname{diff.}
\expandafter\def\csname r@ax-br-fs-q3-c\endcsname{$-$1.6 [$-$5.0, +1.8]}
\expandafter\def\csname r@ax-br-fs-q3-c-ci\endcsname{[$-$5.0, +1.8]}
\expandafter\def\csname r@ax-br-fs-q3-c-ci95\endcsname{[$-$5.0, +1.8]}
\expandafter\def\csname r@ax-br-fs-q3-c-d\endcsname{$-$1.6}
\expandafter\def\csname r@ax-br-fs-q3-c-p\endcsname{--}
\expandafter\def\csname r@ax-br-fs-q3-c-v\endcsname{n.d.}
\expandafter\def\csname r@ax-br-fs-q3-gainshare\endcsname{-82}
\expandafter\def\csname r@ax-br-fs-q3-miss\endcsname{+1.2 [$-$1.3, +3.8]}
\expandafter\def\csname r@ax-br-fs-q3-miss-ci\endcsname{[$-$1.3, +3.8]}
\expandafter\def\csname r@ax-br-fs-q3-miss-ci95\endcsname{[$-$1.3, +3.8]}
\expandafter\def\csname r@ax-br-fs-q3-miss-d\endcsname{+1.2}
\expandafter\def\csname r@ax-br-fs-q3-miss-p\endcsname{--}
\expandafter\def\csname r@ax-br-fs-q3-miss-v\endcsname{n.d.}
\expandafter\def\csname r@ax-br-fs-q3-none\endcsname{--}
\expandafter\def\csname r@ax-br-fs-q3-none-ci\endcsname{--}
\expandafter\def\csname r@ax-br-fs-q3-none-d\endcsname{--}
\expandafter\def\csname r@ax-br-fs-q3-none-p\endcsname{--}
\expandafter\def\csname r@ax-br-fs-q3-none-v\endcsname{--}
\expandafter\def\csname r@ax-br-fs-q3-yes\endcsname{$-$0.4 [$-$2.6, +2.0]}
\expandafter\def\csname r@ax-br-fs-q3-yes-ci\endcsname{[$-$2.6, +2.0]}
\expandafter\def\csname r@ax-br-fs-q3-yes-ci95\endcsname{[$-$2.6, +2.0]}
\expandafter\def\csname r@ax-br-fs-q3-yes-d\endcsname{$-$0.4}
\expandafter\def\csname r@ax-br-fs-q3-yes-p\endcsname{--}
\expandafter\def\csname r@ax-br-fs-q3-yes-v\endcsname{n.d.}
\expandafter\def\csname r@ax-br-fs-rr-c\endcsname{+0.9 [$-$3.8, +5.7]}
\expandafter\def\csname r@ax-br-fs-rr-c-ci\endcsname{[$-$3.8, +5.7]}
\expandafter\def\csname r@ax-br-fs-rr-c-ci95\endcsname{[$-$3.8, +5.7]}
\expandafter\def\csname r@ax-br-fs-rr-c-d\endcsname{+0.9}
\expandafter\def\csname r@ax-br-fs-rr-c-p\endcsname{--}
\expandafter\def\csname r@ax-br-fs-rr-c-v\endcsname{n.d.}
\expandafter\def\csname r@ax-br-fs-rr-gainshare\endcsname{89}
\expandafter\def\csname r@ax-br-fs-rr-miss\endcsname{+0.2 [$-$3.6, +4.3]}
\expandafter\def\csname r@ax-br-fs-rr-miss-ci\endcsname{[$-$3.6, +4.3]}
\expandafter\def\csname r@ax-br-fs-rr-miss-ci95\endcsname{[$-$3.6, +4.3]}
\expandafter\def\csname r@ax-br-fs-rr-miss-d\endcsname{+0.2}
\expandafter\def\csname r@ax-br-fs-rr-miss-p\endcsname{--}
\expandafter\def\csname r@ax-br-fs-rr-miss-v\endcsname{n.d.}
\expandafter\def\csname r@ax-br-fs-rr-none\endcsname{--}
\expandafter\def\csname r@ax-br-fs-rr-none-ci\endcsname{--}
\expandafter\def\csname r@ax-br-fs-rr-none-d\endcsname{--}
\expandafter\def\csname r@ax-br-fs-rr-none-p\endcsname{--}
\expandafter\def\csname r@ax-br-fs-rr-none-v\endcsname{--}
\expandafter\def\csname r@ax-br-fs-rr-yes\endcsname{+1.2 [$-$1.4, +3.9]}
\expandafter\def\csname r@ax-br-fs-rr-yes-ci\endcsname{[$-$1.4, +3.9]}
\expandafter\def\csname r@ax-br-fs-rr-yes-ci95\endcsname{[$-$1.4, +3.9]}
\expandafter\def\csname r@ax-br-fs-rr-yes-d\endcsname{+1.2}
\expandafter\def\csname r@ax-br-fs-rr-yes-p\endcsname{--}
\expandafter\def\csname r@ax-br-fs-rr-yes-v\endcsname{n.d.}
\expandafter\def\csname r@ax-br-fs-share\endcsname{61}
\expandafter\def\csname r@ax-br-qasper-bm25-c\endcsname{+21.2 [+15.4, +27.6]}
\expandafter\def\csname r@ax-br-qasper-bm25-c-ci\endcsname{[+15.4, +27.6]}
\expandafter\def\csname r@ax-br-qasper-bm25-c-ci95\endcsname{[+15.4, +27.6]}
\expandafter\def\csname r@ax-br-qasper-bm25-c-d\endcsname{+21.2}
\expandafter\def\csname r@ax-br-qasper-bm25-c-p\endcsname{--}
\expandafter\def\csname r@ax-br-qasper-bm25-c-v\endcsname{diff.}
\expandafter\def\csname r@ax-br-qasper-bm25-gainshare\endcsname{56}
\expandafter\def\csname r@ax-br-qasper-bm25-lossn\endcsname{54}
\expandafter\def\csname r@ax-br-qasper-bm25-lossshare\endcsname{2}
\expandafter\def\csname r@ax-br-qasper-bm25-miss\endcsname{+3.2 [+0.9, +5.6]}
\expandafter\def\csname r@ax-br-qasper-bm25-miss-ci\endcsname{[+0.9, +5.6]}
\expandafter\def\csname r@ax-br-qasper-bm25-miss-ci95\endcsname{[+0.9, +5.6]}
\expandafter\def\csname r@ax-br-qasper-bm25-miss-d\endcsname{+3.2}
\expandafter\def\csname r@ax-br-qasper-bm25-miss-p\endcsname{--}
\expandafter\def\csname r@ax-br-qasper-bm25-miss-v\endcsname{diff.}
\expandafter\def\csname r@ax-br-qasper-bm25-none\endcsname{+13.6 [+7.4, +21.2]}
\expandafter\def\csname r@ax-br-qasper-bm25-none-ci\endcsname{[+7.4, +21.2]}
\expandafter\def\csname r@ax-br-qasper-bm25-none-ci95\endcsname{[+7.4, +21.2]}
\expandafter\def\csname r@ax-br-qasper-bm25-none-d\endcsname{+13.6}
\expandafter\def\csname r@ax-br-qasper-bm25-none-p\endcsname{--}
\expandafter\def\csname r@ax-br-qasper-bm25-none-v\endcsname{diff.}
\expandafter\def\csname r@ax-br-qasper-bm25-tien\endcsname{721}
\expandafter\def\csname r@ax-br-qasper-bm25-tieshare\endcsname{16}
\expandafter\def\csname r@ax-br-qasper-bm25-winn\endcsname{176}
\expandafter\def\csname r@ax-br-qasper-bm25-winshare\endcsname{41}
\expandafter\def\csname r@ax-br-qasper-bm25-yes\endcsname{+24.4 [+19.2, +30.2]}
\expandafter\def\csname r@ax-br-qasper-bm25-yes-ci\endcsname{[+19.2, +30.2]}
\expandafter\def\csname r@ax-br-qasper-bm25-yes-ci95\endcsname{[+19.2, +30.2]}
\expandafter\def\csname r@ax-br-qasper-bm25-yes-d\endcsname{+24.4}
\expandafter\def\csname r@ax-br-qasper-bm25-yes-p\endcsname{--}
\expandafter\def\csname r@ax-br-qasper-bm25-yes-v\endcsname{diff.}
\expandafter\def\csname r@ax-br-qasper-hq3-c\endcsname{+15.7 [+10.1, +21.7]}
\expandafter\def\csname r@ax-br-qasper-hq3-c-ci\endcsname{[+10.1, +21.7]}
\expandafter\def\csname r@ax-br-qasper-hq3-c-ci95\endcsname{[+10.1, +21.7]}
\expandafter\def\csname r@ax-br-qasper-hq3-c-d\endcsname{+15.7}
\expandafter\def\csname r@ax-br-qasper-hq3-c-p\endcsname{--}
\expandafter\def\csname r@ax-br-qasper-hq3-c-v\endcsname{diff.}
\expandafter\def\csname r@ax-br-qasper-hq3-gainshare\endcsname{71}
\expandafter\def\csname r@ax-br-qasper-hq3-miss\endcsname{+0.5 [$-$2.5, +3.5]}
\expandafter\def\csname r@ax-br-qasper-hq3-miss-ci\endcsname{[$-$2.5, +3.5]}
\expandafter\def\csname r@ax-br-qasper-hq3-miss-ci95\endcsname{[$-$2.5, +3.5]}
\expandafter\def\csname r@ax-br-qasper-hq3-miss-d\endcsname{+0.5}
\expandafter\def\csname r@ax-br-qasper-hq3-miss-p\endcsname{--}
\expandafter\def\csname r@ax-br-qasper-hq3-miss-v\endcsname{n.d.}
\expandafter\def\csname r@ax-br-qasper-hq3-none\endcsname{+8.4 [+1.9, +15.2]}
\expandafter\def\csname r@ax-br-qasper-hq3-none-ci\endcsname{[+1.9, +15.2]}
\expandafter\def\csname r@ax-br-qasper-hq3-none-ci95\endcsname{[+1.9, +15.2]}
\expandafter\def\csname r@ax-br-qasper-hq3-none-d\endcsname{+8.4}
\expandafter\def\csname r@ax-br-qasper-hq3-none-p\endcsname{--}
\expandafter\def\csname r@ax-br-qasper-hq3-none-v\endcsname{diff.}
\expandafter\def\csname r@ax-br-qasper-hq3-yes\endcsname{+16.1 [+11.1, +21.8]}
\expandafter\def\csname r@ax-br-qasper-hq3-yes-ci\endcsname{[+11.1, +21.8]}
\expandafter\def\csname r@ax-br-qasper-hq3-yes-ci95\endcsname{[+11.1, +21.8]}
\expandafter\def\csname r@ax-br-qasper-hq3-yes-d\endcsname{+16.1}
\expandafter\def\csname r@ax-br-qasper-hq3-yes-p\endcsname{--}
\expandafter\def\csname r@ax-br-qasper-hq3-yes-v\endcsname{diff.}
\expandafter\def\csname r@ax-br-qasper-hyb-c\endcsname{+16.8 [+10.1, +23.7]}
\expandafter\def\csname r@ax-br-qasper-hyb-c-ci\endcsname{[+10.1, +23.7]}
\expandafter\def\csname r@ax-br-qasper-hyb-c-ci95\endcsname{[+10.1, +23.7]}
\expandafter\def\csname r@ax-br-qasper-hyb-c-d\endcsname{+16.8}
\expandafter\def\csname r@ax-br-qasper-hyb-c-p\endcsname{--}
\expandafter\def\csname r@ax-br-qasper-hyb-c-v\endcsname{diff.}
\expandafter\def\csname r@ax-br-qasper-hyb-gainshare\endcsname{66}
\expandafter\def\csname r@ax-br-qasper-hyb-miss\endcsname{+1.4 [$-$1.7, +4.4]}
\expandafter\def\csname r@ax-br-qasper-hyb-miss-ci\endcsname{[$-$1.7, +4.4]}
\expandafter\def\csname r@ax-br-qasper-hyb-miss-ci95\endcsname{[$-$1.7, +4.4]}
\expandafter\def\csname r@ax-br-qasper-hyb-miss-d\endcsname{+1.4}
\expandafter\def\csname r@ax-br-qasper-hyb-miss-p\endcsname{--}
\expandafter\def\csname r@ax-br-qasper-hyb-miss-v\endcsname{n.d.}
\expandafter\def\csname r@ax-br-qasper-hyb-none\endcsname{+7.3 [+1.2, +13.8]}
\expandafter\def\csname r@ax-br-qasper-hyb-none-ci\endcsname{[+1.2, +13.8]}
\expandafter\def\csname r@ax-br-qasper-hyb-none-ci95\endcsname{[+1.2, +13.8]}
\expandafter\def\csname r@ax-br-qasper-hyb-none-d\endcsname{+7.3}
\expandafter\def\csname r@ax-br-qasper-hyb-none-p\endcsname{--}
\expandafter\def\csname r@ax-br-qasper-hyb-none-v\endcsname{diff.}
\expandafter\def\csname r@ax-br-qasper-hyb-yes\endcsname{+18.2 [+12.2, +24.4]}
\expandafter\def\csname r@ax-br-qasper-hyb-yes-ci\endcsname{[+12.2, +24.4]}
\expandafter\def\csname r@ax-br-qasper-hyb-yes-ci95\endcsname{[+12.2, +24.4]}
\expandafter\def\csname r@ax-br-qasper-hyb-yes-d\endcsname{+18.2}
\expandafter\def\csname r@ax-br-qasper-hyb-yes-p\endcsname{--}
\expandafter\def\csname r@ax-br-qasper-hyb-yes-v\endcsname{diff.}
\expandafter\def\csname r@ax-br-qasper-missbridged\endcsname{11}
\expandafter\def\csname r@ax-br-qasper-missing\endcsname{1.9}
\expandafter\def\csname r@ax-br-qasper-mxbai-c\endcsname{+4.8 [$-$0.1, +10.4]}
\expandafter\def\csname r@ax-br-qasper-mxbai-c-ci\endcsname{[$-$0.1, +10.4]}
\expandafter\def\csname r@ax-br-qasper-mxbai-c-ci95\endcsname{[$-$0.1, +10.4]}
\expandafter\def\csname r@ax-br-qasper-mxbai-c-d\endcsname{+4.8}
\expandafter\def\csname r@ax-br-qasper-mxbai-c-p\endcsname{--}
\expandafter\def\csname r@ax-br-qasper-mxbai-c-v\endcsname{n.d.}
\expandafter\def\csname r@ax-br-qasper-mxbai-gainshare\endcsname{128}
\expandafter\def\csname r@ax-br-qasper-mxbai-miss\endcsname{$-$0.4 [$-$3.7, +2.8]}
\expandafter\def\csname r@ax-br-qasper-mxbai-miss-ci\endcsname{[$-$3.7, +2.8]}
\expandafter\def\csname r@ax-br-qasper-mxbai-miss-ci95\endcsname{[$-$3.7, +2.8]}
\expandafter\def\csname r@ax-br-qasper-mxbai-miss-d\endcsname{$-$0.4}
\expandafter\def\csname r@ax-br-qasper-mxbai-miss-p\endcsname{--}
\expandafter\def\csname r@ax-br-qasper-mxbai-miss-v\endcsname{n.d.}
\expandafter\def\csname r@ax-br-qasper-mxbai-none\endcsname{+0.6 [$-$5.0, +6.6]}
\expandafter\def\csname r@ax-br-qasper-mxbai-none-ci\endcsname{[$-$5.0, +6.6]}
\expandafter\def\csname r@ax-br-qasper-mxbai-none-ci95\endcsname{[$-$5.0, +6.6]}
\expandafter\def\csname r@ax-br-qasper-mxbai-none-d\endcsname{+0.6}
\expandafter\def\csname r@ax-br-qasper-mxbai-none-p\endcsname{--}
\expandafter\def\csname r@ax-br-qasper-mxbai-none-v\endcsname{n.d.}
\expandafter\def\csname r@ax-br-qasper-mxbai-yes\endcsname{+4.4 [+0.2, +9.2]}
\expandafter\def\csname r@ax-br-qasper-mxbai-yes-ci\endcsname{[+0.2, +9.2]}
\expandafter\def\csname r@ax-br-qasper-mxbai-yes-ci95\endcsname{[+0.2, +9.2]}
\expandafter\def\csname r@ax-br-qasper-mxbai-yes-d\endcsname{+4.4}
\expandafter\def\csname r@ax-br-qasper-mxbai-yes-p\endcsname{--}
\expandafter\def\csname r@ax-br-qasper-mxbai-yes-v\endcsname{diff.}
\expandafter\def\csname r@ax-br-qasper-n\endcsname{190}
\expandafter\def\csname r@ax-br-qasper-nmiss\endcsname{644}
\expandafter\def\csname r@ax-br-qasper-nnone\endcsname{117}
\expandafter\def\csname r@ax-br-qasper-nomic-c\endcsname{+7.5 [+1.1, +13.6]}
\expandafter\def\csname r@ax-br-qasper-nomic-c-ci\endcsname{[+1.1, +13.6]}
\expandafter\def\csname r@ax-br-qasper-nomic-c-ci95\endcsname{[+1.1, +13.6]}
\expandafter\def\csname r@ax-br-qasper-nomic-c-d\endcsname{+7.5}
\expandafter\def\csname r@ax-br-qasper-nomic-c-p\endcsname{--}
\expandafter\def\csname r@ax-br-qasper-nomic-c-v\endcsname{diff.}
\expandafter\def\csname r@ax-br-qasper-nomic-gainshare\endcsname{158}
\expandafter\def\csname r@ax-br-qasper-nomic-miss\endcsname{$-$0.7 [$-$4.0, +2.5]}
\expandafter\def\csname r@ax-br-qasper-nomic-miss-ci\endcsname{[$-$4.0, +2.5]}
\expandafter\def\csname r@ax-br-qasper-nomic-miss-ci95\endcsname{[$-$4.0, +2.5]}
\expandafter\def\csname r@ax-br-qasper-nomic-miss-d\endcsname{$-$0.7}
\expandafter\def\csname r@ax-br-qasper-nomic-miss-p\endcsname{--}
\expandafter\def\csname r@ax-br-qasper-nomic-miss-v\endcsname{n.d.}
\expandafter\def\csname r@ax-br-qasper-nomic-none\endcsname{$-$0.0 [$-$6.4, +6.2]}
\expandafter\def\csname r@ax-br-qasper-nomic-none-ci\endcsname{[$-$6.4, +6.2]}
\expandafter\def\csname r@ax-br-qasper-nomic-none-ci95\endcsname{[$-$6.4, +6.2]}
\expandafter\def\csname r@ax-br-qasper-nomic-none-d\endcsname{$-$0.0}
\expandafter\def\csname r@ax-br-qasper-nomic-none-p\endcsname{--}
\expandafter\def\csname r@ax-br-qasper-nomic-none-v\endcsname{n.d.}
\expandafter\def\csname r@ax-br-qasper-nomic-yes\endcsname{+6.8 [+1.3, +12.1]}
\expandafter\def\csname r@ax-br-qasper-nomic-yes-ci\endcsname{[+1.3, +12.1]}
\expandafter\def\csname r@ax-br-qasper-nomic-yes-ci95\endcsname{[+1.3, +12.1]}
\expandafter\def\csname r@ax-br-qasper-nomic-yes-d\endcsname{+6.8}
\expandafter\def\csname r@ax-br-qasper-nomic-yes-p\endcsname{--}
\expandafter\def\csname r@ax-br-qasper-nomic-yes-v\endcsname{diff.}
\expandafter\def\csname r@ax-br-qasper-q3-c\endcsname{+4.3 [$-$1.4, +10.0]}
\expandafter\def\csname r@ax-br-qasper-q3-c-ci\endcsname{[$-$1.4, +10.0]}
\expandafter\def\csname r@ax-br-qasper-q3-c-ci95\endcsname{[$-$1.4, +10.0]}
\expandafter\def\csname r@ax-br-qasper-q3-c-d\endcsname{+4.3}
\expandafter\def\csname r@ax-br-qasper-q3-c-p\endcsname{--}
\expandafter\def\csname r@ax-br-qasper-q3-c-v\endcsname{n.d.}
\expandafter\def\csname r@ax-br-qasper-q3-gainshare\endcsname{65}
\expandafter\def\csname r@ax-br-qasper-q3-miss\endcsname{+0.6 [$-$2.6, +4.0]}
\expandafter\def\csname r@ax-br-qasper-q3-miss-ci\endcsname{[$-$2.6, +4.0]}
\expandafter\def\csname r@ax-br-qasper-q3-miss-ci95\endcsname{[$-$2.6, +4.0]}
\expandafter\def\csname r@ax-br-qasper-q3-miss-d\endcsname{+0.6}
\expandafter\def\csname r@ax-br-qasper-q3-miss-p\endcsname{--}
\expandafter\def\csname r@ax-br-qasper-q3-miss-v\endcsname{n.d.}
\expandafter\def\csname r@ax-br-qasper-q3-none\endcsname{+0.7 [$-$5.5, +7.1]}
\expandafter\def\csname r@ax-br-qasper-q3-none-ci\endcsname{[$-$5.5, +7.1]}
\expandafter\def\csname r@ax-br-qasper-q3-none-ci95\endcsname{[$-$5.5, +7.1]}
\expandafter\def\csname r@ax-br-qasper-q3-none-d\endcsname{+0.7}
\expandafter\def\csname r@ax-br-qasper-q3-none-p\endcsname{--}
\expandafter\def\csname r@ax-br-qasper-q3-none-v\endcsname{n.d.}
\expandafter\def\csname r@ax-br-qasper-q3-yes\endcsname{+5.0 [+0.5, +9.7]}
\expandafter\def\csname r@ax-br-qasper-q3-yes-ci\endcsname{[+0.5, +9.7]}
\expandafter\def\csname r@ax-br-qasper-q3-yes-ci95\endcsname{[+0.5, +9.7]}
\expandafter\def\csname r@ax-br-qasper-q3-yes-d\endcsname{+5.0}
\expandafter\def\csname r@ax-br-qasper-q3-yes-p\endcsname{--}
\expandafter\def\csname r@ax-br-qasper-q3-yes-v\endcsname{diff.}
\expandafter\def\csname r@ax-br-qasper-rr-c\endcsname{+4.2 [$-$1.2, +9.3]}
\expandafter\def\csname r@ax-br-qasper-rr-c-ci\endcsname{[$-$1.2, +9.3]}
\expandafter\def\csname r@ax-br-qasper-rr-c-ci95\endcsname{[$-$1.2, +9.3]}
\expandafter\def\csname r@ax-br-qasper-rr-c-d\endcsname{+4.2}
\expandafter\def\csname r@ax-br-qasper-rr-c-p\endcsname{--}
\expandafter\def\csname r@ax-br-qasper-rr-c-v\endcsname{n.d.}
\expandafter\def\csname r@ax-br-qasper-rr-gainshare\endcsname{182}
\expandafter\def\csname r@ax-br-qasper-rr-miss\endcsname{$-$0.6 [$-$3.2, +2.1]}
\expandafter\def\csname r@ax-br-qasper-rr-miss-ci\endcsname{[$-$3.2, +2.1]}
\expandafter\def\csname r@ax-br-qasper-rr-miss-ci95\endcsname{[$-$3.2, +2.1]}
\expandafter\def\csname r@ax-br-qasper-rr-miss-d\endcsname{$-$0.6}
\expandafter\def\csname r@ax-br-qasper-rr-miss-p\endcsname{--}
\expandafter\def\csname r@ax-br-qasper-rr-miss-v\endcsname{n.d.}
\expandafter\def\csname r@ax-br-qasper-rr-none\endcsname{+0.7 [$-$2.4, +4.1]}
\expandafter\def\csname r@ax-br-qasper-rr-none-ci\endcsname{[$-$2.4, +4.1]}
\expandafter\def\csname r@ax-br-qasper-rr-none-ci95\endcsname{[$-$2.4, +4.1]}
\expandafter\def\csname r@ax-br-qasper-rr-none-d\endcsname{+0.7}
\expandafter\def\csname r@ax-br-qasper-rr-none-p\endcsname{--}
\expandafter\def\csname r@ax-br-qasper-rr-none-v\endcsname{n.d.}
\expandafter\def\csname r@ax-br-qasper-rr-yes\endcsname{+3.6 [$-$1.2, +8.3]}
\expandafter\def\csname r@ax-br-qasper-rr-yes-ci\endcsname{[$-$1.2, +8.3]}
\expandafter\def\csname r@ax-br-qasper-rr-yes-ci95\endcsname{[$-$1.2, +8.3]}
\expandafter\def\csname r@ax-br-qasper-rr-yes-d\endcsname{+3.6}
\expandafter\def\csname r@ax-br-qasper-rr-yes-p\endcsname{--}
\expandafter\def\csname r@ax-br-qasper-rr-yes-v\endcsname{n.d.}
\expandafter\def\csname r@ax-br-qasper-share\endcsname{20}
\expandafter\def\csname r@ax-bud-fs-E-CR-bm25-hit@1\endcsname{+0.4 [$-$3.4, +4.7]}
\expandafter\def\csname r@ax-bud-fs-E-CR-bm25-hit@1-ci\endcsname{[$-$3.4, +4.7]}
\expandafter\def\csname r@ax-bud-fs-E-CR-bm25-hit@1-ci95\endcsname{[$-$3.4, +4.7]}
\expandafter\def\csname r@ax-bud-fs-E-CR-bm25-hit@1-d\endcsname{+0.4}
\expandafter\def\csname r@ax-bud-fs-E-CR-bm25-hit@1-p\endcsname{--}
\expandafter\def\csname r@ax-bud-fs-E-CR-bm25-hit@1-v\endcsname{n.d.}
\expandafter\def\csname r@ax-bud-fs-E-CR-bm25-hit@5\endcsname{+3.4 [$-$0.9, +8.1]}
\expandafter\def\csname r@ax-bud-fs-E-CR-bm25-hit@5-ci\endcsname{[$-$0.9, +8.1]}
\expandafter\def\csname r@ax-bud-fs-E-CR-bm25-hit@5-ci95\endcsname{[$-$0.9, +8.1]}
\expandafter\def\csname r@ax-bud-fs-E-CR-bm25-hit@5-d\endcsname{+3.4}
\expandafter\def\csname r@ax-bud-fs-E-CR-bm25-hit@5-p\endcsname{--}
\expandafter\def\csname r@ax-bud-fs-E-CR-bm25-hit@5-v\endcsname{n.d.}
\expandafter\def\csname r@ax-bud-fs-E-CR-bm25-mrr@10\endcsname{+1.9 [$-$1.1, +5.1]}
\expandafter\def\csname r@ax-bud-fs-E-CR-bm25-mrr@10-ci\endcsname{[$-$1.1, +5.1]}
\expandafter\def\csname r@ax-bud-fs-E-CR-bm25-mrr@10-ci95\endcsname{[$-$1.1, +5.1]}
\expandafter\def\csname r@ax-bud-fs-E-CR-bm25-mrr@10-d\endcsname{+1.9}
\expandafter\def\csname r@ax-bud-fs-E-CR-bm25-mrr@10-p\endcsname{--}
\expandafter\def\csname r@ax-bud-fs-E-CR-bm25-mrr@10-v\endcsname{n.d.}
\expandafter\def\csname r@ax-bud-fs-E-CR-bm25-prec@1024t\endcsname{+2.1 [+0.5, +3.9]}
\expandafter\def\csname r@ax-bud-fs-E-CR-bm25-prec@1024t-ci\endcsname{[+0.5, +3.9]}
\expandafter\def\csname r@ax-bud-fs-E-CR-bm25-prec@1024t-ci95\endcsname{[+0.5, +3.9]}
\expandafter\def\csname r@ax-bud-fs-E-CR-bm25-prec@1024t-d\endcsname{+2.1}
\expandafter\def\csname r@ax-bud-fs-E-CR-bm25-prec@1024t-p\endcsname{--}
\expandafter\def\csname r@ax-bud-fs-E-CR-bm25-prec@1024t-v\endcsname{diff.}
\expandafter\def\csname r@ax-bud-fs-E-CR-bm25-prec@2048t\endcsname{+0.9 [$-$0.1, +2.0]}
\expandafter\def\csname r@ax-bud-fs-E-CR-bm25-prec@2048t-ci\endcsname{[$-$0.1, +2.0]}
\expandafter\def\csname r@ax-bud-fs-E-CR-bm25-prec@2048t-ci95\endcsname{[$-$0.1, +2.0]}
\expandafter\def\csname r@ax-bud-fs-E-CR-bm25-prec@2048t-d\endcsname{+0.9}
\expandafter\def\csname r@ax-bud-fs-E-CR-bm25-prec@2048t-p\endcsname{--}
\expandafter\def\csname r@ax-bud-fs-E-CR-bm25-prec@2048t-v\endcsname{n.d.}
\expandafter\def\csname r@ax-bud-fs-E-CR-bm25-prec@512t\endcsname{+2.2 [+0.2, +4.4]}
\expandafter\def\csname r@ax-bud-fs-E-CR-bm25-prec@512t-ci\endcsname{[+0.2, +4.4]}
\expandafter\def\csname r@ax-bud-fs-E-CR-bm25-prec@512t-ci95\endcsname{[+0.2, +4.4]}
\expandafter\def\csname r@ax-bud-fs-E-CR-bm25-prec@512t-d\endcsname{+2.2}
\expandafter\def\csname r@ax-bud-fs-E-CR-bm25-prec@512t-p\endcsname{--}
\expandafter\def\csname r@ax-bud-fs-E-CR-bm25-prec@512t-v\endcsname{diff.}
\expandafter\def\csname r@ax-bud-fs-E-CR-bm25-rec@1024t\endcsname{+0.8 [+0.2, +1.8]}
\expandafter\def\csname r@ax-bud-fs-E-CR-bm25-rec@1024t-ci\endcsname{[+0.2, +1.8]}
\expandafter\def\csname r@ax-bud-fs-E-CR-bm25-rec@1024t-ci95\endcsname{[+0.2, +1.8]}
\expandafter\def\csname r@ax-bud-fs-E-CR-bm25-rec@1024t-d\endcsname{+0.8}
\expandafter\def\csname r@ax-bud-fs-E-CR-bm25-rec@1024t-p\endcsname{--}
\expandafter\def\csname r@ax-bud-fs-E-CR-bm25-rec@1024t-v\endcsname{diff.}
\expandafter\def\csname r@ax-bud-fs-E-CR-hyb-hit@1\endcsname{+1.7 [$-$3.8, +7.2]}
\expandafter\def\csname r@ax-bud-fs-E-CR-hyb-hit@1-ci\endcsname{[$-$3.8, +7.2]}
\expandafter\def\csname r@ax-bud-fs-E-CR-hyb-hit@1-ci95\endcsname{[$-$3.8, +7.2]}
\expandafter\def\csname r@ax-bud-fs-E-CR-hyb-hit@1-d\endcsname{+1.7}
\expandafter\def\csname r@ax-bud-fs-E-CR-hyb-hit@1-p\endcsname{--}
\expandafter\def\csname r@ax-bud-fs-E-CR-hyb-hit@1-v\endcsname{n.d.}
\expandafter\def\csname r@ax-bud-fs-E-CR-hyb-hit@5\endcsname{+3.4 [$-$0.4, +7.2]}
\expandafter\def\csname r@ax-bud-fs-E-CR-hyb-hit@5-ci\endcsname{[$-$0.4, +7.2]}
\expandafter\def\csname r@ax-bud-fs-E-CR-hyb-hit@5-ci95\endcsname{[$-$0.4, +7.2]}
\expandafter\def\csname r@ax-bud-fs-E-CR-hyb-hit@5-d\endcsname{+3.4}
\expandafter\def\csname r@ax-bud-fs-E-CR-hyb-hit@5-p\endcsname{--}
\expandafter\def\csname r@ax-bud-fs-E-CR-hyb-hit@5-v\endcsname{n.d.}
\expandafter\def\csname r@ax-bud-fs-E-CR-hyb-mrr@10\endcsname{+2.2 [$-$1.4, +6.0]}
\expandafter\def\csname r@ax-bud-fs-E-CR-hyb-mrr@10-ci\endcsname{[$-$1.4, +6.0]}
\expandafter\def\csname r@ax-bud-fs-E-CR-hyb-mrr@10-ci95\endcsname{[$-$1.4, +6.0]}
\expandafter\def\csname r@ax-bud-fs-E-CR-hyb-mrr@10-d\endcsname{+2.2}
\expandafter\def\csname r@ax-bud-fs-E-CR-hyb-mrr@10-p\endcsname{--}
\expandafter\def\csname r@ax-bud-fs-E-CR-hyb-mrr@10-v\endcsname{n.d.}
\expandafter\def\csname r@ax-bud-fs-E-CR-hyb-prec@1024t\endcsname{+1.8 [$-$0.1, +3.7]}
\expandafter\def\csname r@ax-bud-fs-E-CR-hyb-prec@1024t-ci\endcsname{[$-$0.1, +3.7]}
\expandafter\def\csname r@ax-bud-fs-E-CR-hyb-prec@1024t-ci95\endcsname{[$-$0.1, +3.7]}
\expandafter\def\csname r@ax-bud-fs-E-CR-hyb-prec@1024t-d\endcsname{+1.8}
\expandafter\def\csname r@ax-bud-fs-E-CR-hyb-prec@1024t-p\endcsname{--}
\expandafter\def\csname r@ax-bud-fs-E-CR-hyb-prec@1024t-v\endcsname{n.d.}
\expandafter\def\csname r@ax-bud-fs-E-CR-hyb-prec@2048t\endcsname{+1.5 [+0.2, +2.9]}
\expandafter\def\csname r@ax-bud-fs-E-CR-hyb-prec@2048t-ci\endcsname{[+0.2, +2.9]}
\expandafter\def\csname r@ax-bud-fs-E-CR-hyb-prec@2048t-ci95\endcsname{[+0.2, +2.9]}
\expandafter\def\csname r@ax-bud-fs-E-CR-hyb-prec@2048t-d\endcsname{+1.5}
\expandafter\def\csname r@ax-bud-fs-E-CR-hyb-prec@2048t-p\endcsname{--}
\expandafter\def\csname r@ax-bud-fs-E-CR-hyb-prec@2048t-v\endcsname{diff.}
\expandafter\def\csname r@ax-bud-fs-E-CR-hyb-prec@512t\endcsname{+1.0 [$-$2.0, +4.3]}
\expandafter\def\csname r@ax-bud-fs-E-CR-hyb-prec@512t-ci\endcsname{[$-$2.0, +4.3]}
\expandafter\def\csname r@ax-bud-fs-E-CR-hyb-prec@512t-ci95\endcsname{[$-$2.0, +4.3]}
\expandafter\def\csname r@ax-bud-fs-E-CR-hyb-prec@512t-d\endcsname{+1.0}
\expandafter\def\csname r@ax-bud-fs-E-CR-hyb-prec@512t-p\endcsname{--}
\expandafter\def\csname r@ax-bud-fs-E-CR-hyb-prec@512t-v\endcsname{n.d.}
\expandafter\def\csname r@ax-bud-fs-E-CR-hyb-rec@1024t\endcsname{+0.4 [$-$0.2, +1.0]}
\expandafter\def\csname r@ax-bud-fs-E-CR-hyb-rec@1024t-ci\endcsname{[$-$0.2, +1.0]}
\expandafter\def\csname r@ax-bud-fs-E-CR-hyb-rec@1024t-ci95\endcsname{[$-$0.2, +1.0]}
\expandafter\def\csname r@ax-bud-fs-E-CR-hyb-rec@1024t-d\endcsname{+0.4}
\expandafter\def\csname r@ax-bud-fs-E-CR-hyb-rec@1024t-p\endcsname{--}
\expandafter\def\csname r@ax-bud-fs-E-CR-hyb-rec@1024t-v\endcsname{n.d.}
\expandafter\def\csname r@ax-bud-fs-E-CR-nomic-hit@1\endcsname{+3.0 [$-$1.7, +8.1]}
\expandafter\def\csname r@ax-bud-fs-E-CR-nomic-hit@1-ci\endcsname{[$-$1.7, +8.1]}
\expandafter\def\csname r@ax-bud-fs-E-CR-nomic-hit@1-ci95\endcsname{[$-$1.7, +8.1]}
\expandafter\def\csname r@ax-bud-fs-E-CR-nomic-hit@1-d\endcsname{+3.0}
\expandafter\def\csname r@ax-bud-fs-E-CR-nomic-hit@1-p\endcsname{--}
\expandafter\def\csname r@ax-bud-fs-E-CR-nomic-hit@1-v\endcsname{n.d.}
\expandafter\def\csname r@ax-bud-fs-E-CR-nomic-hit@5\endcsname{+2.1 [$-$1.3, +6.0]}
\expandafter\def\csname r@ax-bud-fs-E-CR-nomic-hit@5-ci\endcsname{[$-$1.3, +6.0]}
\expandafter\def\csname r@ax-bud-fs-E-CR-nomic-hit@5-ci95\endcsname{[$-$1.3, +6.0]}
\expandafter\def\csname r@ax-bud-fs-E-CR-nomic-hit@5-d\endcsname{+2.1}
\expandafter\def\csname r@ax-bud-fs-E-CR-nomic-hit@5-p\endcsname{--}
\expandafter\def\csname r@ax-bud-fs-E-CR-nomic-hit@5-v\endcsname{n.d.}
\expandafter\def\csname r@ax-bud-fs-E-CR-nomic-mrr@10\endcsname{+3.2 [$-$0.1, +6.8]}
\expandafter\def\csname r@ax-bud-fs-E-CR-nomic-mrr@10-ci\endcsname{[$-$0.1, +6.8]}
\expandafter\def\csname r@ax-bud-fs-E-CR-nomic-mrr@10-ci95\endcsname{[$-$0.1, +6.8]}
\expandafter\def\csname r@ax-bud-fs-E-CR-nomic-mrr@10-d\endcsname{+3.2}
\expandafter\def\csname r@ax-bud-fs-E-CR-nomic-mrr@10-p\endcsname{--}
\expandafter\def\csname r@ax-bud-fs-E-CR-nomic-mrr@10-v\endcsname{n.d.}
\expandafter\def\csname r@ax-bud-fs-E-CR-nomic-prec@1024t\endcsname{+2.2 [+0.3, +4.3]}
\expandafter\def\csname r@ax-bud-fs-E-CR-nomic-prec@1024t-ci\endcsname{[+0.3, +4.3]}
\expandafter\def\csname r@ax-bud-fs-E-CR-nomic-prec@1024t-ci95\endcsname{[+0.3, +4.3]}
\expandafter\def\csname r@ax-bud-fs-E-CR-nomic-prec@1024t-d\endcsname{+2.2}
\expandafter\def\csname r@ax-bud-fs-E-CR-nomic-prec@1024t-p\endcsname{--}
\expandafter\def\csname r@ax-bud-fs-E-CR-nomic-prec@1024t-v\endcsname{diff.}
\expandafter\def\csname r@ax-bud-fs-E-CR-nomic-prec@2048t\endcsname{+1.2 [$-$0.1, +2.4]}
\expandafter\def\csname r@ax-bud-fs-E-CR-nomic-prec@2048t-ci\endcsname{[$-$0.1, +2.4]}
\expandafter\def\csname r@ax-bud-fs-E-CR-nomic-prec@2048t-ci95\endcsname{[$-$0.1, +2.4]}
\expandafter\def\csname r@ax-bud-fs-E-CR-nomic-prec@2048t-d\endcsname{+1.2}
\expandafter\def\csname r@ax-bud-fs-E-CR-nomic-prec@2048t-p\endcsname{--}
\expandafter\def\csname r@ax-bud-fs-E-CR-nomic-prec@2048t-v\endcsname{n.d.}
\expandafter\def\csname r@ax-bud-fs-E-CR-nomic-prec@512t\endcsname{+2.6 [$-$0.2, +5.3]}
\expandafter\def\csname r@ax-bud-fs-E-CR-nomic-prec@512t-ci\endcsname{[$-$0.2, +5.3]}
\expandafter\def\csname r@ax-bud-fs-E-CR-nomic-prec@512t-ci95\endcsname{[$-$0.2, +5.3]}
\expandafter\def\csname r@ax-bud-fs-E-CR-nomic-prec@512t-d\endcsname{+2.6}
\expandafter\def\csname r@ax-bud-fs-E-CR-nomic-prec@512t-p\endcsname{--}
\expandafter\def\csname r@ax-bud-fs-E-CR-nomic-prec@512t-v\endcsname{n.d.}
\expandafter\def\csname r@ax-bud-fs-E-CR-nomic-rec@1024t\endcsname{+0.5 [$-$0.0, +1.0]}
\expandafter\def\csname r@ax-bud-fs-E-CR-nomic-rec@1024t-ci\endcsname{[$-$0.0, +1.0]}
\expandafter\def\csname r@ax-bud-fs-E-CR-nomic-rec@1024t-ci95\endcsname{[$-$0.0, +1.0]}
\expandafter\def\csname r@ax-bud-fs-E-CR-nomic-rec@1024t-d\endcsname{+0.5}
\expandafter\def\csname r@ax-bud-fs-E-CR-nomic-rec@1024t-p\endcsname{--}
\expandafter\def\csname r@ax-bud-fs-E-CR-nomic-rec@1024t-v\endcsname{n.d.}
\expandafter\def\csname r@ax-bud-fs-E-CR-q3-hit@1\endcsname{+3.0 [$-$2.1, +8.5]}
\expandafter\def\csname r@ax-bud-fs-E-CR-q3-hit@1-ci\endcsname{[$-$2.1, +8.5]}
\expandafter\def\csname r@ax-bud-fs-E-CR-q3-hit@1-ci95\endcsname{[$-$2.1, +8.5]}
\expandafter\def\csname r@ax-bud-fs-E-CR-q3-hit@1-d\endcsname{+3.0}
\expandafter\def\csname r@ax-bud-fs-E-CR-q3-hit@1-p\endcsname{--}
\expandafter\def\csname r@ax-bud-fs-E-CR-q3-hit@1-v\endcsname{n.d.}
\expandafter\def\csname r@ax-bud-fs-E-CR-q3-hit@5\endcsname{+2.6 [$-$0.9, +6.0]}
\expandafter\def\csname r@ax-bud-fs-E-CR-q3-hit@5-ci\endcsname{[$-$0.9, +6.0]}
\expandafter\def\csname r@ax-bud-fs-E-CR-q3-hit@5-ci95\endcsname{[$-$0.9, +6.0]}
\expandafter\def\csname r@ax-bud-fs-E-CR-q3-hit@5-d\endcsname{+2.6}
\expandafter\def\csname r@ax-bud-fs-E-CR-q3-hit@5-p\endcsname{--}
\expandafter\def\csname r@ax-bud-fs-E-CR-q3-hit@5-v\endcsname{n.d.}
\expandafter\def\csname r@ax-bud-fs-E-CR-q3-mrr@10\endcsname{+2.7 [$-$0.8, +6.4]}
\expandafter\def\csname r@ax-bud-fs-E-CR-q3-mrr@10-ci\endcsname{[$-$0.8, +6.4]}
\expandafter\def\csname r@ax-bud-fs-E-CR-q3-mrr@10-ci95\endcsname{[$-$0.8, +6.4]}
\expandafter\def\csname r@ax-bud-fs-E-CR-q3-mrr@10-d\endcsname{+2.7}
\expandafter\def\csname r@ax-bud-fs-E-CR-q3-mrr@10-p\endcsname{--}
\expandafter\def\csname r@ax-bud-fs-E-CR-q3-mrr@10-v\endcsname{n.d.}
\expandafter\def\csname r@ax-bud-fs-E-CR-q3-prec@1024t\endcsname{$-$0.6 [$-$2.8, +1.5]}
\expandafter\def\csname r@ax-bud-fs-E-CR-q3-prec@1024t-ci\endcsname{[$-$2.8, +1.5]}
\expandafter\def\csname r@ax-bud-fs-E-CR-q3-prec@1024t-ci95\endcsname{[$-$2.8, +1.5]}
\expandafter\def\csname r@ax-bud-fs-E-CR-q3-prec@1024t-d\endcsname{$-$0.6}
\expandafter\def\csname r@ax-bud-fs-E-CR-q3-prec@1024t-p\endcsname{--}
\expandafter\def\csname r@ax-bud-fs-E-CR-q3-prec@1024t-v\endcsname{n.d.}
\expandafter\def\csname r@ax-bud-fs-E-CR-q3-prec@2048t\endcsname{$-$1.1 [$-$2.7, +0.4]}
\expandafter\def\csname r@ax-bud-fs-E-CR-q3-prec@2048t-ci\endcsname{[$-$2.7, +0.4]}
\expandafter\def\csname r@ax-bud-fs-E-CR-q3-prec@2048t-ci95\endcsname{[$-$2.7, +0.4]}
\expandafter\def\csname r@ax-bud-fs-E-CR-q3-prec@2048t-d\endcsname{$-$1.1}
\expandafter\def\csname r@ax-bud-fs-E-CR-q3-prec@2048t-p\endcsname{--}
\expandafter\def\csname r@ax-bud-fs-E-CR-q3-prec@2048t-v\endcsname{n.d.}
\expandafter\def\csname r@ax-bud-fs-E-CR-q3-prec@512t\endcsname{+2.0 [$-$0.6, +4.6]}
\expandafter\def\csname r@ax-bud-fs-E-CR-q3-prec@512t-ci\endcsname{[$-$0.6, +4.6]}
\expandafter\def\csname r@ax-bud-fs-E-CR-q3-prec@512t-ci95\endcsname{[$-$0.6, +4.6]}
\expandafter\def\csname r@ax-bud-fs-E-CR-q3-prec@512t-d\endcsname{+2.0}
\expandafter\def\csname r@ax-bud-fs-E-CR-q3-prec@512t-p\endcsname{--}
\expandafter\def\csname r@ax-bud-fs-E-CR-q3-prec@512t-v\endcsname{n.d.}
\expandafter\def\csname r@ax-bud-fs-E-CR-q3-rec@1024t\endcsname{$-$0.2 [$-$0.9, +0.4]}
\expandafter\def\csname r@ax-bud-fs-E-CR-q3-rec@1024t-ci\endcsname{[$-$0.9, +0.4]}
\expandafter\def\csname r@ax-bud-fs-E-CR-q3-rec@1024t-ci95\endcsname{[$-$0.9, +0.4]}
\expandafter\def\csname r@ax-bud-fs-E-CR-q3-rec@1024t-d\endcsname{$-$0.2}
\expandafter\def\csname r@ax-bud-fs-E-CR-q3-rec@1024t-p\endcsname{--}
\expandafter\def\csname r@ax-bud-fs-E-CR-q3-rec@1024t-v\endcsname{n.d.}
\expandafter\def\csname r@ax-bud-fs-E-CR-rr-hit@1\endcsname{+0.9 [$-$4.3, +6.0]}
\expandafter\def\csname r@ax-bud-fs-E-CR-rr-hit@1-ci\endcsname{[$-$4.3, +6.0]}
\expandafter\def\csname r@ax-bud-fs-E-CR-rr-hit@1-ci95\endcsname{[$-$4.3, +6.0]}
\expandafter\def\csname r@ax-bud-fs-E-CR-rr-hit@1-d\endcsname{+0.9}
\expandafter\def\csname r@ax-bud-fs-E-CR-rr-hit@1-p\endcsname{--}
\expandafter\def\csname r@ax-bud-fs-E-CR-rr-hit@1-v\endcsname{n.d.}
\expandafter\def\csname r@ax-bud-fs-E-CR-rr-hit@5\endcsname{+0.9 [$-$3.4, +5.1]}
\expandafter\def\csname r@ax-bud-fs-E-CR-rr-hit@5-ci\endcsname{[$-$3.4, +5.1]}
\expandafter\def\csname r@ax-bud-fs-E-CR-rr-hit@5-ci95\endcsname{[$-$3.4, +5.1]}
\expandafter\def\csname r@ax-bud-fs-E-CR-rr-hit@5-d\endcsname{+0.9}
\expandafter\def\csname r@ax-bud-fs-E-CR-rr-hit@5-p\endcsname{--}
\expandafter\def\csname r@ax-bud-fs-E-CR-rr-hit@5-v\endcsname{n.d.}
\expandafter\def\csname r@ax-bud-fs-E-CR-rr-mrr@10\endcsname{+1.5 [$-$2.2, +5.0]}
\expandafter\def\csname r@ax-bud-fs-E-CR-rr-mrr@10-ci\endcsname{[$-$2.2, +5.0]}
\expandafter\def\csname r@ax-bud-fs-E-CR-rr-mrr@10-ci95\endcsname{[$-$2.2, +5.0]}
\expandafter\def\csname r@ax-bud-fs-E-CR-rr-mrr@10-d\endcsname{+1.5}
\expandafter\def\csname r@ax-bud-fs-E-CR-rr-mrr@10-p\endcsname{--}
\expandafter\def\csname r@ax-bud-fs-E-CR-rr-mrr@10-v\endcsname{n.d.}
\expandafter\def\csname r@ax-bud-fs-E-CR-rr-prec@1024t\endcsname{+0.9 [$-$1.4, +3.5]}
\expandafter\def\csname r@ax-bud-fs-E-CR-rr-prec@1024t-ci\endcsname{[$-$1.4, +3.5]}
\expandafter\def\csname r@ax-bud-fs-E-CR-rr-prec@1024t-ci95\endcsname{[$-$1.4, +3.5]}
\expandafter\def\csname r@ax-bud-fs-E-CR-rr-prec@1024t-d\endcsname{+0.9}
\expandafter\def\csname r@ax-bud-fs-E-CR-rr-prec@1024t-p\endcsname{--}
\expandafter\def\csname r@ax-bud-fs-E-CR-rr-prec@1024t-v\endcsname{n.d.}
\expandafter\def\csname r@ax-bud-fs-E-CR-rr-prec@2048t\endcsname{+0.9 [$-$0.5, +2.3]}
\expandafter\def\csname r@ax-bud-fs-E-CR-rr-prec@2048t-ci\endcsname{[$-$0.5, +2.3]}
\expandafter\def\csname r@ax-bud-fs-E-CR-rr-prec@2048t-ci95\endcsname{[$-$0.5, +2.3]}
\expandafter\def\csname r@ax-bud-fs-E-CR-rr-prec@2048t-d\endcsname{+0.9}
\expandafter\def\csname r@ax-bud-fs-E-CR-rr-prec@2048t-p\endcsname{--}
\expandafter\def\csname r@ax-bud-fs-E-CR-rr-prec@2048t-v\endcsname{n.d.}
\expandafter\def\csname r@ax-bud-fs-E-CR-rr-prec@512t\endcsname{+2.1 [$-$0.6, +5.2]}
\expandafter\def\csname r@ax-bud-fs-E-CR-rr-prec@512t-ci\endcsname{[$-$0.6, +5.2]}
\expandafter\def\csname r@ax-bud-fs-E-CR-rr-prec@512t-ci95\endcsname{[$-$0.6, +5.2]}
\expandafter\def\csname r@ax-bud-fs-E-CR-rr-prec@512t-d\endcsname{+2.1}
\expandafter\def\csname r@ax-bud-fs-E-CR-rr-prec@512t-p\endcsname{--}
\expandafter\def\csname r@ax-bud-fs-E-CR-rr-prec@512t-v\endcsname{n.d.}
\expandafter\def\csname r@ax-bud-fs-E-CR-rr-rec@1024t\endcsname{+0.2 [$-$0.5, +0.9]}
\expandafter\def\csname r@ax-bud-fs-E-CR-rr-rec@1024t-ci\endcsname{[$-$0.5, +0.9]}
\expandafter\def\csname r@ax-bud-fs-E-CR-rr-rec@1024t-ci95\endcsname{[$-$0.5, +0.9]}
\expandafter\def\csname r@ax-bud-fs-E-CR-rr-rec@1024t-d\endcsname{+0.2}
\expandafter\def\csname r@ax-bud-fs-E-CR-rr-rec@1024t-p\endcsname{--}
\expandafter\def\csname r@ax-bud-fs-E-CR-rr-rec@1024t-v\endcsname{n.d.}
\expandafter\def\csname r@ax-bud-fs-E-SpT-bm25-hit@1\endcsname{+1.3 [$-$3.4, +6.0]}
\expandafter\def\csname r@ax-bud-fs-E-SpT-bm25-hit@1-ci\endcsname{[$-$3.4, +6.0]}
\expandafter\def\csname r@ax-bud-fs-E-SpT-bm25-hit@1-ci95\endcsname{[$-$3.4, +6.0]}
\expandafter\def\csname r@ax-bud-fs-E-SpT-bm25-hit@1-d\endcsname{+1.3}
\expandafter\def\csname r@ax-bud-fs-E-SpT-bm25-hit@1-p\endcsname{--}
\expandafter\def\csname r@ax-bud-fs-E-SpT-bm25-hit@1-v\endcsname{n.d.}
\expandafter\def\csname r@ax-bud-fs-E-SpT-bm25-hit@5\endcsname{+1.7 [$-$2.6, +6.0]}
\expandafter\def\csname r@ax-bud-fs-E-SpT-bm25-hit@5-ci\endcsname{[$-$2.6, +6.0]}
\expandafter\def\csname r@ax-bud-fs-E-SpT-bm25-hit@5-ci95\endcsname{[$-$2.6, +6.0]}
\expandafter\def\csname r@ax-bud-fs-E-SpT-bm25-hit@5-d\endcsname{+1.7}
\expandafter\def\csname r@ax-bud-fs-E-SpT-bm25-hit@5-p\endcsname{--}
\expandafter\def\csname r@ax-bud-fs-E-SpT-bm25-hit@5-v\endcsname{n.d.}
\expandafter\def\csname r@ax-bud-fs-E-SpT-bm25-mrr@10\endcsname{+1.9 [$-$1.3, +5.2]}
\expandafter\def\csname r@ax-bud-fs-E-SpT-bm25-mrr@10-ci\endcsname{[$-$1.3, +5.2]}
\expandafter\def\csname r@ax-bud-fs-E-SpT-bm25-mrr@10-ci95\endcsname{[$-$1.3, +5.2]}
\expandafter\def\csname r@ax-bud-fs-E-SpT-bm25-mrr@10-d\endcsname{+1.9}
\expandafter\def\csname r@ax-bud-fs-E-SpT-bm25-mrr@10-p\endcsname{--}
\expandafter\def\csname r@ax-bud-fs-E-SpT-bm25-mrr@10-v\endcsname{n.d.}
\expandafter\def\csname r@ax-bud-fs-E-SpT-bm25-prec@1024t\endcsname{+2.4 [+0.9, +4.3]}
\expandafter\def\csname r@ax-bud-fs-E-SpT-bm25-prec@1024t-ci\endcsname{[+0.9, +4.3]}
\expandafter\def\csname r@ax-bud-fs-E-SpT-bm25-prec@1024t-ci95\endcsname{[+0.9, +4.3]}
\expandafter\def\csname r@ax-bud-fs-E-SpT-bm25-prec@1024t-d\endcsname{+2.4}
\expandafter\def\csname r@ax-bud-fs-E-SpT-bm25-prec@1024t-p\endcsname{--}
\expandafter\def\csname r@ax-bud-fs-E-SpT-bm25-prec@1024t-v\endcsname{diff.}
\expandafter\def\csname r@ax-bud-fs-E-SpT-bm25-prec@2048t\endcsname{+1.3 [+0.0, +2.7]}
\expandafter\def\csname r@ax-bud-fs-E-SpT-bm25-prec@2048t-ci\endcsname{[+0.0, +2.7]}
\expandafter\def\csname r@ax-bud-fs-E-SpT-bm25-prec@2048t-ci95\endcsname{[+0.0, +2.7]}
\expandafter\def\csname r@ax-bud-fs-E-SpT-bm25-prec@2048t-d\endcsname{+1.3}
\expandafter\def\csname r@ax-bud-fs-E-SpT-bm25-prec@2048t-p\endcsname{--}
\expandafter\def\csname r@ax-bud-fs-E-SpT-bm25-prec@2048t-v\endcsname{diff.}
\expandafter\def\csname r@ax-bud-fs-E-SpT-bm25-prec@512t\endcsname{+1.6 [$-$0.4, +3.8]}
\expandafter\def\csname r@ax-bud-fs-E-SpT-bm25-prec@512t-ci\endcsname{[$-$0.4, +3.8]}
\expandafter\def\csname r@ax-bud-fs-E-SpT-bm25-prec@512t-ci95\endcsname{[$-$0.4, +3.8]}
\expandafter\def\csname r@ax-bud-fs-E-SpT-bm25-prec@512t-d\endcsname{+1.6}
\expandafter\def\csname r@ax-bud-fs-E-SpT-bm25-prec@512t-p\endcsname{--}
\expandafter\def\csname r@ax-bud-fs-E-SpT-bm25-prec@512t-v\endcsname{n.d.}
\expandafter\def\csname r@ax-bud-fs-E-SpT-bm25-rec@1024t\endcsname{+0.9 [+0.4, +1.5]}
\expandafter\def\csname r@ax-bud-fs-E-SpT-bm25-rec@1024t-ci\endcsname{[+0.4, +1.5]}
\expandafter\def\csname r@ax-bud-fs-E-SpT-bm25-rec@1024t-ci95\endcsname{[+0.4, +1.5]}
\expandafter\def\csname r@ax-bud-fs-E-SpT-bm25-rec@1024t-d\endcsname{+0.9}
\expandafter\def\csname r@ax-bud-fs-E-SpT-bm25-rec@1024t-p\endcsname{--}
\expandafter\def\csname r@ax-bud-fs-E-SpT-bm25-rec@1024t-v\endcsname{diff.}
\expandafter\def\csname r@ax-bud-fs-E-SpT-hyb-hit@1\endcsname{+2.6 [$-$3.4, +8.5]}
\expandafter\def\csname r@ax-bud-fs-E-SpT-hyb-hit@1-ci\endcsname{[$-$3.4, +8.5]}
\expandafter\def\csname r@ax-bud-fs-E-SpT-hyb-hit@1-ci95\endcsname{[$-$3.4, +8.5]}
\expandafter\def\csname r@ax-bud-fs-E-SpT-hyb-hit@1-d\endcsname{+2.6}
\expandafter\def\csname r@ax-bud-fs-E-SpT-hyb-hit@1-p\endcsname{--}
\expandafter\def\csname r@ax-bud-fs-E-SpT-hyb-hit@1-v\endcsname{n.d.}
\expandafter\def\csname r@ax-bud-fs-E-SpT-hyb-hit@5\endcsname{+2.1 [$-$2.1, +6.8]}
\expandafter\def\csname r@ax-bud-fs-E-SpT-hyb-hit@5-ci\endcsname{[$-$2.1, +6.8]}
\expandafter\def\csname r@ax-bud-fs-E-SpT-hyb-hit@5-ci95\endcsname{[$-$2.1, +6.8]}
\expandafter\def\csname r@ax-bud-fs-E-SpT-hyb-hit@5-d\endcsname{+2.1}
\expandafter\def\csname r@ax-bud-fs-E-SpT-hyb-hit@5-p\endcsname{--}
\expandafter\def\csname r@ax-bud-fs-E-SpT-hyb-hit@5-v\endcsname{n.d.}
\expandafter\def\csname r@ax-bud-fs-E-SpT-hyb-mrr@10\endcsname{+2.7 [$-$1.3, +6.7]}
\expandafter\def\csname r@ax-bud-fs-E-SpT-hyb-mrr@10-ci\endcsname{[$-$1.3, +6.7]}
\expandafter\def\csname r@ax-bud-fs-E-SpT-hyb-mrr@10-ci95\endcsname{[$-$1.3, +6.7]}
\expandafter\def\csname r@ax-bud-fs-E-SpT-hyb-mrr@10-d\endcsname{+2.7}
\expandafter\def\csname r@ax-bud-fs-E-SpT-hyb-mrr@10-p\endcsname{--}
\expandafter\def\csname r@ax-bud-fs-E-SpT-hyb-mrr@10-v\endcsname{n.d.}
\expandafter\def\csname r@ax-bud-fs-E-SpT-hyb-prec@1024t\endcsname{+2.7 [+0.5, +5.1]}
\expandafter\def\csname r@ax-bud-fs-E-SpT-hyb-prec@1024t-ci\endcsname{[+0.5, +5.1]}
\expandafter\def\csname r@ax-bud-fs-E-SpT-hyb-prec@1024t-ci95\endcsname{[+0.5, +5.1]}
\expandafter\def\csname r@ax-bud-fs-E-SpT-hyb-prec@1024t-d\endcsname{+2.7}
\expandafter\def\csname r@ax-bud-fs-E-SpT-hyb-prec@1024t-p\endcsname{--}
\expandafter\def\csname r@ax-bud-fs-E-SpT-hyb-prec@1024t-v\endcsname{diff.}
\expandafter\def\csname r@ax-bud-fs-E-SpT-hyb-prec@2048t\endcsname{+2.3 [+0.8, +3.8]}
\expandafter\def\csname r@ax-bud-fs-E-SpT-hyb-prec@2048t-ci\endcsname{[+0.8, +3.8]}
\expandafter\def\csname r@ax-bud-fs-E-SpT-hyb-prec@2048t-ci95\endcsname{[+0.8, +3.8]}
\expandafter\def\csname r@ax-bud-fs-E-SpT-hyb-prec@2048t-d\endcsname{+2.3}
\expandafter\def\csname r@ax-bud-fs-E-SpT-hyb-prec@2048t-p\endcsname{--}
\expandafter\def\csname r@ax-bud-fs-E-SpT-hyb-prec@2048t-v\endcsname{diff.}
\expandafter\def\csname r@ax-bud-fs-E-SpT-hyb-prec@512t\endcsname{+1.5 [$-$1.5, +4.7]}
\expandafter\def\csname r@ax-bud-fs-E-SpT-hyb-prec@512t-ci\endcsname{[$-$1.5, +4.7]}
\expandafter\def\csname r@ax-bud-fs-E-SpT-hyb-prec@512t-ci95\endcsname{[$-$1.5, +4.7]}
\expandafter\def\csname r@ax-bud-fs-E-SpT-hyb-prec@512t-d\endcsname{+1.5}
\expandafter\def\csname r@ax-bud-fs-E-SpT-hyb-prec@512t-p\endcsname{--}
\expandafter\def\csname r@ax-bud-fs-E-SpT-hyb-prec@512t-v\endcsname{n.d.}
\expandafter\def\csname r@ax-bud-fs-E-SpT-hyb-rec@1024t\endcsname{+0.6 [$-$0.1, +1.3]}
\expandafter\def\csname r@ax-bud-fs-E-SpT-hyb-rec@1024t-ci\endcsname{[$-$0.1, +1.3]}
\expandafter\def\csname r@ax-bud-fs-E-SpT-hyb-rec@1024t-ci95\endcsname{[$-$0.1, +1.3]}
\expandafter\def\csname r@ax-bud-fs-E-SpT-hyb-rec@1024t-d\endcsname{+0.6}
\expandafter\def\csname r@ax-bud-fs-E-SpT-hyb-rec@1024t-p\endcsname{--}
\expandafter\def\csname r@ax-bud-fs-E-SpT-hyb-rec@1024t-v\endcsname{n.d.}
\expandafter\def\csname r@ax-bud-fs-E-SpT-nomic-hit@1\endcsname{+1.7 [$-$3.8, +7.7]}
\expandafter\def\csname r@ax-bud-fs-E-SpT-nomic-hit@1-ci\endcsname{[$-$3.8, +7.7]}
\expandafter\def\csname r@ax-bud-fs-E-SpT-nomic-hit@1-ci95\endcsname{[$-$3.8, +7.7]}
\expandafter\def\csname r@ax-bud-fs-E-SpT-nomic-hit@1-d\endcsname{+1.7}
\expandafter\def\csname r@ax-bud-fs-E-SpT-nomic-hit@1-p\endcsname{--}
\expandafter\def\csname r@ax-bud-fs-E-SpT-nomic-hit@1-v\endcsname{n.d.}
\expandafter\def\csname r@ax-bud-fs-E-SpT-nomic-hit@5\endcsname{+5.5 [+0.9, +10.6]}
\expandafter\def\csname r@ax-bud-fs-E-SpT-nomic-hit@5-ci\endcsname{[+0.9, +10.6]}
\expandafter\def\csname r@ax-bud-fs-E-SpT-nomic-hit@5-ci95\endcsname{[+0.9, +10.6]}
\expandafter\def\csname r@ax-bud-fs-E-SpT-nomic-hit@5-d\endcsname{+5.5}
\expandafter\def\csname r@ax-bud-fs-E-SpT-nomic-hit@5-p\endcsname{--}
\expandafter\def\csname r@ax-bud-fs-E-SpT-nomic-hit@5-v\endcsname{diff.}
\expandafter\def\csname r@ax-bud-fs-E-SpT-nomic-mrr@10\endcsname{+2.8 [$-$1.0, +7.0]}
\expandafter\def\csname r@ax-bud-fs-E-SpT-nomic-mrr@10-ci\endcsname{[$-$1.0, +7.0]}
\expandafter\def\csname r@ax-bud-fs-E-SpT-nomic-mrr@10-ci95\endcsname{[$-$1.0, +7.0]}
\expandafter\def\csname r@ax-bud-fs-E-SpT-nomic-mrr@10-d\endcsname{+2.8}
\expandafter\def\csname r@ax-bud-fs-E-SpT-nomic-mrr@10-p\endcsname{--}
\expandafter\def\csname r@ax-bud-fs-E-SpT-nomic-mrr@10-v\endcsname{n.d.}
\expandafter\def\csname r@ax-bud-fs-E-SpT-nomic-prec@1024t\endcsname{+2.6 [+0.3, +5.0]}
\expandafter\def\csname r@ax-bud-fs-E-SpT-nomic-prec@1024t-ci\endcsname{[+0.3, +5.0]}
\expandafter\def\csname r@ax-bud-fs-E-SpT-nomic-prec@1024t-ci95\endcsname{[+0.3, +5.0]}
\expandafter\def\csname r@ax-bud-fs-E-SpT-nomic-prec@1024t-d\endcsname{+2.6}
\expandafter\def\csname r@ax-bud-fs-E-SpT-nomic-prec@1024t-p\endcsname{--}
\expandafter\def\csname r@ax-bud-fs-E-SpT-nomic-prec@1024t-v\endcsname{diff.}
\expandafter\def\csname r@ax-bud-fs-E-SpT-nomic-prec@2048t\endcsname{+0.8 [$-$0.9, +2.4]}
\expandafter\def\csname r@ax-bud-fs-E-SpT-nomic-prec@2048t-ci\endcsname{[$-$0.9, +2.4]}
\expandafter\def\csname r@ax-bud-fs-E-SpT-nomic-prec@2048t-ci95\endcsname{[$-$0.9, +2.4]}
\expandafter\def\csname r@ax-bud-fs-E-SpT-nomic-prec@2048t-d\endcsname{+0.8}
\expandafter\def\csname r@ax-bud-fs-E-SpT-nomic-prec@2048t-p\endcsname{--}
\expandafter\def\csname r@ax-bud-fs-E-SpT-nomic-prec@2048t-v\endcsname{n.d.}
\expandafter\def\csname r@ax-bud-fs-E-SpT-nomic-prec@512t\endcsname{+3.1 [$-$0.1, +6.1]}
\expandafter\def\csname r@ax-bud-fs-E-SpT-nomic-prec@512t-ci\endcsname{[$-$0.1, +6.1]}
\expandafter\def\csname r@ax-bud-fs-E-SpT-nomic-prec@512t-ci95\endcsname{[$-$0.1, +6.1]}
\expandafter\def\csname r@ax-bud-fs-E-SpT-nomic-prec@512t-d\endcsname{+3.1}
\expandafter\def\csname r@ax-bud-fs-E-SpT-nomic-prec@512t-p\endcsname{--}
\expandafter\def\csname r@ax-bud-fs-E-SpT-nomic-prec@512t-v\endcsname{n.d.}
\expandafter\def\csname r@ax-bud-fs-E-SpT-nomic-rec@1024t\endcsname{+0.8 [+0.1, +1.5]}
\expandafter\def\csname r@ax-bud-fs-E-SpT-nomic-rec@1024t-ci\endcsname{[+0.1, +1.5]}
\expandafter\def\csname r@ax-bud-fs-E-SpT-nomic-rec@1024t-ci95\endcsname{[+0.1, +1.5]}
\expandafter\def\csname r@ax-bud-fs-E-SpT-nomic-rec@1024t-d\endcsname{+0.8}
\expandafter\def\csname r@ax-bud-fs-E-SpT-nomic-rec@1024t-p\endcsname{--}
\expandafter\def\csname r@ax-bud-fs-E-SpT-nomic-rec@1024t-v\endcsname{diff.}
\expandafter\def\csname r@ax-bud-fs-E-SpT-q3-hit@1\endcsname{+0.0 [$-$4.7, +4.7]}
\expandafter\def\csname r@ax-bud-fs-E-SpT-q3-hit@1-ci\endcsname{[$-$4.7, +4.7]}
\expandafter\def\csname r@ax-bud-fs-E-SpT-q3-hit@1-ci95\endcsname{[$-$4.7, +4.7]}
\expandafter\def\csname r@ax-bud-fs-E-SpT-q3-hit@1-d\endcsname{+0.0}
\expandafter\def\csname r@ax-bud-fs-E-SpT-q3-hit@1-p\endcsname{--}
\expandafter\def\csname r@ax-bud-fs-E-SpT-q3-hit@1-v\endcsname{n.d.}
\expandafter\def\csname r@ax-bud-fs-E-SpT-q3-hit@5\endcsname{+2.1 [$-$1.3, +5.5]}
\expandafter\def\csname r@ax-bud-fs-E-SpT-q3-hit@5-ci\endcsname{[$-$1.3, +5.5]}
\expandafter\def\csname r@ax-bud-fs-E-SpT-q3-hit@5-ci95\endcsname{[$-$1.3, +5.5]}
\expandafter\def\csname r@ax-bud-fs-E-SpT-q3-hit@5-d\endcsname{+2.1}
\expandafter\def\csname r@ax-bud-fs-E-SpT-q3-hit@5-p\endcsname{--}
\expandafter\def\csname r@ax-bud-fs-E-SpT-q3-hit@5-v\endcsname{n.d.}
\expandafter\def\csname r@ax-bud-fs-E-SpT-q3-mrr@10\endcsname{+1.0 [$-$2.1, +4.2]}
\expandafter\def\csname r@ax-bud-fs-E-SpT-q3-mrr@10-ci\endcsname{[$-$2.1, +4.2]}
\expandafter\def\csname r@ax-bud-fs-E-SpT-q3-mrr@10-ci95\endcsname{[$-$2.1, +4.2]}
\expandafter\def\csname r@ax-bud-fs-E-SpT-q3-mrr@10-d\endcsname{+1.0}
\expandafter\def\csname r@ax-bud-fs-E-SpT-q3-mrr@10-p\endcsname{--}
\expandafter\def\csname r@ax-bud-fs-E-SpT-q3-mrr@10-v\endcsname{n.d.}
\expandafter\def\csname r@ax-bud-fs-E-SpT-q3-prec@1024t\endcsname{+0.3 [$-$1.4, +2.0]}
\expandafter\def\csname r@ax-bud-fs-E-SpT-q3-prec@1024t-ci\endcsname{[$-$1.4, +2.0]}
\expandafter\def\csname r@ax-bud-fs-E-SpT-q3-prec@1024t-ci95\endcsname{[$-$1.4, +2.0]}
\expandafter\def\csname r@ax-bud-fs-E-SpT-q3-prec@1024t-d\endcsname{+0.3}
\expandafter\def\csname r@ax-bud-fs-E-SpT-q3-prec@1024t-p\endcsname{--}
\expandafter\def\csname r@ax-bud-fs-E-SpT-q3-prec@1024t-v\endcsname{n.d.}
\expandafter\def\csname r@ax-bud-fs-E-SpT-q3-prec@2048t\endcsname{+0.6 [$-$0.8, +2.0]}
\expandafter\def\csname r@ax-bud-fs-E-SpT-q3-prec@2048t-ci\endcsname{[$-$0.8, +2.0]}
\expandafter\def\csname r@ax-bud-fs-E-SpT-q3-prec@2048t-ci95\endcsname{[$-$0.8, +2.0]}
\expandafter\def\csname r@ax-bud-fs-E-SpT-q3-prec@2048t-d\endcsname{+0.6}
\expandafter\def\csname r@ax-bud-fs-E-SpT-q3-prec@2048t-p\endcsname{--}
\expandafter\def\csname r@ax-bud-fs-E-SpT-q3-prec@2048t-v\endcsname{n.d.}
\expandafter\def\csname r@ax-bud-fs-E-SpT-q3-prec@512t\endcsname{+0.1 [$-$2.2, +2.6]}
\expandafter\def\csname r@ax-bud-fs-E-SpT-q3-prec@512t-ci\endcsname{[$-$2.2, +2.6]}
\expandafter\def\csname r@ax-bud-fs-E-SpT-q3-prec@512t-ci95\endcsname{[$-$2.2, +2.6]}
\expandafter\def\csname r@ax-bud-fs-E-SpT-q3-prec@512t-d\endcsname{+0.1}
\expandafter\def\csname r@ax-bud-fs-E-SpT-q3-prec@512t-p\endcsname{--}
\expandafter\def\csname r@ax-bud-fs-E-SpT-q3-prec@512t-v\endcsname{n.d.}
\expandafter\def\csname r@ax-bud-fs-E-SpT-q3-rec@1024t\endcsname{+0.2 [$-$0.3, +0.8]}
\expandafter\def\csname r@ax-bud-fs-E-SpT-q3-rec@1024t-ci\endcsname{[$-$0.3, +0.8]}
\expandafter\def\csname r@ax-bud-fs-E-SpT-q3-rec@1024t-ci95\endcsname{[$-$0.3, +0.8]}
\expandafter\def\csname r@ax-bud-fs-E-SpT-q3-rec@1024t-d\endcsname{+0.2}
\expandafter\def\csname r@ax-bud-fs-E-SpT-q3-rec@1024t-p\endcsname{--}
\expandafter\def\csname r@ax-bud-fs-E-SpT-q3-rec@1024t-v\endcsname{n.d.}
\expandafter\def\csname r@ax-bud-fs-E-SpT-rr-hit@1\endcsname{+4.7 [$-$0.9, +10.6]}
\expandafter\def\csname r@ax-bud-fs-E-SpT-rr-hit@1-ci\endcsname{[$-$0.9, +10.6]}
\expandafter\def\csname r@ax-bud-fs-E-SpT-rr-hit@1-ci95\endcsname{[$-$0.9, +10.6]}
\expandafter\def\csname r@ax-bud-fs-E-SpT-rr-hit@1-d\endcsname{+4.7}
\expandafter\def\csname r@ax-bud-fs-E-SpT-rr-hit@1-p\endcsname{--}
\expandafter\def\csname r@ax-bud-fs-E-SpT-rr-hit@1-v\endcsname{n.d.}
\expandafter\def\csname r@ax-bud-fs-E-SpT-rr-hit@5\endcsname{+0.9 [$-$3.4, +5.1]}
\expandafter\def\csname r@ax-bud-fs-E-SpT-rr-hit@5-ci\endcsname{[$-$3.4, +5.1]}
\expandafter\def\csname r@ax-bud-fs-E-SpT-rr-hit@5-ci95\endcsname{[$-$3.4, +5.1]}
\expandafter\def\csname r@ax-bud-fs-E-SpT-rr-hit@5-d\endcsname{+0.9}
\expandafter\def\csname r@ax-bud-fs-E-SpT-rr-hit@5-p\endcsname{--}
\expandafter\def\csname r@ax-bud-fs-E-SpT-rr-hit@5-v\endcsname{n.d.}
\expandafter\def\csname r@ax-bud-fs-E-SpT-rr-mrr@10\endcsname{+2.7 [$-$1.1, +6.6]}
\expandafter\def\csname r@ax-bud-fs-E-SpT-rr-mrr@10-ci\endcsname{[$-$1.1, +6.6]}
\expandafter\def\csname r@ax-bud-fs-E-SpT-rr-mrr@10-ci95\endcsname{[$-$1.1, +6.6]}
\expandafter\def\csname r@ax-bud-fs-E-SpT-rr-mrr@10-d\endcsname{+2.7}
\expandafter\def\csname r@ax-bud-fs-E-SpT-rr-mrr@10-p\endcsname{--}
\expandafter\def\csname r@ax-bud-fs-E-SpT-rr-mrr@10-v\endcsname{n.d.}
\expandafter\def\csname r@ax-bud-fs-E-SpT-rr-prec@1024t\endcsname{+0.8 [$-$1.4, +3.0]}
\expandafter\def\csname r@ax-bud-fs-E-SpT-rr-prec@1024t-ci\endcsname{[$-$1.4, +3.0]}
\expandafter\def\csname r@ax-bud-fs-E-SpT-rr-prec@1024t-ci95\endcsname{[$-$1.4, +3.0]}
\expandafter\def\csname r@ax-bud-fs-E-SpT-rr-prec@1024t-d\endcsname{+0.8}
\expandafter\def\csname r@ax-bud-fs-E-SpT-rr-prec@1024t-p\endcsname{--}
\expandafter\def\csname r@ax-bud-fs-E-SpT-rr-prec@1024t-v\endcsname{n.d.}
\expandafter\def\csname r@ax-bud-fs-E-SpT-rr-prec@2048t\endcsname{+0.7 [$-$0.9, +2.3]}
\expandafter\def\csname r@ax-bud-fs-E-SpT-rr-prec@2048t-ci\endcsname{[$-$0.9, +2.3]}
\expandafter\def\csname r@ax-bud-fs-E-SpT-rr-prec@2048t-ci95\endcsname{[$-$0.9, +2.3]}
\expandafter\def\csname r@ax-bud-fs-E-SpT-rr-prec@2048t-d\endcsname{+0.7}
\expandafter\def\csname r@ax-bud-fs-E-SpT-rr-prec@2048t-p\endcsname{--}
\expandafter\def\csname r@ax-bud-fs-E-SpT-rr-prec@2048t-v\endcsname{n.d.}
\expandafter\def\csname r@ax-bud-fs-E-SpT-rr-prec@512t\endcsname{+0.2 [$-$2.5, +3.0]}
\expandafter\def\csname r@ax-bud-fs-E-SpT-rr-prec@512t-ci\endcsname{[$-$2.5, +3.0]}
\expandafter\def\csname r@ax-bud-fs-E-SpT-rr-prec@512t-ci95\endcsname{[$-$2.5, +3.0]}
\expandafter\def\csname r@ax-bud-fs-E-SpT-rr-prec@512t-d\endcsname{+0.2}
\expandafter\def\csname r@ax-bud-fs-E-SpT-rr-prec@512t-p\endcsname{--}
\expandafter\def\csname r@ax-bud-fs-E-SpT-rr-prec@512t-v\endcsname{n.d.}
\expandafter\def\csname r@ax-bud-fs-E-SpT-rr-rec@1024t\endcsname{+0.4 [$-$0.3, +1.3]}
\expandafter\def\csname r@ax-bud-fs-E-SpT-rr-rec@1024t-ci\endcsname{[$-$0.3, +1.3]}
\expandafter\def\csname r@ax-bud-fs-E-SpT-rr-rec@1024t-ci95\endcsname{[$-$0.3, +1.3]}
\expandafter\def\csname r@ax-bud-fs-E-SpT-rr-rec@1024t-d\endcsname{+0.4}
\expandafter\def\csname r@ax-bud-fs-E-SpT-rr-rec@1024t-p\endcsname{--}
\expandafter\def\csname r@ax-bud-fs-E-SpT-rr-rec@1024t-v\endcsname{n.d.}
\expandafter\def\csname r@ax-bud-fs-S-F256t-bm25-hit@1\endcsname{$-$1.3 [$-$5.5, +3.0]}
\expandafter\def\csname r@ax-bud-fs-S-F256t-bm25-hit@1-ci\endcsname{[$-$5.5, +3.0]}
\expandafter\def\csname r@ax-bud-fs-S-F256t-bm25-hit@1-ci95\endcsname{[$-$5.5, +3.0]}
\expandafter\def\csname r@ax-bud-fs-S-F256t-bm25-hit@1-d\endcsname{$-$1.3}
\expandafter\def\csname r@ax-bud-fs-S-F256t-bm25-hit@1-p\endcsname{--}
\expandafter\def\csname r@ax-bud-fs-S-F256t-bm25-hit@1-v\endcsname{n.d.}
\expandafter\def\csname r@ax-bud-fs-S-F256t-bm25-hit@5\endcsname{+2.6 [$-$2.1, +7.2]}
\expandafter\def\csname r@ax-bud-fs-S-F256t-bm25-hit@5-ci\endcsname{[$-$2.1, +7.2]}
\expandafter\def\csname r@ax-bud-fs-S-F256t-bm25-hit@5-ci95\endcsname{[$-$2.1, +7.2]}
\expandafter\def\csname r@ax-bud-fs-S-F256t-bm25-hit@5-d\endcsname{+2.6}
\expandafter\def\csname r@ax-bud-fs-S-F256t-bm25-hit@5-p\endcsname{--}
\expandafter\def\csname r@ax-bud-fs-S-F256t-bm25-hit@5-v\endcsname{n.d.}
\expandafter\def\csname r@ax-bud-fs-S-F256t-bm25-mrr@10\endcsname{+0.1 [$-$3.1, +3.2]}
\expandafter\def\csname r@ax-bud-fs-S-F256t-bm25-mrr@10-ci\endcsname{[$-$3.1, +3.2]}
\expandafter\def\csname r@ax-bud-fs-S-F256t-bm25-mrr@10-ci95\endcsname{[$-$3.1, +3.2]}
\expandafter\def\csname r@ax-bud-fs-S-F256t-bm25-mrr@10-d\endcsname{+0.1}
\expandafter\def\csname r@ax-bud-fs-S-F256t-bm25-mrr@10-p\endcsname{--}
\expandafter\def\csname r@ax-bud-fs-S-F256t-bm25-mrr@10-v\endcsname{n.d.}
\expandafter\def\csname r@ax-bud-fs-S-F256t-bm25-prec@1024t\endcsname{$-$1.8 [$-$4.1, +0.5]}
\expandafter\def\csname r@ax-bud-fs-S-F256t-bm25-prec@1024t-ci\endcsname{[$-$4.1, +0.5]}
\expandafter\def\csname r@ax-bud-fs-S-F256t-bm25-prec@1024t-ci95\endcsname{[$-$4.1, +0.5]}
\expandafter\def\csname r@ax-bud-fs-S-F256t-bm25-prec@1024t-d\endcsname{$-$1.8}
\expandafter\def\csname r@ax-bud-fs-S-F256t-bm25-prec@1024t-p\endcsname{--}
\expandafter\def\csname r@ax-bud-fs-S-F256t-bm25-prec@1024t-v\endcsname{n.d.}
\expandafter\def\csname r@ax-bud-fs-S-F256t-bm25-prec@2048t\endcsname{$-$1.4 [$-$3.1, +0.3]}
\expandafter\def\csname r@ax-bud-fs-S-F256t-bm25-prec@2048t-ci\endcsname{[$-$3.1, +0.3]}
\expandafter\def\csname r@ax-bud-fs-S-F256t-bm25-prec@2048t-ci95\endcsname{[$-$3.1, +0.3]}
\expandafter\def\csname r@ax-bud-fs-S-F256t-bm25-prec@2048t-d\endcsname{$-$1.4}
\expandafter\def\csname r@ax-bud-fs-S-F256t-bm25-prec@2048t-p\endcsname{--}
\expandafter\def\csname r@ax-bud-fs-S-F256t-bm25-prec@2048t-v\endcsname{n.d.}
\expandafter\def\csname r@ax-bud-fs-S-F256t-bm25-prec@512t\endcsname{$-$1.1 [$-$4.1, +1.8]}
\expandafter\def\csname r@ax-bud-fs-S-F256t-bm25-prec@512t-ci\endcsname{[$-$4.1, +1.8]}
\expandafter\def\csname r@ax-bud-fs-S-F256t-bm25-prec@512t-ci95\endcsname{[$-$4.1, +1.8]}
\expandafter\def\csname r@ax-bud-fs-S-F256t-bm25-prec@512t-d\endcsname{$-$1.1}
\expandafter\def\csname r@ax-bud-fs-S-F256t-bm25-prec@512t-p\endcsname{--}
\expandafter\def\csname r@ax-bud-fs-S-F256t-bm25-prec@512t-v\endcsname{n.d.}
\expandafter\def\csname r@ax-bud-fs-S-F256t-bm25-rec@1024t\endcsname{$-$1.0 [$-$2.1, $-$0.1]}
\expandafter\def\csname r@ax-bud-fs-S-F256t-bm25-rec@1024t-ci\endcsname{[$-$2.1, $-$0.1]}
\expandafter\def\csname r@ax-bud-fs-S-F256t-bm25-rec@1024t-ci95\endcsname{[$-$2.1, $-$0.1]}
\expandafter\def\csname r@ax-bud-fs-S-F256t-bm25-rec@1024t-d\endcsname{$-$1.0}
\expandafter\def\csname r@ax-bud-fs-S-F256t-bm25-rec@1024t-p\endcsname{--}
\expandafter\def\csname r@ax-bud-fs-S-F256t-bm25-rec@1024t-v\endcsname{diff.}
\expandafter\def\csname r@ax-bud-fs-S-F256t-hyb-hit@1\endcsname{$-$3.4 [$-$8.9, +2.1]}
\expandafter\def\csname r@ax-bud-fs-S-F256t-hyb-hit@1-ci\endcsname{[$-$8.9, +2.1]}
\expandafter\def\csname r@ax-bud-fs-S-F256t-hyb-hit@1-ci95\endcsname{[$-$8.9, +2.1]}
\expandafter\def\csname r@ax-bud-fs-S-F256t-hyb-hit@1-d\endcsname{$-$3.4}
\expandafter\def\csname r@ax-bud-fs-S-F256t-hyb-hit@1-p\endcsname{--}
\expandafter\def\csname r@ax-bud-fs-S-F256t-hyb-hit@1-v\endcsname{n.d.}
\expandafter\def\csname r@ax-bud-fs-S-F256t-hyb-hit@5\endcsname{$-$0.9 [$-$5.1, +3.4]}
\expandafter\def\csname r@ax-bud-fs-S-F256t-hyb-hit@5-ci\endcsname{[$-$5.1, +3.4]}
\expandafter\def\csname r@ax-bud-fs-S-F256t-hyb-hit@5-ci95\endcsname{[$-$5.1, +3.4]}
\expandafter\def\csname r@ax-bud-fs-S-F256t-hyb-hit@5-d\endcsname{$-$0.9}
\expandafter\def\csname r@ax-bud-fs-S-F256t-hyb-hit@5-p\endcsname{--}
\expandafter\def\csname r@ax-bud-fs-S-F256t-hyb-hit@5-v\endcsname{n.d.}
\expandafter\def\csname r@ax-bud-fs-S-F256t-hyb-mrr@10\endcsname{$-$1.0 [$-$4.7, +2.7]}
\expandafter\def\csname r@ax-bud-fs-S-F256t-hyb-mrr@10-ci\endcsname{[$-$4.7, +2.7]}
\expandafter\def\csname r@ax-bud-fs-S-F256t-hyb-mrr@10-ci95\endcsname{[$-$4.7, +2.7]}
\expandafter\def\csname r@ax-bud-fs-S-F256t-hyb-mrr@10-d\endcsname{$-$1.0}
\expandafter\def\csname r@ax-bud-fs-S-F256t-hyb-mrr@10-p\endcsname{--}
\expandafter\def\csname r@ax-bud-fs-S-F256t-hyb-mrr@10-v\endcsname{n.d.}
\expandafter\def\csname r@ax-bud-fs-S-F256t-hyb-prec@1024t\endcsname{$-$2.9 [$-$5.4, $-$0.3]}
\expandafter\def\csname r@ax-bud-fs-S-F256t-hyb-prec@1024t-ci\endcsname{[$-$5.4, $-$0.3]}
\expandafter\def\csname r@ax-bud-fs-S-F256t-hyb-prec@1024t-ci95\endcsname{[$-$5.4, $-$0.3]}
\expandafter\def\csname r@ax-bud-fs-S-F256t-hyb-prec@1024t-d\endcsname{$-$2.9}
\expandafter\def\csname r@ax-bud-fs-S-F256t-hyb-prec@1024t-p\endcsname{--}
\expandafter\def\csname r@ax-bud-fs-S-F256t-hyb-prec@1024t-v\endcsname{diff.}
\expandafter\def\csname r@ax-bud-fs-S-F256t-hyb-prec@2048t\endcsname{$-$2.6 [$-$4.4, $-$0.9]}
\expandafter\def\csname r@ax-bud-fs-S-F256t-hyb-prec@2048t-ci\endcsname{[$-$4.4, $-$0.9]}
\expandafter\def\csname r@ax-bud-fs-S-F256t-hyb-prec@2048t-ci95\endcsname{[$-$4.4, $-$0.9]}
\expandafter\def\csname r@ax-bud-fs-S-F256t-hyb-prec@2048t-d\endcsname{$-$2.6}
\expandafter\def\csname r@ax-bud-fs-S-F256t-hyb-prec@2048t-p\endcsname{--}
\expandafter\def\csname r@ax-bud-fs-S-F256t-hyb-prec@2048t-v\endcsname{diff.}
\expandafter\def\csname r@ax-bud-fs-S-F256t-hyb-prec@512t\endcsname{$-$0.8 [$-$4.3, +2.8]}
\expandafter\def\csname r@ax-bud-fs-S-F256t-hyb-prec@512t-ci\endcsname{[$-$4.3, +2.8]}
\expandafter\def\csname r@ax-bud-fs-S-F256t-hyb-prec@512t-ci95\endcsname{[$-$4.3, +2.8]}
\expandafter\def\csname r@ax-bud-fs-S-F256t-hyb-prec@512t-d\endcsname{$-$0.8}
\expandafter\def\csname r@ax-bud-fs-S-F256t-hyb-prec@512t-p\endcsname{--}
\expandafter\def\csname r@ax-bud-fs-S-F256t-hyb-prec@512t-v\endcsname{n.d.}
\expandafter\def\csname r@ax-bud-fs-S-F256t-hyb-rec@1024t\endcsname{$-$0.9 [$-$1.6, $-$0.1]}
\expandafter\def\csname r@ax-bud-fs-S-F256t-hyb-rec@1024t-ci\endcsname{[$-$1.6, $-$0.1]}
\expandafter\def\csname r@ax-bud-fs-S-F256t-hyb-rec@1024t-ci95\endcsname{[$-$1.6, $-$0.1]}
\expandafter\def\csname r@ax-bud-fs-S-F256t-hyb-rec@1024t-d\endcsname{$-$0.9}
\expandafter\def\csname r@ax-bud-fs-S-F256t-hyb-rec@1024t-p\endcsname{--}
\expandafter\def\csname r@ax-bud-fs-S-F256t-hyb-rec@1024t-v\endcsname{diff.}
\expandafter\def\csname r@ax-bud-fs-S-F256t-nomic-hit@1\endcsname{+2.6 [$-$2.1, +7.2]}
\expandafter\def\csname r@ax-bud-fs-S-F256t-nomic-hit@1-ci\endcsname{[$-$2.1, +7.2]}
\expandafter\def\csname r@ax-bud-fs-S-F256t-nomic-hit@1-ci95\endcsname{[$-$2.1, +7.2]}
\expandafter\def\csname r@ax-bud-fs-S-F256t-nomic-hit@1-d\endcsname{+2.6}
\expandafter\def\csname r@ax-bud-fs-S-F256t-nomic-hit@1-p\endcsname{--}
\expandafter\def\csname r@ax-bud-fs-S-F256t-nomic-hit@1-v\endcsname{n.d.}
\expandafter\def\csname r@ax-bud-fs-S-F256t-nomic-hit@5\endcsname{+2.6 [$-$1.7, +6.8]}
\expandafter\def\csname r@ax-bud-fs-S-F256t-nomic-hit@5-ci\endcsname{[$-$1.7, +6.8]}
\expandafter\def\csname r@ax-bud-fs-S-F256t-nomic-hit@5-ci95\endcsname{[$-$1.7, +6.8]}
\expandafter\def\csname r@ax-bud-fs-S-F256t-nomic-hit@5-d\endcsname{+2.6}
\expandafter\def\csname r@ax-bud-fs-S-F256t-nomic-hit@5-p\endcsname{--}
\expandafter\def\csname r@ax-bud-fs-S-F256t-nomic-hit@5-v\endcsname{n.d.}
\expandafter\def\csname r@ax-bud-fs-S-F256t-nomic-mrr@10\endcsname{+1.6 [$-$1.7, +5.1]}
\expandafter\def\csname r@ax-bud-fs-S-F256t-nomic-mrr@10-ci\endcsname{[$-$1.7, +5.1]}
\expandafter\def\csname r@ax-bud-fs-S-F256t-nomic-mrr@10-ci95\endcsname{[$-$1.7, +5.1]}
\expandafter\def\csname r@ax-bud-fs-S-F256t-nomic-mrr@10-d\endcsname{+1.6}
\expandafter\def\csname r@ax-bud-fs-S-F256t-nomic-mrr@10-p\endcsname{--}
\expandafter\def\csname r@ax-bud-fs-S-F256t-nomic-mrr@10-v\endcsname{n.d.}
\expandafter\def\csname r@ax-bud-fs-S-F256t-nomic-prec@1024t\endcsname{$-$3.5 [$-$5.9, $-$1.2]}
\expandafter\def\csname r@ax-bud-fs-S-F256t-nomic-prec@1024t-ci\endcsname{[$-$5.9, $-$1.2]}
\expandafter\def\csname r@ax-bud-fs-S-F256t-nomic-prec@1024t-ci95\endcsname{[$-$5.9, $-$1.2]}
\expandafter\def\csname r@ax-bud-fs-S-F256t-nomic-prec@1024t-d\endcsname{$-$3.5}
\expandafter\def\csname r@ax-bud-fs-S-F256t-nomic-prec@1024t-p\endcsname{--}
\expandafter\def\csname r@ax-bud-fs-S-F256t-nomic-prec@1024t-v\endcsname{diff.}
\expandafter\def\csname r@ax-bud-fs-S-F256t-nomic-prec@2048t\endcsname{$-$1.9 [$-$3.5, $-$0.3]}
\expandafter\def\csname r@ax-bud-fs-S-F256t-nomic-prec@2048t-ci\endcsname{[$-$3.5, $-$0.3]}
\expandafter\def\csname r@ax-bud-fs-S-F256t-nomic-prec@2048t-ci95\endcsname{[$-$3.5, $-$0.3]}
\expandafter\def\csname r@ax-bud-fs-S-F256t-nomic-prec@2048t-d\endcsname{$-$1.9}
\expandafter\def\csname r@ax-bud-fs-S-F256t-nomic-prec@2048t-p\endcsname{--}
\expandafter\def\csname r@ax-bud-fs-S-F256t-nomic-prec@2048t-v\endcsname{diff.}
\expandafter\def\csname r@ax-bud-fs-S-F256t-nomic-prec@512t\endcsname{+0.1 [$-$3.1, +3.4]}
\expandafter\def\csname r@ax-bud-fs-S-F256t-nomic-prec@512t-ci\endcsname{[$-$3.1, +3.4]}
\expandafter\def\csname r@ax-bud-fs-S-F256t-nomic-prec@512t-ci95\endcsname{[$-$3.1, +3.4]}
\expandafter\def\csname r@ax-bud-fs-S-F256t-nomic-prec@512t-d\endcsname{+0.1}
\expandafter\def\csname r@ax-bud-fs-S-F256t-nomic-prec@512t-p\endcsname{--}
\expandafter\def\csname r@ax-bud-fs-S-F256t-nomic-prec@512t-v\endcsname{n.d.}
\expandafter\def\csname r@ax-bud-fs-S-F256t-nomic-rec@1024t\endcsname{$-$1.5 [$-$2.4, $-$0.8]}
\expandafter\def\csname r@ax-bud-fs-S-F256t-nomic-rec@1024t-ci\endcsname{[$-$2.4, $-$0.8]}
\expandafter\def\csname r@ax-bud-fs-S-F256t-nomic-rec@1024t-ci95\endcsname{[$-$2.4, $-$0.8]}
\expandafter\def\csname r@ax-bud-fs-S-F256t-nomic-rec@1024t-d\endcsname{$-$1.5}
\expandafter\def\csname r@ax-bud-fs-S-F256t-nomic-rec@1024t-p\endcsname{--}
\expandafter\def\csname r@ax-bud-fs-S-F256t-nomic-rec@1024t-v\endcsname{diff.}
\expandafter\def\csname r@ax-bud-fs-S-F256t-q3-hit@1\endcsname{+0.9 [$-$4.7, +6.0]}
\expandafter\def\csname r@ax-bud-fs-S-F256t-q3-hit@1-ci\endcsname{[$-$4.7, +6.0]}
\expandafter\def\csname r@ax-bud-fs-S-F256t-q3-hit@1-ci95\endcsname{[$-$4.7, +6.0]}
\expandafter\def\csname r@ax-bud-fs-S-F256t-q3-hit@1-d\endcsname{+0.9}
\expandafter\def\csname r@ax-bud-fs-S-F256t-q3-hit@1-p\endcsname{--}
\expandafter\def\csname r@ax-bud-fs-S-F256t-q3-hit@1-v\endcsname{n.d.}
\expandafter\def\csname r@ax-bud-fs-S-F256t-q3-hit@5\endcsname{+1.7 [$-$3.4, +6.4]}
\expandafter\def\csname r@ax-bud-fs-S-F256t-q3-hit@5-ci\endcsname{[$-$3.4, +6.4]}
\expandafter\def\csname r@ax-bud-fs-S-F256t-q3-hit@5-ci95\endcsname{[$-$3.4, +6.4]}
\expandafter\def\csname r@ax-bud-fs-S-F256t-q3-hit@5-d\endcsname{+1.7}
\expandafter\def\csname r@ax-bud-fs-S-F256t-q3-hit@5-p\endcsname{--}
\expandafter\def\csname r@ax-bud-fs-S-F256t-q3-hit@5-v\endcsname{n.d.}
\expandafter\def\csname r@ax-bud-fs-S-F256t-q3-mrr@10\endcsname{+1.3 [$-$2.3, +4.8]}
\expandafter\def\csname r@ax-bud-fs-S-F256t-q3-mrr@10-ci\endcsname{[$-$2.3, +4.8]}
\expandafter\def\csname r@ax-bud-fs-S-F256t-q3-mrr@10-ci95\endcsname{[$-$2.3, +4.8]}
\expandafter\def\csname r@ax-bud-fs-S-F256t-q3-mrr@10-d\endcsname{+1.3}
\expandafter\def\csname r@ax-bud-fs-S-F256t-q3-mrr@10-p\endcsname{--}
\expandafter\def\csname r@ax-bud-fs-S-F256t-q3-mrr@10-v\endcsname{n.d.}
\expandafter\def\csname r@ax-bud-fs-S-F256t-q3-prec@1024t\endcsname{$-$2.6 [$-$4.9, $-$0.5]}
\expandafter\def\csname r@ax-bud-fs-S-F256t-q3-prec@1024t-ci\endcsname{[$-$4.9, $-$0.5]}
\expandafter\def\csname r@ax-bud-fs-S-F256t-q3-prec@1024t-ci95\endcsname{[$-$4.9, $-$0.5]}
\expandafter\def\csname r@ax-bud-fs-S-F256t-q3-prec@1024t-d\endcsname{$-$2.6}
\expandafter\def\csname r@ax-bud-fs-S-F256t-q3-prec@1024t-p\endcsname{--}
\expandafter\def\csname r@ax-bud-fs-S-F256t-q3-prec@1024t-v\endcsname{diff.}
\expandafter\def\csname r@ax-bud-fs-S-F256t-q3-prec@2048t\endcsname{$-$2.5 [$-$3.9, $-$1.1]}
\expandafter\def\csname r@ax-bud-fs-S-F256t-q3-prec@2048t-ci\endcsname{[$-$3.9, $-$1.1]}
\expandafter\def\csname r@ax-bud-fs-S-F256t-q3-prec@2048t-ci95\endcsname{[$-$3.9, $-$1.1]}
\expandafter\def\csname r@ax-bud-fs-S-F256t-q3-prec@2048t-d\endcsname{$-$2.5}
\expandafter\def\csname r@ax-bud-fs-S-F256t-q3-prec@2048t-p\endcsname{--}
\expandafter\def\csname r@ax-bud-fs-S-F256t-q3-prec@2048t-v\endcsname{diff.}
\expandafter\def\csname r@ax-bud-fs-S-F256t-q3-prec@512t\endcsname{$-$1.9 [$-$5.1, +1.2]}
\expandafter\def\csname r@ax-bud-fs-S-F256t-q3-prec@512t-ci\endcsname{[$-$5.1, +1.2]}
\expandafter\def\csname r@ax-bud-fs-S-F256t-q3-prec@512t-ci95\endcsname{[$-$5.1, +1.2]}
\expandafter\def\csname r@ax-bud-fs-S-F256t-q3-prec@512t-d\endcsname{$-$1.9}
\expandafter\def\csname r@ax-bud-fs-S-F256t-q3-prec@512t-p\endcsname{--}
\expandafter\def\csname r@ax-bud-fs-S-F256t-q3-prec@512t-v\endcsname{n.d.}
\expandafter\def\csname r@ax-bud-fs-S-F256t-q3-rec@1024t\endcsname{$-$1.0 [$-$2.0, $-$0.3]}
\expandafter\def\csname r@ax-bud-fs-S-F256t-q3-rec@1024t-ci\endcsname{[$-$2.0, $-$0.3]}
\expandafter\def\csname r@ax-bud-fs-S-F256t-q3-rec@1024t-ci95\endcsname{[$-$2.0, $-$0.3]}
\expandafter\def\csname r@ax-bud-fs-S-F256t-q3-rec@1024t-d\endcsname{$-$1.0}
\expandafter\def\csname r@ax-bud-fs-S-F256t-q3-rec@1024t-p\endcsname{--}
\expandafter\def\csname r@ax-bud-fs-S-F256t-q3-rec@1024t-v\endcsname{diff.}
\expandafter\def\csname r@ax-bud-fs-S-F256t-rr-hit@1\endcsname{$-$2.1 [$-$7.7, +3.4]}
\expandafter\def\csname r@ax-bud-fs-S-F256t-rr-hit@1-ci\endcsname{[$-$7.7, +3.4]}
\expandafter\def\csname r@ax-bud-fs-S-F256t-rr-hit@1-ci95\endcsname{[$-$7.7, +3.4]}
\expandafter\def\csname r@ax-bud-fs-S-F256t-rr-hit@1-d\endcsname{$-$2.1}
\expandafter\def\csname r@ax-bud-fs-S-F256t-rr-hit@1-p\endcsname{--}
\expandafter\def\csname r@ax-bud-fs-S-F256t-rr-hit@1-v\endcsname{n.d.}
\expandafter\def\csname r@ax-bud-fs-S-F256t-rr-hit@5\endcsname{$-$0.9 [$-$5.5, +3.4]}
\expandafter\def\csname r@ax-bud-fs-S-F256t-rr-hit@5-ci\endcsname{[$-$5.5, +3.4]}
\expandafter\def\csname r@ax-bud-fs-S-F256t-rr-hit@5-ci95\endcsname{[$-$5.5, +3.4]}
\expandafter\def\csname r@ax-bud-fs-S-F256t-rr-hit@5-d\endcsname{$-$0.9}
\expandafter\def\csname r@ax-bud-fs-S-F256t-rr-hit@5-p\endcsname{--}
\expandafter\def\csname r@ax-bud-fs-S-F256t-rr-hit@5-v\endcsname{n.d.}
\expandafter\def\csname r@ax-bud-fs-S-F256t-rr-mrr@10\endcsname{$-$2.8 [$-$6.7, +1.1]}
\expandafter\def\csname r@ax-bud-fs-S-F256t-rr-mrr@10-ci\endcsname{[$-$6.7, +1.1]}
\expandafter\def\csname r@ax-bud-fs-S-F256t-rr-mrr@10-ci95\endcsname{[$-$6.7, +1.1]}
\expandafter\def\csname r@ax-bud-fs-S-F256t-rr-mrr@10-d\endcsname{$-$2.8}
\expandafter\def\csname r@ax-bud-fs-S-F256t-rr-mrr@10-p\endcsname{--}
\expandafter\def\csname r@ax-bud-fs-S-F256t-rr-mrr@10-v\endcsname{n.d.}
\expandafter\def\csname r@ax-bud-fs-S-F256t-rr-prec@1024t\endcsname{$-$3.9 [$-$6.1, $-$1.4]}
\expandafter\def\csname r@ax-bud-fs-S-F256t-rr-prec@1024t-ci\endcsname{[$-$6.1, $-$1.4]}
\expandafter\def\csname r@ax-bud-fs-S-F256t-rr-prec@1024t-ci95\endcsname{[$-$6.1, $-$1.4]}
\expandafter\def\csname r@ax-bud-fs-S-F256t-rr-prec@1024t-d\endcsname{$-$3.9}
\expandafter\def\csname r@ax-bud-fs-S-F256t-rr-prec@1024t-p\endcsname{--}
\expandafter\def\csname r@ax-bud-fs-S-F256t-rr-prec@1024t-v\endcsname{diff.}
\expandafter\def\csname r@ax-bud-fs-S-F256t-rr-prec@2048t\endcsname{$-$3.9 [$-$5.7, $-$2.2]}
\expandafter\def\csname r@ax-bud-fs-S-F256t-rr-prec@2048t-ci\endcsname{[$-$5.7, $-$2.2]}
\expandafter\def\csname r@ax-bud-fs-S-F256t-rr-prec@2048t-ci95\endcsname{[$-$5.7, $-$2.2]}
\expandafter\def\csname r@ax-bud-fs-S-F256t-rr-prec@2048t-d\endcsname{$-$3.9}
\expandafter\def\csname r@ax-bud-fs-S-F256t-rr-prec@2048t-p\endcsname{--}
\expandafter\def\csname r@ax-bud-fs-S-F256t-rr-prec@2048t-v\endcsname{diff.}
\expandafter\def\csname r@ax-bud-fs-S-F256t-rr-prec@512t\endcsname{$-$2.7 [$-$6.0, +0.6]}
\expandafter\def\csname r@ax-bud-fs-S-F256t-rr-prec@512t-ci\endcsname{[$-$6.0, +0.6]}
\expandafter\def\csname r@ax-bud-fs-S-F256t-rr-prec@512t-ci95\endcsname{[$-$6.0, +0.6]}
\expandafter\def\csname r@ax-bud-fs-S-F256t-rr-prec@512t-d\endcsname{$-$2.7}
\expandafter\def\csname r@ax-bud-fs-S-F256t-rr-prec@512t-p\endcsname{--}
\expandafter\def\csname r@ax-bud-fs-S-F256t-rr-prec@512t-v\endcsname{n.d.}
\expandafter\def\csname r@ax-bud-fs-S-F256t-rr-rec@1024t\endcsname{$-$1.7 [$-$2.7, $-$0.8]}
\expandafter\def\csname r@ax-bud-fs-S-F256t-rr-rec@1024t-ci\endcsname{[$-$2.7, $-$0.8]}
\expandafter\def\csname r@ax-bud-fs-S-F256t-rr-rec@1024t-ci95\endcsname{[$-$2.7, $-$0.8]}
\expandafter\def\csname r@ax-bud-fs-S-F256t-rr-rec@1024t-d\endcsname{$-$1.7}
\expandafter\def\csname r@ax-bud-fs-S-F256t-rr-rec@1024t-p\endcsname{--}
\expandafter\def\csname r@ax-bud-fs-S-F256t-rr-rec@1024t-v\endcsname{diff.}
\expandafter\def\csname r@ax-bud-fs-nrev\endcsname{7}
\expandafter\def\csname r@ax-bud-fs-nrevstrict\endcsname{0}
\expandafter\def\csname r@ax-bud-qasper-E-CR-bm25-hit@1\endcsname{+4.9 [+2.6, +7.5]}
\expandafter\def\csname r@ax-bud-qasper-E-CR-bm25-hit@1-ci\endcsname{[+2.6, +7.5]}
\expandafter\def\csname r@ax-bud-qasper-E-CR-bm25-hit@1-ci95\endcsname{[+2.6, +7.5]}
\expandafter\def\csname r@ax-bud-qasper-E-CR-bm25-hit@1-d\endcsname{+4.9}
\expandafter\def\csname r@ax-bud-qasper-E-CR-bm25-hit@1-p\endcsname{--}
\expandafter\def\csname r@ax-bud-qasper-E-CR-bm25-hit@1-v\endcsname{diff.}
\expandafter\def\csname r@ax-bud-qasper-E-CR-bm25-hit@5\endcsname{+3.3 [+0.6, +5.8]}
\expandafter\def\csname r@ax-bud-qasper-E-CR-bm25-hit@5-ci\endcsname{[+0.6, +5.8]}
\expandafter\def\csname r@ax-bud-qasper-E-CR-bm25-hit@5-ci95\endcsname{[+0.6, +5.8]}
\expandafter\def\csname r@ax-bud-qasper-E-CR-bm25-hit@5-d\endcsname{+3.3}
\expandafter\def\csname r@ax-bud-qasper-E-CR-bm25-hit@5-p\endcsname{--}
\expandafter\def\csname r@ax-bud-qasper-E-CR-bm25-hit@5-v\endcsname{diff.}
\expandafter\def\csname r@ax-bud-qasper-E-CR-bm25-rec@1024t\endcsname{+3.7 [+1.4, +6.1]}
\expandafter\def\csname r@ax-bud-qasper-E-CR-bm25-rec@1024t-ci\endcsname{[+1.4, +6.1]}
\expandafter\def\csname r@ax-bud-qasper-E-CR-bm25-rec@1024t-ci95\endcsname{[+1.4, +6.1]}
\expandafter\def\csname r@ax-bud-qasper-E-CR-bm25-rec@1024t-d\endcsname{+3.7}
\expandafter\def\csname r@ax-bud-qasper-E-CR-bm25-rec@1024t-p\endcsname{--}
\expandafter\def\csname r@ax-bud-qasper-E-CR-bm25-rec@1024t-v\endcsname{diff.}
\expandafter\def\csname r@ax-bud-qasper-E-CR-bm25-rec@256t\endcsname{+4.2 [+2.5, +6.2]}
\expandafter\def\csname r@ax-bud-qasper-E-CR-bm25-rec@256t-ci\endcsname{[+2.5, +6.2]}
\expandafter\def\csname r@ax-bud-qasper-E-CR-bm25-rec@256t-ci95\endcsname{[+2.5, +6.2]}
\expandafter\def\csname r@ax-bud-qasper-E-CR-bm25-rec@256t-d\endcsname{+4.2}
\expandafter\def\csname r@ax-bud-qasper-E-CR-bm25-rec@256t-p\endcsname{--}
\expandafter\def\csname r@ax-bud-qasper-E-CR-bm25-rec@256t-v\endcsname{diff.}
\expandafter\def\csname r@ax-bud-qasper-E-CR-bm25-rec@5\endcsname{+2.7 [+0.6, +5.0]}
\expandafter\def\csname r@ax-bud-qasper-E-CR-bm25-rec@5-ci\endcsname{[+0.6, +5.0]}
\expandafter\def\csname r@ax-bud-qasper-E-CR-bm25-rec@5-ci95\endcsname{[+0.6, +5.0]}
\expandafter\def\csname r@ax-bud-qasper-E-CR-bm25-rec@5-d\endcsname{+2.7}
\expandafter\def\csname r@ax-bud-qasper-E-CR-bm25-rec@5-p\endcsname{--}
\expandafter\def\csname r@ax-bud-qasper-E-CR-bm25-rec@5-v\endcsname{diff.}
\expandafter\def\csname r@ax-bud-qasper-E-CR-bm25-rec@512t\endcsname{+5.0 [+2.7, +7.4]}
\expandafter\def\csname r@ax-bud-qasper-E-CR-bm25-rec@512t-ci\endcsname{[+2.7, +7.4]}
\expandafter\def\csname r@ax-bud-qasper-E-CR-bm25-rec@512t-ci95\endcsname{[+2.7, +7.4]}
\expandafter\def\csname r@ax-bud-qasper-E-CR-bm25-rec@512t-d\endcsname{+5.0}
\expandafter\def\csname r@ax-bud-qasper-E-CR-bm25-rec@512t-p\endcsname{--}
\expandafter\def\csname r@ax-bud-qasper-E-CR-bm25-rec@512t-v\endcsname{diff.}
\expandafter\def\csname r@ax-bud-qasper-E-CR-hyb-hit@1\endcsname{+2.0 [$-$1.0, +5.1]}
\expandafter\def\csname r@ax-bud-qasper-E-CR-hyb-hit@1-ci\endcsname{[$-$1.0, +5.1]}
\expandafter\def\csname r@ax-bud-qasper-E-CR-hyb-hit@1-ci95\endcsname{[$-$1.0, +5.1]}
\expandafter\def\csname r@ax-bud-qasper-E-CR-hyb-hit@1-d\endcsname{+2.0}
\expandafter\def\csname r@ax-bud-qasper-E-CR-hyb-hit@1-p\endcsname{--}
\expandafter\def\csname r@ax-bud-qasper-E-CR-hyb-hit@1-v\endcsname{n.d.}
\expandafter\def\csname r@ax-bud-qasper-E-CR-hyb-hit@5\endcsname{+0.2 [$-$2.3, +2.7]}
\expandafter\def\csname r@ax-bud-qasper-E-CR-hyb-hit@5-ci\endcsname{[$-$2.3, +2.7]}
\expandafter\def\csname r@ax-bud-qasper-E-CR-hyb-hit@5-ci95\endcsname{[$-$2.3, +2.7]}
\expandafter\def\csname r@ax-bud-qasper-E-CR-hyb-hit@5-d\endcsname{+0.2}
\expandafter\def\csname r@ax-bud-qasper-E-CR-hyb-hit@5-p\endcsname{--}
\expandafter\def\csname r@ax-bud-qasper-E-CR-hyb-hit@5-v\endcsname{n.d.}
\expandafter\def\csname r@ax-bud-qasper-E-CR-hyb-rec@1024t\endcsname{+0.1 [$-$2.1, +2.5]}
\expandafter\def\csname r@ax-bud-qasper-E-CR-hyb-rec@1024t-ci\endcsname{[$-$2.1, +2.5]}
\expandafter\def\csname r@ax-bud-qasper-E-CR-hyb-rec@1024t-ci95\endcsname{[$-$2.1, +2.5]}
\expandafter\def\csname r@ax-bud-qasper-E-CR-hyb-rec@1024t-d\endcsname{+0.1}
\expandafter\def\csname r@ax-bud-qasper-E-CR-hyb-rec@1024t-p\endcsname{--}
\expandafter\def\csname r@ax-bud-qasper-E-CR-hyb-rec@1024t-v\endcsname{n.d.}
\expandafter\def\csname r@ax-bud-qasper-E-CR-hyb-rec@256t\endcsname{+0.6 [$-$1.7, +3.0]}
\expandafter\def\csname r@ax-bud-qasper-E-CR-hyb-rec@256t-ci\endcsname{[$-$1.7, +3.0]}
\expandafter\def\csname r@ax-bud-qasper-E-CR-hyb-rec@256t-ci95\endcsname{[$-$1.7, +3.0]}
\expandafter\def\csname r@ax-bud-qasper-E-CR-hyb-rec@256t-d\endcsname{+0.6}
\expandafter\def\csname r@ax-bud-qasper-E-CR-hyb-rec@256t-p\endcsname{--}
\expandafter\def\csname r@ax-bud-qasper-E-CR-hyb-rec@256t-v\endcsname{n.d.}
\expandafter\def\csname r@ax-bud-qasper-E-CR-hyb-rec@5\endcsname{$-$0.1 [$-$2.4, +2.3]}
\expandafter\def\csname r@ax-bud-qasper-E-CR-hyb-rec@5-ci\endcsname{[$-$2.4, +2.3]}
\expandafter\def\csname r@ax-bud-qasper-E-CR-hyb-rec@5-ci95\endcsname{[$-$2.4, +2.3]}
\expandafter\def\csname r@ax-bud-qasper-E-CR-hyb-rec@5-d\endcsname{$-$0.1}
\expandafter\def\csname r@ax-bud-qasper-E-CR-hyb-rec@5-p\endcsname{--}
\expandafter\def\csname r@ax-bud-qasper-E-CR-hyb-rec@5-v\endcsname{n.d.}
\expandafter\def\csname r@ax-bud-qasper-E-CR-hyb-rec@512t\endcsname{+2.1 [$-$0.3, +4.4]}
\expandafter\def\csname r@ax-bud-qasper-E-CR-hyb-rec@512t-ci\endcsname{[$-$0.3, +4.4]}
\expandafter\def\csname r@ax-bud-qasper-E-CR-hyb-rec@512t-ci95\endcsname{[$-$0.3, +4.4]}
\expandafter\def\csname r@ax-bud-qasper-E-CR-hyb-rec@512t-d\endcsname{+2.1}
\expandafter\def\csname r@ax-bud-qasper-E-CR-hyb-rec@512t-p\endcsname{--}
\expandafter\def\csname r@ax-bud-qasper-E-CR-hyb-rec@512t-v\endcsname{n.d.}
\expandafter\def\csname r@ax-bud-qasper-E-CR-nomic-hit@1\endcsname{+0.5 [$-$2.3, +3.4]}
\expandafter\def\csname r@ax-bud-qasper-E-CR-nomic-hit@1-ci\endcsname{[$-$2.3, +3.4]}
\expandafter\def\csname r@ax-bud-qasper-E-CR-nomic-hit@1-ci95\endcsname{[$-$2.3, +3.4]}
\expandafter\def\csname r@ax-bud-qasper-E-CR-nomic-hit@1-d\endcsname{+0.5}
\expandafter\def\csname r@ax-bud-qasper-E-CR-nomic-hit@1-p\endcsname{--}
\expandafter\def\csname r@ax-bud-qasper-E-CR-nomic-hit@1-v\endcsname{n.d.}
\expandafter\def\csname r@ax-bud-qasper-E-CR-nomic-hit@5\endcsname{$-$0.5 [$-$2.9, +1.8]}
\expandafter\def\csname r@ax-bud-qasper-E-CR-nomic-hit@5-ci\endcsname{[$-$2.9, +1.8]}
\expandafter\def\csname r@ax-bud-qasper-E-CR-nomic-hit@5-ci95\endcsname{[$-$2.9, +1.8]}
\expandafter\def\csname r@ax-bud-qasper-E-CR-nomic-hit@5-d\endcsname{$-$0.5}
\expandafter\def\csname r@ax-bud-qasper-E-CR-nomic-hit@5-p\endcsname{--}
\expandafter\def\csname r@ax-bud-qasper-E-CR-nomic-hit@5-v\endcsname{n.d.}
\expandafter\def\csname r@ax-bud-qasper-E-CR-nomic-rec@1024t\endcsname{$-$1.5 [$-$3.7, +0.6]}
\expandafter\def\csname r@ax-bud-qasper-E-CR-nomic-rec@1024t-ci\endcsname{[$-$3.7, +0.6]}
\expandafter\def\csname r@ax-bud-qasper-E-CR-nomic-rec@1024t-ci95\endcsname{[$-$3.7, +0.6]}
\expandafter\def\csname r@ax-bud-qasper-E-CR-nomic-rec@1024t-d\endcsname{$-$1.5}
\expandafter\def\csname r@ax-bud-qasper-E-CR-nomic-rec@1024t-p\endcsname{--}
\expandafter\def\csname r@ax-bud-qasper-E-CR-nomic-rec@1024t-v\endcsname{n.d.}
\expandafter\def\csname r@ax-bud-qasper-E-CR-nomic-rec@256t\endcsname{$-$0.0 [$-$2.2, +2.2]}
\expandafter\def\csname r@ax-bud-qasper-E-CR-nomic-rec@256t-ci\endcsname{[$-$2.2, +2.2]}
\expandafter\def\csname r@ax-bud-qasper-E-CR-nomic-rec@256t-ci95\endcsname{[$-$2.2, +2.2]}
\expandafter\def\csname r@ax-bud-qasper-E-CR-nomic-rec@256t-d\endcsname{$-$0.0}
\expandafter\def\csname r@ax-bud-qasper-E-CR-nomic-rec@256t-p\endcsname{--}
\expandafter\def\csname r@ax-bud-qasper-E-CR-nomic-rec@256t-v\endcsname{n.d.}
\expandafter\def\csname r@ax-bud-qasper-E-CR-nomic-rec@5\endcsname{$-$0.2 [$-$2.5, +2.1]}
\expandafter\def\csname r@ax-bud-qasper-E-CR-nomic-rec@5-ci\endcsname{[$-$2.5, +2.1]}
\expandafter\def\csname r@ax-bud-qasper-E-CR-nomic-rec@5-ci95\endcsname{[$-$2.5, +2.1]}
\expandafter\def\csname r@ax-bud-qasper-E-CR-nomic-rec@5-d\endcsname{$-$0.2}
\expandafter\def\csname r@ax-bud-qasper-E-CR-nomic-rec@5-p\endcsname{--}
\expandafter\def\csname r@ax-bud-qasper-E-CR-nomic-rec@5-v\endcsname{n.d.}
\expandafter\def\csname r@ax-bud-qasper-E-CR-nomic-rec@512t\endcsname{$-$1.2 [$-$3.7, +1.2]}
\expandafter\def\csname r@ax-bud-qasper-E-CR-nomic-rec@512t-ci\endcsname{[$-$3.7, +1.2]}
\expandafter\def\csname r@ax-bud-qasper-E-CR-nomic-rec@512t-ci95\endcsname{[$-$3.7, +1.2]}
\expandafter\def\csname r@ax-bud-qasper-E-CR-nomic-rec@512t-d\endcsname{$-$1.2}
\expandafter\def\csname r@ax-bud-qasper-E-CR-nomic-rec@512t-p\endcsname{--}
\expandafter\def\csname r@ax-bud-qasper-E-CR-nomic-rec@512t-v\endcsname{n.d.}
\expandafter\def\csname r@ax-bud-qasper-E-CR-q3-hit@1\endcsname{+0.1 [$-$2.8, +3.1]}
\expandafter\def\csname r@ax-bud-qasper-E-CR-q3-hit@1-ci\endcsname{[$-$2.8, +3.1]}
\expandafter\def\csname r@ax-bud-qasper-E-CR-q3-hit@1-ci95\endcsname{[$-$2.8, +3.1]}
\expandafter\def\csname r@ax-bud-qasper-E-CR-q3-hit@1-d\endcsname{+0.1}
\expandafter\def\csname r@ax-bud-qasper-E-CR-q3-hit@1-p\endcsname{--}
\expandafter\def\csname r@ax-bud-qasper-E-CR-q3-hit@1-v\endcsname{n.d.}
\expandafter\def\csname r@ax-bud-qasper-E-CR-q3-hit@5\endcsname{$-$1.2 [$-$3.4, +1.1]}
\expandafter\def\csname r@ax-bud-qasper-E-CR-q3-hit@5-ci\endcsname{[$-$3.4, +1.1]}
\expandafter\def\csname r@ax-bud-qasper-E-CR-q3-hit@5-ci95\endcsname{[$-$3.4, +1.1]}
\expandafter\def\csname r@ax-bud-qasper-E-CR-q3-hit@5-d\endcsname{$-$1.2}
\expandafter\def\csname r@ax-bud-qasper-E-CR-q3-hit@5-p\endcsname{--}
\expandafter\def\csname r@ax-bud-qasper-E-CR-q3-hit@5-v\endcsname{n.d.}
\expandafter\def\csname r@ax-bud-qasper-E-CR-q3-rec@1024t\endcsname{$-$2.6 [$-$4.7, $-$0.4]}
\expandafter\def\csname r@ax-bud-qasper-E-CR-q3-rec@1024t-ci\endcsname{[$-$4.7, $-$0.4]}
\expandafter\def\csname r@ax-bud-qasper-E-CR-q3-rec@1024t-ci95\endcsname{[$-$4.7, $-$0.4]}
\expandafter\def\csname r@ax-bud-qasper-E-CR-q3-rec@1024t-d\endcsname{$-$2.6}
\expandafter\def\csname r@ax-bud-qasper-E-CR-q3-rec@1024t-p\endcsname{--}
\expandafter\def\csname r@ax-bud-qasper-E-CR-q3-rec@1024t-v\endcsname{diff.}
\expandafter\def\csname r@ax-bud-qasper-E-CR-q3-rec@256t\endcsname{+0.9 [$-$1.3, +3.3]}
\expandafter\def\csname r@ax-bud-qasper-E-CR-q3-rec@256t-ci\endcsname{[$-$1.3, +3.3]}
\expandafter\def\csname r@ax-bud-qasper-E-CR-q3-rec@256t-ci95\endcsname{[$-$1.3, +3.3]}
\expandafter\def\csname r@ax-bud-qasper-E-CR-q3-rec@256t-d\endcsname{+0.9}
\expandafter\def\csname r@ax-bud-qasper-E-CR-q3-rec@256t-p\endcsname{--}
\expandafter\def\csname r@ax-bud-qasper-E-CR-q3-rec@256t-v\endcsname{n.d.}
\expandafter\def\csname r@ax-bud-qasper-E-CR-q3-rec@5\endcsname{$-$1.1 [$-$3.3, +1.2]}
\expandafter\def\csname r@ax-bud-qasper-E-CR-q3-rec@5-ci\endcsname{[$-$3.3, +1.2]}
\expandafter\def\csname r@ax-bud-qasper-E-CR-q3-rec@5-ci95\endcsname{[$-$3.3, +1.2]}
\expandafter\def\csname r@ax-bud-qasper-E-CR-q3-rec@5-d\endcsname{$-$1.1}
\expandafter\def\csname r@ax-bud-qasper-E-CR-q3-rec@5-p\endcsname{--}
\expandafter\def\csname r@ax-bud-qasper-E-CR-q3-rec@5-v\endcsname{n.d.}
\expandafter\def\csname r@ax-bud-qasper-E-CR-q3-rec@512t\endcsname{$-$0.6 [$-$3.1, +1.9]}
\expandafter\def\csname r@ax-bud-qasper-E-CR-q3-rec@512t-ci\endcsname{[$-$3.1, +1.9]}
\expandafter\def\csname r@ax-bud-qasper-E-CR-q3-rec@512t-ci95\endcsname{[$-$3.1, +1.9]}
\expandafter\def\csname r@ax-bud-qasper-E-CR-q3-rec@512t-d\endcsname{$-$0.6}
\expandafter\def\csname r@ax-bud-qasper-E-CR-q3-rec@512t-p\endcsname{--}
\expandafter\def\csname r@ax-bud-qasper-E-CR-q3-rec@512t-v\endcsname{n.d.}
\expandafter\def\csname r@ax-bud-qasper-E-CR-rr-hit@1\endcsname{+0.7 [$-$2.3, +3.8]}
\expandafter\def\csname r@ax-bud-qasper-E-CR-rr-hit@1-ci\endcsname{[$-$2.3, +3.8]}
\expandafter\def\csname r@ax-bud-qasper-E-CR-rr-hit@1-ci95\endcsname{[$-$2.3, +3.8]}
\expandafter\def\csname r@ax-bud-qasper-E-CR-rr-hit@1-d\endcsname{+0.7}
\expandafter\def\csname r@ax-bud-qasper-E-CR-rr-hit@1-p\endcsname{--}
\expandafter\def\csname r@ax-bud-qasper-E-CR-rr-hit@1-v\endcsname{n.d.}
\expandafter\def\csname r@ax-bud-qasper-E-CR-rr-hit@5\endcsname{$-$1.7 [$-$3.7, +0.3]}
\expandafter\def\csname r@ax-bud-qasper-E-CR-rr-hit@5-ci\endcsname{[$-$3.7, +0.3]}
\expandafter\def\csname r@ax-bud-qasper-E-CR-rr-hit@5-ci95\endcsname{[$-$3.7, +0.3]}
\expandafter\def\csname r@ax-bud-qasper-E-CR-rr-hit@5-d\endcsname{$-$1.7}
\expandafter\def\csname r@ax-bud-qasper-E-CR-rr-hit@5-p\endcsname{--}
\expandafter\def\csname r@ax-bud-qasper-E-CR-rr-hit@5-v\endcsname{n.d.}
\expandafter\def\csname r@ax-bud-qasper-E-CR-rr-rec@1024t\endcsname{$-$1.6 [$-$3.5, +0.3]}
\expandafter\def\csname r@ax-bud-qasper-E-CR-rr-rec@1024t-ci\endcsname{[$-$3.5, +0.3]}
\expandafter\def\csname r@ax-bud-qasper-E-CR-rr-rec@1024t-ci95\endcsname{[$-$3.5, +0.3]}
\expandafter\def\csname r@ax-bud-qasper-E-CR-rr-rec@1024t-d\endcsname{$-$1.6}
\expandafter\def\csname r@ax-bud-qasper-E-CR-rr-rec@1024t-p\endcsname{--}
\expandafter\def\csname r@ax-bud-qasper-E-CR-rr-rec@1024t-v\endcsname{n.d.}
\expandafter\def\csname r@ax-bud-qasper-E-CR-rr-rec@256t\endcsname{+0.8 [$-$1.5, +3.2]}
\expandafter\def\csname r@ax-bud-qasper-E-CR-rr-rec@256t-ci\endcsname{[$-$1.5, +3.2]}
\expandafter\def\csname r@ax-bud-qasper-E-CR-rr-rec@256t-ci95\endcsname{[$-$1.5, +3.2]}
\expandafter\def\csname r@ax-bud-qasper-E-CR-rr-rec@256t-d\endcsname{+0.8}
\expandafter\def\csname r@ax-bud-qasper-E-CR-rr-rec@256t-p\endcsname{--}
\expandafter\def\csname r@ax-bud-qasper-E-CR-rr-rec@256t-v\endcsname{n.d.}
\expandafter\def\csname r@ax-bud-qasper-E-CR-rr-rec@5\endcsname{$-$1.7 [$-$3.6, +0.2]}
\expandafter\def\csname r@ax-bud-qasper-E-CR-rr-rec@5-ci\endcsname{[$-$3.6, +0.2]}
\expandafter\def\csname r@ax-bud-qasper-E-CR-rr-rec@5-ci95\endcsname{[$-$3.6, +0.2]}
\expandafter\def\csname r@ax-bud-qasper-E-CR-rr-rec@5-d\endcsname{$-$1.7}
\expandafter\def\csname r@ax-bud-qasper-E-CR-rr-rec@5-p\endcsname{--}
\expandafter\def\csname r@ax-bud-qasper-E-CR-rr-rec@5-v\endcsname{n.d.}
\expandafter\def\csname r@ax-bud-qasper-E-CR-rr-rec@512t\endcsname{+0.3 [$-$1.9, +2.5]}
\expandafter\def\csname r@ax-bud-qasper-E-CR-rr-rec@512t-ci\endcsname{[$-$1.9, +2.5]}
\expandafter\def\csname r@ax-bud-qasper-E-CR-rr-rec@512t-ci95\endcsname{[$-$1.9, +2.5]}
\expandafter\def\csname r@ax-bud-qasper-E-CR-rr-rec@512t-d\endcsname{+0.3}
\expandafter\def\csname r@ax-bud-qasper-E-CR-rr-rec@512t-p\endcsname{--}
\expandafter\def\csname r@ax-bud-qasper-E-CR-rr-rec@512t-v\endcsname{n.d.}
\expandafter\def\csname r@ax-bud-qasper-E-SpT-bm25-hit@1\endcsname{+7.0 [+4.5, +9.8]}
\expandafter\def\csname r@ax-bud-qasper-E-SpT-bm25-hit@1-ci\endcsname{[+4.5, +9.8]}
\expandafter\def\csname r@ax-bud-qasper-E-SpT-bm25-hit@1-ci95\endcsname{[+4.5, +9.8]}
\expandafter\def\csname r@ax-bud-qasper-E-SpT-bm25-hit@1-d\endcsname{+7.0}
\expandafter\def\csname r@ax-bud-qasper-E-SpT-bm25-hit@1-p\endcsname{--}
\expandafter\def\csname r@ax-bud-qasper-E-SpT-bm25-hit@1-v\endcsname{diff.}
\expandafter\def\csname r@ax-bud-qasper-E-SpT-bm25-hit@5\endcsname{+6.9 [+4.4, +9.4]}
\expandafter\def\csname r@ax-bud-qasper-E-SpT-bm25-hit@5-ci\endcsname{[+4.4, +9.4]}
\expandafter\def\csname r@ax-bud-qasper-E-SpT-bm25-hit@5-ci95\endcsname{[+4.4, +9.4]}
\expandafter\def\csname r@ax-bud-qasper-E-SpT-bm25-hit@5-d\endcsname{+6.9}
\expandafter\def\csname r@ax-bud-qasper-E-SpT-bm25-hit@5-p\endcsname{--}
\expandafter\def\csname r@ax-bud-qasper-E-SpT-bm25-hit@5-v\endcsname{diff.}
\expandafter\def\csname r@ax-bud-qasper-E-SpT-bm25-rec@1024t\endcsname{+7.5 [+5.4, +9.8]}
\expandafter\def\csname r@ax-bud-qasper-E-SpT-bm25-rec@1024t-ci\endcsname{[+5.4, +9.8]}
\expandafter\def\csname r@ax-bud-qasper-E-SpT-bm25-rec@1024t-ci95\endcsname{[+5.4, +9.8]}
\expandafter\def\csname r@ax-bud-qasper-E-SpT-bm25-rec@1024t-d\endcsname{+7.5}
\expandafter\def\csname r@ax-bud-qasper-E-SpT-bm25-rec@1024t-p\endcsname{--}
\expandafter\def\csname r@ax-bud-qasper-E-SpT-bm25-rec@1024t-v\endcsname{diff.}
\expandafter\def\csname r@ax-bud-qasper-E-SpT-bm25-rec@256t\endcsname{+6.0 [+4.2, +8.1]}
\expandafter\def\csname r@ax-bud-qasper-E-SpT-bm25-rec@256t-ci\endcsname{[+4.2, +8.1]}
\expandafter\def\csname r@ax-bud-qasper-E-SpT-bm25-rec@256t-ci95\endcsname{[+4.2, +8.1]}
\expandafter\def\csname r@ax-bud-qasper-E-SpT-bm25-rec@256t-d\endcsname{+6.0}
\expandafter\def\csname r@ax-bud-qasper-E-SpT-bm25-rec@256t-p\endcsname{--}
\expandafter\def\csname r@ax-bud-qasper-E-SpT-bm25-rec@256t-v\endcsname{diff.}
\expandafter\def\csname r@ax-bud-qasper-E-SpT-bm25-rec@5\endcsname{+6.4 [+4.2, +8.7]}
\expandafter\def\csname r@ax-bud-qasper-E-SpT-bm25-rec@5-ci\endcsname{[+4.2, +8.7]}
\expandafter\def\csname r@ax-bud-qasper-E-SpT-bm25-rec@5-ci95\endcsname{[+4.2, +8.7]}
\expandafter\def\csname r@ax-bud-qasper-E-SpT-bm25-rec@5-d\endcsname{+6.4}
\expandafter\def\csname r@ax-bud-qasper-E-SpT-bm25-rec@5-p\endcsname{--}
\expandafter\def\csname r@ax-bud-qasper-E-SpT-bm25-rec@5-v\endcsname{diff.}
\expandafter\def\csname r@ax-bud-qasper-E-SpT-bm25-rec@512t\endcsname{+8.7 [+6.6, +10.8]}
\expandafter\def\csname r@ax-bud-qasper-E-SpT-bm25-rec@512t-ci\endcsname{[+6.6, +10.8]}
\expandafter\def\csname r@ax-bud-qasper-E-SpT-bm25-rec@512t-ci95\endcsname{[+6.6, +10.8]}
\expandafter\def\csname r@ax-bud-qasper-E-SpT-bm25-rec@512t-d\endcsname{+8.7}
\expandafter\def\csname r@ax-bud-qasper-E-SpT-bm25-rec@512t-p\endcsname{--}
\expandafter\def\csname r@ax-bud-qasper-E-SpT-bm25-rec@512t-v\endcsname{diff.}
\expandafter\def\csname r@ax-bud-qasper-E-SpT-hyb-hit@1\endcsname{+5.2 [+2.2, +8.2]}
\expandafter\def\csname r@ax-bud-qasper-E-SpT-hyb-hit@1-ci\endcsname{[+2.2, +8.2]}
\expandafter\def\csname r@ax-bud-qasper-E-SpT-hyb-hit@1-ci95\endcsname{[+2.2, +8.2]}
\expandafter\def\csname r@ax-bud-qasper-E-SpT-hyb-hit@1-d\endcsname{+5.2}
\expandafter\def\csname r@ax-bud-qasper-E-SpT-hyb-hit@1-p\endcsname{--}
\expandafter\def\csname r@ax-bud-qasper-E-SpT-hyb-hit@1-v\endcsname{diff.}
\expandafter\def\csname r@ax-bud-qasper-E-SpT-hyb-hit@5\endcsname{+2.7 [+0.2, +5.3]}
\expandafter\def\csname r@ax-bud-qasper-E-SpT-hyb-hit@5-ci\endcsname{[+0.2, +5.3]}
\expandafter\def\csname r@ax-bud-qasper-E-SpT-hyb-hit@5-ci95\endcsname{[+0.2, +5.3]}
\expandafter\def\csname r@ax-bud-qasper-E-SpT-hyb-hit@5-d\endcsname{+2.7}
\expandafter\def\csname r@ax-bud-qasper-E-SpT-hyb-hit@5-p\endcsname{--}
\expandafter\def\csname r@ax-bud-qasper-E-SpT-hyb-hit@5-v\endcsname{diff.}
\expandafter\def\csname r@ax-bud-qasper-E-SpT-hyb-rec@1024t\endcsname{+2.6 [+0.4, +4.9]}
\expandafter\def\csname r@ax-bud-qasper-E-SpT-hyb-rec@1024t-ci\endcsname{[+0.4, +4.9]}
\expandafter\def\csname r@ax-bud-qasper-E-SpT-hyb-rec@1024t-ci95\endcsname{[+0.4, +4.9]}
\expandafter\def\csname r@ax-bud-qasper-E-SpT-hyb-rec@1024t-d\endcsname{+2.6}
\expandafter\def\csname r@ax-bud-qasper-E-SpT-hyb-rec@1024t-p\endcsname{--}
\expandafter\def\csname r@ax-bud-qasper-E-SpT-hyb-rec@1024t-v\endcsname{diff.}
\expandafter\def\csname r@ax-bud-qasper-E-SpT-hyb-rec@256t\endcsname{+3.6 [+1.3, +5.9]}
\expandafter\def\csname r@ax-bud-qasper-E-SpT-hyb-rec@256t-ci\endcsname{[+1.3, +5.9]}
\expandafter\def\csname r@ax-bud-qasper-E-SpT-hyb-rec@256t-ci95\endcsname{[+1.3, +5.9]}
\expandafter\def\csname r@ax-bud-qasper-E-SpT-hyb-rec@256t-d\endcsname{+3.6}
\expandafter\def\csname r@ax-bud-qasper-E-SpT-hyb-rec@256t-p\endcsname{--}
\expandafter\def\csname r@ax-bud-qasper-E-SpT-hyb-rec@256t-v\endcsname{diff.}
\expandafter\def\csname r@ax-bud-qasper-E-SpT-hyb-rec@5\endcsname{+2.7 [+0.4, +5.2]}
\expandafter\def\csname r@ax-bud-qasper-E-SpT-hyb-rec@5-ci\endcsname{[+0.4, +5.2]}
\expandafter\def\csname r@ax-bud-qasper-E-SpT-hyb-rec@5-ci95\endcsname{[+0.4, +5.2]}
\expandafter\def\csname r@ax-bud-qasper-E-SpT-hyb-rec@5-d\endcsname{+2.7}
\expandafter\def\csname r@ax-bud-qasper-E-SpT-hyb-rec@5-p\endcsname{--}
\expandafter\def\csname r@ax-bud-qasper-E-SpT-hyb-rec@5-v\endcsname{diff.}
\expandafter\def\csname r@ax-bud-qasper-E-SpT-hyb-rec@512t\endcsname{+5.5 [+2.9, +8.1]}
\expandafter\def\csname r@ax-bud-qasper-E-SpT-hyb-rec@512t-ci\endcsname{[+2.9, +8.1]}
\expandafter\def\csname r@ax-bud-qasper-E-SpT-hyb-rec@512t-ci95\endcsname{[+2.9, +8.1]}
\expandafter\def\csname r@ax-bud-qasper-E-SpT-hyb-rec@512t-d\endcsname{+5.5}
\expandafter\def\csname r@ax-bud-qasper-E-SpT-hyb-rec@512t-p\endcsname{--}
\expandafter\def\csname r@ax-bud-qasper-E-SpT-hyb-rec@512t-v\endcsname{diff.}
\expandafter\def\csname r@ax-bud-qasper-E-SpT-nomic-hit@1\endcsname{+2.7 [$-$0.3, +5.8]}
\expandafter\def\csname r@ax-bud-qasper-E-SpT-nomic-hit@1-ci\endcsname{[$-$0.3, +5.8]}
\expandafter\def\csname r@ax-bud-qasper-E-SpT-nomic-hit@1-ci95\endcsname{[$-$0.3, +5.8]}
\expandafter\def\csname r@ax-bud-qasper-E-SpT-nomic-hit@1-d\endcsname{+2.7}
\expandafter\def\csname r@ax-bud-qasper-E-SpT-nomic-hit@1-p\endcsname{--}
\expandafter\def\csname r@ax-bud-qasper-E-SpT-nomic-hit@1-v\endcsname{n.d.}
\expandafter\def\csname r@ax-bud-qasper-E-SpT-nomic-hit@5\endcsname{+1.8 [$-$0.9, +4.4]}
\expandafter\def\csname r@ax-bud-qasper-E-SpT-nomic-hit@5-ci\endcsname{[$-$0.9, +4.4]}
\expandafter\def\csname r@ax-bud-qasper-E-SpT-nomic-hit@5-ci95\endcsname{[$-$0.9, +4.4]}
\expandafter\def\csname r@ax-bud-qasper-E-SpT-nomic-hit@5-d\endcsname{+1.8}
\expandafter\def\csname r@ax-bud-qasper-E-SpT-nomic-hit@5-p\endcsname{--}
\expandafter\def\csname r@ax-bud-qasper-E-SpT-nomic-hit@5-v\endcsname{n.d.}
\expandafter\def\csname r@ax-bud-qasper-E-SpT-nomic-rec@1024t\endcsname{+2.5 [+0.3, +4.9]}
\expandafter\def\csname r@ax-bud-qasper-E-SpT-nomic-rec@1024t-ci\endcsname{[+0.3, +4.9]}
\expandafter\def\csname r@ax-bud-qasper-E-SpT-nomic-rec@1024t-ci95\endcsname{[+0.3, +4.9]}
\expandafter\def\csname r@ax-bud-qasper-E-SpT-nomic-rec@1024t-d\endcsname{+2.5}
\expandafter\def\csname r@ax-bud-qasper-E-SpT-nomic-rec@1024t-p\endcsname{--}
\expandafter\def\csname r@ax-bud-qasper-E-SpT-nomic-rec@1024t-v\endcsname{diff.}
\expandafter\def\csname r@ax-bud-qasper-E-SpT-nomic-rec@256t\endcsname{+2.4 [$-$0.1, +4.9]}
\expandafter\def\csname r@ax-bud-qasper-E-SpT-nomic-rec@256t-ci\endcsname{[$-$0.1, +4.9]}
\expandafter\def\csname r@ax-bud-qasper-E-SpT-nomic-rec@256t-ci95\endcsname{[$-$0.1, +4.9]}
\expandafter\def\csname r@ax-bud-qasper-E-SpT-nomic-rec@256t-d\endcsname{+2.4}
\expandafter\def\csname r@ax-bud-qasper-E-SpT-nomic-rec@256t-p\endcsname{--}
\expandafter\def\csname r@ax-bud-qasper-E-SpT-nomic-rec@256t-v\endcsname{n.d.}
\expandafter\def\csname r@ax-bud-qasper-E-SpT-nomic-rec@5\endcsname{+1.8 [$-$0.6, +4.2]}
\expandafter\def\csname r@ax-bud-qasper-E-SpT-nomic-rec@5-ci\endcsname{[$-$0.6, +4.2]}
\expandafter\def\csname r@ax-bud-qasper-E-SpT-nomic-rec@5-ci95\endcsname{[$-$0.6, +4.2]}
\expandafter\def\csname r@ax-bud-qasper-E-SpT-nomic-rec@5-d\endcsname{+1.8}
\expandafter\def\csname r@ax-bud-qasper-E-SpT-nomic-rec@5-p\endcsname{--}
\expandafter\def\csname r@ax-bud-qasper-E-SpT-nomic-rec@5-v\endcsname{n.d.}
\expandafter\def\csname r@ax-bud-qasper-E-SpT-nomic-rec@512t\endcsname{+0.9 [$-$1.7, +3.3]}
\expandafter\def\csname r@ax-bud-qasper-E-SpT-nomic-rec@512t-ci\endcsname{[$-$1.7, +3.3]}
\expandafter\def\csname r@ax-bud-qasper-E-SpT-nomic-rec@512t-ci95\endcsname{[$-$1.7, +3.3]}
\expandafter\def\csname r@ax-bud-qasper-E-SpT-nomic-rec@512t-d\endcsname{+0.9}
\expandafter\def\csname r@ax-bud-qasper-E-SpT-nomic-rec@512t-p\endcsname{--}
\expandafter\def\csname r@ax-bud-qasper-E-SpT-nomic-rec@512t-v\endcsname{n.d.}
\expandafter\def\csname r@ax-bud-qasper-E-SpT-q3-hit@1\endcsname{+2.9 [$-$0.1, +6.0]}
\expandafter\def\csname r@ax-bud-qasper-E-SpT-q3-hit@1-ci\endcsname{[$-$0.1, +6.0]}
\expandafter\def\csname r@ax-bud-qasper-E-SpT-q3-hit@1-ci95\endcsname{[$-$0.1, +6.0]}
\expandafter\def\csname r@ax-bud-qasper-E-SpT-q3-hit@1-d\endcsname{+2.9}
\expandafter\def\csname r@ax-bud-qasper-E-SpT-q3-hit@1-p\endcsname{--}
\expandafter\def\csname r@ax-bud-qasper-E-SpT-q3-hit@1-v\endcsname{n.d.}
\expandafter\def\csname r@ax-bud-qasper-E-SpT-q3-hit@5\endcsname{+1.4 [$-$0.9, +3.7]}
\expandafter\def\csname r@ax-bud-qasper-E-SpT-q3-hit@5-ci\endcsname{[$-$0.9, +3.7]}
\expandafter\def\csname r@ax-bud-qasper-E-SpT-q3-hit@5-ci95\endcsname{[$-$0.9, +3.7]}
\expandafter\def\csname r@ax-bud-qasper-E-SpT-q3-hit@5-d\endcsname{+1.4}
\expandafter\def\csname r@ax-bud-qasper-E-SpT-q3-hit@5-p\endcsname{--}
\expandafter\def\csname r@ax-bud-qasper-E-SpT-q3-hit@5-v\endcsname{n.d.}
\expandafter\def\csname r@ax-bud-qasper-E-SpT-q3-rec@1024t\endcsname{$-$0.1 [$-$2.2, +2.1]}
\expandafter\def\csname r@ax-bud-qasper-E-SpT-q3-rec@1024t-ci\endcsname{[$-$2.2, +2.1]}
\expandafter\def\csname r@ax-bud-qasper-E-SpT-q3-rec@1024t-ci95\endcsname{[$-$2.2, +2.1]}
\expandafter\def\csname r@ax-bud-qasper-E-SpT-q3-rec@1024t-d\endcsname{$-$0.1}
\expandafter\def\csname r@ax-bud-qasper-E-SpT-q3-rec@1024t-p\endcsname{--}
\expandafter\def\csname r@ax-bud-qasper-E-SpT-q3-rec@1024t-v\endcsname{n.d.}
\expandafter\def\csname r@ax-bud-qasper-E-SpT-q3-rec@256t\endcsname{+2.3 [$-$0.0, +4.7]}
\expandafter\def\csname r@ax-bud-qasper-E-SpT-q3-rec@256t-ci\endcsname{[$-$0.0, +4.7]}
\expandafter\def\csname r@ax-bud-qasper-E-SpT-q3-rec@256t-ci95\endcsname{[$-$0.0, +4.7]}
\expandafter\def\csname r@ax-bud-qasper-E-SpT-q3-rec@256t-d\endcsname{+2.3}
\expandafter\def\csname r@ax-bud-qasper-E-SpT-q3-rec@256t-p\endcsname{--}
\expandafter\def\csname r@ax-bud-qasper-E-SpT-q3-rec@256t-v\endcsname{n.d.}
\expandafter\def\csname r@ax-bud-qasper-E-SpT-q3-rec@5\endcsname{+0.9 [$-$1.3, +3.1]}
\expandafter\def\csname r@ax-bud-qasper-E-SpT-q3-rec@5-ci\endcsname{[$-$1.3, +3.1]}
\expandafter\def\csname r@ax-bud-qasper-E-SpT-q3-rec@5-ci95\endcsname{[$-$1.3, +3.1]}
\expandafter\def\csname r@ax-bud-qasper-E-SpT-q3-rec@5-d\endcsname{+0.9}
\expandafter\def\csname r@ax-bud-qasper-E-SpT-q3-rec@5-p\endcsname{--}
\expandafter\def\csname r@ax-bud-qasper-E-SpT-q3-rec@5-v\endcsname{n.d.}
\expandafter\def\csname r@ax-bud-qasper-E-SpT-q3-rec@512t\endcsname{+1.5 [$-$1.0, +3.9]}
\expandafter\def\csname r@ax-bud-qasper-E-SpT-q3-rec@512t-ci\endcsname{[$-$1.0, +3.9]}
\expandafter\def\csname r@ax-bud-qasper-E-SpT-q3-rec@512t-ci95\endcsname{[$-$1.0, +3.9]}
\expandafter\def\csname r@ax-bud-qasper-E-SpT-q3-rec@512t-d\endcsname{+1.5}
\expandafter\def\csname r@ax-bud-qasper-E-SpT-q3-rec@512t-p\endcsname{--}
\expandafter\def\csname r@ax-bud-qasper-E-SpT-q3-rec@512t-v\endcsname{n.d.}
\expandafter\def\csname r@ax-bud-qasper-E-SpT-rr-hit@1\endcsname{+2.5 [$-$0.4, +5.5]}
\expandafter\def\csname r@ax-bud-qasper-E-SpT-rr-hit@1-ci\endcsname{[$-$0.4, +5.5]}
\expandafter\def\csname r@ax-bud-qasper-E-SpT-rr-hit@1-ci95\endcsname{[$-$0.4, +5.5]}
\expandafter\def\csname r@ax-bud-qasper-E-SpT-rr-hit@1-d\endcsname{+2.5}
\expandafter\def\csname r@ax-bud-qasper-E-SpT-rr-hit@1-p\endcsname{--}
\expandafter\def\csname r@ax-bud-qasper-E-SpT-rr-hit@1-v\endcsname{n.d.}
\expandafter\def\csname r@ax-bud-qasper-E-SpT-rr-hit@5\endcsname{$-$2.2 [$-$4.1, $-$0.3]}
\expandafter\def\csname r@ax-bud-qasper-E-SpT-rr-hit@5-ci\endcsname{[$-$4.1, $-$0.3]}
\expandafter\def\csname r@ax-bud-qasper-E-SpT-rr-hit@5-ci95\endcsname{[$-$4.1, $-$0.3]}
\expandafter\def\csname r@ax-bud-qasper-E-SpT-rr-hit@5-d\endcsname{$-$2.2}
\expandafter\def\csname r@ax-bud-qasper-E-SpT-rr-hit@5-p\endcsname{--}
\expandafter\def\csname r@ax-bud-qasper-E-SpT-rr-hit@5-v\endcsname{diff.}
\expandafter\def\csname r@ax-bud-qasper-E-SpT-rr-rec@1024t\endcsname{$-$1.9 [$-$4.0, $-$0.1]}
\expandafter\def\csname r@ax-bud-qasper-E-SpT-rr-rec@1024t-ci\endcsname{[$-$4.0, $-$0.1]}
\expandafter\def\csname r@ax-bud-qasper-E-SpT-rr-rec@1024t-ci95\endcsname{[$-$4.0, $-$0.1]}
\expandafter\def\csname r@ax-bud-qasper-E-SpT-rr-rec@1024t-d\endcsname{$-$1.9}
\expandafter\def\csname r@ax-bud-qasper-E-SpT-rr-rec@1024t-p\endcsname{--}
\expandafter\def\csname r@ax-bud-qasper-E-SpT-rr-rec@1024t-v\endcsname{diff.}
\expandafter\def\csname r@ax-bud-qasper-E-SpT-rr-rec@256t\endcsname{+1.8 [$-$0.4, +4.1]}
\expandafter\def\csname r@ax-bud-qasper-E-SpT-rr-rec@256t-ci\endcsname{[$-$0.4, +4.1]}
\expandafter\def\csname r@ax-bud-qasper-E-SpT-rr-rec@256t-ci95\endcsname{[$-$0.4, +4.1]}
\expandafter\def\csname r@ax-bud-qasper-E-SpT-rr-rec@256t-d\endcsname{+1.8}
\expandafter\def\csname r@ax-bud-qasper-E-SpT-rr-rec@256t-p\endcsname{--}
\expandafter\def\csname r@ax-bud-qasper-E-SpT-rr-rec@256t-v\endcsname{n.d.}
\expandafter\def\csname r@ax-bud-qasper-E-SpT-rr-rec@5\endcsname{$-$2.1 [$-$3.9, $-$0.3]}
\expandafter\def\csname r@ax-bud-qasper-E-SpT-rr-rec@5-ci\endcsname{[$-$3.9, $-$0.3]}
\expandafter\def\csname r@ax-bud-qasper-E-SpT-rr-rec@5-ci95\endcsname{[$-$3.9, $-$0.3]}
\expandafter\def\csname r@ax-bud-qasper-E-SpT-rr-rec@5-d\endcsname{$-$2.1}
\expandafter\def\csname r@ax-bud-qasper-E-SpT-rr-rec@5-p\endcsname{--}
\expandafter\def\csname r@ax-bud-qasper-E-SpT-rr-rec@5-v\endcsname{diff.}
\expandafter\def\csname r@ax-bud-qasper-E-SpT-rr-rec@512t\endcsname{+0.4 [$-$1.7, +2.5]}
\expandafter\def\csname r@ax-bud-qasper-E-SpT-rr-rec@512t-ci\endcsname{[$-$1.7, +2.5]}
\expandafter\def\csname r@ax-bud-qasper-E-SpT-rr-rec@512t-ci95\endcsname{[$-$1.7, +2.5]}
\expandafter\def\csname r@ax-bud-qasper-E-SpT-rr-rec@512t-d\endcsname{+0.4}
\expandafter\def\csname r@ax-bud-qasper-E-SpT-rr-rec@512t-p\endcsname{--}
\expandafter\def\csname r@ax-bud-qasper-E-SpT-rr-rec@512t-v\endcsname{n.d.}
\expandafter\def\csname r@ax-bud-qasper-S-F256t-bm25-hit@1\endcsname{+1.1 [$-$1.6, +3.7]}
\expandafter\def\csname r@ax-bud-qasper-S-F256t-bm25-hit@1-ci\endcsname{[$-$1.6, +3.7]}
\expandafter\def\csname r@ax-bud-qasper-S-F256t-bm25-hit@1-ci95\endcsname{[$-$1.6, +3.7]}
\expandafter\def\csname r@ax-bud-qasper-S-F256t-bm25-hit@1-d\endcsname{+1.1}
\expandafter\def\csname r@ax-bud-qasper-S-F256t-bm25-hit@1-p\endcsname{--}
\expandafter\def\csname r@ax-bud-qasper-S-F256t-bm25-hit@1-v\endcsname{n.d.}
\expandafter\def\csname r@ax-bud-qasper-S-F256t-bm25-hit@5\endcsname{$-$0.1 [$-$3.0, +2.8]}
\expandafter\def\csname r@ax-bud-qasper-S-F256t-bm25-hit@5-ci\endcsname{[$-$3.0, +2.8]}
\expandafter\def\csname r@ax-bud-qasper-S-F256t-bm25-hit@5-ci95\endcsname{[$-$3.0, +2.8]}
\expandafter\def\csname r@ax-bud-qasper-S-F256t-bm25-hit@5-d\endcsname{$-$0.1}
\expandafter\def\csname r@ax-bud-qasper-S-F256t-bm25-hit@5-p\endcsname{--}
\expandafter\def\csname r@ax-bud-qasper-S-F256t-bm25-hit@5-v\endcsname{n.d.}
\expandafter\def\csname r@ax-bud-qasper-S-F256t-bm25-rec@1024t\endcsname{+5.5 [+2.9, +8.2]}
\expandafter\def\csname r@ax-bud-qasper-S-F256t-bm25-rec@1024t-ci\endcsname{[+2.9, +8.2]}
\expandafter\def\csname r@ax-bud-qasper-S-F256t-bm25-rec@1024t-ci95\endcsname{[+2.9, +8.2]}
\expandafter\def\csname r@ax-bud-qasper-S-F256t-bm25-rec@1024t-d\endcsname{+5.5}
\expandafter\def\csname r@ax-bud-qasper-S-F256t-bm25-rec@1024t-p\endcsname{--}
\expandafter\def\csname r@ax-bud-qasper-S-F256t-bm25-rec@1024t-v\endcsname{diff.}
\expandafter\def\csname r@ax-bud-qasper-S-F256t-bm25-rec@256t\endcsname{+4.0 [+2.0, +6.0]}
\expandafter\def\csname r@ax-bud-qasper-S-F256t-bm25-rec@256t-ci\endcsname{[+2.0, +6.0]}
\expandafter\def\csname r@ax-bud-qasper-S-F256t-bm25-rec@256t-ci95\endcsname{[+2.0, +6.0]}
\expandafter\def\csname r@ax-bud-qasper-S-F256t-bm25-rec@256t-d\endcsname{+4.0}
\expandafter\def\csname r@ax-bud-qasper-S-F256t-bm25-rec@256t-p\endcsname{--}
\expandafter\def\csname r@ax-bud-qasper-S-F256t-bm25-rec@256t-v\endcsname{diff.}
\expandafter\def\csname r@ax-bud-qasper-S-F256t-bm25-rec@5\endcsname{+0.2 [$-$2.3, +2.8]}
\expandafter\def\csname r@ax-bud-qasper-S-F256t-bm25-rec@5-ci\endcsname{[$-$2.3, +2.8]}
\expandafter\def\csname r@ax-bud-qasper-S-F256t-bm25-rec@5-ci95\endcsname{[$-$2.3, +2.8]}
\expandafter\def\csname r@ax-bud-qasper-S-F256t-bm25-rec@5-d\endcsname{+0.2}
\expandafter\def\csname r@ax-bud-qasper-S-F256t-bm25-rec@5-p\endcsname{--}
\expandafter\def\csname r@ax-bud-qasper-S-F256t-bm25-rec@5-v\endcsname{n.d.}
\expandafter\def\csname r@ax-bud-qasper-S-F256t-bm25-rec@512t\endcsname{+5.7 [+3.5, +7.8]}
\expandafter\def\csname r@ax-bud-qasper-S-F256t-bm25-rec@512t-ci\endcsname{[+3.5, +7.8]}
\expandafter\def\csname r@ax-bud-qasper-S-F256t-bm25-rec@512t-ci95\endcsname{[+3.5, +7.8]}
\expandafter\def\csname r@ax-bud-qasper-S-F256t-bm25-rec@512t-d\endcsname{+5.7}
\expandafter\def\csname r@ax-bud-qasper-S-F256t-bm25-rec@512t-p\endcsname{--}
\expandafter\def\csname r@ax-bud-qasper-S-F256t-bm25-rec@512t-v\endcsname{diff.}
\expandafter\def\csname r@ax-bud-qasper-S-F256t-hyb-hit@1\endcsname{+2.2 [$-$0.8, +5.2]}
\expandafter\def\csname r@ax-bud-qasper-S-F256t-hyb-hit@1-ci\endcsname{[$-$0.8, +5.2]}
\expandafter\def\csname r@ax-bud-qasper-S-F256t-hyb-hit@1-ci95\endcsname{[$-$0.8, +5.2]}
\expandafter\def\csname r@ax-bud-qasper-S-F256t-hyb-hit@1-d\endcsname{+2.2}
\expandafter\def\csname r@ax-bud-qasper-S-F256t-hyb-hit@1-p\endcsname{--}
\expandafter\def\csname r@ax-bud-qasper-S-F256t-hyb-hit@1-v\endcsname{n.d.}
\expandafter\def\csname r@ax-bud-qasper-S-F256t-hyb-hit@5\endcsname{+3.5 [+0.5, +6.2]}
\expandafter\def\csname r@ax-bud-qasper-S-F256t-hyb-hit@5-ci\endcsname{[+0.5, +6.2]}
\expandafter\def\csname r@ax-bud-qasper-S-F256t-hyb-hit@5-ci95\endcsname{[+0.5, +6.2]}
\expandafter\def\csname r@ax-bud-qasper-S-F256t-hyb-hit@5-d\endcsname{+3.5}
\expandafter\def\csname r@ax-bud-qasper-S-F256t-hyb-hit@5-p\endcsname{--}
\expandafter\def\csname r@ax-bud-qasper-S-F256t-hyb-hit@5-v\endcsname{diff.}
\expandafter\def\csname r@ax-bud-qasper-S-F256t-hyb-rec@1024t\endcsname{+9.2 [+6.7, +11.8]}
\expandafter\def\csname r@ax-bud-qasper-S-F256t-hyb-rec@1024t-ci\endcsname{[+6.7, +11.8]}
\expandafter\def\csname r@ax-bud-qasper-S-F256t-hyb-rec@1024t-ci95\endcsname{[+6.7, +11.8]}
\expandafter\def\csname r@ax-bud-qasper-S-F256t-hyb-rec@1024t-d\endcsname{+9.2}
\expandafter\def\csname r@ax-bud-qasper-S-F256t-hyb-rec@1024t-p\endcsname{--}
\expandafter\def\csname r@ax-bud-qasper-S-F256t-hyb-rec@1024t-v\endcsname{diff.}
\expandafter\def\csname r@ax-bud-qasper-S-F256t-hyb-rec@256t\endcsname{+6.7 [+4.4, +9.0]}
\expandafter\def\csname r@ax-bud-qasper-S-F256t-hyb-rec@256t-ci\endcsname{[+4.4, +9.0]}
\expandafter\def\csname r@ax-bud-qasper-S-F256t-hyb-rec@256t-ci95\endcsname{[+4.4, +9.0]}
\expandafter\def\csname r@ax-bud-qasper-S-F256t-hyb-rec@256t-d\endcsname{+6.7}
\expandafter\def\csname r@ax-bud-qasper-S-F256t-hyb-rec@256t-p\endcsname{--}
\expandafter\def\csname r@ax-bud-qasper-S-F256t-hyb-rec@256t-v\endcsname{diff.}
\expandafter\def\csname r@ax-bud-qasper-S-F256t-hyb-rec@5\endcsname{+3.4 [+0.7, +6.0]}
\expandafter\def\csname r@ax-bud-qasper-S-F256t-hyb-rec@5-ci\endcsname{[+0.7, +6.0]}
\expandafter\def\csname r@ax-bud-qasper-S-F256t-hyb-rec@5-ci95\endcsname{[+0.7, +6.0]}
\expandafter\def\csname r@ax-bud-qasper-S-F256t-hyb-rec@5-d\endcsname{+3.4}
\expandafter\def\csname r@ax-bud-qasper-S-F256t-hyb-rec@5-p\endcsname{--}
\expandafter\def\csname r@ax-bud-qasper-S-F256t-hyb-rec@5-v\endcsname{diff.}
\expandafter\def\csname r@ax-bud-qasper-S-F256t-hyb-rec@512t\endcsname{+7.5 [+5.0, +10.1]}
\expandafter\def\csname r@ax-bud-qasper-S-F256t-hyb-rec@512t-ci\endcsname{[+5.0, +10.1]}
\expandafter\def\csname r@ax-bud-qasper-S-F256t-hyb-rec@512t-ci95\endcsname{[+5.0, +10.1]}
\expandafter\def\csname r@ax-bud-qasper-S-F256t-hyb-rec@512t-d\endcsname{+7.5}
\expandafter\def\csname r@ax-bud-qasper-S-F256t-hyb-rec@512t-p\endcsname{--}
\expandafter\def\csname r@ax-bud-qasper-S-F256t-hyb-rec@512t-v\endcsname{diff.}
\expandafter\def\csname r@ax-bud-qasper-S-F256t-nomic-hit@1\endcsname{+3.7 [+0.3, +7.0]}
\expandafter\def\csname r@ax-bud-qasper-S-F256t-nomic-hit@1-ci\endcsname{[+0.3, +7.0]}
\expandafter\def\csname r@ax-bud-qasper-S-F256t-nomic-hit@1-ci95\endcsname{[+0.3, +7.0]}
\expandafter\def\csname r@ax-bud-qasper-S-F256t-nomic-hit@1-d\endcsname{+3.7}
\expandafter\def\csname r@ax-bud-qasper-S-F256t-nomic-hit@1-p\endcsname{--}
\expandafter\def\csname r@ax-bud-qasper-S-F256t-nomic-hit@1-v\endcsname{diff.}
\expandafter\def\csname r@ax-bud-qasper-S-F256t-nomic-hit@5\endcsname{+3.2 [+0.2, +6.1]}
\expandafter\def\csname r@ax-bud-qasper-S-F256t-nomic-hit@5-ci\endcsname{[+0.2, +6.1]}
\expandafter\def\csname r@ax-bud-qasper-S-F256t-nomic-hit@5-ci95\endcsname{[+0.2, +6.1]}
\expandafter\def\csname r@ax-bud-qasper-S-F256t-nomic-hit@5-d\endcsname{+3.2}
\expandafter\def\csname r@ax-bud-qasper-S-F256t-nomic-hit@5-p\endcsname{--}
\expandafter\def\csname r@ax-bud-qasper-S-F256t-nomic-hit@5-v\endcsname{diff.}
\expandafter\def\csname r@ax-bud-qasper-S-F256t-nomic-rec@1024t\endcsname{+9.0 [+6.2, +12.1]}
\expandafter\def\csname r@ax-bud-qasper-S-F256t-nomic-rec@1024t-ci\endcsname{[+6.2, +12.1]}
\expandafter\def\csname r@ax-bud-qasper-S-F256t-nomic-rec@1024t-ci95\endcsname{[+6.2, +12.1]}
\expandafter\def\csname r@ax-bud-qasper-S-F256t-nomic-rec@1024t-d\endcsname{+9.0}
\expandafter\def\csname r@ax-bud-qasper-S-F256t-nomic-rec@1024t-p\endcsname{--}
\expandafter\def\csname r@ax-bud-qasper-S-F256t-nomic-rec@1024t-v\endcsname{diff.}
\expandafter\def\csname r@ax-bud-qasper-S-F256t-nomic-rec@256t\endcsname{+8.8 [+6.1, +11.5]}
\expandafter\def\csname r@ax-bud-qasper-S-F256t-nomic-rec@256t-ci\endcsname{[+6.1, +11.5]}
\expandafter\def\csname r@ax-bud-qasper-S-F256t-nomic-rec@256t-ci95\endcsname{[+6.1, +11.5]}
\expandafter\def\csname r@ax-bud-qasper-S-F256t-nomic-rec@256t-d\endcsname{+8.8}
\expandafter\def\csname r@ax-bud-qasper-S-F256t-nomic-rec@256t-p\endcsname{--}
\expandafter\def\csname r@ax-bud-qasper-S-F256t-nomic-rec@256t-v\endcsname{diff.}
\expandafter\def\csname r@ax-bud-qasper-S-F256t-nomic-rec@5\endcsname{+2.7 [$-$0.1, +5.5]}
\expandafter\def\csname r@ax-bud-qasper-S-F256t-nomic-rec@5-ci\endcsname{[$-$0.1, +5.5]}
\expandafter\def\csname r@ax-bud-qasper-S-F256t-nomic-rec@5-ci95\endcsname{[$-$0.1, +5.5]}
\expandafter\def\csname r@ax-bud-qasper-S-F256t-nomic-rec@5-d\endcsname{+2.7}
\expandafter\def\csname r@ax-bud-qasper-S-F256t-nomic-rec@5-p\endcsname{--}
\expandafter\def\csname r@ax-bud-qasper-S-F256t-nomic-rec@5-v\endcsname{n.d.}
\expandafter\def\csname r@ax-bud-qasper-S-F256t-nomic-rec@512t\endcsname{+10.4 [+7.7, +13.4]}
\expandafter\def\csname r@ax-bud-qasper-S-F256t-nomic-rec@512t-ci\endcsname{[+7.7, +13.4]}
\expandafter\def\csname r@ax-bud-qasper-S-F256t-nomic-rec@512t-ci95\endcsname{[+7.7, +13.4]}
\expandafter\def\csname r@ax-bud-qasper-S-F256t-nomic-rec@512t-d\endcsname{+10.4}
\expandafter\def\csname r@ax-bud-qasper-S-F256t-nomic-rec@512t-p\endcsname{--}
\expandafter\def\csname r@ax-bud-qasper-S-F256t-nomic-rec@512t-v\endcsname{diff.}
\expandafter\def\csname r@ax-bud-qasper-S-F256t-q3-hit@1\endcsname{+0.5 [$-$2.8, +3.7]}
\expandafter\def\csname r@ax-bud-qasper-S-F256t-q3-hit@1-ci\endcsname{[$-$2.8, +3.7]}
\expandafter\def\csname r@ax-bud-qasper-S-F256t-q3-hit@1-ci95\endcsname{[$-$2.8, +3.7]}
\expandafter\def\csname r@ax-bud-qasper-S-F256t-q3-hit@1-d\endcsname{+0.5}
\expandafter\def\csname r@ax-bud-qasper-S-F256t-q3-hit@1-p\endcsname{--}
\expandafter\def\csname r@ax-bud-qasper-S-F256t-q3-hit@1-v\endcsname{n.d.}
\expandafter\def\csname r@ax-bud-qasper-S-F256t-q3-hit@5\endcsname{+0.2 [$-$2.3, +2.8]}
\expandafter\def\csname r@ax-bud-qasper-S-F256t-q3-hit@5-ci\endcsname{[$-$2.3, +2.8]}
\expandafter\def\csname r@ax-bud-qasper-S-F256t-q3-hit@5-ci95\endcsname{[$-$2.3, +2.8]}
\expandafter\def\csname r@ax-bud-qasper-S-F256t-q3-hit@5-d\endcsname{+0.2}
\expandafter\def\csname r@ax-bud-qasper-S-F256t-q3-hit@5-p\endcsname{--}
\expandafter\def\csname r@ax-bud-qasper-S-F256t-q3-hit@5-v\endcsname{n.d.}
\expandafter\def\csname r@ax-bud-qasper-S-F256t-q3-rec@1024t\endcsname{+6.2 [+3.7, +8.6]}
\expandafter\def\csname r@ax-bud-qasper-S-F256t-q3-rec@1024t-ci\endcsname{[+3.7, +8.6]}
\expandafter\def\csname r@ax-bud-qasper-S-F256t-q3-rec@1024t-ci95\endcsname{[+3.7, +8.6]}
\expandafter\def\csname r@ax-bud-qasper-S-F256t-q3-rec@1024t-d\endcsname{+6.2}
\expandafter\def\csname r@ax-bud-qasper-S-F256t-q3-rec@1024t-p\endcsname{--}
\expandafter\def\csname r@ax-bud-qasper-S-F256t-q3-rec@1024t-v\endcsname{diff.}
\expandafter\def\csname r@ax-bud-qasper-S-F256t-q3-rec@256t\endcsname{+7.2 [+4.6, +9.8]}
\expandafter\def\csname r@ax-bud-qasper-S-F256t-q3-rec@256t-ci\endcsname{[+4.6, +9.8]}
\expandafter\def\csname r@ax-bud-qasper-S-F256t-q3-rec@256t-ci95\endcsname{[+4.6, +9.8]}
\expandafter\def\csname r@ax-bud-qasper-S-F256t-q3-rec@256t-d\endcsname{+7.2}
\expandafter\def\csname r@ax-bud-qasper-S-F256t-q3-rec@256t-p\endcsname{--}
\expandafter\def\csname r@ax-bud-qasper-S-F256t-q3-rec@256t-v\endcsname{diff.}
\expandafter\def\csname r@ax-bud-qasper-S-F256t-q3-rec@5\endcsname{$-$0.1 [$-$2.6, +2.4]}
\expandafter\def\csname r@ax-bud-qasper-S-F256t-q3-rec@5-ci\endcsname{[$-$2.6, +2.4]}
\expandafter\def\csname r@ax-bud-qasper-S-F256t-q3-rec@5-ci95\endcsname{[$-$2.6, +2.4]}
\expandafter\def\csname r@ax-bud-qasper-S-F256t-q3-rec@5-d\endcsname{$-$0.1}
\expandafter\def\csname r@ax-bud-qasper-S-F256t-q3-rec@5-p\endcsname{--}
\expandafter\def\csname r@ax-bud-qasper-S-F256t-q3-rec@5-v\endcsname{n.d.}
\expandafter\def\csname r@ax-bud-qasper-S-F256t-q3-rec@512t\endcsname{+7.3 [+4.9, +9.6]}
\expandafter\def\csname r@ax-bud-qasper-S-F256t-q3-rec@512t-ci\endcsname{[+4.9, +9.6]}
\expandafter\def\csname r@ax-bud-qasper-S-F256t-q3-rec@512t-ci95\endcsname{[+4.9, +9.6]}
\expandafter\def\csname r@ax-bud-qasper-S-F256t-q3-rec@512t-d\endcsname{+7.3}
\expandafter\def\csname r@ax-bud-qasper-S-F256t-q3-rec@512t-p\endcsname{--}
\expandafter\def\csname r@ax-bud-qasper-S-F256t-q3-rec@512t-v\endcsname{diff.}
\expandafter\def\csname r@ax-bud-qasper-S-F256t-rr-hit@1\endcsname{+4.3 [+1.3, +7.5]}
\expandafter\def\csname r@ax-bud-qasper-S-F256t-rr-hit@1-ci\endcsname{[+1.3, +7.5]}
\expandafter\def\csname r@ax-bud-qasper-S-F256t-rr-hit@1-ci95\endcsname{[+1.3, +7.5]}
\expandafter\def\csname r@ax-bud-qasper-S-F256t-rr-hit@1-d\endcsname{+4.3}
\expandafter\def\csname r@ax-bud-qasper-S-F256t-rr-hit@1-p\endcsname{--}
\expandafter\def\csname r@ax-bud-qasper-S-F256t-rr-hit@1-v\endcsname{diff.}
\expandafter\def\csname r@ax-bud-qasper-S-F256t-rr-hit@5\endcsname{+2.8 [+0.6, +5.1]}
\expandafter\def\csname r@ax-bud-qasper-S-F256t-rr-hit@5-ci\endcsname{[+0.6, +5.1]}
\expandafter\def\csname r@ax-bud-qasper-S-F256t-rr-hit@5-ci95\endcsname{[+0.6, +5.1]}
\expandafter\def\csname r@ax-bud-qasper-S-F256t-rr-hit@5-d\endcsname{+2.8}
\expandafter\def\csname r@ax-bud-qasper-S-F256t-rr-hit@5-p\endcsname{--}
\expandafter\def\csname r@ax-bud-qasper-S-F256t-rr-hit@5-v\endcsname{diff.}
\expandafter\def\csname r@ax-bud-qasper-S-F256t-rr-rec@1024t\endcsname{+10.4 [+8.3, +12.7]}
\expandafter\def\csname r@ax-bud-qasper-S-F256t-rr-rec@1024t-ci\endcsname{[+8.3, +12.7]}
\expandafter\def\csname r@ax-bud-qasper-S-F256t-rr-rec@1024t-ci95\endcsname{[+8.3, +12.7]}
\expandafter\def\csname r@ax-bud-qasper-S-F256t-rr-rec@1024t-d\endcsname{+10.4}
\expandafter\def\csname r@ax-bud-qasper-S-F256t-rr-rec@1024t-p\endcsname{--}
\expandafter\def\csname r@ax-bud-qasper-S-F256t-rr-rec@1024t-v\endcsname{diff.}
\expandafter\def\csname r@ax-bud-qasper-S-F256t-rr-rec@256t\endcsname{+9.0 [+6.5, +11.6]}
\expandafter\def\csname r@ax-bud-qasper-S-F256t-rr-rec@256t-ci\endcsname{[+6.5, +11.6]}
\expandafter\def\csname r@ax-bud-qasper-S-F256t-rr-rec@256t-ci95\endcsname{[+6.5, +11.6]}
\expandafter\def\csname r@ax-bud-qasper-S-F256t-rr-rec@256t-d\endcsname{+9.0}
\expandafter\def\csname r@ax-bud-qasper-S-F256t-rr-rec@256t-p\endcsname{--}
\expandafter\def\csname r@ax-bud-qasper-S-F256t-rr-rec@256t-v\endcsname{diff.}
\expandafter\def\csname r@ax-bud-qasper-S-F256t-rr-rec@5\endcsname{+3.5 [+1.3, +5.8]}
\expandafter\def\csname r@ax-bud-qasper-S-F256t-rr-rec@5-ci\endcsname{[+1.3, +5.8]}
\expandafter\def\csname r@ax-bud-qasper-S-F256t-rr-rec@5-ci95\endcsname{[+1.3, +5.8]}
\expandafter\def\csname r@ax-bud-qasper-S-F256t-rr-rec@5-d\endcsname{+3.5}
\expandafter\def\csname r@ax-bud-qasper-S-F256t-rr-rec@5-p\endcsname{--}
\expandafter\def\csname r@ax-bud-qasper-S-F256t-rr-rec@5-v\endcsname{diff.}
\expandafter\def\csname r@ax-bud-qasper-S-F256t-rr-rec@512t\endcsname{+9.3 [+6.6, +12.2]}
\expandafter\def\csname r@ax-bud-qasper-S-F256t-rr-rec@512t-ci\endcsname{[+6.6, +12.2]}
\expandafter\def\csname r@ax-bud-qasper-S-F256t-rr-rec@512t-ci95\endcsname{[+6.6, +12.2]}
\expandafter\def\csname r@ax-bud-qasper-S-F256t-rr-rec@512t-d\endcsname{+9.3}
\expandafter\def\csname r@ax-bud-qasper-S-F256t-rr-rec@512t-p\endcsname{--}
\expandafter\def\csname r@ax-bud-qasper-S-F256t-rr-rec@512t-v\endcsname{diff.}
\expandafter\def\csname r@ax-bud-qasper-nrev\endcsname{5}
\expandafter\def\csname r@ax-bud-qasper-nrevstrict\endcsname{3}
\expandafter\def\csname r@ax-f1-abstractive\endcsname{$-$2.2 [$-$8.0, +2.9]}
\expandafter\def\csname r@ax-f1-abstractive-ci\endcsname{[$-$8.0, +2.9]}
\expandafter\def\csname r@ax-f1-abstractive-ci95\endcsname{[$-$8.0, +2.9]}
\expandafter\def\csname r@ax-f1-abstractive-d\endcsname{$-$2.2}
\expandafter\def\csname r@ax-f1-abstractive-p\endcsname{--}
\expandafter\def\csname r@ax-f1-abstractive-v\endcsname{n.d.}
\expandafter\def\csname r@ax-f1-extractive\endcsname{+1.5 [$-$1.8, +4.5]}
\expandafter\def\csname r@ax-f1-extractive-ci\endcsname{[$-$1.8, +4.5]}
\expandafter\def\csname r@ax-f1-extractive-ci95\endcsname{[$-$1.8, +4.5]}
\expandafter\def\csname r@ax-f1-extractive-d\endcsname{+1.5}
\expandafter\def\csname r@ax-f1-extractive-p\endcsname{--}
\expandafter\def\csname r@ax-f1-extractive-v\endcsname{n.d.}
\expandafter\def\csname r@ax-f1-mixed\endcsname{+1.8 [$-$1.7, +5.5]}
\expandafter\def\csname r@ax-f1-mixed-ci\endcsname{[$-$1.7, +5.5]}
\expandafter\def\csname r@ax-f1-mixed-ci95\endcsname{[$-$1.7, +5.5]}
\expandafter\def\csname r@ax-f1-mixed-d\endcsname{+1.8}
\expandafter\def\csname r@ax-f1-mixed-p\endcsname{--}
\expandafter\def\csname r@ax-f1-mixed-v\endcsname{n.d.}
\expandafter\def\csname r@ax-f1-recchanged\endcsname{29}
\expandafter\def\csname r@ax-f1-recdown\endcsname{$-$16.3 [$-$23.4, $-$9.8]}
\expandafter\def\csname r@ax-f1-recdown-ci\endcsname{[$-$23.4, $-$9.8]}
\expandafter\def\csname r@ax-f1-recdown-ci95\endcsname{[$-$23.4, $-$9.8]}
\expandafter\def\csname r@ax-f1-recdown-d\endcsname{$-$16.3}
\expandafter\def\csname r@ax-f1-recdown-n\endcsname{106}
\expandafter\def\csname r@ax-f1-recdown-p\endcsname{--}
\expandafter\def\csname r@ax-f1-recdown-v\endcsname{diff.}
\expandafter\def\csname r@ax-f1-recsame\endcsname{$-$0.2 [$-$1.9, +1.5]}
\expandafter\def\csname r@ax-f1-recsame-ci\endcsname{[$-$1.9, +1.5]}
\expandafter\def\csname r@ax-f1-recsame-ci95\endcsname{[$-$1.9, +1.5]}
\expandafter\def\csname r@ax-f1-recsame-d\endcsname{$-$0.2}
\expandafter\def\csname r@ax-f1-recsame-n\endcsname{677}
\expandafter\def\csname r@ax-f1-recsame-p\endcsname{--}
\expandafter\def\csname r@ax-f1-recsame-v\endcsname{n.d.}
\expandafter\def\csname r@ax-f1-recup\endcsname{+18.9 [+12.4, +25.3]}
\expandafter\def\csname r@ax-f1-recup-ci\endcsname{[+12.4, +25.3]}
\expandafter\def\csname r@ax-f1-recup-ci95\endcsname{[+12.4, +25.3]}
\expandafter\def\csname r@ax-f1-recup-d\endcsname{+18.9}
\expandafter\def\csname r@ax-f1-recup-n\endcsname{168}
\expandafter\def\csname r@ax-f1-recup-p\endcsname{--}
\expandafter\def\csname r@ax-f1-recup-v\endcsname{diff.}
\expandafter\def\csname r@ax-f1-rho\endcsname{0.33}
\expandafter\def\csname r@ax-f1-updown\endcsname{+35.2 [+26.1, +44.5]}
\expandafter\def\csname r@ax-f1-updown-ci\endcsname{[+26.1, +44.5]}
\expandafter\def\csname r@ax-f1-updown-ci95\endcsname{[+26.1, +44.5]}
\expandafter\def\csname r@ax-f1-updown-d\endcsname{+35.2}
\expandafter\def\csname r@ax-f1-updown-p\endcsname{--}
\expandafter\def\csname r@ax-f1-updown-v\endcsname{diff.}
\expandafter\def\csname r@ax-f1-yesno\endcsname{+2.9 [$-$1.4, +7.7]}
\expandafter\def\csname r@ax-f1-yesno-ci\endcsname{[$-$1.4, +7.7]}
\expandafter\def\csname r@ax-f1-yesno-ci95\endcsname{[$-$1.4, +7.7]}
\expandafter\def\csname r@ax-f1-yesno-d\endcsname{+2.9}
\expandafter\def\csname r@ax-f1-yesno-p\endcsname{--}
\expandafter\def\csname r@ax-f1-yesno-v\endcsname{n.d.}
\expandafter\def\csname r@ax-fr-fs-CRq3-STq3\endcsname{+0.9 [$-$1.0, +2.8]}
\expandafter\def\csname r@ax-fr-fs-CRq3-STq3-ci\endcsname{[$-$1.0, +2.8]}
\expandafter\def\csname r@ax-fr-fs-CRq3-STq3-ci95\endcsname{[$-$1.0, +2.8]}
\expandafter\def\csname r@ax-fr-fs-CRq3-STq3-d\endcsname{+0.9}
\expandafter\def\csname r@ax-fr-fs-CRq3-STq3-p\endcsname{--}
\expandafter\def\csname r@ax-fr-fs-CRq3-STq3-v\endcsname{equiv.}
\expandafter\def\csname r@ax-fr-fs-Ehyb-SThyb\endcsname{+2.7 [+0.5, +5.1]}
\expandafter\def\csname r@ax-fr-fs-Ehyb-SThyb-ci\endcsname{[+0.5, +5.1]}
\expandafter\def\csname r@ax-fr-fs-Ehyb-SThyb-ci95\endcsname{[+0.5, +5.1]}
\expandafter\def\csname r@ax-fr-fs-Ehyb-SThyb-d\endcsname{+2.7}
\expandafter\def\csname r@ax-fr-fs-Ehyb-SThyb-p\endcsname{--}
\expandafter\def\csname r@ax-fr-fs-Ehyb-SThyb-v\endcsname{diff.}
\expandafter\def\csname r@ax-fr-fs-Enomic-Ehyb\endcsname{$-$1.3 [$-$3.9, +1.3]}
\expandafter\def\csname r@ax-fr-fs-Enomic-Ehyb-ci\endcsname{[$-$3.9, +1.3]}
\expandafter\def\csname r@ax-fr-fs-Enomic-Ehyb-ci95\endcsname{[$-$3.9, +1.3]}
\expandafter\def\csname r@ax-fr-fs-Enomic-Ehyb-d\endcsname{$-$1.3}
\expandafter\def\csname r@ax-fr-fs-Enomic-Ehyb-p\endcsname{--}
\expandafter\def\csname r@ax-fr-fs-Enomic-Ehyb-v\endcsname{equiv.}
\expandafter\def\csname r@ax-fr-fs-Eq3-Err\endcsname{$-$0.1 [$-$2.8, +2.5]}
\expandafter\def\csname r@ax-fr-fs-Eq3-Err-ci\endcsname{[$-$2.8, +2.5]}
\expandafter\def\csname r@ax-fr-fs-Eq3-Err-ci95\endcsname{[$-$2.8, +2.5]}
\expandafter\def\csname r@ax-fr-fs-Eq3-Err-d\endcsname{$-$0.1}
\expandafter\def\csname r@ax-fr-fs-Eq3-Err-p\endcsname{--}
\expandafter\def\csname r@ax-fr-fs-Eq3-Err-v\endcsname{equiv.}
\expandafter\def\csname r@ax-fr-fs-Eq3-STq3\endcsname{+0.3 [$-$1.4, +2.0]}
\expandafter\def\csname r@ax-fr-fs-Eq3-STq3-ci\endcsname{[$-$1.4, +2.0]}
\expandafter\def\csname r@ax-fr-fs-Eq3-STq3-ci95\endcsname{[$-$1.4, +2.0]}
\expandafter\def\csname r@ax-fr-fs-Eq3-STq3-d\endcsname{+0.3}
\expandafter\def\csname r@ax-fr-fs-Eq3-STq3-p\endcsname{--}
\expandafter\def\csname r@ax-fr-fs-Eq3-STq3-v\endcsname{equiv.}
\expandafter\def\csname r@ax-fr-fs-Err-STrr\endcsname{+0.8 [$-$1.4, +3.0]}
\expandafter\def\csname r@ax-fr-fs-Err-STrr-ci\endcsname{[$-$1.4, +3.0]}
\expandafter\def\csname r@ax-fr-fs-Err-STrr-ci95\endcsname{[$-$1.4, +3.0]}
\expandafter\def\csname r@ax-fr-fs-Err-STrr-d\endcsname{+0.8}
\expandafter\def\csname r@ax-fr-fs-Err-STrr-p\endcsname{--}
\expandafter\def\csname r@ax-fr-fs-Err-STrr-v\endcsname{equiv.}
\expandafter\def\csname r@ax-fr-fs-Esrr-STq3\endcsname{+1.3 [$-$1.3, +4.1]}
\expandafter\def\csname r@ax-fr-fs-Esrr-STq3-ci\endcsname{[$-$1.3, +4.1]}
\expandafter\def\csname r@ax-fr-fs-Esrr-STq3-ci95\endcsname{[$-$1.3, +4.1]}
\expandafter\def\csname r@ax-fr-fs-Esrr-STq3-d\endcsname{+1.3}
\expandafter\def\csname r@ax-fr-fs-Esrr-STq3-p\endcsname{--}
\expandafter\def\csname r@ax-fr-fs-Esrr-STq3-v\endcsname{equiv.}
\expandafter\def\csname r@ax-fr-fs-F256tq3-STq3\endcsname{$-$0.1 [$-$2.7, +2.7]}
\expandafter\def\csname r@ax-fr-fs-F256tq3-STq3-ci\endcsname{[$-$2.7, +2.7]}
\expandafter\def\csname r@ax-fr-fs-F256tq3-STq3-ci95\endcsname{[$-$2.7, +2.7]}
\expandafter\def\csname r@ax-fr-fs-F256tq3-STq3-d\endcsname{$-$0.1}
\expandafter\def\csname r@ax-fr-fs-F256tq3-STq3-p\endcsname{--}
\expandafter\def\csname r@ax-fr-fs-F256tq3-STq3-v\endcsname{equiv.}
\expandafter\def\csname r@ax-fr-fs-PPrr-STrr\endcsname{+2.0 [$-$0.8, +4.8]}
\expandafter\def\csname r@ax-fr-fs-PPrr-STrr-ci\endcsname{[$-$0.8, +4.8]}
\expandafter\def\csname r@ax-fr-fs-PPrr-STrr-ci95\endcsname{[$-$0.8, +4.8]}
\expandafter\def\csname r@ax-fr-fs-PPrr-STrr-d\endcsname{+2.0}
\expandafter\def\csname r@ax-fr-fs-PPrr-STrr-p\endcsname{--}
\expandafter\def\csname r@ax-fr-fs-PPrr-STrr-v\endcsname{incon.}
\expandafter\def\csname r@ax-fr-fs-STnomic-SThyb\endcsname{$-$1.2 [$-$3.5, +1.3]}
\expandafter\def\csname r@ax-fr-fs-STnomic-SThyb-ci\endcsname{[$-$3.5, +1.3]}
\expandafter\def\csname r@ax-fr-fs-STnomic-SThyb-ci95\endcsname{[$-$3.5, +1.3]}
\expandafter\def\csname r@ax-fr-fs-STnomic-SThyb-d\endcsname{$-$1.2}
\expandafter\def\csname r@ax-fr-fs-STnomic-SThyb-p\endcsname{--}
\expandafter\def\csname r@ax-fr-fs-STnomic-SThyb-v\endcsname{equiv.}
\expandafter\def\csname r@ax-fr-fs-STq3-Ehyb\endcsname{+3.8 [+0.5, +7.0]}
\expandafter\def\csname r@ax-fr-fs-STq3-Ehyb-ci\endcsname{[+0.5, +7.0]}
\expandafter\def\csname r@ax-fr-fs-STq3-Ehyb-ci95\endcsname{[+0.5, +7.0]}
\expandafter\def\csname r@ax-fr-fs-STq3-Ehyb-d\endcsname{+3.8}
\expandafter\def\csname r@ax-fr-fs-STq3-Ehyb-p\endcsname{--}
\expandafter\def\csname r@ax-fr-fs-STq3-Ehyb-v\endcsname{diff.}
\expandafter\def\csname r@ax-fr-fs-STq3-SThyb\endcsname{+6.5 [+3.6, +9.6]}
\expandafter\def\csname r@ax-fr-fs-STq3-SThyb-ci\endcsname{[+3.6, +9.6]}
\expandafter\def\csname r@ax-fr-fs-STq3-SThyb-ci95\endcsname{[+3.6, +9.6]}
\expandafter\def\csname r@ax-fr-fs-STq3-SThyb-d\endcsname{+6.5}
\expandafter\def\csname r@ax-fr-fs-STq3-SThyb-p\endcsname{--}
\expandafter\def\csname r@ax-fr-fs-STq3-SThyb-v\endcsname{diff.}
\expandafter\def\csname r@ax-fr-fs-STq3-STnomic\endcsname{+7.7 [+4.6, +10.7]}
\expandafter\def\csname r@ax-fr-fs-STq3-STnomic-ci\endcsname{[+4.6, +10.7]}
\expandafter\def\csname r@ax-fr-fs-STq3-STnomic-ci95\endcsname{[+4.6, +10.7]}
\expandafter\def\csname r@ax-fr-fs-STq3-STnomic-d\endcsname{+7.7}
\expandafter\def\csname r@ax-fr-fs-STq3-STnomic-p\endcsname{--}
\expandafter\def\csname r@ax-fr-fs-STq3-STnomic-v\endcsname{diff.}
\expandafter\def\csname r@ax-fr-fs-STq3-STrr\endcsname{+0.4 [$-$1.9, +2.8]}
\expandafter\def\csname r@ax-fr-fs-STq3-STrr-ci\endcsname{[$-$1.9, +2.8]}
\expandafter\def\csname r@ax-fr-fs-STq3-STrr-ci95\endcsname{[$-$1.9, +2.8]}
\expandafter\def\csname r@ax-fr-fs-STq3-STrr-d\endcsname{+0.4}
\expandafter\def\csname r@ax-fr-fs-STq3-STrr-p\endcsname{--}
\expandafter\def\csname r@ax-fr-fs-STq3-STrr-v\endcsname{equiv.}
\expandafter\def\csname r@ax-fr-fs-STrr-Ehyb\endcsname{+3.4 [+0.4, +6.5]}
\expandafter\def\csname r@ax-fr-fs-STrr-Ehyb-ci\endcsname{[+0.4, +6.5]}
\expandafter\def\csname r@ax-fr-fs-STrr-Ehyb-ci95\endcsname{[+0.4, +6.5]}
\expandafter\def\csname r@ax-fr-fs-STrr-Ehyb-d\endcsname{+3.4}
\expandafter\def\csname r@ax-fr-fs-STrr-Ehyb-p\endcsname{--}
\expandafter\def\csname r@ax-fr-fs-STrr-Ehyb-v\endcsname{diff.}
\expandafter\def\csname r@ax-fr-fs-STrr-SThyb\endcsname{+6.1 [+3.4, +9.2]}
\expandafter\def\csname r@ax-fr-fs-STrr-SThyb-ci\endcsname{[+3.4, +9.2]}
\expandafter\def\csname r@ax-fr-fs-STrr-SThyb-ci95\endcsname{[+3.4, +9.2]}
\expandafter\def\csname r@ax-fr-fs-STrr-SThyb-d\endcsname{+6.1}
\expandafter\def\csname r@ax-fr-fs-STrr-SThyb-p\endcsname{--}
\expandafter\def\csname r@ax-fr-fs-STrr-SThyb-v\endcsname{diff.}
\expandafter\def\csname r@ax-fr-fs-Snomic-Shyb\endcsname{$-$2.4 [$-$5.0, $-$0.1]}
\expandafter\def\csname r@ax-fr-fs-Snomic-Shyb-ci\endcsname{[$-$5.0, $-$0.1]}
\expandafter\def\csname r@ax-fr-fs-Snomic-Shyb-ci95\endcsname{[$-$5.0, $-$0.1]}
\expandafter\def\csname r@ax-fr-fs-Snomic-Shyb-d\endcsname{$-$2.4}
\expandafter\def\csname r@ax-fr-fs-Snomic-Shyb-p\endcsname{--}
\expandafter\def\csname r@ax-fr-fs-Snomic-Shyb-v\endcsname{diff.}
\expandafter\def\csname r@ax-fr-fs-best\endcsname{PP + rerank}
\expandafter\def\csname r@ax-fr-fs-best-m\endcsname{36.2}
\expandafter\def\csname r@ax-fr-fs-bestfree\endcsname{PP + rerank}
\expandafter\def\csname r@ax-fr-fs-bestfree-bestfreenorr\endcsname{+1.6 [$-$1.6, +4.7]}
\expandafter\def\csname r@ax-fr-fs-bestfree-bestfreenorr-ci\endcsname{[$-$1.6, +4.7]}
\expandafter\def\csname r@ax-fr-fs-bestfree-bestfreenorr-ci95\endcsname{[$-$1.6, +4.7]}
\expandafter\def\csname r@ax-fr-fs-bestfree-bestfreenorr-d\endcsname{+1.6}
\expandafter\def\csname r@ax-fr-fs-bestfree-bestfreenorr-p\endcsname{--}
\expandafter\def\csname r@ax-fr-fs-bestfree-bestfreenorr-v\endcsname{n.d.}
\expandafter\def\csname r@ax-fr-fs-bestfree-m\endcsname{36.2}
\expandafter\def\csname r@ax-fr-fs-bestfree-norr\endcsname{F256t + hybrid-qwen3}
\expandafter\def\csname r@ax-fr-fs-bestfree-norr-m\endcsname{34.6}
\expandafter\def\csname r@ax-fr-qasper-CRq3-STq3\endcsname{+2.1 [+0.1, +4.1]}
\expandafter\def\csname r@ax-fr-qasper-CRq3-STq3-ci\endcsname{[+0.1, +4.1]}
\expandafter\def\csname r@ax-fr-qasper-CRq3-STq3-ci95\endcsname{[+0.1, +4.1]}
\expandafter\def\csname r@ax-fr-qasper-CRq3-STq3-d\endcsname{+2.1}
\expandafter\def\csname r@ax-fr-qasper-CRq3-STq3-p\endcsname{--}
\expandafter\def\csname r@ax-fr-qasper-CRq3-STq3-v\endcsname{diff., equiv.}
\expandafter\def\csname r@ax-fr-qasper-Ehyb-SThyb\endcsname{+5.5 [+2.9, +8.1]}
\expandafter\def\csname r@ax-fr-qasper-Ehyb-SThyb-ci\endcsname{[+2.9, +8.1]}
\expandafter\def\csname r@ax-fr-qasper-Ehyb-SThyb-ci95\endcsname{[+2.9, +8.1]}
\expandafter\def\csname r@ax-fr-qasper-Ehyb-SThyb-d\endcsname{+5.5}
\expandafter\def\csname r@ax-fr-qasper-Ehyb-SThyb-p\endcsname{--}
\expandafter\def\csname r@ax-fr-qasper-Ehyb-SThyb-v\endcsname{diff.}
\expandafter\def\csname r@ax-fr-qasper-Enomic-Ehyb\endcsname{+0.5 [$-$1.8, +2.8]}
\expandafter\def\csname r@ax-fr-qasper-Enomic-Ehyb-ci\endcsname{[$-$1.8, +2.8]}
\expandafter\def\csname r@ax-fr-qasper-Enomic-Ehyb-ci95\endcsname{[$-$1.8, +2.8]}
\expandafter\def\csname r@ax-fr-qasper-Enomic-Ehyb-d\endcsname{+0.5}
\expandafter\def\csname r@ax-fr-qasper-Enomic-Ehyb-p\endcsname{--}
\expandafter\def\csname r@ax-fr-qasper-Enomic-Ehyb-v\endcsname{equiv.}
\expandafter\def\csname r@ax-fr-qasper-Eq3-Err\endcsname{+0.3 [$-$2.0, +2.7]}
\expandafter\def\csname r@ax-fr-qasper-Eq3-Err-ci\endcsname{[$-$2.0, +2.7]}
\expandafter\def\csname r@ax-fr-qasper-Eq3-Err-ci95\endcsname{[$-$2.0, +2.7]}
\expandafter\def\csname r@ax-fr-qasper-Eq3-Err-d\endcsname{+0.3}
\expandafter\def\csname r@ax-fr-qasper-Eq3-Err-p\endcsname{--}
\expandafter\def\csname r@ax-fr-qasper-Eq3-Err-v\endcsname{equiv.}
\expandafter\def\csname r@ax-fr-qasper-Eq3-STq3\endcsname{+1.5 [$-$1.0, +3.9]}
\expandafter\def\csname r@ax-fr-qasper-Eq3-STq3-ci\endcsname{[$-$1.0, +3.9]}
\expandafter\def\csname r@ax-fr-qasper-Eq3-STq3-ci95\endcsname{[$-$1.0, +3.9]}
\expandafter\def\csname r@ax-fr-qasper-Eq3-STq3-d\endcsname{+1.5}
\expandafter\def\csname r@ax-fr-qasper-Eq3-STq3-p\endcsname{--}
\expandafter\def\csname r@ax-fr-qasper-Eq3-STq3-v\endcsname{equiv.}
\expandafter\def\csname r@ax-fr-qasper-Err-STrr\endcsname{+0.4 [$-$1.7, +2.5]}
\expandafter\def\csname r@ax-fr-qasper-Err-STrr-ci\endcsname{[$-$1.7, +2.5]}
\expandafter\def\csname r@ax-fr-qasper-Err-STrr-ci95\endcsname{[$-$1.7, +2.5]}
\expandafter\def\csname r@ax-fr-qasper-Err-STrr-d\endcsname{+0.4}
\expandafter\def\csname r@ax-fr-qasper-Err-STrr-p\endcsname{--}
\expandafter\def\csname r@ax-fr-qasper-Err-STrr-v\endcsname{equiv.}
\expandafter\def\csname r@ax-fr-qasper-Esrr-STq3\endcsname{+3.3 [+0.5, +6.1]}
\expandafter\def\csname r@ax-fr-qasper-Esrr-STq3-ci\endcsname{[+0.5, +6.1]}
\expandafter\def\csname r@ax-fr-qasper-Esrr-STq3-ci95\endcsname{[+0.5, +6.1]}
\expandafter\def\csname r@ax-fr-qasper-Esrr-STq3-d\endcsname{+3.3}
\expandafter\def\csname r@ax-fr-qasper-Esrr-STq3-p\endcsname{--}
\expandafter\def\csname r@ax-fr-qasper-Esrr-STq3-v\endcsname{diff.}
\expandafter\def\csname r@ax-fr-qasper-F256tq3-STq3\endcsname{$-$9.0 [$-$11.5, $-$6.4]}
\expandafter\def\csname r@ax-fr-qasper-F256tq3-STq3-ci\endcsname{[$-$11.5, $-$6.4]}
\expandafter\def\csname r@ax-fr-qasper-F256tq3-STq3-ci95\endcsname{[$-$11.5, $-$6.4]}
\expandafter\def\csname r@ax-fr-qasper-F256tq3-STq3-d\endcsname{$-$9.0}
\expandafter\def\csname r@ax-fr-qasper-F256tq3-STq3-p\endcsname{--}
\expandafter\def\csname r@ax-fr-qasper-F256tq3-STq3-v\endcsname{diff.}
\expandafter\def\csname r@ax-fr-qasper-PPrr-STrr\endcsname{$-$7.1 [$-$9.4, $-$4.7]}
\expandafter\def\csname r@ax-fr-qasper-PPrr-STrr-ci\endcsname{[$-$9.4, $-$4.7]}
\expandafter\def\csname r@ax-fr-qasper-PPrr-STrr-ci95\endcsname{[$-$9.4, $-$4.7]}
\expandafter\def\csname r@ax-fr-qasper-PPrr-STrr-d\endcsname{$-$7.1}
\expandafter\def\csname r@ax-fr-qasper-PPrr-STrr-p\endcsname{--}
\expandafter\def\csname r@ax-fr-qasper-PPrr-STrr-v\endcsname{diff.}
\expandafter\def\csname r@ax-fr-qasper-STnomic-SThyb\endcsname{+5.1 [+2.6, +7.8]}
\expandafter\def\csname r@ax-fr-qasper-STnomic-SThyb-ci\endcsname{[+2.6, +7.8]}
\expandafter\def\csname r@ax-fr-qasper-STnomic-SThyb-ci95\endcsname{[+2.6, +7.8]}
\expandafter\def\csname r@ax-fr-qasper-STnomic-SThyb-d\endcsname{+5.1}
\expandafter\def\csname r@ax-fr-qasper-STnomic-SThyb-p\endcsname{--}
\expandafter\def\csname r@ax-fr-qasper-STnomic-SThyb-v\endcsname{diff.}
\expandafter\def\csname r@ax-fr-qasper-STq3-Ehyb\endcsname{+5.5 [+2.7, +8.2]}
\expandafter\def\csname r@ax-fr-qasper-STq3-Ehyb-ci\endcsname{[+2.7, +8.2]}
\expandafter\def\csname r@ax-fr-qasper-STq3-Ehyb-ci95\endcsname{[+2.7, +8.2]}
\expandafter\def\csname r@ax-fr-qasper-STq3-Ehyb-d\endcsname{+5.5}
\expandafter\def\csname r@ax-fr-qasper-STq3-Ehyb-p\endcsname{--}
\expandafter\def\csname r@ax-fr-qasper-STq3-Ehyb-v\endcsname{diff.}
\expandafter\def\csname r@ax-fr-qasper-STq3-SThyb\endcsname{+10.9 [+7.9, +14.0]}
\expandafter\def\csname r@ax-fr-qasper-STq3-SThyb-ci\endcsname{[+7.9, +14.0]}
\expandafter\def\csname r@ax-fr-qasper-STq3-SThyb-ci95\endcsname{[+7.9, +14.0]}
\expandafter\def\csname r@ax-fr-qasper-STq3-SThyb-d\endcsname{+10.9}
\expandafter\def\csname r@ax-fr-qasper-STq3-SThyb-p\endcsname{--}
\expandafter\def\csname r@ax-fr-qasper-STq3-SThyb-v\endcsname{diff.}
\expandafter\def\csname r@ax-fr-qasper-STq3-STnomic\endcsname{+5.8 [+3.2, +8.6]}
\expandafter\def\csname r@ax-fr-qasper-STq3-STnomic-ci\endcsname{[+3.2, +8.6]}
\expandafter\def\csname r@ax-fr-qasper-STq3-STnomic-ci95\endcsname{[+3.2, +8.6]}
\expandafter\def\csname r@ax-fr-qasper-STq3-STnomic-d\endcsname{+5.8}
\expandafter\def\csname r@ax-fr-qasper-STq3-STnomic-p\endcsname{--}
\expandafter\def\csname r@ax-fr-qasper-STq3-STnomic-v\endcsname{diff.}
\expandafter\def\csname r@ax-fr-qasper-STq3-STrr\endcsname{$-$0.9 [$-$3.4, +1.7]}
\expandafter\def\csname r@ax-fr-qasper-STq3-STrr-ci\endcsname{[$-$3.4, +1.7]}
\expandafter\def\csname r@ax-fr-qasper-STq3-STrr-ci95\endcsname{[$-$3.4, +1.7]}
\expandafter\def\csname r@ax-fr-qasper-STq3-STrr-d\endcsname{$-$0.9}
\expandafter\def\csname r@ax-fr-qasper-STq3-STrr-p\endcsname{--}
\expandafter\def\csname r@ax-fr-qasper-STq3-STrr-v\endcsname{equiv.}
\expandafter\def\csname r@ax-fr-qasper-STrr-Ehyb\endcsname{+6.3 [+3.4, +9.2]}
\expandafter\def\csname r@ax-fr-qasper-STrr-Ehyb-ci\endcsname{[+3.4, +9.2]}
\expandafter\def\csname r@ax-fr-qasper-STrr-Ehyb-ci95\endcsname{[+3.4, +9.2]}
\expandafter\def\csname r@ax-fr-qasper-STrr-Ehyb-d\endcsname{+6.3}
\expandafter\def\csname r@ax-fr-qasper-STrr-Ehyb-p\endcsname{--}
\expandafter\def\csname r@ax-fr-qasper-STrr-Ehyb-v\endcsname{diff.}
\expandafter\def\csname r@ax-fr-qasper-STrr-SThyb\endcsname{+11.8 [+8.8, +14.7]}
\expandafter\def\csname r@ax-fr-qasper-STrr-SThyb-ci\endcsname{[+8.8, +14.7]}
\expandafter\def\csname r@ax-fr-qasper-STrr-SThyb-ci95\endcsname{[+8.8, +14.7]}
\expandafter\def\csname r@ax-fr-qasper-STrr-SThyb-d\endcsname{+11.8}
\expandafter\def\csname r@ax-fr-qasper-STrr-SThyb-p\endcsname{--}
\expandafter\def\csname r@ax-fr-qasper-STrr-SThyb-v\endcsname{diff.}
\expandafter\def\csname r@ax-fr-qasper-Snomic-Shyb\endcsname{+5.4 [+2.8, +8.2]}
\expandafter\def\csname r@ax-fr-qasper-Snomic-Shyb-ci\endcsname{[+2.8, +8.2]}
\expandafter\def\csname r@ax-fr-qasper-Snomic-Shyb-ci95\endcsname{[+2.8, +8.2]}
\expandafter\def\csname r@ax-fr-qasper-Snomic-Shyb-d\endcsname{+5.4}
\expandafter\def\csname r@ax-fr-qasper-Snomic-Shyb-p\endcsname{--}
\expandafter\def\csname r@ax-fr-qasper-Snomic-Shyb-v\endcsname{diff.}
\expandafter\def\csname r@ax-fr-qasper-best\endcsname{CR-strong + rerank}
\expandafter\def\csname r@ax-fr-qasper-best-bestfree\endcsname{+2.5 [+0.4, +4.6]}
\expandafter\def\csname r@ax-fr-qasper-best-bestfree-ci\endcsname{[+0.4, +4.6]}
\expandafter\def\csname r@ax-fr-qasper-best-bestfree-ci95\endcsname{[+0.4, +4.6]}
\expandafter\def\csname r@ax-fr-qasper-best-bestfree-d\endcsname{+2.5}
\expandafter\def\csname r@ax-fr-qasper-best-bestfree-p\endcsname{--}
\expandafter\def\csname r@ax-fr-qasper-best-bestfree-v\endcsname{diff.}
\expandafter\def\csname r@ax-fr-qasper-best-m\endcsname{57.0}
\expandafter\def\csname r@ax-fr-qasper-bestfree\endcsname{S+T + rerank}
\expandafter\def\csname r@ax-fr-qasper-bestfree-bestfreenorr\endcsname{+0.9 [$-$1.7, +3.4]}
\expandafter\def\csname r@ax-fr-qasper-bestfree-bestfreenorr-ci\endcsname{[$-$1.7, +3.4]}
\expandafter\def\csname r@ax-fr-qasper-bestfree-bestfreenorr-ci95\endcsname{[$-$1.7, +3.4]}
\expandafter\def\csname r@ax-fr-qasper-bestfree-bestfreenorr-d\endcsname{+0.9}
\expandafter\def\csname r@ax-fr-qasper-bestfree-bestfreenorr-p\endcsname{--}
\expandafter\def\csname r@ax-fr-qasper-bestfree-bestfreenorr-v\endcsname{n.d.}
\expandafter\def\csname r@ax-fr-qasper-bestfree-m\endcsname{54.5}
\expandafter\def\csname r@ax-fr-qasper-bestfree-norr\endcsname{S+T + qwen3}
\expandafter\def\csname r@ax-fr-qasper-bestfree-norr-m\endcsname{53.6}
\expandafter\def\csname r@ax-gran-fs-E-len\endcsname{171}
\expandafter\def\csname r@ax-gran-fs-E-noRK-len\endcsname{171}
\expandafter\def\csname r@ax-gran-fs-F256t-len\endcsname{248}
\expandafter\def\csname r@ax-gran-fs-F512c-len\endcsname{112}
\expandafter\def\csname r@ax-gran-fs-FL-len\endcsname{144}
\expandafter\def\csname r@ax-gran-fs-M-TP-c\endcsname{+1.5 [$-$3.6, +6.4]}
\expandafter\def\csname r@ax-gran-fs-M-TP-c-ci\endcsname{[$-$3.6, +6.4]}
\expandafter\def\csname r@ax-gran-fs-M-TP-c-ci95\endcsname{[$-$3.6, +6.4]}
\expandafter\def\csname r@ax-gran-fs-M-TP-c-d\endcsname{+1.5}
\expandafter\def\csname r@ax-gran-fs-M-TP-c-p\endcsname{--}
\expandafter\def\csname r@ax-gran-fs-M-TP-c-v\endcsname{n.d.}
\expandafter\def\csname r@ax-gran-fs-M-TP-high\endcsname{+4.9 [+1.1, +8.8]}
\expandafter\def\csname r@ax-gran-fs-M-TP-high-ci\endcsname{[+1.1, +8.8]}
\expandafter\def\csname r@ax-gran-fs-M-TP-high-ci95\endcsname{[+1.1, +8.8]}
\expandafter\def\csname r@ax-gran-fs-M-TP-high-d\endcsname{+4.9}
\expandafter\def\csname r@ax-gran-fs-M-TP-high-p\endcsname{--}
\expandafter\def\csname r@ax-gran-fs-M-TP-high-v\endcsname{diff.}
\expandafter\def\csname r@ax-gran-fs-M-TP-len\endcsname{227}
\expandafter\def\csname r@ax-gran-fs-M-TP-low\endcsname{+3.4 [+0.6, +7.0]}
\expandafter\def\csname r@ax-gran-fs-M-TP-low-ci\endcsname{[+0.6, +7.0]}
\expandafter\def\csname r@ax-gran-fs-M-TP-low-ci95\endcsname{[+0.6, +7.0]}
\expandafter\def\csname r@ax-gran-fs-M-TP-low-d\endcsname{+3.4}
\expandafter\def\csname r@ax-gran-fs-M-TP-low-p\endcsname{--}
\expandafter\def\csname r@ax-gran-fs-M-TP-low-v\endcsname{diff.}
\expandafter\def\csname r@ax-gran-fs-M-TP-mid\endcsname{+4.9 [+0.6, +9.5]}
\expandafter\def\csname r@ax-gran-fs-M-TP-mid-ci\endcsname{[+0.6, +9.5]}
\expandafter\def\csname r@ax-gran-fs-M-TP-mid-ci95\endcsname{[+0.6, +9.5]}
\expandafter\def\csname r@ax-gran-fs-M-TP-mid-d\endcsname{+4.9}
\expandafter\def\csname r@ax-gran-fs-M-TP-mid-p\endcsname{--}
\expandafter\def\csname r@ax-gran-fs-M-TP-mid-v\endcsname{diff.}
\expandafter\def\csname r@ax-gran-fs-M-c\endcsname{+0.1 [$-$2.6, +3.0]}
\expandafter\def\csname r@ax-gran-fs-M-c-ci\endcsname{[$-$2.6, +3.0]}
\expandafter\def\csname r@ax-gran-fs-M-c-ci95\endcsname{[$-$2.6, +3.0]}
\expandafter\def\csname r@ax-gran-fs-M-c-d\endcsname{+0.1}
\expandafter\def\csname r@ax-gran-fs-M-c-p\endcsname{--}
\expandafter\def\csname r@ax-gran-fs-M-c-v\endcsname{n.d.}
\expandafter\def\csname r@ax-gran-fs-M-high\endcsname{+0.3 [$-$2.0, +2.7]}
\expandafter\def\csname r@ax-gran-fs-M-high-ci\endcsname{[$-$2.0, +2.7]}
\expandafter\def\csname r@ax-gran-fs-M-high-ci95\endcsname{[$-$2.0, +2.7]}
\expandafter\def\csname r@ax-gran-fs-M-high-d\endcsname{+0.3}
\expandafter\def\csname r@ax-gran-fs-M-high-p\endcsname{--}
\expandafter\def\csname r@ax-gran-fs-M-high-v\endcsname{n.d.}
\expandafter\def\csname r@ax-gran-fs-M-len\endcsname{195}
\expandafter\def\csname r@ax-gran-fs-M-low\endcsname{+0.2 [$-$1.3, +1.5]}
\expandafter\def\csname r@ax-gran-fs-M-low-ci\endcsname{[$-$1.3, +1.5]}
\expandafter\def\csname r@ax-gran-fs-M-low-ci95\endcsname{[$-$1.3, +1.5]}
\expandafter\def\csname r@ax-gran-fs-M-low-d\endcsname{+0.2}
\expandafter\def\csname r@ax-gran-fs-M-low-p\endcsname{--}
\expandafter\def\csname r@ax-gran-fs-M-low-v\endcsname{n.d.}
\expandafter\def\csname r@ax-gran-fs-M-mid\endcsname{+0.3 [$-$2.3, +3.4]}
\expandafter\def\csname r@ax-gran-fs-M-mid-ci\endcsname{[$-$2.3, +3.4]}
\expandafter\def\csname r@ax-gran-fs-M-mid-ci95\endcsname{[$-$2.3, +3.4]}
\expandafter\def\csname r@ax-gran-fs-M-mid-d\endcsname{+0.3}
\expandafter\def\csname r@ax-gran-fs-M-mid-p\endcsname{--}
\expandafter\def\csname r@ax-gran-fs-M-mid-v\endcsname{n.d.}
\expandafter\def\csname r@ax-gran-fs-M-noRK-len\endcsname{180}
\expandafter\def\csname r@ax-gran-fs-PP-len\endcsname{296}
\expandafter\def\csname r@ax-gran-fs-RM-TP-c\endcsname{+2.9 [$-$1.6, +7.1]}
\expandafter\def\csname r@ax-gran-fs-RM-TP-c-ci\endcsname{[$-$1.6, +7.1]}
\expandafter\def\csname r@ax-gran-fs-RM-TP-c-ci95\endcsname{[$-$1.6, +7.1]}
\expandafter\def\csname r@ax-gran-fs-RM-TP-c-d\endcsname{+2.9}
\expandafter\def\csname r@ax-gran-fs-RM-TP-c-p\endcsname{--}
\expandafter\def\csname r@ax-gran-fs-RM-TP-c-v\endcsname{n.d.}
\expandafter\def\csname r@ax-gran-fs-RM-TP-high\endcsname{+3.9 [+0.2, +7.6]}
\expandafter\def\csname r@ax-gran-fs-RM-TP-high-ci\endcsname{[+0.2, +7.6]}
\expandafter\def\csname r@ax-gran-fs-RM-TP-high-ci95\endcsname{[+0.2, +7.6]}
\expandafter\def\csname r@ax-gran-fs-RM-TP-high-d\endcsname{+3.9}
\expandafter\def\csname r@ax-gran-fs-RM-TP-high-p\endcsname{--}
\expandafter\def\csname r@ax-gran-fs-RM-TP-high-v\endcsname{diff.}
\expandafter\def\csname r@ax-gran-fs-RM-TP-len\endcsname{227}
\expandafter\def\csname r@ax-gran-fs-RM-TP-low\endcsname{+1.0 [$-$1.1, +3.2]}
\expandafter\def\csname r@ax-gran-fs-RM-TP-low-ci\endcsname{[$-$1.1, +3.2]}
\expandafter\def\csname r@ax-gran-fs-RM-TP-low-ci95\endcsname{[$-$1.1, +3.2]}
\expandafter\def\csname r@ax-gran-fs-RM-TP-low-d\endcsname{+1.0}
\expandafter\def\csname r@ax-gran-fs-RM-TP-low-p\endcsname{--}
\expandafter\def\csname r@ax-gran-fs-RM-TP-low-v\endcsname{n.d.}
\expandafter\def\csname r@ax-gran-fs-RM-TP-mid\endcsname{+1.5 [$-$1.5, +4.7]}
\expandafter\def\csname r@ax-gran-fs-RM-TP-mid-ci\endcsname{[$-$1.5, +4.7]}
\expandafter\def\csname r@ax-gran-fs-RM-TP-mid-ci95\endcsname{[$-$1.5, +4.7]}
\expandafter\def\csname r@ax-gran-fs-RM-TP-mid-d\endcsname{+1.5}
\expandafter\def\csname r@ax-gran-fs-RM-TP-mid-p\endcsname{--}
\expandafter\def\csname r@ax-gran-fs-RM-TP-mid-v\endcsname{n.d.}
\expandafter\def\csname r@ax-gran-fs-RM-len\endcsname{195}
\expandafter\def\csname r@ax-gran-fs-S-len\endcsname{171}
\expandafter\def\csname r@ax-gran-fs-SM-TP-c\endcsname{+4.5 [+0.1, +9.1]}
\expandafter\def\csname r@ax-gran-fs-SM-TP-c-ci\endcsname{[+0.1, +9.1]}
\expandafter\def\csname r@ax-gran-fs-SM-TP-c-ci95\endcsname{[+0.1, +9.1]}
\expandafter\def\csname r@ax-gran-fs-SM-TP-c-d\endcsname{+4.5}
\expandafter\def\csname r@ax-gran-fs-SM-TP-c-p\endcsname{--}
\expandafter\def\csname r@ax-gran-fs-SM-TP-c-v\endcsname{diff.}
\expandafter\def\csname r@ax-gran-fs-SM-TP-high\endcsname{+4.7 [+1.1, +8.4]}
\expandafter\def\csname r@ax-gran-fs-SM-TP-high-ci\endcsname{[+1.1, +8.4]}
\expandafter\def\csname r@ax-gran-fs-SM-TP-high-ci95\endcsname{[+1.1, +8.4]}
\expandafter\def\csname r@ax-gran-fs-SM-TP-high-d\endcsname{+4.7}
\expandafter\def\csname r@ax-gran-fs-SM-TP-high-p\endcsname{--}
\expandafter\def\csname r@ax-gran-fs-SM-TP-high-v\endcsname{diff.}
\expandafter\def\csname r@ax-gran-fs-SM-TP-len\endcsname{227}
\expandafter\def\csname r@ax-gran-fs-SM-TP-low\endcsname{+0.2 [$-$2.3, +2.7]}
\expandafter\def\csname r@ax-gran-fs-SM-TP-low-ci\endcsname{[$-$2.3, +2.7]}
\expandafter\def\csname r@ax-gran-fs-SM-TP-low-ci95\endcsname{[$-$2.3, +2.7]}
\expandafter\def\csname r@ax-gran-fs-SM-TP-low-d\endcsname{+0.2}
\expandafter\def\csname r@ax-gran-fs-SM-TP-low-p\endcsname{--}
\expandafter\def\csname r@ax-gran-fs-SM-TP-low-v\endcsname{n.d.}
\expandafter\def\csname r@ax-gran-fs-SM-TP-mid\endcsname{+2.5 [$-$0.9, +6.8]}
\expandafter\def\csname r@ax-gran-fs-SM-TP-mid-ci\endcsname{[$-$0.9, +6.8]}
\expandafter\def\csname r@ax-gran-fs-SM-TP-mid-ci95\endcsname{[$-$0.9, +6.8]}
\expandafter\def\csname r@ax-gran-fs-SM-TP-mid-d\endcsname{+2.5}
\expandafter\def\csname r@ax-gran-fs-SM-TP-mid-p\endcsname{--}
\expandafter\def\csname r@ax-gran-fs-SM-TP-mid-v\endcsname{n.d.}
\expandafter\def\csname r@ax-gran-fs-SM-len\endcsname{195}
\expandafter\def\csname r@ax-gran-fs-meta-n\endcsname{9}
\expandafter\def\csname r@ax-gran-fs-meta-rho\endcsname{0.85}
\expandafter\def\csname r@ax-gran-fs-text-n\endcsname{5}
\expandafter\def\csname r@ax-gran-fs-text-rho\endcsname{0.90}
\expandafter\def\csname r@ax-gran-qasper-E-len\endcsname{201}
\expandafter\def\csname r@ax-gran-qasper-E-noRK-len\endcsname{201}
\expandafter\def\csname r@ax-gran-qasper-F256t-len\endcsname{251}
\expandafter\def\csname r@ax-gran-qasper-F512c-len\endcsname{106}
\expandafter\def\csname r@ax-gran-qasper-FL-len\endcsname{198}
\expandafter\def\csname r@ax-gran-qasper-M-TP-c\endcsname{+6.1 [+0.5, +11.6]}
\expandafter\def\csname r@ax-gran-qasper-M-TP-c-ci\endcsname{[+0.5, +11.6]}
\expandafter\def\csname r@ax-gran-qasper-M-TP-c-ci95\endcsname{[+0.5, +11.6]}
\expandafter\def\csname r@ax-gran-qasper-M-TP-c-d\endcsname{+6.1}
\expandafter\def\csname r@ax-gran-qasper-M-TP-c-p\endcsname{--}
\expandafter\def\csname r@ax-gran-qasper-M-TP-c-v\endcsname{diff.}
\expandafter\def\csname r@ax-gran-qasper-M-TP-high\endcsname{$-$2.8 [$-$6.0, +0.0]}
\expandafter\def\csname r@ax-gran-qasper-M-TP-high-ci\endcsname{[$-$6.0, +0.0]}
\expandafter\def\csname r@ax-gran-qasper-M-TP-high-ci95\endcsname{[$-$6.0, +0.0]}
\expandafter\def\csname r@ax-gran-qasper-M-TP-high-d\endcsname{$-$2.8}
\expandafter\def\csname r@ax-gran-qasper-M-TP-high-p\endcsname{--}
\expandafter\def\csname r@ax-gran-qasper-M-TP-high-v\endcsname{n.d.}
\expandafter\def\csname r@ax-gran-qasper-M-TP-len\endcsname{279}
\expandafter\def\csname r@ax-gran-qasper-M-TP-low\endcsname{$-$8.9 [$-$13.6, $-$4.5]}
\expandafter\def\csname r@ax-gran-qasper-M-TP-low-ci\endcsname{[$-$13.6, $-$4.5]}
\expandafter\def\csname r@ax-gran-qasper-M-TP-low-ci95\endcsname{[$-$13.6, $-$4.5]}
\expandafter\def\csname r@ax-gran-qasper-M-TP-low-d\endcsname{$-$8.9}
\expandafter\def\csname r@ax-gran-qasper-M-TP-low-p\endcsname{--}
\expandafter\def\csname r@ax-gran-qasper-M-TP-low-v\endcsname{diff.}
\expandafter\def\csname r@ax-gran-qasper-M-TP-mid\endcsname{$-$5.1 [$-$9.1, $-$1.0]}
\expandafter\def\csname r@ax-gran-qasper-M-TP-mid-ci\endcsname{[$-$9.1, $-$1.0]}
\expandafter\def\csname r@ax-gran-qasper-M-TP-mid-ci95\endcsname{[$-$9.1, $-$1.0]}
\expandafter\def\csname r@ax-gran-qasper-M-TP-mid-d\endcsname{$-$5.1}
\expandafter\def\csname r@ax-gran-qasper-M-TP-mid-p\endcsname{--}
\expandafter\def\csname r@ax-gran-qasper-M-TP-mid-v\endcsname{diff.}
\expandafter\def\csname r@ax-gran-qasper-M-c\endcsname{$-$2.0 [$-$5.9, +2.0]}
\expandafter\def\csname r@ax-gran-qasper-M-c-ci\endcsname{[$-$5.9, +2.0]}
\expandafter\def\csname r@ax-gran-qasper-M-c-ci95\endcsname{[$-$5.9, +2.0]}
\expandafter\def\csname r@ax-gran-qasper-M-c-d\endcsname{$-$2.0}
\expandafter\def\csname r@ax-gran-qasper-M-c-p\endcsname{--}
\expandafter\def\csname r@ax-gran-qasper-M-c-v\endcsname{n.d.}
\expandafter\def\csname r@ax-gran-qasper-M-high\endcsname{$-$2.9 [$-$5.4, $-$0.6]}
\expandafter\def\csname r@ax-gran-qasper-M-high-ci\endcsname{[$-$5.4, $-$0.6]}
\expandafter\def\csname r@ax-gran-qasper-M-high-ci95\endcsname{[$-$5.4, $-$0.6]}
\expandafter\def\csname r@ax-gran-qasper-M-high-d\endcsname{$-$2.9}
\expandafter\def\csname r@ax-gran-qasper-M-high-p\endcsname{--}
\expandafter\def\csname r@ax-gran-qasper-M-high-v\endcsname{diff.}
\expandafter\def\csname r@ax-gran-qasper-M-len\endcsname{233}
\expandafter\def\csname r@ax-gran-qasper-M-low\endcsname{$-$0.9 [$-$4.2, +2.2]}
\expandafter\def\csname r@ax-gran-qasper-M-low-ci\endcsname{[$-$4.2, +2.2]}
\expandafter\def\csname r@ax-gran-qasper-M-low-ci95\endcsname{[$-$4.2, +2.2]}
\expandafter\def\csname r@ax-gran-qasper-M-low-d\endcsname{$-$0.9}
\expandafter\def\csname r@ax-gran-qasper-M-low-p\endcsname{--}
\expandafter\def\csname r@ax-gran-qasper-M-low-v\endcsname{n.d.}
\expandafter\def\csname r@ax-gran-qasper-M-mid\endcsname{$-$2.9 [$-$6.2, +0.1]}
\expandafter\def\csname r@ax-gran-qasper-M-mid-ci\endcsname{[$-$6.2, +0.1]}
\expandafter\def\csname r@ax-gran-qasper-M-mid-ci95\endcsname{[$-$6.2, +0.1]}
\expandafter\def\csname r@ax-gran-qasper-M-mid-d\endcsname{$-$2.9}
\expandafter\def\csname r@ax-gran-qasper-M-mid-p\endcsname{--}
\expandafter\def\csname r@ax-gran-qasper-M-mid-v\endcsname{n.d.}
\expandafter\def\csname r@ax-gran-qasper-M-noRK-len\endcsname{212}
\expandafter\def\csname r@ax-gran-qasper-PP-len\endcsname{245}
\expandafter\def\csname r@ax-gran-qasper-RM-TP-c\endcsname{+6.3 [+1.8, +10.8]}
\expandafter\def\csname r@ax-gran-qasper-RM-TP-c-ci\endcsname{[+1.8, +10.8]}
\expandafter\def\csname r@ax-gran-qasper-RM-TP-c-ci95\endcsname{[+1.8, +10.8]}
\expandafter\def\csname r@ax-gran-qasper-RM-TP-c-d\endcsname{+6.3}
\expandafter\def\csname r@ax-gran-qasper-RM-TP-c-p\endcsname{--}
\expandafter\def\csname r@ax-gran-qasper-RM-TP-c-v\endcsname{diff.}
\expandafter\def\csname r@ax-gran-qasper-RM-TP-high\endcsname{$-$3.5 [$-$6.6, $-$0.8]}
\expandafter\def\csname r@ax-gran-qasper-RM-TP-high-ci\endcsname{[$-$6.6, $-$0.8]}
\expandafter\def\csname r@ax-gran-qasper-RM-TP-high-ci95\endcsname{[$-$6.6, $-$0.8]}
\expandafter\def\csname r@ax-gran-qasper-RM-TP-high-d\endcsname{$-$3.5}
\expandafter\def\csname r@ax-gran-qasper-RM-TP-high-p\endcsname{--}
\expandafter\def\csname r@ax-gran-qasper-RM-TP-high-v\endcsname{diff.}
\expandafter\def\csname r@ax-gran-qasper-RM-TP-len\endcsname{279}
\expandafter\def\csname r@ax-gran-qasper-RM-TP-low\endcsname{$-$9.8 [$-$13.7, $-$6.5]}
\expandafter\def\csname r@ax-gran-qasper-RM-TP-low-ci\endcsname{[$-$13.7, $-$6.5]}
\expandafter\def\csname r@ax-gran-qasper-RM-TP-low-ci95\endcsname{[$-$13.7, $-$6.5]}
\expandafter\def\csname r@ax-gran-qasper-RM-TP-low-d\endcsname{$-$9.8}
\expandafter\def\csname r@ax-gran-qasper-RM-TP-low-p\endcsname{--}
\expandafter\def\csname r@ax-gran-qasper-RM-TP-low-v\endcsname{diff.}
\expandafter\def\csname r@ax-gran-qasper-RM-TP-mid\endcsname{$-$10.1 [$-$13.3, $-$7.2]}
\expandafter\def\csname r@ax-gran-qasper-RM-TP-mid-ci\endcsname{[$-$13.3, $-$7.2]}
\expandafter\def\csname r@ax-gran-qasper-RM-TP-mid-ci95\endcsname{[$-$13.3, $-$7.2]}
\expandafter\def\csname r@ax-gran-qasper-RM-TP-mid-d\endcsname{$-$10.1}
\expandafter\def\csname r@ax-gran-qasper-RM-TP-mid-p\endcsname{--}
\expandafter\def\csname r@ax-gran-qasper-RM-TP-mid-v\endcsname{diff.}
\expandafter\def\csname r@ax-gran-qasper-RM-len\endcsname{233}
\expandafter\def\csname r@ax-gran-qasper-S-len\endcsname{201}
\expandafter\def\csname r@ax-gran-qasper-SM-TP-c\endcsname{+3.2 [$-$2.5, +9.5]}
\expandafter\def\csname r@ax-gran-qasper-SM-TP-c-ci\endcsname{[$-$2.5, +9.5]}
\expandafter\def\csname r@ax-gran-qasper-SM-TP-c-ci95\endcsname{[$-$2.5, +9.5]}
\expandafter\def\csname r@ax-gran-qasper-SM-TP-c-d\endcsname{+3.2}
\expandafter\def\csname r@ax-gran-qasper-SM-TP-c-p\endcsname{--}
\expandafter\def\csname r@ax-gran-qasper-SM-TP-c-v\endcsname{n.d.}
\expandafter\def\csname r@ax-gran-qasper-SM-TP-high\endcsname{$-$2.4 [$-$5.8, +0.8]}
\expandafter\def\csname r@ax-gran-qasper-SM-TP-high-ci\endcsname{[$-$5.8, +0.8]}
\expandafter\def\csname r@ax-gran-qasper-SM-TP-high-ci95\endcsname{[$-$5.8, +0.8]}
\expandafter\def\csname r@ax-gran-qasper-SM-TP-high-d\endcsname{$-$2.4}
\expandafter\def\csname r@ax-gran-qasper-SM-TP-high-p\endcsname{--}
\expandafter\def\csname r@ax-gran-qasper-SM-TP-high-v\endcsname{n.d.}
\expandafter\def\csname r@ax-gran-qasper-SM-TP-len\endcsname{279}
\expandafter\def\csname r@ax-gran-qasper-SM-TP-low\endcsname{$-$5.6 [$-$11.1, $-$0.9]}
\expandafter\def\csname r@ax-gran-qasper-SM-TP-low-ci\endcsname{[$-$11.1, $-$0.9]}
\expandafter\def\csname r@ax-gran-qasper-SM-TP-low-ci95\endcsname{[$-$11.1, $-$0.9]}
\expandafter\def\csname r@ax-gran-qasper-SM-TP-low-d\endcsname{$-$5.6}
\expandafter\def\csname r@ax-gran-qasper-SM-TP-low-p\endcsname{--}
\expandafter\def\csname r@ax-gran-qasper-SM-TP-low-v\endcsname{diff.}
\expandafter\def\csname r@ax-gran-qasper-SM-TP-mid\endcsname{$-$8.9 [$-$13.1, $-$4.8]}
\expandafter\def\csname r@ax-gran-qasper-SM-TP-mid-ci\endcsname{[$-$13.1, $-$4.8]}
\expandafter\def\csname r@ax-gran-qasper-SM-TP-mid-ci95\endcsname{[$-$13.1, $-$4.8]}
\expandafter\def\csname r@ax-gran-qasper-SM-TP-mid-d\endcsname{$-$8.9}
\expandafter\def\csname r@ax-gran-qasper-SM-TP-mid-p\endcsname{--}
\expandafter\def\csname r@ax-gran-qasper-SM-TP-mid-v\endcsname{diff.}
\expandafter\def\csname r@ax-gran-qasper-SM-len\endcsname{233}
\expandafter\def\csname r@ax-gran-qasper-meta-n\endcsname{9}
\expandafter\def\csname r@ax-gran-qasper-meta-rho\endcsname{$-$0.88}
\expandafter\def\csname r@ax-gran-qasper-text-n\endcsname{5}
\expandafter\def\csname r@ax-gran-qasper-text-rho\endcsname{0.50}
\expandafter\def\csname r@ax-het-fs-angular-bm25\endcsname{+1.0 [$-$1.2, +3.3]}
\expandafter\def\csname r@ax-het-fs-angular-bm25-ci\endcsname{[$-$1.2, +3.3]}
\expandafter\def\csname r@ax-het-fs-angular-bm25-ci95\endcsname{[$-$1.2, +3.3]}
\expandafter\def\csname r@ax-het-fs-angular-bm25-d\endcsname{+1.0}
\expandafter\def\csname r@ax-het-fs-angular-bm25-p\endcsname{--}
\expandafter\def\csname r@ax-het-fs-angular-bm25-v\endcsname{n.d.}
\expandafter\def\csname r@ax-het-fs-angular-q3\endcsname{$-$0.5 [$-$2.8, +1.6]}
\expandafter\def\csname r@ax-het-fs-angular-q3-ci\endcsname{[$-$2.8, +1.6]}
\expandafter\def\csname r@ax-het-fs-angular-q3-ci95\endcsname{[$-$2.8, +1.6]}
\expandafter\def\csname r@ax-het-fs-angular-q3-d\endcsname{$-$0.5}
\expandafter\def\csname r@ax-het-fs-angular-q3-p\endcsname{--}
\expandafter\def\csname r@ax-het-fs-angular-q3-v\endcsname{n.d.}
\expandafter\def\csname r@ax-het-fs-angular-rr\endcsname{+1.5 [$-$1.8, +4.7]}
\expandafter\def\csname r@ax-het-fs-angular-rr-ci\endcsname{[$-$1.8, +4.7]}
\expandafter\def\csname r@ax-het-fs-angular-rr-ci95\endcsname{[$-$1.8, +4.7]}
\expandafter\def\csname r@ax-het-fs-angular-rr-d\endcsname{+1.5}
\expandafter\def\csname r@ax-het-fs-angular-rr-p\endcsname{--}
\expandafter\def\csname r@ax-het-fs-angular-rr-v\endcsname{n.d.}
\expandafter\def\csname r@ax-het-fs-gold-high-bm25\endcsname{+1.8 [$-$1.1, +6.1]}
\expandafter\def\csname r@ax-het-fs-gold-high-bm25-ci\endcsname{[$-$1.1, +6.1]}
\expandafter\def\csname r@ax-het-fs-gold-high-bm25-ci95\endcsname{[$-$1.1, +6.1]}
\expandafter\def\csname r@ax-het-fs-gold-high-bm25-d\endcsname{+1.8}
\expandafter\def\csname r@ax-het-fs-gold-high-bm25-p\endcsname{--}
\expandafter\def\csname r@ax-het-fs-gold-high-bm25-v\endcsname{n.d.}
\expandafter\def\csname r@ax-het-fs-gold-high-hyb\endcsname{+2.5 [$-$2.2, +7.3]}
\expandafter\def\csname r@ax-het-fs-gold-high-hyb-ci\endcsname{[$-$2.2, +7.3]}
\expandafter\def\csname r@ax-het-fs-gold-high-hyb-ci95\endcsname{[$-$2.2, +7.3]}
\expandafter\def\csname r@ax-het-fs-gold-high-hyb-d\endcsname{+2.5}
\expandafter\def\csname r@ax-het-fs-gold-high-hyb-p\endcsname{--}
\expandafter\def\csname r@ax-het-fs-gold-high-hyb-v\endcsname{n.d.}
\expandafter\def\csname r@ax-het-fs-gold-high-rr\endcsname{$-$0.9 [$-$5.3, +4.0]}
\expandafter\def\csname r@ax-het-fs-gold-high-rr-ci\endcsname{[$-$5.3, +4.0]}
\expandafter\def\csname r@ax-het-fs-gold-high-rr-ci95\endcsname{[$-$5.3, +4.0]}
\expandafter\def\csname r@ax-het-fs-gold-high-rr-d\endcsname{$-$0.9}
\expandafter\def\csname r@ax-het-fs-gold-high-rr-p\endcsname{--}
\expandafter\def\csname r@ax-het-fs-gold-high-rr-v\endcsname{n.d.}
\expandafter\def\csname r@ax-het-fs-gold-low-bm25\endcsname{+2.8 [+0.8, +5.1]}
\expandafter\def\csname r@ax-het-fs-gold-low-bm25-ci\endcsname{[+0.8, +5.1]}
\expandafter\def\csname r@ax-het-fs-gold-low-bm25-ci95\endcsname{[+0.8, +5.1]}
\expandafter\def\csname r@ax-het-fs-gold-low-bm25-d\endcsname{+2.8}
\expandafter\def\csname r@ax-het-fs-gold-low-bm25-p\endcsname{--}
\expandafter\def\csname r@ax-het-fs-gold-low-bm25-v\endcsname{diff.}
\expandafter\def\csname r@ax-het-fs-gold-low-hyb\endcsname{+0.8 [$-$2.4, +4.5]}
\expandafter\def\csname r@ax-het-fs-gold-low-hyb-ci\endcsname{[$-$2.4, +4.5]}
\expandafter\def\csname r@ax-het-fs-gold-low-hyb-ci95\endcsname{[$-$2.4, +4.5]}
\expandafter\def\csname r@ax-het-fs-gold-low-hyb-d\endcsname{+0.8}
\expandafter\def\csname r@ax-het-fs-gold-low-hyb-p\endcsname{--}
\expandafter\def\csname r@ax-het-fs-gold-low-hyb-v\endcsname{n.d.}
\expandafter\def\csname r@ax-het-fs-gold-low-rr\endcsname{+0.2 [$-$2.8, +3.8]}
\expandafter\def\csname r@ax-het-fs-gold-low-rr-ci\endcsname{[$-$2.8, +3.8]}
\expandafter\def\csname r@ax-het-fs-gold-low-rr-ci95\endcsname{[$-$2.8, +3.8]}
\expandafter\def\csname r@ax-het-fs-gold-low-rr-d\endcsname{+0.2}
\expandafter\def\csname r@ax-het-fs-gold-low-rr-p\endcsname{--}
\expandafter\def\csname r@ax-het-fs-gold-low-rr-v\endcsname{n.d.}
\expandafter\def\csname r@ax-het-fs-gold-mid-bm25\endcsname{+2.6 [+0.2, +6.0]}
\expandafter\def\csname r@ax-het-fs-gold-mid-bm25-ci\endcsname{[+0.2, +6.0]}
\expandafter\def\csname r@ax-het-fs-gold-mid-bm25-ci95\endcsname{[+0.2, +6.0]}
\expandafter\def\csname r@ax-het-fs-gold-mid-bm25-d\endcsname{+2.6}
\expandafter\def\csname r@ax-het-fs-gold-mid-bm25-p\endcsname{--}
\expandafter\def\csname r@ax-het-fs-gold-mid-bm25-v\endcsname{diff.}
\expandafter\def\csname r@ax-het-fs-gold-mid-hyb\endcsname{+4.9 [+1.7, +8.4]}
\expandafter\def\csname r@ax-het-fs-gold-mid-hyb-ci\endcsname{[+1.7, +8.4]}
\expandafter\def\csname r@ax-het-fs-gold-mid-hyb-ci95\endcsname{[+1.7, +8.4]}
\expandafter\def\csname r@ax-het-fs-gold-mid-hyb-d\endcsname{+4.9}
\expandafter\def\csname r@ax-het-fs-gold-mid-hyb-p\endcsname{--}
\expandafter\def\csname r@ax-het-fs-gold-mid-hyb-v\endcsname{diff.}
\expandafter\def\csname r@ax-het-fs-gold-mid-rr\endcsname{+3.0 [$-$0.5, +6.9]}
\expandafter\def\csname r@ax-het-fs-gold-mid-rr-ci\endcsname{[$-$0.5, +6.9]}
\expandafter\def\csname r@ax-het-fs-gold-mid-rr-ci95\endcsname{[$-$0.5, +6.9]}
\expandafter\def\csname r@ax-het-fs-gold-mid-rr-d\endcsname{+3.0}
\expandafter\def\csname r@ax-het-fs-gold-mid-rr-p\endcsname{--}
\expandafter\def\csname r@ax-het-fs-gold-mid-rr-v\endcsname{n.d.}
\expandafter\def\csname r@ax-het-fs-goldhl-bm25\endcsname{$-$1.0 [$-$4.8, +3.8]}
\expandafter\def\csname r@ax-het-fs-goldhl-bm25-ci\endcsname{[$-$4.8, +3.8]}
\expandafter\def\csname r@ax-het-fs-goldhl-bm25-ci95\endcsname{[$-$4.8, +3.8]}
\expandafter\def\csname r@ax-het-fs-goldhl-bm25-d\endcsname{$-$1.0}
\expandafter\def\csname r@ax-het-fs-goldhl-bm25-p\endcsname{--}
\expandafter\def\csname r@ax-het-fs-goldhl-bm25-v\endcsname{n.d.}
\expandafter\def\csname r@ax-het-fs-goldhl-hyb\endcsname{+1.6 [$-$4.3, +7.5]}
\expandafter\def\csname r@ax-het-fs-goldhl-hyb-ci\endcsname{[$-$4.3, +7.5]}
\expandafter\def\csname r@ax-het-fs-goldhl-hyb-ci95\endcsname{[$-$4.3, +7.5]}
\expandafter\def\csname r@ax-het-fs-goldhl-hyb-d\endcsname{+1.6}
\expandafter\def\csname r@ax-het-fs-goldhl-hyb-p\endcsname{--}
\expandafter\def\csname r@ax-het-fs-goldhl-hyb-v\endcsname{n.d.}
\expandafter\def\csname r@ax-het-fs-laravel-bm25\endcsname{+4.0 [+1.7, +8.1]}
\expandafter\def\csname r@ax-het-fs-laravel-bm25-ci\endcsname{[+1.7, +8.1]}
\expandafter\def\csname r@ax-het-fs-laravel-bm25-ci95\endcsname{[+1.7, +8.1]}
\expandafter\def\csname r@ax-het-fs-laravel-bm25-d\endcsname{+4.0}
\expandafter\def\csname r@ax-het-fs-laravel-bm25-p\endcsname{--}
\expandafter\def\csname r@ax-het-fs-laravel-bm25-v\endcsname{diff.}
\expandafter\def\csname r@ax-het-fs-laravel-q3\endcsname{+1.0 [$-$2.1, +4.4]}
\expandafter\def\csname r@ax-het-fs-laravel-q3-ci\endcsname{[$-$2.1, +4.4]}
\expandafter\def\csname r@ax-het-fs-laravel-q3-ci95\endcsname{[$-$2.1, +4.4]}
\expandafter\def\csname r@ax-het-fs-laravel-q3-d\endcsname{+1.0}
\expandafter\def\csname r@ax-het-fs-laravel-q3-p\endcsname{--}
\expandafter\def\csname r@ax-het-fs-laravel-q3-v\endcsname{n.d.}
\expandafter\def\csname r@ax-het-fs-laravel-rr\endcsname{+0.9 [$-$2.5, +4.5]}
\expandafter\def\csname r@ax-het-fs-laravel-rr-ci\endcsname{[$-$2.5, +4.5]}
\expandafter\def\csname r@ax-het-fs-laravel-rr-ci95\endcsname{[$-$2.5, +4.5]}
\expandafter\def\csname r@ax-het-fs-laravel-rr-d\endcsname{+0.9}
\expandafter\def\csname r@ax-het-fs-laravel-rr-p\endcsname{--}
\expandafter\def\csname r@ax-het-fs-laravel-rr-v\endcsname{n.d.}
\expandafter\def\csname r@ax-het-fs-yolo-bm25\endcsname{+2.3 [$-$1.1, +7.8]}
\expandafter\def\csname r@ax-het-fs-yolo-bm25-ci\endcsname{[$-$1.1, +7.8]}
\expandafter\def\csname r@ax-het-fs-yolo-bm25-ci95\endcsname{[$-$1.1, +7.8]}
\expandafter\def\csname r@ax-het-fs-yolo-bm25-d\endcsname{+2.3}
\expandafter\def\csname r@ax-het-fs-yolo-bm25-p\endcsname{--}
\expandafter\def\csname r@ax-het-fs-yolo-bm25-v\endcsname{n.d.}
\expandafter\def\csname r@ax-het-fs-yolo-q3\endcsname{+0.5 [$-$3.2, +4.9]}
\expandafter\def\csname r@ax-het-fs-yolo-q3-ci\endcsname{[$-$3.2, +4.9]}
\expandafter\def\csname r@ax-het-fs-yolo-q3-ci95\endcsname{[$-$3.2, +4.9]}
\expandafter\def\csname r@ax-het-fs-yolo-q3-d\endcsname{+0.5}
\expandafter\def\csname r@ax-het-fs-yolo-q3-p\endcsname{--}
\expandafter\def\csname r@ax-het-fs-yolo-q3-v\endcsname{n.d.}
\expandafter\def\csname r@ax-het-fs-yolo-rr\endcsname{$-$0.9 [$-$6.7, +5.7]}
\expandafter\def\csname r@ax-het-fs-yolo-rr-ci\endcsname{[$-$6.7, +5.7]}
\expandafter\def\csname r@ax-het-fs-yolo-rr-ci95\endcsname{[$-$6.7, +5.7]}
\expandafter\def\csname r@ax-het-fs-yolo-rr-d\endcsname{$-$0.9}
\expandafter\def\csname r@ax-het-fs-yolo-rr-p\endcsname{--}
\expandafter\def\csname r@ax-het-fs-yolo-rr-v\endcsname{n.d.}
\expandafter\def\csname r@ax-het-qasper-answertype-abstractive-bm25\endcsname{+2.8 [$-$3.5, +9.8]}
\expandafter\def\csname r@ax-het-qasper-answertype-abstractive-bm25-ci\endcsname{[$-$3.5, +9.8]}
\expandafter\def\csname r@ax-het-qasper-answertype-abstractive-bm25-ci95\endcsname{[$-$3.5, +9.8]}
\expandafter\def\csname r@ax-het-qasper-answertype-abstractive-bm25-d\endcsname{+2.8}
\expandafter\def\csname r@ax-het-qasper-answertype-abstractive-bm25-p\endcsname{--}
\expandafter\def\csname r@ax-het-qasper-answertype-abstractive-bm25-v\endcsname{n.d.}
\expandafter\def\csname r@ax-het-qasper-answertype-abstractive-hyb\endcsname{+6.5 [$-$2.2, +15.8]}
\expandafter\def\csname r@ax-het-qasper-answertype-abstractive-hyb-ci\endcsname{[$-$2.2, +15.8]}
\expandafter\def\csname r@ax-het-qasper-answertype-abstractive-hyb-ci95\endcsname{[$-$2.2, +15.8]}
\expandafter\def\csname r@ax-het-qasper-answertype-abstractive-hyb-d\endcsname{+6.5}
\expandafter\def\csname r@ax-het-qasper-answertype-abstractive-hyb-p\endcsname{--}
\expandafter\def\csname r@ax-het-qasper-answertype-abstractive-hyb-v\endcsname{n.d.}
\expandafter\def\csname r@ax-het-qasper-answertype-abstractive-n\endcsname{106}
\expandafter\def\csname r@ax-het-qasper-answertype-abstractive-rr\endcsname{+0.8 [$-$6.3, +8.0]}
\expandafter\def\csname r@ax-het-qasper-answertype-abstractive-rr-ci\endcsname{[$-$6.3, +8.0]}
\expandafter\def\csname r@ax-het-qasper-answertype-abstractive-rr-ci95\endcsname{[$-$6.3, +8.0]}
\expandafter\def\csname r@ax-het-qasper-answertype-abstractive-rr-d\endcsname{+0.8}
\expandafter\def\csname r@ax-het-qasper-answertype-abstractive-rr-p\endcsname{--}
\expandafter\def\csname r@ax-het-qasper-answertype-abstractive-rr-v\endcsname{n.d.}
\expandafter\def\csname r@ax-het-qasper-answertype-extractive-bm25\endcsname{+9.8 [+6.7, +13.2]}
\expandafter\def\csname r@ax-het-qasper-answertype-extractive-bm25-ci\endcsname{[+6.7, +13.2]}
\expandafter\def\csname r@ax-het-qasper-answertype-extractive-bm25-ci95\endcsname{[+6.7, +13.2]}
\expandafter\def\csname r@ax-het-qasper-answertype-extractive-bm25-d\endcsname{+9.8}
\expandafter\def\csname r@ax-het-qasper-answertype-extractive-bm25-p\endcsname{--}
\expandafter\def\csname r@ax-het-qasper-answertype-extractive-bm25-v\endcsname{diff.}
\expandafter\def\csname r@ax-het-qasper-answertype-extractive-hyb\endcsname{+4.5 [+0.9, +8.2]}
\expandafter\def\csname r@ax-het-qasper-answertype-extractive-hyb-ci\endcsname{[+0.9, +8.2]}
\expandafter\def\csname r@ax-het-qasper-answertype-extractive-hyb-ci95\endcsname{[+0.9, +8.2]}
\expandafter\def\csname r@ax-het-qasper-answertype-extractive-hyb-d\endcsname{+4.5}
\expandafter\def\csname r@ax-het-qasper-answertype-extractive-hyb-p\endcsname{--}
\expandafter\def\csname r@ax-het-qasper-answertype-extractive-hyb-v\endcsname{diff.}
\expandafter\def\csname r@ax-het-qasper-answertype-extractive-n\endcsname{446}
\expandafter\def\csname r@ax-het-qasper-answertype-extractive-rr\endcsname{+1.1 [$-$2.0, +4.2]}
\expandafter\def\csname r@ax-het-qasper-answertype-extractive-rr-ci\endcsname{[$-$2.0, +4.2]}
\expandafter\def\csname r@ax-het-qasper-answertype-extractive-rr-ci95\endcsname{[$-$2.0, +4.2]}
\expandafter\def\csname r@ax-het-qasper-answertype-extractive-rr-d\endcsname{+1.1}
\expandafter\def\csname r@ax-het-qasper-answertype-extractive-rr-p\endcsname{--}
\expandafter\def\csname r@ax-het-qasper-answertype-extractive-rr-v\endcsname{n.d.}
\expandafter\def\csname r@ax-het-qasper-answertype-mixed-bm25\endcsname{+13.4 [+9.4, +17.9]}
\expandafter\def\csname r@ax-het-qasper-answertype-mixed-bm25-ci\endcsname{[+9.4, +17.9]}
\expandafter\def\csname r@ax-het-qasper-answertype-mixed-bm25-ci95\endcsname{[+9.4, +17.9]}
\expandafter\def\csname r@ax-het-qasper-answertype-mixed-bm25-d\endcsname{+13.4}
\expandafter\def\csname r@ax-het-qasper-answertype-mixed-bm25-p\endcsname{--}
\expandafter\def\csname r@ax-het-qasper-answertype-mixed-bm25-v\endcsname{diff.}
\expandafter\def\csname r@ax-het-qasper-answertype-mixed-hyb\endcsname{+9.6 [+4.9, +14.5]}
\expandafter\def\csname r@ax-het-qasper-answertype-mixed-hyb-ci\endcsname{[+4.9, +14.5]}
\expandafter\def\csname r@ax-het-qasper-answertype-mixed-hyb-ci95\endcsname{[+4.9, +14.5]}
\expandafter\def\csname r@ax-het-qasper-answertype-mixed-hyb-d\endcsname{+9.6}
\expandafter\def\csname r@ax-het-qasper-answertype-mixed-hyb-p\endcsname{--}
\expandafter\def\csname r@ax-het-qasper-answertype-mixed-hyb-v\endcsname{diff.}
\expandafter\def\csname r@ax-het-qasper-answertype-mixed-n\endcsname{256}
\expandafter\def\csname r@ax-het-qasper-answertype-mixed-rr\endcsname{+0.3 [$-$3.6, +4.5]}
\expandafter\def\csname r@ax-het-qasper-answertype-mixed-rr-ci\endcsname{[$-$3.6, +4.5]}
\expandafter\def\csname r@ax-het-qasper-answertype-mixed-rr-ci95\endcsname{[$-$3.6, +4.5]}
\expandafter\def\csname r@ax-het-qasper-answertype-mixed-rr-d\endcsname{+0.3}
\expandafter\def\csname r@ax-het-qasper-answertype-mixed-rr-p\endcsname{--}
\expandafter\def\csname r@ax-het-qasper-answertype-mixed-rr-v\endcsname{n.d.}
\expandafter\def\csname r@ax-het-qasper-answertype-yesno-bm25\endcsname{+1.2 [$-$3.1, +5.9]}
\expandafter\def\csname r@ax-het-qasper-answertype-yesno-bm25-ci\endcsname{[$-$3.1, +5.9]}
\expandafter\def\csname r@ax-het-qasper-answertype-yesno-bm25-ci95\endcsname{[$-$3.1, +5.9]}
\expandafter\def\csname r@ax-het-qasper-answertype-yesno-bm25-d\endcsname{+1.2}
\expandafter\def\csname r@ax-het-qasper-answertype-yesno-bm25-p\endcsname{--}
\expandafter\def\csname r@ax-het-qasper-answertype-yesno-bm25-v\endcsname{n.d.}
\expandafter\def\csname r@ax-het-qasper-answertype-yesno-hyb\endcsname{+0.3 [$-$4.8, +5.5]}
\expandafter\def\csname r@ax-het-qasper-answertype-yesno-hyb-ci\endcsname{[$-$4.8, +5.5]}
\expandafter\def\csname r@ax-het-qasper-answertype-yesno-hyb-ci95\endcsname{[$-$4.8, +5.5]}
\expandafter\def\csname r@ax-het-qasper-answertype-yesno-hyb-d\endcsname{+0.3}
\expandafter\def\csname r@ax-het-qasper-answertype-yesno-hyb-p\endcsname{--}
\expandafter\def\csname r@ax-het-qasper-answertype-yesno-hyb-v\endcsname{n.d.}
\expandafter\def\csname r@ax-het-qasper-answertype-yesno-n\endcsname{143}
\expandafter\def\csname r@ax-het-qasper-answertype-yesno-rr\endcsname{$-$2.0 [$-$6.6, +2.3]}
\expandafter\def\csname r@ax-het-qasper-answertype-yesno-rr-ci\endcsname{[$-$6.6, +2.3]}
\expandafter\def\csname r@ax-het-qasper-answertype-yesno-rr-ci95\endcsname{[$-$6.6, +2.3]}
\expandafter\def\csname r@ax-het-qasper-answertype-yesno-rr-d\endcsname{$-$2.0}
\expandafter\def\csname r@ax-het-qasper-answertype-yesno-rr-p\endcsname{--}
\expandafter\def\csname r@ax-het-qasper-answertype-yesno-rr-v\endcsname{n.d.}
\expandafter\def\csname r@ax-het-qasper-anyunanswerable-False-bm25\endcsname{+9.3 [+7.1, +11.6]}
\expandafter\def\csname r@ax-het-qasper-anyunanswerable-False-bm25-ci\endcsname{[+7.1, +11.6]}
\expandafter\def\csname r@ax-het-qasper-anyunanswerable-False-bm25-ci95\endcsname{[+7.1, +11.6]}
\expandafter\def\csname r@ax-het-qasper-anyunanswerable-False-bm25-d\endcsname{+9.3}
\expandafter\def\csname r@ax-het-qasper-anyunanswerable-False-bm25-p\endcsname{--}
\expandafter\def\csname r@ax-het-qasper-anyunanswerable-False-bm25-v\endcsname{diff.}
\expandafter\def\csname r@ax-het-qasper-anyunanswerable-False-hyb\endcsname{+5.9 [+3.2, +8.6]}
\expandafter\def\csname r@ax-het-qasper-anyunanswerable-False-hyb-ci\endcsname{[+3.2, +8.6]}
\expandafter\def\csname r@ax-het-qasper-anyunanswerable-False-hyb-ci95\endcsname{[+3.2, +8.6]}
\expandafter\def\csname r@ax-het-qasper-anyunanswerable-False-hyb-d\endcsname{+5.9}
\expandafter\def\csname r@ax-het-qasper-anyunanswerable-False-hyb-p\endcsname{--}
\expandafter\def\csname r@ax-het-qasper-anyunanswerable-False-hyb-v\endcsname{diff.}
\expandafter\def\csname r@ax-het-qasper-anyunanswerable-False-n\endcsname{845}
\expandafter\def\csname r@ax-het-qasper-anyunanswerable-False-rr\endcsname{+0.2 [$-$2.0, +2.4]}
\expandafter\def\csname r@ax-het-qasper-anyunanswerable-False-rr-ci\endcsname{[$-$2.0, +2.4]}
\expandafter\def\csname r@ax-het-qasper-anyunanswerable-False-rr-ci95\endcsname{[$-$2.0, +2.4]}
\expandafter\def\csname r@ax-het-qasper-anyunanswerable-False-rr-d\endcsname{+0.2}
\expandafter\def\csname r@ax-het-qasper-anyunanswerable-False-rr-p\endcsname{--}
\expandafter\def\csname r@ax-het-qasper-anyunanswerable-False-rr-v\endcsname{n.d.}
\expandafter\def\csname r@ax-het-qasper-anyunanswerable-True-bm25\endcsname{+3.6 [$-$2.5, +9.7]}
\expandafter\def\csname r@ax-het-qasper-anyunanswerable-True-bm25-ci\endcsname{[$-$2.5, +9.7]}
\expandafter\def\csname r@ax-het-qasper-anyunanswerable-True-bm25-ci95\endcsname{[$-$2.5, +9.7]}
\expandafter\def\csname r@ax-het-qasper-anyunanswerable-True-bm25-d\endcsname{+3.6}
\expandafter\def\csname r@ax-het-qasper-anyunanswerable-True-bm25-p\endcsname{--}
\expandafter\def\csname r@ax-het-qasper-anyunanswerable-True-bm25-v\endcsname{n.d.}
\expandafter\def\csname r@ax-het-qasper-anyunanswerable-True-hyb\endcsname{+2.2 [$-$5.3, +10.5]}
\expandafter\def\csname r@ax-het-qasper-anyunanswerable-True-hyb-ci\endcsname{[$-$5.3, +10.5]}
\expandafter\def\csname r@ax-het-qasper-anyunanswerable-True-hyb-ci95\endcsname{[$-$5.3, +10.5]}
\expandafter\def\csname r@ax-het-qasper-anyunanswerable-True-hyb-d\endcsname{+2.2}
\expandafter\def\csname r@ax-het-qasper-anyunanswerable-True-hyb-p\endcsname{--}
\expandafter\def\csname r@ax-het-qasper-anyunanswerable-True-hyb-v\endcsname{n.d.}
\expandafter\def\csname r@ax-het-qasper-anyunanswerable-True-n\endcsname{106}
\expandafter\def\csname r@ax-het-qasper-anyunanswerable-True-rr\endcsname{+2.2 [$-$4.8, +10.8]}
\expandafter\def\csname r@ax-het-qasper-anyunanswerable-True-rr-ci\endcsname{[$-$4.8, +10.8]}
\expandafter\def\csname r@ax-het-qasper-anyunanswerable-True-rr-ci95\endcsname{[$-$4.8, +10.8]}
\expandafter\def\csname r@ax-het-qasper-anyunanswerable-True-rr-d\endcsname{+2.2}
\expandafter\def\csname r@ax-het-qasper-anyunanswerable-True-rr-p\endcsname{--}
\expandafter\def\csname r@ax-het-qasper-anyunanswerable-True-rr-v\endcsname{n.d.}
\expandafter\def\csname r@ax-het-qasper-ev4v1-bm25\endcsname{$-$6.3 [$-$11.4, $-$0.2]}
\expandafter\def\csname r@ax-het-qasper-ev4v1-bm25-ci\endcsname{[$-$11.4, $-$0.2]}
\expandafter\def\csname r@ax-het-qasper-ev4v1-bm25-ci95\endcsname{[$-$11.4, $-$0.2]}
\expandafter\def\csname r@ax-het-qasper-ev4v1-bm25-d\endcsname{$-$6.3}
\expandafter\def\csname r@ax-het-qasper-ev4v1-bm25-p\endcsname{--}
\expandafter\def\csname r@ax-het-qasper-ev4v1-bm25-v\endcsname{diff.}
\expandafter\def\csname r@ax-het-qasper-ev4v1-hyb\endcsname{$-$5.6 [$-$11.6, +0.4]}
\expandafter\def\csname r@ax-het-qasper-ev4v1-hyb-ci\endcsname{[$-$11.6, +0.4]}
\expandafter\def\csname r@ax-het-qasper-ev4v1-hyb-ci95\endcsname{[$-$11.6, +0.4]}
\expandafter\def\csname r@ax-het-qasper-ev4v1-hyb-d\endcsname{$-$5.6}
\expandafter\def\csname r@ax-het-qasper-ev4v1-hyb-p\endcsname{--}
\expandafter\def\csname r@ax-het-qasper-ev4v1-hyb-v\endcsname{n.d.}
\expandafter\def\csname r@ax-het-qasper-lenhl-bm25\endcsname{$-$0.8 [$-$6.1, +5.0]}
\expandafter\def\csname r@ax-het-qasper-lenhl-bm25-ci\endcsname{[$-$6.1, +5.0]}
\expandafter\def\csname r@ax-het-qasper-lenhl-bm25-ci95\endcsname{[$-$6.1, +5.0]}
\expandafter\def\csname r@ax-het-qasper-lenhl-bm25-d\endcsname{$-$0.8}
\expandafter\def\csname r@ax-het-qasper-lenhl-bm25-p\endcsname{--}
\expandafter\def\csname r@ax-het-qasper-lenhl-bm25-v\endcsname{n.d.}
\expandafter\def\csname r@ax-het-qasper-lenhl-hyb\endcsname{$-$1.3 [$-$7.7, +5.3]}
\expandafter\def\csname r@ax-het-qasper-lenhl-hyb-ci\endcsname{[$-$7.7, +5.3]}
\expandafter\def\csname r@ax-het-qasper-lenhl-hyb-ci95\endcsname{[$-$7.7, +5.3]}
\expandafter\def\csname r@ax-het-qasper-lenhl-hyb-d\endcsname{$-$1.3}
\expandafter\def\csname r@ax-het-qasper-lenhl-hyb-p\endcsname{--}
\expandafter\def\csname r@ax-het-qasper-lenhl-hyb-v\endcsname{n.d.}
\expandafter\def\csname r@ax-het-qasper-nevidence-1-bm25\endcsname{+10.6 [+7.1, +14.5]}
\expandafter\def\csname r@ax-het-qasper-nevidence-1-bm25-ci\endcsname{[+7.1, +14.5]}
\expandafter\def\csname r@ax-het-qasper-nevidence-1-bm25-ci95\endcsname{[+7.1, +14.5]}
\expandafter\def\csname r@ax-het-qasper-nevidence-1-bm25-d\endcsname{+10.6}
\expandafter\def\csname r@ax-het-qasper-nevidence-1-bm25-p\endcsname{--}
\expandafter\def\csname r@ax-het-qasper-nevidence-1-bm25-v\endcsname{diff.}
\expandafter\def\csname r@ax-het-qasper-nevidence-1-hyb\endcsname{+8.6 [+3.8, +13.3]}
\expandafter\def\csname r@ax-het-qasper-nevidence-1-hyb-ci\endcsname{[+3.8, +13.3]}
\expandafter\def\csname r@ax-het-qasper-nevidence-1-hyb-ci95\endcsname{[+3.8, +13.3]}
\expandafter\def\csname r@ax-het-qasper-nevidence-1-hyb-d\endcsname{+8.6}
\expandafter\def\csname r@ax-het-qasper-nevidence-1-hyb-p\endcsname{--}
\expandafter\def\csname r@ax-het-qasper-nevidence-1-hyb-v\endcsname{diff.}
\expandafter\def\csname r@ax-het-qasper-nevidence-1-n\endcsname{432}
\expandafter\def\csname r@ax-het-qasper-nevidence-1-rr\endcsname{+1.2 [$-$2.6, +5.0]}
\expandafter\def\csname r@ax-het-qasper-nevidence-1-rr-ci\endcsname{[$-$2.6, +5.0]}
\expandafter\def\csname r@ax-het-qasper-nevidence-1-rr-ci95\endcsname{[$-$2.6, +5.0]}
\expandafter\def\csname r@ax-het-qasper-nevidence-1-rr-d\endcsname{+1.2}
\expandafter\def\csname r@ax-het-qasper-nevidence-1-rr-p\endcsname{--}
\expandafter\def\csname r@ax-het-qasper-nevidence-1-rr-v\endcsname{n.d.}
\expandafter\def\csname r@ax-het-qasper-nevidence-2-bm25\endcsname{+8.0 [+4.2, +11.9]}
\expandafter\def\csname r@ax-het-qasper-nevidence-2-bm25-ci\endcsname{[+4.2, +11.9]}
\expandafter\def\csname r@ax-het-qasper-nevidence-2-bm25-ci95\endcsname{[+4.2, +11.9]}
\expandafter\def\csname r@ax-het-qasper-nevidence-2-bm25-d\endcsname{+8.0}
\expandafter\def\csname r@ax-het-qasper-nevidence-2-bm25-p\endcsname{--}
\expandafter\def\csname r@ax-het-qasper-nevidence-2-bm25-v\endcsname{diff.}
\expandafter\def\csname r@ax-het-qasper-nevidence-2-hyb\endcsname{+1.9 [$-$1.7, +5.6]}
\expandafter\def\csname r@ax-het-qasper-nevidence-2-hyb-ci\endcsname{[$-$1.7, +5.6]}
\expandafter\def\csname r@ax-het-qasper-nevidence-2-hyb-ci95\endcsname{[$-$1.7, +5.6]}
\expandafter\def\csname r@ax-het-qasper-nevidence-2-hyb-d\endcsname{+1.9}
\expandafter\def\csname r@ax-het-qasper-nevidence-2-hyb-p\endcsname{--}
\expandafter\def\csname r@ax-het-qasper-nevidence-2-hyb-v\endcsname{n.d.}
\expandafter\def\csname r@ax-het-qasper-nevidence-2-n\endcsname{269}
\expandafter\def\csname r@ax-het-qasper-nevidence-2-rr\endcsname{+0.7 [$-$2.6, +4.0]}
\expandafter\def\csname r@ax-het-qasper-nevidence-2-rr-ci\endcsname{[$-$2.6, +4.0]}
\expandafter\def\csname r@ax-het-qasper-nevidence-2-rr-ci95\endcsname{[$-$2.6, +4.0]}
\expandafter\def\csname r@ax-het-qasper-nevidence-2-rr-d\endcsname{+0.7}
\expandafter\def\csname r@ax-het-qasper-nevidence-2-rr-p\endcsname{--}
\expandafter\def\csname r@ax-het-qasper-nevidence-2-rr-v\endcsname{n.d.}
\expandafter\def\csname r@ax-het-qasper-nevidence-3-bm25\endcsname{+8.7 [+2.8, +13.8]}
\expandafter\def\csname r@ax-het-qasper-nevidence-3-bm25-ci\endcsname{[+2.8, +13.8]}
\expandafter\def\csname r@ax-het-qasper-nevidence-3-bm25-ci95\endcsname{[+2.8, +13.8]}
\expandafter\def\csname r@ax-het-qasper-nevidence-3-bm25-d\endcsname{+8.7}
\expandafter\def\csname r@ax-het-qasper-nevidence-3-bm25-p\endcsname{--}
\expandafter\def\csname r@ax-het-qasper-nevidence-3-bm25-v\endcsname{diff.}
\expandafter\def\csname r@ax-het-qasper-nevidence-3-hyb\endcsname{+5.7 [+0.3, +11.4]}
\expandafter\def\csname r@ax-het-qasper-nevidence-3-hyb-ci\endcsname{[+0.3, +11.4]}
\expandafter\def\csname r@ax-het-qasper-nevidence-3-hyb-ci95\endcsname{[+0.3, +11.4]}
\expandafter\def\csname r@ax-het-qasper-nevidence-3-hyb-d\endcsname{+5.7}
\expandafter\def\csname r@ax-het-qasper-nevidence-3-hyb-p\endcsname{--}
\expandafter\def\csname r@ax-het-qasper-nevidence-3-hyb-v\endcsname{diff.}
\expandafter\def\csname r@ax-het-qasper-nevidence-3-n\endcsname{100}
\expandafter\def\csname r@ax-het-qasper-nevidence-3-rr\endcsname{$-$3.0 [$-$7.7, +1.7]}
\expandafter\def\csname r@ax-het-qasper-nevidence-3-rr-ci\endcsname{[$-$7.7, +1.7]}
\expandafter\def\csname r@ax-het-qasper-nevidence-3-rr-ci95\endcsname{[$-$7.7, +1.7]}
\expandafter\def\csname r@ax-het-qasper-nevidence-3-rr-d\endcsname{$-$3.0}
\expandafter\def\csname r@ax-het-qasper-nevidence-3-rr-p\endcsname{--}
\expandafter\def\csname r@ax-het-qasper-nevidence-3-rr-v\endcsname{n.d.}
\expandafter\def\csname r@ax-het-qasper-nevidence-4p-bm25\endcsname{+4.4 [+0.7, +9.5]}
\expandafter\def\csname r@ax-het-qasper-nevidence-4p-bm25-ci\endcsname{[+0.7, +9.5]}
\expandafter\def\csname r@ax-het-qasper-nevidence-4p-bm25-ci95\endcsname{[+0.7, +9.5]}
\expandafter\def\csname r@ax-het-qasper-nevidence-4p-bm25-d\endcsname{+4.4}
\expandafter\def\csname r@ax-het-qasper-nevidence-4p-bm25-p\endcsname{--}
\expandafter\def\csname r@ax-het-qasper-nevidence-4p-bm25-v\endcsname{diff.}
\expandafter\def\csname r@ax-het-qasper-nevidence-4p-hyb\endcsname{+3.0 [$-$1.0, +7.3]}
\expandafter\def\csname r@ax-het-qasper-nevidence-4p-hyb-ci\endcsname{[$-$1.0, +7.3]}
\expandafter\def\csname r@ax-het-qasper-nevidence-4p-hyb-ci95\endcsname{[$-$1.0, +7.3]}
\expandafter\def\csname r@ax-het-qasper-nevidence-4p-hyb-d\endcsname{+3.0}
\expandafter\def\csname r@ax-het-qasper-nevidence-4p-hyb-p\endcsname{--}
\expandafter\def\csname r@ax-het-qasper-nevidence-4p-hyb-v\endcsname{n.d.}
\expandafter\def\csname r@ax-het-qasper-nevidence-4p-n\endcsname{150}
\expandafter\def\csname r@ax-het-qasper-nevidence-4p-rr\endcsname{$-$0.2 [$-$4.1, +4.2]}
\expandafter\def\csname r@ax-het-qasper-nevidence-4p-rr-ci\endcsname{[$-$4.1, +4.2]}
\expandafter\def\csname r@ax-het-qasper-nevidence-4p-rr-ci95\endcsname{[$-$4.1, +4.2]}
\expandafter\def\csname r@ax-het-qasper-nevidence-4p-rr-d\endcsname{$-$0.2}
\expandafter\def\csname r@ax-het-qasper-nevidence-4p-rr-p\endcsname{--}
\expandafter\def\csname r@ax-het-qasper-nevidence-4p-rr-v\endcsname{n.d.}
\expandafter\def\csname r@ax-het-qasper-paperchunks-high-bm25\endcsname{+7.5 [+3.9, +11.5]}
\expandafter\def\csname r@ax-het-qasper-paperchunks-high-bm25-ci\endcsname{[+3.9, +11.5]}
\expandafter\def\csname r@ax-het-qasper-paperchunks-high-bm25-ci95\endcsname{[+3.9, +11.5]}
\expandafter\def\csname r@ax-het-qasper-paperchunks-high-bm25-d\endcsname{+7.5}
\expandafter\def\csname r@ax-het-qasper-paperchunks-high-bm25-p\endcsname{--}
\expandafter\def\csname r@ax-het-qasper-paperchunks-high-bm25-v\endcsname{diff.}
\expandafter\def\csname r@ax-het-qasper-paperchunks-high-hyb\endcsname{+3.2 [$-$0.9, +7.9]}
\expandafter\def\csname r@ax-het-qasper-paperchunks-high-hyb-ci\endcsname{[$-$0.9, +7.9]}
\expandafter\def\csname r@ax-het-qasper-paperchunks-high-hyb-ci95\endcsname{[$-$0.9, +7.9]}
\expandafter\def\csname r@ax-het-qasper-paperchunks-high-hyb-d\endcsname{+3.2}
\expandafter\def\csname r@ax-het-qasper-paperchunks-high-hyb-p\endcsname{--}
\expandafter\def\csname r@ax-het-qasper-paperchunks-high-hyb-v\endcsname{n.d.}
\expandafter\def\csname r@ax-het-qasper-paperchunks-high-n\endcsname{281}
\expandafter\def\csname r@ax-het-qasper-paperchunks-high-rr\endcsname{$-$0.9 [$-$4.3, +2.2]}
\expandafter\def\csname r@ax-het-qasper-paperchunks-high-rr-ci\endcsname{[$-$4.3, +2.2]}
\expandafter\def\csname r@ax-het-qasper-paperchunks-high-rr-ci95\endcsname{[$-$4.3, +2.2]}
\expandafter\def\csname r@ax-het-qasper-paperchunks-high-rr-d\endcsname{$-$0.9}
\expandafter\def\csname r@ax-het-qasper-paperchunks-high-rr-p\endcsname{--}
\expandafter\def\csname r@ax-het-qasper-paperchunks-high-rr-v\endcsname{n.d.}
\expandafter\def\csname r@ax-het-qasper-paperchunks-low-bm25\endcsname{+8.3 [+4.5, +12.5]}
\expandafter\def\csname r@ax-het-qasper-paperchunks-low-bm25-ci\endcsname{[+4.5, +12.5]}
\expandafter\def\csname r@ax-het-qasper-paperchunks-low-bm25-ci95\endcsname{[+4.5, +12.5]}
\expandafter\def\csname r@ax-het-qasper-paperchunks-low-bm25-d\endcsname{+8.3}
\expandafter\def\csname r@ax-het-qasper-paperchunks-low-bm25-p\endcsname{--}
\expandafter\def\csname r@ax-het-qasper-paperchunks-low-bm25-v\endcsname{diff.}
\expandafter\def\csname r@ax-het-qasper-paperchunks-low-hyb\endcsname{+4.5 [$-$0.3, +9.2]}
\expandafter\def\csname r@ax-het-qasper-paperchunks-low-hyb-ci\endcsname{[$-$0.3, +9.2]}
\expandafter\def\csname r@ax-het-qasper-paperchunks-low-hyb-ci95\endcsname{[$-$0.3, +9.2]}
\expandafter\def\csname r@ax-het-qasper-paperchunks-low-hyb-d\endcsname{+4.5}
\expandafter\def\csname r@ax-het-qasper-paperchunks-low-hyb-p\endcsname{--}
\expandafter\def\csname r@ax-het-qasper-paperchunks-low-hyb-v\endcsname{n.d.}
\expandafter\def\csname r@ax-het-qasper-paperchunks-low-n\endcsname{318}
\expandafter\def\csname r@ax-het-qasper-paperchunks-low-rr\endcsname{+2.3 [$-$1.4, +6.7]}
\expandafter\def\csname r@ax-het-qasper-paperchunks-low-rr-ci\endcsname{[$-$1.4, +6.7]}
\expandafter\def\csname r@ax-het-qasper-paperchunks-low-rr-ci95\endcsname{[$-$1.4, +6.7]}
\expandafter\def\csname r@ax-het-qasper-paperchunks-low-rr-d\endcsname{+2.3}
\expandafter\def\csname r@ax-het-qasper-paperchunks-low-rr-p\endcsname{--}
\expandafter\def\csname r@ax-het-qasper-paperchunks-low-rr-v\endcsname{n.d.}
\expandafter\def\csname r@ax-het-qasper-paperchunks-mid-bm25\endcsname{+10.0 [+6.7, +13.2]}
\expandafter\def\csname r@ax-het-qasper-paperchunks-mid-bm25-ci\endcsname{[+6.7, +13.2]}
\expandafter\def\csname r@ax-het-qasper-paperchunks-mid-bm25-ci95\endcsname{[+6.7, +13.2]}
\expandafter\def\csname r@ax-het-qasper-paperchunks-mid-bm25-d\endcsname{+10.0}
\expandafter\def\csname r@ax-het-qasper-paperchunks-mid-bm25-p\endcsname{--}
\expandafter\def\csname r@ax-het-qasper-paperchunks-mid-bm25-v\endcsname{diff.}
\expandafter\def\csname r@ax-het-qasper-paperchunks-mid-hyb\endcsname{+8.2 [+4.0, +12.6]}
\expandafter\def\csname r@ax-het-qasper-paperchunks-mid-hyb-ci\endcsname{[+4.0, +12.6]}
\expandafter\def\csname r@ax-het-qasper-paperchunks-mid-hyb-ci95\endcsname{[+4.0, +12.6]}
\expandafter\def\csname r@ax-het-qasper-paperchunks-mid-hyb-d\endcsname{+8.2}
\expandafter\def\csname r@ax-het-qasper-paperchunks-mid-hyb-p\endcsname{--}
\expandafter\def\csname r@ax-het-qasper-paperchunks-mid-hyb-v\endcsname{diff.}
\expandafter\def\csname r@ax-het-qasper-paperchunks-mid-n\endcsname{352}
\expandafter\def\csname r@ax-het-qasper-paperchunks-mid-rr\endcsname{$-$0.3 [$-$3.9, +3.2]}
\expandafter\def\csname r@ax-het-qasper-paperchunks-mid-rr-ci\endcsname{[$-$3.9, +3.2]}
\expandafter\def\csname r@ax-het-qasper-paperchunks-mid-rr-ci95\endcsname{[$-$3.9, +3.2]}
\expandafter\def\csname r@ax-het-qasper-paperchunks-mid-rr-d\endcsname{$-$0.3}
\expandafter\def\csname r@ax-het-qasper-paperchunks-mid-rr-p\endcsname{--}
\expandafter\def\csname r@ax-het-qasper-paperchunks-mid-rr-v\endcsname{n.d.}
\expandafter\def\csname r@ax-key-fs-E-adj\endcsname{50}
\expandafter\def\csname r@ax-key-fs-E-distmed\endcsname{1}
\expandafter\def\csname r@ax-key-fs-E-evictdocs\endcsname{28}
\expandafter\def\csname r@ax-key-fs-E-gt10\endcsname{16}
\expandafter\def\csname r@ax-key-fs-E-keytokintext\endcsname{79}
\expandafter\def\csname r@ax-key-fs-E-kwnew\endcsname{16}
\expandafter\def\csname r@ax-key-fs-E-outside\endcsname{26}
\expandafter\def\csname r@ax-key-fs-E-qnew\endcsname{28}
\expandafter\def\csname r@ax-key-fs-E-reuses\endcsname{933}
\expandafter\def\csname r@ax-key-fs-E-verbatim\endcsname{33}
\expandafter\def\csname r@ax-key-fs-E-within3\endcsname{65}
\expandafter\def\csname r@ax-key-fs-Enork-adj\endcsname{41}
\expandafter\def\csname r@ax-key-fs-Enork-distmed\endcsname{2}
\expandafter\def\csname r@ax-key-fs-Enork-evictdocs\endcsname{30}
\expandafter\def\csname r@ax-key-fs-Enork-gt10\endcsname{23}
\expandafter\def\csname r@ax-key-fs-Enork-keytokintext\endcsname{82}
\expandafter\def\csname r@ax-key-fs-Enork-kwnew\endcsname{15}
\expandafter\def\csname r@ax-key-fs-Enork-outside\endcsname{20}
\expandafter\def\csname r@ax-key-fs-Enork-qnew\endcsname{29}
\expandafter\def\csname r@ax-key-fs-Enork-reuses\endcsname{357}
\expandafter\def\csname r@ax-key-fs-Enork-verbatim\endcsname{37}
\expandafter\def\csname r@ax-key-fs-Enork-within3\endcsname{58}
\expandafter\def\csname r@ax-key-qasper-E-adj\endcsname{37}
\expandafter\def\csname r@ax-key-qasper-E-distmed\endcsname{2}
\expandafter\def\csname r@ax-key-qasper-E-evictdocs\endcsname{6}
\expandafter\def\csname r@ax-key-qasper-E-gt10\endcsname{13}
\expandafter\def\csname r@ax-key-qasper-E-keytokintext\endcsname{79}
\expandafter\def\csname r@ax-key-qasper-E-kwnew\endcsname{10}
\expandafter\def\csname r@ax-key-qasper-E-outside\endcsname{0}
\expandafter\def\csname r@ax-key-qasper-E-qnew\endcsname{31}
\expandafter\def\csname r@ax-key-qasper-E-reuses\endcsname{1,171}
\expandafter\def\csname r@ax-key-qasper-E-verbatim\endcsname{33}
\expandafter\def\csname r@ax-key-qasper-E-within3\endcsname{64}
\expandafter\def\csname r@ax-key-qasper-Enork-adj\endcsname{31}
\expandafter\def\csname r@ax-key-qasper-Enork-distmed\endcsname{3}
\expandafter\def\csname r@ax-key-qasper-Enork-evictdocs\endcsname{11}
\expandafter\def\csname r@ax-key-qasper-Enork-gt10\endcsname{22}
\expandafter\def\csname r@ax-key-qasper-Enork-keytokintext\endcsname{82}
\expandafter\def\csname r@ax-key-qasper-Enork-kwnew\endcsname{9}
\expandafter\def\csname r@ax-key-qasper-Enork-outside\endcsname{2}
\expandafter\def\csname r@ax-key-qasper-Enork-qnew\endcsname{30}
\expandafter\def\csname r@ax-key-qasper-Enork-reuses\endcsname{441}
\expandafter\def\csname r@ax-key-qasper-Enork-verbatim\endcsname{35}
\expandafter\def\csname r@ax-key-qasper-Enork-within3\endcsname{53}
\expandafter\def\csname r@ax-lc-dcos-c\endcsname{$-$2.5 [$-$10.2, +5.3]}
\expandafter\def\csname r@ax-lc-dcos-c-ci\endcsname{[$-$10.2, +5.3]}
\expandafter\def\csname r@ax-lc-dcos-c-ci95\endcsname{[$-$10.2, +5.3]}
\expandafter\def\csname r@ax-lc-dcos-c-d\endcsname{$-$2.5}
\expandafter\def\csname r@ax-lc-dcos-c-p\endcsname{--}
\expandafter\def\csname r@ax-lc-dcos-c-v\endcsname{n.d.}
\expandafter\def\csname r@ax-lc-rho-dcos-nchunks\endcsname{0.31}
\expandafter\def\csname r@ax-lc-rho-dcos-nchunks-ci\endcsname{[0.20, 0.41]}
\expandafter\def\csname r@ax-lc-rho-loss-coslate\endcsname{$-$0.08}
\expandafter\def\csname r@ax-lc-rho-loss-coslate-ci\endcsname{[$-$0.19, 0.03]}
\expandafter\def\csname r@ax-lc-rho-loss-dcos\endcsname{$-$0.05}
\expandafter\def\csname r@ax-lc-rho-loss-dcos-ci\endcsname{[$-$0.17, 0.07]}
\expandafter\def\csname r@ax-lc-rho-loss-nchunks\endcsname{$-$0.12}
\expandafter\def\csname r@ax-lc-rho-loss-nchunks-ci\endcsname{[$-$0.24, $-$0.01]}
\expandafter\def\csname r@ax-lc-rho-loss-tokens\endcsname{$-$0.08}
\expandafter\def\csname r@ax-lc-rho-loss-tokens-ci\endcsname{[$-$0.20, 0.03]}
\expandafter\def\csname r@ax-lc-share-ge90\endcsname{97.7}
\expandafter\def\csname r@ax-lc-win-c\endcsname{$-$7.6 [$-$16.3, +0.5]}
\expandafter\def\csname r@ax-lc-win-c-ci\endcsname{[$-$16.3, +0.5]}
\expandafter\def\csname r@ax-lc-win-c-ci95\endcsname{[$-$16.3, +0.5]}
\expandafter\def\csname r@ax-lc-win-c-d\endcsname{$-$7.6}
\expandafter\def\csname r@ax-lc-win-c-p\endcsname{--}
\expandafter\def\csname r@ax-lc-win-c-v\endcsname{n.d.}
\expandafter\def\csname r@ax-lc-win-multi\endcsname{$-$18.2 [$-$26.3, $-$10.9]}
\expandafter\def\csname r@ax-lc-win-multi-ci\endcsname{[$-$26.3, $-$10.9]}
\expandafter\def\csname r@ax-lc-win-multi-ci95\endcsname{[$-$26.3, $-$10.9]}
\expandafter\def\csname r@ax-lc-win-multi-d\endcsname{$-$18.2}
\expandafter\def\csname r@ax-lc-win-multi-n\endcsname{35}
\expandafter\def\csname r@ax-lc-win-multi-p\endcsname{--}
\expandafter\def\csname r@ax-lc-win-multi-v\endcsname{diff.}
\expandafter\def\csname r@ax-lc-win-one\endcsname{$-$10.5 [$-$14.0, $-$7.2]}
\expandafter\def\csname r@ax-lc-win-one-ci\endcsname{[$-$14.0, $-$7.2]}
\expandafter\def\csname r@ax-lc-win-one-ci95\endcsname{[$-$14.0, $-$7.2]}
\expandafter\def\csname r@ax-lc-win-one-d\endcsname{$-$10.5}
\expandafter\def\csname r@ax-lc-win-one-n\endcsname{265}
\expandafter\def\csname r@ax-lc-win-one-p\endcsname{--}
\expandafter\def\csname r@ax-lc-win-one-v\endcsname{diff.}
\expandafter\def\csname r@ax-ovl-fs-bm25-high\endcsname{+2.9 [$-$0.4, +7.6]}
\expandafter\def\csname r@ax-ovl-fs-bm25-high-ci\endcsname{[$-$0.4, +7.6]}
\expandafter\def\csname r@ax-ovl-fs-bm25-high-ci95\endcsname{[$-$0.4, +7.6]}
\expandafter\def\csname r@ax-ovl-fs-bm25-high-d\endcsname{+2.9}
\expandafter\def\csname r@ax-ovl-fs-bm25-high-p\endcsname{--}
\expandafter\def\csname r@ax-ovl-fs-bm25-high-v\endcsname{n.d.}
\expandafter\def\csname r@ax-ovl-fs-bm25-lmh\endcsname{$-$0.7 [$-$5.7, +3.6]}
\expandafter\def\csname r@ax-ovl-fs-bm25-lmh-ci\endcsname{[$-$5.7, +3.6]}
\expandafter\def\csname r@ax-ovl-fs-bm25-lmh-ci95\endcsname{[$-$5.7, +3.6]}
\expandafter\def\csname r@ax-ovl-fs-bm25-lmh-d\endcsname{$-$0.7}
\expandafter\def\csname r@ax-ovl-fs-bm25-lmh-p\endcsname{--}
\expandafter\def\csname r@ax-ovl-fs-bm25-lmh-v\endcsname{n.d.}
\expandafter\def\csname r@ax-ovl-fs-bm25-low\endcsname{+2.2 [+0.1, +5.4]}
\expandafter\def\csname r@ax-ovl-fs-bm25-low-ci\endcsname{[+0.1, +5.4]}
\expandafter\def\csname r@ax-ovl-fs-bm25-low-ci95\endcsname{[+0.1, +5.4]}
\expandafter\def\csname r@ax-ovl-fs-bm25-low-d\endcsname{+2.2}
\expandafter\def\csname r@ax-ovl-fs-bm25-low-p\endcsname{--}
\expandafter\def\csname r@ax-ovl-fs-bm25-low-v\endcsname{diff.}
\expandafter\def\csname r@ax-ovl-fs-bm25-mid\endcsname{+2.0 [+0.3, +4.4]}
\expandafter\def\csname r@ax-ovl-fs-bm25-mid-ci\endcsname{[+0.3, +4.4]}
\expandafter\def\csname r@ax-ovl-fs-bm25-mid-ci95\endcsname{[+0.3, +4.4]}
\expandafter\def\csname r@ax-ovl-fs-bm25-mid-d\endcsname{+2.0}
\expandafter\def\csname r@ax-ovl-fs-bm25-mid-p\endcsname{--}
\expandafter\def\csname r@ax-ovl-fs-bm25-mid-v\endcsname{diff.}
\expandafter\def\csname r@ax-ovl-fs-cut1\endcsname{36}
\expandafter\def\csname r@ax-ovl-fs-cut2\endcsname{52}
\expandafter\def\csname r@ax-ovl-fs-hq3-high\endcsname{+0.7 [$-$2.8, +3.9]}
\expandafter\def\csname r@ax-ovl-fs-hq3-high-ci\endcsname{[$-$2.8, +3.9]}
\expandafter\def\csname r@ax-ovl-fs-hq3-high-ci95\endcsname{[$-$2.8, +3.9]}
\expandafter\def\csname r@ax-ovl-fs-hq3-high-d\endcsname{+0.7}
\expandafter\def\csname r@ax-ovl-fs-hq3-high-p\endcsname{--}
\expandafter\def\csname r@ax-ovl-fs-hq3-high-v\endcsname{n.d.}
\expandafter\def\csname r@ax-ovl-fs-hq3-lmh\endcsname{$-$0.6 [$-$4.7, +3.5]}
\expandafter\def\csname r@ax-ovl-fs-hq3-lmh-ci\endcsname{[$-$4.7, +3.5]}
\expandafter\def\csname r@ax-ovl-fs-hq3-lmh-ci95\endcsname{[$-$4.7, +3.5]}
\expandafter\def\csname r@ax-ovl-fs-hq3-lmh-d\endcsname{$-$0.6}
\expandafter\def\csname r@ax-ovl-fs-hq3-lmh-p\endcsname{--}
\expandafter\def\csname r@ax-ovl-fs-hq3-lmh-v\endcsname{n.d.}
\expandafter\def\csname r@ax-ovl-fs-hq3-low\endcsname{+0.1 [$-$2.3, +2.4]}
\expandafter\def\csname r@ax-ovl-fs-hq3-low-ci\endcsname{[$-$2.3, +2.4]}
\expandafter\def\csname r@ax-ovl-fs-hq3-low-ci95\endcsname{[$-$2.3, +2.4]}
\expandafter\def\csname r@ax-ovl-fs-hq3-low-d\endcsname{+0.1}
\expandafter\def\csname r@ax-ovl-fs-hq3-low-p\endcsname{--}
\expandafter\def\csname r@ax-ovl-fs-hq3-low-v\endcsname{n.d.}
\expandafter\def\csname r@ax-ovl-fs-hq3-mid\endcsname{+2.4 [$-$2.1, +6.2]}
\expandafter\def\csname r@ax-ovl-fs-hq3-mid-ci\endcsname{[$-$2.1, +6.2]}
\expandafter\def\csname r@ax-ovl-fs-hq3-mid-ci95\endcsname{[$-$2.1, +6.2]}
\expandafter\def\csname r@ax-ovl-fs-hq3-mid-d\endcsname{+2.4}
\expandafter\def\csname r@ax-ovl-fs-hq3-mid-p\endcsname{--}
\expandafter\def\csname r@ax-ovl-fs-hq3-mid-v\endcsname{n.d.}
\expandafter\def\csname r@ax-ovl-fs-hyb-high\endcsname{+1.1 [$-$3.4, +5.4]}
\expandafter\def\csname r@ax-ovl-fs-hyb-high-ci\endcsname{[$-$3.4, +5.4]}
\expandafter\def\csname r@ax-ovl-fs-hyb-high-ci95\endcsname{[$-$3.4, +5.4]}
\expandafter\def\csname r@ax-ovl-fs-hyb-high-d\endcsname{+1.1}
\expandafter\def\csname r@ax-ovl-fs-hyb-high-p\endcsname{--}
\expandafter\def\csname r@ax-ovl-fs-hyb-high-v\endcsname{n.d.}
\expandafter\def\csname r@ax-ovl-fs-hyb-lmh\endcsname{+1.9 [$-$3.2, +7.4]}
\expandafter\def\csname r@ax-ovl-fs-hyb-lmh-ci\endcsname{[$-$3.2, +7.4]}
\expandafter\def\csname r@ax-ovl-fs-hyb-lmh-ci95\endcsname{[$-$3.2, +7.4]}
\expandafter\def\csname r@ax-ovl-fs-hyb-lmh-d\endcsname{+1.9}
\expandafter\def\csname r@ax-ovl-fs-hyb-lmh-p\endcsname{--}
\expandafter\def\csname r@ax-ovl-fs-hyb-lmh-v\endcsname{n.d.}
\expandafter\def\csname r@ax-ovl-fs-hyb-low\endcsname{+3.0 [+0.3, +6.2]}
\expandafter\def\csname r@ax-ovl-fs-hyb-low-ci\endcsname{[+0.3, +6.2]}
\expandafter\def\csname r@ax-ovl-fs-hyb-low-ci95\endcsname{[+0.3, +6.2]}
\expandafter\def\csname r@ax-ovl-fs-hyb-low-d\endcsname{+3.0}
\expandafter\def\csname r@ax-ovl-fs-hyb-low-p\endcsname{--}
\expandafter\def\csname r@ax-ovl-fs-hyb-low-v\endcsname{diff.}
\expandafter\def\csname r@ax-ovl-fs-hyb-mid\endcsname{+4.1 [+0.0, +8.6]}
\expandafter\def\csname r@ax-ovl-fs-hyb-mid-ci\endcsname{[+0.0, +8.6]}
\expandafter\def\csname r@ax-ovl-fs-hyb-mid-ci95\endcsname{[+0.0, +8.6]}
\expandafter\def\csname r@ax-ovl-fs-hyb-mid-d\endcsname{+4.1}
\expandafter\def\csname r@ax-ovl-fs-hyb-mid-p\endcsname{--}
\expandafter\def\csname r@ax-ovl-fs-hyb-mid-v\endcsname{diff.}
\expandafter\def\csname r@ax-ovl-fs-mean\endcsname{45}
\expandafter\def\csname r@ax-ovl-fs-mxbai-high\endcsname{+1.7 [$-$2.6, +6.0]}
\expandafter\def\csname r@ax-ovl-fs-mxbai-high-ci\endcsname{[$-$2.6, +6.0]}
\expandafter\def\csname r@ax-ovl-fs-mxbai-high-ci95\endcsname{[$-$2.6, +6.0]}
\expandafter\def\csname r@ax-ovl-fs-mxbai-high-d\endcsname{+1.7}
\expandafter\def\csname r@ax-ovl-fs-mxbai-high-p\endcsname{--}
\expandafter\def\csname r@ax-ovl-fs-mxbai-high-v\endcsname{n.d.}
\expandafter\def\csname r@ax-ovl-fs-mxbai-lmh\endcsname{$-$0.5 [$-$5.6, +4.5]}
\expandafter\def\csname r@ax-ovl-fs-mxbai-lmh-ci\endcsname{[$-$5.6, +4.5]}
\expandafter\def\csname r@ax-ovl-fs-mxbai-lmh-ci95\endcsname{[$-$5.6, +4.5]}
\expandafter\def\csname r@ax-ovl-fs-mxbai-lmh-d\endcsname{$-$0.5}
\expandafter\def\csname r@ax-ovl-fs-mxbai-lmh-p\endcsname{--}
\expandafter\def\csname r@ax-ovl-fs-mxbai-lmh-v\endcsname{n.d.}
\expandafter\def\csname r@ax-ovl-fs-mxbai-low\endcsname{+1.2 [$-$1.4, +3.7]}
\expandafter\def\csname r@ax-ovl-fs-mxbai-low-ci\endcsname{[$-$1.4, +3.7]}
\expandafter\def\csname r@ax-ovl-fs-mxbai-low-ci95\endcsname{[$-$1.4, +3.7]}
\expandafter\def\csname r@ax-ovl-fs-mxbai-low-d\endcsname{+1.2}
\expandafter\def\csname r@ax-ovl-fs-mxbai-low-p\endcsname{--}
\expandafter\def\csname r@ax-ovl-fs-mxbai-low-v\endcsname{n.d.}
\expandafter\def\csname r@ax-ovl-fs-mxbai-mid\endcsname{$-$2.9 [$-$7.2, +1.6]}
\expandafter\def\csname r@ax-ovl-fs-mxbai-mid-ci\endcsname{[$-$7.2, +1.6]}
\expandafter\def\csname r@ax-ovl-fs-mxbai-mid-ci95\endcsname{[$-$7.2, +1.6]}
\expandafter\def\csname r@ax-ovl-fs-mxbai-mid-d\endcsname{$-$2.9}
\expandafter\def\csname r@ax-ovl-fs-mxbai-mid-p\endcsname{--}
\expandafter\def\csname r@ax-ovl-fs-mxbai-mid-v\endcsname{n.d.}
\expandafter\def\csname r@ax-ovl-fs-nomic-high\endcsname{+1.3 [$-$3.6, +6.7]}
\expandafter\def\csname r@ax-ovl-fs-nomic-high-ci\endcsname{[$-$3.6, +6.7]}
\expandafter\def\csname r@ax-ovl-fs-nomic-high-ci95\endcsname{[$-$3.6, +6.7]}
\expandafter\def\csname r@ax-ovl-fs-nomic-high-d\endcsname{+1.3}
\expandafter\def\csname r@ax-ovl-fs-nomic-high-p\endcsname{--}
\expandafter\def\csname r@ax-ovl-fs-nomic-high-v\endcsname{n.d.}
\expandafter\def\csname r@ax-ovl-fs-nomic-lmh\endcsname{+1.6 [$-$4.8, +7.5]}
\expandafter\def\csname r@ax-ovl-fs-nomic-lmh-ci\endcsname{[$-$4.8, +7.5]}
\expandafter\def\csname r@ax-ovl-fs-nomic-lmh-ci95\endcsname{[$-$4.8, +7.5]}
\expandafter\def\csname r@ax-ovl-fs-nomic-lmh-d\endcsname{+1.6}
\expandafter\def\csname r@ax-ovl-fs-nomic-lmh-p\endcsname{--}
\expandafter\def\csname r@ax-ovl-fs-nomic-lmh-v\endcsname{n.d.}
\expandafter\def\csname r@ax-ovl-fs-nomic-low\endcsname{+2.9 [$-$0.5, +6.2]}
\expandafter\def\csname r@ax-ovl-fs-nomic-low-ci\endcsname{[$-$0.5, +6.2]}
\expandafter\def\csname r@ax-ovl-fs-nomic-low-ci95\endcsname{[$-$0.5, +6.2]}
\expandafter\def\csname r@ax-ovl-fs-nomic-low-d\endcsname{+2.9}
\expandafter\def\csname r@ax-ovl-fs-nomic-low-p\endcsname{--}
\expandafter\def\csname r@ax-ovl-fs-nomic-low-v\endcsname{n.d.}
\expandafter\def\csname r@ax-ovl-fs-nomic-mid\endcsname{+3.7 [+0.3, +7.8]}
\expandafter\def\csname r@ax-ovl-fs-nomic-mid-ci\endcsname{[+0.3, +7.8]}
\expandafter\def\csname r@ax-ovl-fs-nomic-mid-ci95\endcsname{[+0.3, +7.8]}
\expandafter\def\csname r@ax-ovl-fs-nomic-mid-d\endcsname{+3.7}
\expandafter\def\csname r@ax-ovl-fs-nomic-mid-p\endcsname{--}
\expandafter\def\csname r@ax-ovl-fs-nomic-mid-v\endcsname{diff.}
\expandafter\def\csname r@ax-ovl-fs-q3-high\endcsname{+1.4 [$-$1.9, +5.0]}
\expandafter\def\csname r@ax-ovl-fs-q3-high-ci\endcsname{[$-$1.9, +5.0]}
\expandafter\def\csname r@ax-ovl-fs-q3-high-ci95\endcsname{[$-$1.9, +5.0]}
\expandafter\def\csname r@ax-ovl-fs-q3-high-d\endcsname{+1.4}
\expandafter\def\csname r@ax-ovl-fs-q3-high-p\endcsname{--}
\expandafter\def\csname r@ax-ovl-fs-q3-high-v\endcsname{n.d.}
\expandafter\def\csname r@ax-ovl-fs-q3-lmh\endcsname{$-$1.2 [$-$5.5, +2.9]}
\expandafter\def\csname r@ax-ovl-fs-q3-lmh-ci\endcsname{[$-$5.5, +2.9]}
\expandafter\def\csname r@ax-ovl-fs-q3-lmh-ci95\endcsname{[$-$5.5, +2.9]}
\expandafter\def\csname r@ax-ovl-fs-q3-lmh-d\endcsname{$-$1.2}
\expandafter\def\csname r@ax-ovl-fs-q3-lmh-p\endcsname{--}
\expandafter\def\csname r@ax-ovl-fs-q3-lmh-v\endcsname{n.d.}
\expandafter\def\csname r@ax-ovl-fs-q3-low\endcsname{+0.2 [$-$2.2, +2.4]}
\expandafter\def\csname r@ax-ovl-fs-q3-low-ci\endcsname{[$-$2.2, +2.4]}
\expandafter\def\csname r@ax-ovl-fs-q3-low-ci95\endcsname{[$-$2.2, +2.4]}
\expandafter\def\csname r@ax-ovl-fs-q3-low-d\endcsname{+0.2}
\expandafter\def\csname r@ax-ovl-fs-q3-low-p\endcsname{--}
\expandafter\def\csname r@ax-ovl-fs-q3-low-v\endcsname{n.d.}
\expandafter\def\csname r@ax-ovl-fs-q3-mid\endcsname{$-$0.8 [$-$3.6, +2.4]}
\expandafter\def\csname r@ax-ovl-fs-q3-mid-ci\endcsname{[$-$3.6, +2.4]}
\expandafter\def\csname r@ax-ovl-fs-q3-mid-ci95\endcsname{[$-$3.6, +2.4]}
\expandafter\def\csname r@ax-ovl-fs-q3-mid-d\endcsname{$-$0.8}
\expandafter\def\csname r@ax-ovl-fs-q3-mid-p\endcsname{--}
\expandafter\def\csname r@ax-ovl-fs-q3-mid-v\endcsname{n.d.}
\expandafter\def\csname r@ax-ovl-fs-rr-high\endcsname{+0.2 [$-$3.7, +4.2]}
\expandafter\def\csname r@ax-ovl-fs-rr-high-ci\endcsname{[$-$3.7, +4.2]}
\expandafter\def\csname r@ax-ovl-fs-rr-high-ci95\endcsname{[$-$3.7, +4.2]}
\expandafter\def\csname r@ax-ovl-fs-rr-high-d\endcsname{+0.2}
\expandafter\def\csname r@ax-ovl-fs-rr-high-p\endcsname{--}
\expandafter\def\csname r@ax-ovl-fs-rr-high-v\endcsname{n.d.}
\expandafter\def\csname r@ax-ovl-fs-rr-lmh\endcsname{+1.8 [$-$3.6, +7.4]}
\expandafter\def\csname r@ax-ovl-fs-rr-lmh-ci\endcsname{[$-$3.6, +7.4]}
\expandafter\def\csname r@ax-ovl-fs-rr-lmh-ci95\endcsname{[$-$3.6, +7.4]}
\expandafter\def\csname r@ax-ovl-fs-rr-lmh-d\endcsname{+1.8}
\expandafter\def\csname r@ax-ovl-fs-rr-lmh-p\endcsname{--}
\expandafter\def\csname r@ax-ovl-fs-rr-lmh-v\endcsname{n.d.}
\expandafter\def\csname r@ax-ovl-fs-rr-low\endcsname{+1.9 [$-$1.5, +5.9]}
\expandafter\def\csname r@ax-ovl-fs-rr-low-ci\endcsname{[$-$1.5, +5.9]}
\expandafter\def\csname r@ax-ovl-fs-rr-low-ci95\endcsname{[$-$1.5, +5.9]}
\expandafter\def\csname r@ax-ovl-fs-rr-low-d\endcsname{+1.9}
\expandafter\def\csname r@ax-ovl-fs-rr-low-p\endcsname{--}
\expandafter\def\csname r@ax-ovl-fs-rr-low-v\endcsname{n.d.}
\expandafter\def\csname r@ax-ovl-fs-rr-mid\endcsname{+0.3 [$-$3.4, +4.3]}
\expandafter\def\csname r@ax-ovl-fs-rr-mid-ci\endcsname{[$-$3.4, +4.3]}
\expandafter\def\csname r@ax-ovl-fs-rr-mid-ci95\endcsname{[$-$3.4, +4.3]}
\expandafter\def\csname r@ax-ovl-fs-rr-mid-d\endcsname{+0.3}
\expandafter\def\csname r@ax-ovl-fs-rr-mid-p\endcsname{--}
\expandafter\def\csname r@ax-ovl-fs-rr-mid-v\endcsname{n.d.}
\expandafter\def\csname r@ax-ovl-qasper-bm25-high\endcsname{+9.4 [+5.7, +13.2]}
\expandafter\def\csname r@ax-ovl-qasper-bm25-high-ci\endcsname{[+5.7, +13.2]}
\expandafter\def\csname r@ax-ovl-qasper-bm25-high-ci95\endcsname{[+5.7, +13.2]}
\expandafter\def\csname r@ax-ovl-qasper-bm25-high-d\endcsname{+9.4}
\expandafter\def\csname r@ax-ovl-qasper-bm25-high-p\endcsname{--}
\expandafter\def\csname r@ax-ovl-qasper-bm25-high-v\endcsname{diff.}
\expandafter\def\csname r@ax-ovl-qasper-bm25-lmh\endcsname{+0.1 [$-$5.0, +5.2]}
\expandafter\def\csname r@ax-ovl-qasper-bm25-lmh-ci\endcsname{[$-$5.0, +5.2]}
\expandafter\def\csname r@ax-ovl-qasper-bm25-lmh-ci95\endcsname{[$-$5.0, +5.2]}
\expandafter\def\csname r@ax-ovl-qasper-bm25-lmh-d\endcsname{+0.1}
\expandafter\def\csname r@ax-ovl-qasper-bm25-lmh-p\endcsname{--}
\expandafter\def\csname r@ax-ovl-qasper-bm25-lmh-v\endcsname{n.d.}
\expandafter\def\csname r@ax-ovl-qasper-bm25-low\endcsname{+9.5 [+6.2, +13.0]}
\expandafter\def\csname r@ax-ovl-qasper-bm25-low-ci\endcsname{[+6.2, +13.0]}
\expandafter\def\csname r@ax-ovl-qasper-bm25-low-ci95\endcsname{[+6.2, +13.0]}
\expandafter\def\csname r@ax-ovl-qasper-bm25-low-d\endcsname{+9.5}
\expandafter\def\csname r@ax-ovl-qasper-bm25-low-p\endcsname{--}
\expandafter\def\csname r@ax-ovl-qasper-bm25-low-v\endcsname{diff.}
\expandafter\def\csname r@ax-ovl-qasper-bm25-mid\endcsname{+6.8 [+2.9, +10.9]}
\expandafter\def\csname r@ax-ovl-qasper-bm25-mid-ci\endcsname{[+2.9, +10.9]}
\expandafter\def\csname r@ax-ovl-qasper-bm25-mid-ci95\endcsname{[+2.9, +10.9]}
\expandafter\def\csname r@ax-ovl-qasper-bm25-mid-d\endcsname{+6.8}
\expandafter\def\csname r@ax-ovl-qasper-bm25-mid-p\endcsname{--}
\expandafter\def\csname r@ax-ovl-qasper-bm25-mid-v\endcsname{diff.}
\expandafter\def\csname r@ax-ovl-qasper-cut1\endcsname{33}
\expandafter\def\csname r@ax-ovl-qasper-cut2\endcsname{57}
\expandafter\def\csname r@ax-ovl-qasper-hq3-high\endcsname{+3.7 [$-$0.3, +7.8]}
\expandafter\def\csname r@ax-ovl-qasper-hq3-high-ci\endcsname{[$-$0.3, +7.8]}
\expandafter\def\csname r@ax-ovl-qasper-hq3-high-ci95\endcsname{[$-$0.3, +7.8]}
\expandafter\def\csname r@ax-ovl-qasper-hq3-high-d\endcsname{+3.7}
\expandafter\def\csname r@ax-ovl-qasper-hq3-high-p\endcsname{--}
\expandafter\def\csname r@ax-ovl-qasper-hq3-high-v\endcsname{n.d.}
\expandafter\def\csname r@ax-ovl-qasper-hq3-lmh\endcsname{+3.9 [$-$2.0, +9.7]}
\expandafter\def\csname r@ax-ovl-qasper-hq3-lmh-ci\endcsname{[$-$2.0, +9.7]}
\expandafter\def\csname r@ax-ovl-qasper-hq3-lmh-ci95\endcsname{[$-$2.0, +9.7]}
\expandafter\def\csname r@ax-ovl-qasper-hq3-lmh-d\endcsname{+3.9}
\expandafter\def\csname r@ax-ovl-qasper-hq3-lmh-p\endcsname{--}
\expandafter\def\csname r@ax-ovl-qasper-hq3-lmh-v\endcsname{n.d.}
\expandafter\def\csname r@ax-ovl-qasper-hq3-low\endcsname{+7.6 [+3.5, +12.3]}
\expandafter\def\csname r@ax-ovl-qasper-hq3-low-ci\endcsname{[+3.5, +12.3]}
\expandafter\def\csname r@ax-ovl-qasper-hq3-low-ci95\endcsname{[+3.5, +12.3]}
\expandafter\def\csname r@ax-ovl-qasper-hq3-low-d\endcsname{+7.6}
\expandafter\def\csname r@ax-ovl-qasper-hq3-low-p\endcsname{--}
\expandafter\def\csname r@ax-ovl-qasper-hq3-low-v\endcsname{diff.}
\expandafter\def\csname r@ax-ovl-qasper-hq3-mid\endcsname{+1.2 [$-$3.1, +5.1]}
\expandafter\def\csname r@ax-ovl-qasper-hq3-mid-ci\endcsname{[$-$3.1, +5.1]}
\expandafter\def\csname r@ax-ovl-qasper-hq3-mid-ci95\endcsname{[$-$3.1, +5.1]}
\expandafter\def\csname r@ax-ovl-qasper-hq3-mid-d\endcsname{+1.2}
\expandafter\def\csname r@ax-ovl-qasper-hq3-mid-p\endcsname{--}
\expandafter\def\csname r@ax-ovl-qasper-hq3-mid-v\endcsname{n.d.}
\expandafter\def\csname r@ax-ovl-qasper-hyb-high\endcsname{+5.8 [+1.4, +10.2]}
\expandafter\def\csname r@ax-ovl-qasper-hyb-high-ci\endcsname{[+1.4, +10.2]}
\expandafter\def\csname r@ax-ovl-qasper-hyb-high-ci95\endcsname{[+1.4, +10.2]}
\expandafter\def\csname r@ax-ovl-qasper-hyb-high-d\endcsname{+5.8}
\expandafter\def\csname r@ax-ovl-qasper-hyb-high-p\endcsname{--}
\expandafter\def\csname r@ax-ovl-qasper-hyb-high-v\endcsname{diff.}
\expandafter\def\csname r@ax-ovl-qasper-hyb-lmh\endcsname{$-$0.4 [$-$6.8, +5.9]}
\expandafter\def\csname r@ax-ovl-qasper-hyb-lmh-ci\endcsname{[$-$6.8, +5.9]}
\expandafter\def\csname r@ax-ovl-qasper-hyb-lmh-ci95\endcsname{[$-$6.8, +5.9]}
\expandafter\def\csname r@ax-ovl-qasper-hyb-lmh-d\endcsname{$-$0.4}
\expandafter\def\csname r@ax-ovl-qasper-hyb-lmh-p\endcsname{--}
\expandafter\def\csname r@ax-ovl-qasper-hyb-lmh-v\endcsname{n.d.}
\expandafter\def\csname r@ax-ovl-qasper-hyb-low\endcsname{+5.4 [+1.2, +10.0]}
\expandafter\def\csname r@ax-ovl-qasper-hyb-low-ci\endcsname{[+1.2, +10.0]}
\expandafter\def\csname r@ax-ovl-qasper-hyb-low-ci95\endcsname{[+1.2, +10.0]}
\expandafter\def\csname r@ax-ovl-qasper-hyb-low-d\endcsname{+5.4}
\expandafter\def\csname r@ax-ovl-qasper-hyb-low-p\endcsname{--}
\expandafter\def\csname r@ax-ovl-qasper-hyb-low-v\endcsname{diff.}
\expandafter\def\csname r@ax-ovl-qasper-hyb-mid\endcsname{+5.3 [+1.2, +9.4]}
\expandafter\def\csname r@ax-ovl-qasper-hyb-mid-ci\endcsname{[+1.2, +9.4]}
\expandafter\def\csname r@ax-ovl-qasper-hyb-mid-ci95\endcsname{[+1.2, +9.4]}
\expandafter\def\csname r@ax-ovl-qasper-hyb-mid-d\endcsname{+5.3}
\expandafter\def\csname r@ax-ovl-qasper-hyb-mid-p\endcsname{--}
\expandafter\def\csname r@ax-ovl-qasper-hyb-mid-v\endcsname{diff.}
\expandafter\def\csname r@ax-ovl-qasper-mean\endcsname{45}
\expandafter\def\csname r@ax-ovl-qasper-mxbai-high\endcsname{+2.7 [$-$1.6, +7.3]}
\expandafter\def\csname r@ax-ovl-qasper-mxbai-high-ci\endcsname{[$-$1.6, +7.3]}
\expandafter\def\csname r@ax-ovl-qasper-mxbai-high-ci95\endcsname{[$-$1.6, +7.3]}
\expandafter\def\csname r@ax-ovl-qasper-mxbai-high-d\endcsname{+2.7}
\expandafter\def\csname r@ax-ovl-qasper-mxbai-high-p\endcsname{--}
\expandafter\def\csname r@ax-ovl-qasper-mxbai-high-v\endcsname{n.d.}
\expandafter\def\csname r@ax-ovl-qasper-mxbai-lmh\endcsname{$-$3.8 [$-$9.7, +2.1]}
\expandafter\def\csname r@ax-ovl-qasper-mxbai-lmh-ci\endcsname{[$-$9.7, +2.1]}
\expandafter\def\csname r@ax-ovl-qasper-mxbai-lmh-ci95\endcsname{[$-$9.7, +2.1]}
\expandafter\def\csname r@ax-ovl-qasper-mxbai-lmh-d\endcsname{$-$3.8}
\expandafter\def\csname r@ax-ovl-qasper-mxbai-lmh-p\endcsname{--}
\expandafter\def\csname r@ax-ovl-qasper-mxbai-lmh-v\endcsname{n.d.}
\expandafter\def\csname r@ax-ovl-qasper-mxbai-low\endcsname{$-$1.1 [$-$5.1, +2.8]}
\expandafter\def\csname r@ax-ovl-qasper-mxbai-low-ci\endcsname{[$-$5.1, +2.8]}
\expandafter\def\csname r@ax-ovl-qasper-mxbai-low-ci95\endcsname{[$-$5.1, +2.8]}
\expandafter\def\csname r@ax-ovl-qasper-mxbai-low-d\endcsname{$-$1.1}
\expandafter\def\csname r@ax-ovl-qasper-mxbai-low-p\endcsname{--}
\expandafter\def\csname r@ax-ovl-qasper-mxbai-low-v\endcsname{n.d.}
\expandafter\def\csname r@ax-ovl-qasper-mxbai-mid\endcsname{+1.0 [$-$3.1, +5.0]}
\expandafter\def\csname r@ax-ovl-qasper-mxbai-mid-ci\endcsname{[$-$3.1, +5.0]}
\expandafter\def\csname r@ax-ovl-qasper-mxbai-mid-ci95\endcsname{[$-$3.1, +5.0]}
\expandafter\def\csname r@ax-ovl-qasper-mxbai-mid-d\endcsname{+1.0}
\expandafter\def\csname r@ax-ovl-qasper-mxbai-mid-p\endcsname{--}
\expandafter\def\csname r@ax-ovl-qasper-mxbai-mid-v\endcsname{n.d.}
\expandafter\def\csname r@ax-ovl-qasper-nomic-high\endcsname{+0.3 [$-$3.7, +4.3]}
\expandafter\def\csname r@ax-ovl-qasper-nomic-high-ci\endcsname{[$-$3.7, +4.3]}
\expandafter\def\csname r@ax-ovl-qasper-nomic-high-ci95\endcsname{[$-$3.7, +4.3]}
\expandafter\def\csname r@ax-ovl-qasper-nomic-high-d\endcsname{+0.3}
\expandafter\def\csname r@ax-ovl-qasper-nomic-high-p\endcsname{--}
\expandafter\def\csname r@ax-ovl-qasper-nomic-high-v\endcsname{n.d.}
\expandafter\def\csname r@ax-ovl-qasper-nomic-lmh\endcsname{$-$0.0 [$-$5.8, +6.2]}
\expandafter\def\csname r@ax-ovl-qasper-nomic-lmh-ci\endcsname{[$-$5.8, +6.2]}
\expandafter\def\csname r@ax-ovl-qasper-nomic-lmh-ci95\endcsname{[$-$5.8, +6.2]}
\expandafter\def\csname r@ax-ovl-qasper-nomic-lmh-d\endcsname{$-$0.0}
\expandafter\def\csname r@ax-ovl-qasper-nomic-lmh-p\endcsname{--}
\expandafter\def\csname r@ax-ovl-qasper-nomic-lmh-v\endcsname{n.d.}
\expandafter\def\csname r@ax-ovl-qasper-nomic-low\endcsname{+0.3 [$-$3.8, +4.6]}
\expandafter\def\csname r@ax-ovl-qasper-nomic-low-ci\endcsname{[$-$3.8, +4.6]}
\expandafter\def\csname r@ax-ovl-qasper-nomic-low-ci95\endcsname{[$-$3.8, +4.6]}
\expandafter\def\csname r@ax-ovl-qasper-nomic-low-d\endcsname{+0.3}
\expandafter\def\csname r@ax-ovl-qasper-nomic-low-p\endcsname{--}
\expandafter\def\csname r@ax-ovl-qasper-nomic-low-v\endcsname{n.d.}
\expandafter\def\csname r@ax-ovl-qasper-nomic-mid\endcsname{+2.2 [$-$2.7, +7.2]}
\expandafter\def\csname r@ax-ovl-qasper-nomic-mid-ci\endcsname{[$-$2.7, +7.2]}
\expandafter\def\csname r@ax-ovl-qasper-nomic-mid-ci95\endcsname{[$-$2.7, +7.2]}
\expandafter\def\csname r@ax-ovl-qasper-nomic-mid-d\endcsname{+2.2}
\expandafter\def\csname r@ax-ovl-qasper-nomic-mid-p\endcsname{--}
\expandafter\def\csname r@ax-ovl-qasper-nomic-mid-v\endcsname{n.d.}
\expandafter\def\csname r@ax-ovl-qasper-q3-high\endcsname{+0.1 [$-$3.8, +3.9]}
\expandafter\def\csname r@ax-ovl-qasper-q3-high-ci\endcsname{[$-$3.8, +3.9]}
\expandafter\def\csname r@ax-ovl-qasper-q3-high-ci95\endcsname{[$-$3.8, +3.9]}
\expandafter\def\csname r@ax-ovl-qasper-q3-high-d\endcsname{+0.1}
\expandafter\def\csname r@ax-ovl-qasper-q3-high-p\endcsname{--}
\expandafter\def\csname r@ax-ovl-qasper-q3-high-v\endcsname{n.d.}
\expandafter\def\csname r@ax-ovl-qasper-q3-lmh\endcsname{+4.9 [$-$0.9, +11.0]}
\expandafter\def\csname r@ax-ovl-qasper-q3-lmh-ci\endcsname{[$-$0.9, +11.0]}
\expandafter\def\csname r@ax-ovl-qasper-q3-lmh-ci95\endcsname{[$-$0.9, +11.0]}
\expandafter\def\csname r@ax-ovl-qasper-q3-lmh-d\endcsname{+4.9}
\expandafter\def\csname r@ax-ovl-qasper-q3-lmh-p\endcsname{--}
\expandafter\def\csname r@ax-ovl-qasper-q3-lmh-v\endcsname{n.d.}
\expandafter\def\csname r@ax-ovl-qasper-q3-low\endcsname{+5.0 [+0.8, +9.4]}
\expandafter\def\csname r@ax-ovl-qasper-q3-low-ci\endcsname{[+0.8, +9.4]}
\expandafter\def\csname r@ax-ovl-qasper-q3-low-ci95\endcsname{[+0.8, +9.4]}
\expandafter\def\csname r@ax-ovl-qasper-q3-low-d\endcsname{+5.0}
\expandafter\def\csname r@ax-ovl-qasper-q3-low-p\endcsname{--}
\expandafter\def\csname r@ax-ovl-qasper-q3-low-v\endcsname{diff.}
\expandafter\def\csname r@ax-ovl-qasper-q3-mid\endcsname{$-$1.9 [$-$5.9, +1.9]}
\expandafter\def\csname r@ax-ovl-qasper-q3-mid-ci\endcsname{[$-$5.9, +1.9]}
\expandafter\def\csname r@ax-ovl-qasper-q3-mid-ci95\endcsname{[$-$5.9, +1.9]}
\expandafter\def\csname r@ax-ovl-qasper-q3-mid-d\endcsname{$-$1.9}
\expandafter\def\csname r@ax-ovl-qasper-q3-mid-p\endcsname{--}
\expandafter\def\csname r@ax-ovl-qasper-q3-mid-v\endcsname{n.d.}
\expandafter\def\csname r@ax-ovl-qasper-rr-high\endcsname{+0.7 [$-$2.6, +4.1]}
\expandafter\def\csname r@ax-ovl-qasper-rr-high-ci\endcsname{[$-$2.6, +4.1]}
\expandafter\def\csname r@ax-ovl-qasper-rr-high-ci95\endcsname{[$-$2.6, +4.1]}
\expandafter\def\csname r@ax-ovl-qasper-rr-high-d\endcsname{+0.7}
\expandafter\def\csname r@ax-ovl-qasper-rr-high-p\endcsname{--}
\expandafter\def\csname r@ax-ovl-qasper-rr-high-v\endcsname{n.d.}
\expandafter\def\csname r@ax-ovl-qasper-rr-lmh\endcsname{$-$1.1 [$-$6.4, +3.8]}
\expandafter\def\csname r@ax-ovl-qasper-rr-lmh-ci\endcsname{[$-$6.4, +3.8]}
\expandafter\def\csname r@ax-ovl-qasper-rr-lmh-ci95\endcsname{[$-$6.4, +3.8]}
\expandafter\def\csname r@ax-ovl-qasper-rr-lmh-d\endcsname{$-$1.1}
\expandafter\def\csname r@ax-ovl-qasper-rr-lmh-p\endcsname{--}
\expandafter\def\csname r@ax-ovl-qasper-rr-lmh-v\endcsname{n.d.}
\expandafter\def\csname r@ax-ovl-qasper-rr-low\endcsname{$-$0.4 [$-$4.1, +3.5]}
\expandafter\def\csname r@ax-ovl-qasper-rr-low-ci\endcsname{[$-$4.1, +3.5]}
\expandafter\def\csname r@ax-ovl-qasper-rr-low-ci95\endcsname{[$-$4.1, +3.5]}
\expandafter\def\csname r@ax-ovl-qasper-rr-low-d\endcsname{$-$0.4}
\expandafter\def\csname r@ax-ovl-qasper-rr-low-p\endcsname{--}
\expandafter\def\csname r@ax-ovl-qasper-rr-low-v\endcsname{n.d.}
\expandafter\def\csname r@ax-ovl-qasper-rr-mid\endcsname{+1.1 [$-$2.2, +5.1]}
\expandafter\def\csname r@ax-ovl-qasper-rr-mid-ci\endcsname{[$-$2.2, +5.1]}
\expandafter\def\csname r@ax-ovl-qasper-rr-mid-ci95\endcsname{[$-$2.2, +5.1]}
\expandafter\def\csname r@ax-ovl-qasper-rr-mid-d\endcsname{+1.1}
\expandafter\def\csname r@ax-ovl-qasper-rr-mid-p\endcsname{--}
\expandafter\def\csname r@ax-ovl-qasper-rr-mid-v\endcsname{n.d.}
\expandafter\def\csname r@ax-tg-fs-bm25-c\endcsname{+0.6 [$-$2.6, +4.7]}
\expandafter\def\csname r@ax-tg-fs-bm25-c-ci\endcsname{[$-$2.6, +4.7]}
\expandafter\def\csname r@ax-tg-fs-bm25-c-ci95\endcsname{[$-$2.6, +4.7]}
\expandafter\def\csname r@ax-tg-fs-bm25-c-d\endcsname{+0.6}
\expandafter\def\csname r@ax-tg-fs-bm25-c-p\endcsname{--}
\expandafter\def\csname r@ax-tg-fs-bm25-c-v\endcsname{n.d.}
\expandafter\def\csname r@ax-tg-fs-bm25-high\endcsname{+2.1 [+0.0, +5.4]}
\expandafter\def\csname r@ax-tg-fs-bm25-high-ci\endcsname{[+0.0, +5.4]}
\expandafter\def\csname r@ax-tg-fs-bm25-high-ci95\endcsname{[+0.0, +5.4]}
\expandafter\def\csname r@ax-tg-fs-bm25-high-d\endcsname{+2.1}
\expandafter\def\csname r@ax-tg-fs-bm25-high-p\endcsname{--}
\expandafter\def\csname r@ax-tg-fs-bm25-high-v\endcsname{diff.}
\expandafter\def\csname r@ax-tg-fs-bm25-low\endcsname{+1.6 [$-$0.9, +3.9]}
\expandafter\def\csname r@ax-tg-fs-bm25-low-ci\endcsname{[$-$0.9, +3.9]}
\expandafter\def\csname r@ax-tg-fs-bm25-low-ci95\endcsname{[$-$0.9, +3.9]}
\expandafter\def\csname r@ax-tg-fs-bm25-low-d\endcsname{+1.6}
\expandafter\def\csname r@ax-tg-fs-bm25-low-p\endcsname{--}
\expandafter\def\csname r@ax-tg-fs-bm25-low-v\endcsname{n.d.}
\expandafter\def\csname r@ax-tg-fs-bm25-mid\endcsname{+3.5 [+0.5, +8.2]}
\expandafter\def\csname r@ax-tg-fs-bm25-mid-ci\endcsname{[+0.5, +8.2]}
\expandafter\def\csname r@ax-tg-fs-bm25-mid-ci95\endcsname{[+0.5, +8.2]}
\expandafter\def\csname r@ax-tg-fs-bm25-mid-d\endcsname{+3.5}
\expandafter\def\csname r@ax-tg-fs-bm25-mid-p\endcsname{--}
\expandafter\def\csname r@ax-tg-fs-bm25-mid-v\endcsname{diff.}
\expandafter\def\csname r@ax-tg-fs-gold\endcsname{18.0}
\expandafter\def\csname r@ax-tg-fs-hq3-c\endcsname{$-$3.2 [$-$7.7, +1.2]}
\expandafter\def\csname r@ax-tg-fs-hq3-c-ci\endcsname{[$-$7.7, +1.2]}
\expandafter\def\csname r@ax-tg-fs-hq3-c-ci95\endcsname{[$-$7.7, +1.2]}
\expandafter\def\csname r@ax-tg-fs-hq3-c-d\endcsname{$-$3.2}
\expandafter\def\csname r@ax-tg-fs-hq3-c-p\endcsname{--}
\expandafter\def\csname r@ax-tg-fs-hq3-c-v\endcsname{n.d.}
\expandafter\def\csname r@ax-tg-fs-hq3-high\endcsname{$-$1.9 [$-$6.1, +1.5]}
\expandafter\def\csname r@ax-tg-fs-hq3-high-ci\endcsname{[$-$6.1, +1.5]}
\expandafter\def\csname r@ax-tg-fs-hq3-high-ci95\endcsname{[$-$6.1, +1.5]}
\expandafter\def\csname r@ax-tg-fs-hq3-high-d\endcsname{$-$1.9}
\expandafter\def\csname r@ax-tg-fs-hq3-high-p\endcsname{--}
\expandafter\def\csname r@ax-tg-fs-hq3-high-v\endcsname{n.d.}
\expandafter\def\csname r@ax-tg-fs-hq3-low\endcsname{+1.2 [$-$0.8, +3.5]}
\expandafter\def\csname r@ax-tg-fs-hq3-low-ci\endcsname{[$-$0.8, +3.5]}
\expandafter\def\csname r@ax-tg-fs-hq3-low-ci95\endcsname{[$-$0.8, +3.5]}
\expandafter\def\csname r@ax-tg-fs-hq3-low-d\endcsname{+1.2}
\expandafter\def\csname r@ax-tg-fs-hq3-low-p\endcsname{--}
\expandafter\def\csname r@ax-tg-fs-hq3-low-v\endcsname{n.d.}
\expandafter\def\csname r@ax-tg-fs-hq3-mid\endcsname{+3.8 [+0.3, +7.5]}
\expandafter\def\csname r@ax-tg-fs-hq3-mid-ci\endcsname{[+0.3, +7.5]}
\expandafter\def\csname r@ax-tg-fs-hq3-mid-ci95\endcsname{[+0.3, +7.5]}
\expandafter\def\csname r@ax-tg-fs-hq3-mid-d\endcsname{+3.8}
\expandafter\def\csname r@ax-tg-fs-hq3-mid-p\endcsname{--}
\expandafter\def\csname r@ax-tg-fs-hq3-mid-v\endcsname{diff.}
\expandafter\def\csname r@ax-tg-fs-hyb-c\endcsname{$-$1.1 [$-$6.7, +4.2]}
\expandafter\def\csname r@ax-tg-fs-hyb-c-ci\endcsname{[$-$6.7, +4.2]}
\expandafter\def\csname r@ax-tg-fs-hyb-c-ci95\endcsname{[$-$6.7, +4.2]}
\expandafter\def\csname r@ax-tg-fs-hyb-c-d\endcsname{$-$1.1}
\expandafter\def\csname r@ax-tg-fs-hyb-c-p\endcsname{--}
\expandafter\def\csname r@ax-tg-fs-hyb-c-v\endcsname{n.d.}
\expandafter\def\csname r@ax-tg-fs-hyb-high\endcsname{+0.8 [$-$3.6, +5.2]}
\expandafter\def\csname r@ax-tg-fs-hyb-high-ci\endcsname{[$-$3.6, +5.2]}
\expandafter\def\csname r@ax-tg-fs-hyb-high-ci95\endcsname{[$-$3.6, +5.2]}
\expandafter\def\csname r@ax-tg-fs-hyb-high-d\endcsname{+0.8}
\expandafter\def\csname r@ax-tg-fs-hyb-high-p\endcsname{--}
\expandafter\def\csname r@ax-tg-fs-hyb-high-v\endcsname{n.d.}
\expandafter\def\csname r@ax-tg-fs-hyb-low\endcsname{+1.9 [$-$1.2, +5.3]}
\expandafter\def\csname r@ax-tg-fs-hyb-low-ci\endcsname{[$-$1.2, +5.3]}
\expandafter\def\csname r@ax-tg-fs-hyb-low-ci95\endcsname{[$-$1.2, +5.3]}
\expandafter\def\csname r@ax-tg-fs-hyb-low-d\endcsname{+1.9}
\expandafter\def\csname r@ax-tg-fs-hyb-low-p\endcsname{--}
\expandafter\def\csname r@ax-tg-fs-hyb-low-v\endcsname{n.d.}
\expandafter\def\csname r@ax-tg-fs-hyb-mid\endcsname{+5.5 [+1.8, +9.6]}
\expandafter\def\csname r@ax-tg-fs-hyb-mid-ci\endcsname{[+1.8, +9.6]}
\expandafter\def\csname r@ax-tg-fs-hyb-mid-ci95\endcsname{[+1.8, +9.6]}
\expandafter\def\csname r@ax-tg-fs-hyb-mid-d\endcsname{+5.5}
\expandafter\def\csname r@ax-tg-fs-hyb-mid-p\endcsname{--}
\expandafter\def\csname r@ax-tg-fs-hyb-mid-v\endcsname{diff.}
\expandafter\def\csname r@ax-tg-fs-mxbai-c\endcsname{$-$0.5 [$-$6.2, +4.8]}
\expandafter\def\csname r@ax-tg-fs-mxbai-c-ci\endcsname{[$-$6.2, +4.8]}
\expandafter\def\csname r@ax-tg-fs-mxbai-c-ci95\endcsname{[$-$6.2, +4.8]}
\expandafter\def\csname r@ax-tg-fs-mxbai-c-d\endcsname{$-$0.5}
\expandafter\def\csname r@ax-tg-fs-mxbai-c-p\endcsname{--}
\expandafter\def\csname r@ax-tg-fs-mxbai-c-v\endcsname{n.d.}
\expandafter\def\csname r@ax-tg-fs-mxbai-high\endcsname{$-$1.3 [$-$5.5, +3.1]}
\expandafter\def\csname r@ax-tg-fs-mxbai-high-ci\endcsname{[$-$5.5, +3.1]}
\expandafter\def\csname r@ax-tg-fs-mxbai-high-ci95\endcsname{[$-$5.5, +3.1]}
\expandafter\def\csname r@ax-tg-fs-mxbai-high-d\endcsname{$-$1.3}
\expandafter\def\csname r@ax-tg-fs-mxbai-high-p\endcsname{--}
\expandafter\def\csname r@ax-tg-fs-mxbai-high-v\endcsname{n.d.}
\expandafter\def\csname r@ax-tg-fs-mxbai-low\endcsname{$-$0.8 [$-$3.8, +2.7]}
\expandafter\def\csname r@ax-tg-fs-mxbai-low-ci\endcsname{[$-$3.8, +2.7]}
\expandafter\def\csname r@ax-tg-fs-mxbai-low-ci95\endcsname{[$-$3.8, +2.7]}
\expandafter\def\csname r@ax-tg-fs-mxbai-low-d\endcsname{$-$0.8}
\expandafter\def\csname r@ax-tg-fs-mxbai-low-p\endcsname{--}
\expandafter\def\csname r@ax-tg-fs-mxbai-low-v\endcsname{n.d.}
\expandafter\def\csname r@ax-tg-fs-mxbai-mid\endcsname{+2.2 [$-$1.7, +6.3]}
\expandafter\def\csname r@ax-tg-fs-mxbai-mid-ci\endcsname{[$-$1.7, +6.3]}
\expandafter\def\csname r@ax-tg-fs-mxbai-mid-ci95\endcsname{[$-$1.7, +6.3]}
\expandafter\def\csname r@ax-tg-fs-mxbai-mid-d\endcsname{+2.2}
\expandafter\def\csname r@ax-tg-fs-mxbai-mid-p\endcsname{--}
\expandafter\def\csname r@ax-tg-fs-mxbai-mid-v\endcsname{n.d.}
\expandafter\def\csname r@ax-tg-fs-nomic-c\endcsname{$-$0.2 [$-$5.7, +5.3]}
\expandafter\def\csname r@ax-tg-fs-nomic-c-ci\endcsname{[$-$5.7, +5.3]}
\expandafter\def\csname r@ax-tg-fs-nomic-c-ci95\endcsname{[$-$5.7, +5.3]}
\expandafter\def\csname r@ax-tg-fs-nomic-c-d\endcsname{$-$0.2}
\expandafter\def\csname r@ax-tg-fs-nomic-c-p\endcsname{--}
\expandafter\def\csname r@ax-tg-fs-nomic-c-v\endcsname{n.d.}
\expandafter\def\csname r@ax-tg-fs-nomic-high\endcsname{+1.9 [$-$2.6, +6.6]}
\expandafter\def\csname r@ax-tg-fs-nomic-high-ci\endcsname{[$-$2.6, +6.6]}
\expandafter\def\csname r@ax-tg-fs-nomic-high-ci95\endcsname{[$-$2.6, +6.6]}
\expandafter\def\csname r@ax-tg-fs-nomic-high-d\endcsname{+1.9}
\expandafter\def\csname r@ax-tg-fs-nomic-high-p\endcsname{--}
\expandafter\def\csname r@ax-tg-fs-nomic-high-v\endcsname{n.d.}
\expandafter\def\csname r@ax-tg-fs-nomic-low\endcsname{+2.1 [$-$0.7, +5.3]}
\expandafter\def\csname r@ax-tg-fs-nomic-low-ci\endcsname{[$-$0.7, +5.3]}
\expandafter\def\csname r@ax-tg-fs-nomic-low-ci95\endcsname{[$-$0.7, +5.3]}
\expandafter\def\csname r@ax-tg-fs-nomic-low-d\endcsname{+2.1}
\expandafter\def\csname r@ax-tg-fs-nomic-low-p\endcsname{--}
\expandafter\def\csname r@ax-tg-fs-nomic-low-v\endcsname{n.d.}
\expandafter\def\csname r@ax-tg-fs-nomic-mid\endcsname{+3.9 [$-$0.5, +8.9]}
\expandafter\def\csname r@ax-tg-fs-nomic-mid-ci\endcsname{[$-$0.5, +8.9]}
\expandafter\def\csname r@ax-tg-fs-nomic-mid-ci95\endcsname{[$-$0.5, +8.9]}
\expandafter\def\csname r@ax-tg-fs-nomic-mid-d\endcsname{+3.9}
\expandafter\def\csname r@ax-tg-fs-nomic-mid-p\endcsname{--}
\expandafter\def\csname r@ax-tg-fs-nomic-mid-v\endcsname{n.d.}
\expandafter\def\csname r@ax-tg-fs-other\endcsname{2.1}
\expandafter\def\csname r@ax-tg-fs-q3-c\endcsname{$-$1.7 [$-$5.5, +2.5]}
\expandafter\def\csname r@ax-tg-fs-q3-c-ci\endcsname{[$-$5.5, +2.5]}
\expandafter\def\csname r@ax-tg-fs-q3-c-ci95\endcsname{[$-$5.5, +2.5]}
\expandafter\def\csname r@ax-tg-fs-q3-c-d\endcsname{$-$1.7}
\expandafter\def\csname r@ax-tg-fs-q3-c-p\endcsname{--}
\expandafter\def\csname r@ax-tg-fs-q3-c-v\endcsname{n.d.}
\expandafter\def\csname r@ax-tg-fs-q3-high\endcsname{$-$1.1 [$-$4.3, +2.5]}
\expandafter\def\csname r@ax-tg-fs-q3-high-ci\endcsname{[$-$4.3, +2.5]}
\expandafter\def\csname r@ax-tg-fs-q3-high-ci95\endcsname{[$-$4.3, +2.5]}
\expandafter\def\csname r@ax-tg-fs-q3-high-d\endcsname{$-$1.1}
\expandafter\def\csname r@ax-tg-fs-q3-high-p\endcsname{--}
\expandafter\def\csname r@ax-tg-fs-q3-high-v\endcsname{n.d.}
\expandafter\def\csname r@ax-tg-fs-q3-low\endcsname{+0.6 [$-$1.5, +2.5]}
\expandafter\def\csname r@ax-tg-fs-q3-low-ci\endcsname{[$-$1.5, +2.5]}
\expandafter\def\csname r@ax-tg-fs-q3-low-ci95\endcsname{[$-$1.5, +2.5]}
\expandafter\def\csname r@ax-tg-fs-q3-low-d\endcsname{+0.6}
\expandafter\def\csname r@ax-tg-fs-q3-low-p\endcsname{--}
\expandafter\def\csname r@ax-tg-fs-q3-low-v\endcsname{n.d.}
\expandafter\def\csname r@ax-tg-fs-q3-mid\endcsname{+1.3 [$-$1.7, +4.6]}
\expandafter\def\csname r@ax-tg-fs-q3-mid-ci\endcsname{[$-$1.7, +4.6]}
\expandafter\def\csname r@ax-tg-fs-q3-mid-ci95\endcsname{[$-$1.7, +4.6]}
\expandafter\def\csname r@ax-tg-fs-q3-mid-d\endcsname{+1.3}
\expandafter\def\csname r@ax-tg-fs-q3-mid-p\endcsname{--}
\expandafter\def\csname r@ax-tg-fs-q3-mid-v\endcsname{n.d.}
\expandafter\def\csname r@ax-tg-fs-rr-c\endcsname{+2.3 [$-$3.0, +7.4]}
\expandafter\def\csname r@ax-tg-fs-rr-c-ci\endcsname{[$-$3.0, +7.4]}
\expandafter\def\csname r@ax-tg-fs-rr-c-ci95\endcsname{[$-$3.0, +7.4]}
\expandafter\def\csname r@ax-tg-fs-rr-c-d\endcsname{+2.3}
\expandafter\def\csname r@ax-tg-fs-rr-c-p\endcsname{--}
\expandafter\def\csname r@ax-tg-fs-rr-c-v\endcsname{n.d.}
\expandafter\def\csname r@ax-tg-fs-rr-high\endcsname{+1.0 [$-$3.1, +5.2]}
\expandafter\def\csname r@ax-tg-fs-rr-high-ci\endcsname{[$-$3.1, +5.2]}
\expandafter\def\csname r@ax-tg-fs-rr-high-ci95\endcsname{[$-$3.1, +5.2]}
\expandafter\def\csname r@ax-tg-fs-rr-high-d\endcsname{+1.0}
\expandafter\def\csname r@ax-tg-fs-rr-high-p\endcsname{--}
\expandafter\def\csname r@ax-tg-fs-rr-high-v\endcsname{n.d.}
\expandafter\def\csname r@ax-tg-fs-rr-low\endcsname{$-$1.2 [$-$4.0, +2.0]}
\expandafter\def\csname r@ax-tg-fs-rr-low-ci\endcsname{[$-$4.0, +2.0]}
\expandafter\def\csname r@ax-tg-fs-rr-low-ci95\endcsname{[$-$4.0, +2.0]}
\expandafter\def\csname r@ax-tg-fs-rr-low-d\endcsname{$-$1.2}
\expandafter\def\csname r@ax-tg-fs-rr-low-p\endcsname{--}
\expandafter\def\csname r@ax-tg-fs-rr-low-v\endcsname{n.d.}
\expandafter\def\csname r@ax-tg-fs-rr-mid\endcsname{+2.6 [$-$1.5, +7.0]}
\expandafter\def\csname r@ax-tg-fs-rr-mid-ci\endcsname{[$-$1.5, +7.0]}
\expandafter\def\csname r@ax-tg-fs-rr-mid-ci95\endcsname{[$-$1.5, +7.0]}
\expandafter\def\csname r@ax-tg-fs-rr-mid-d\endcsname{+2.6}
\expandafter\def\csname r@ax-tg-fs-rr-mid-p\endcsname{--}
\expandafter\def\csname r@ax-tg-fs-rr-mid-v\endcsname{n.d.}
\expandafter\def\csname r@ax-tg-qasper-bm25-c\endcsname{+14.7 [+9.9, +19.6]}
\expandafter\def\csname r@ax-tg-qasper-bm25-c-ci\endcsname{[+9.9, +19.6]}
\expandafter\def\csname r@ax-tg-qasper-bm25-c-ci95\endcsname{[+9.9, +19.6]}
\expandafter\def\csname r@ax-tg-qasper-bm25-c-d\endcsname{+14.7}
\expandafter\def\csname r@ax-tg-qasper-bm25-c-p\endcsname{--}
\expandafter\def\csname r@ax-tg-qasper-bm25-c-v\endcsname{diff.}
\expandafter\def\csname r@ax-tg-qasper-bm25-high\endcsname{+14.6 [+11.1, +18.5]}
\expandafter\def\csname r@ax-tg-qasper-bm25-high-ci\endcsname{[+11.1, +18.5]}
\expandafter\def\csname r@ax-tg-qasper-bm25-high-ci95\endcsname{[+11.1, +18.5]}
\expandafter\def\csname r@ax-tg-qasper-bm25-high-d\endcsname{+14.6}
\expandafter\def\csname r@ax-tg-qasper-bm25-high-p\endcsname{--}
\expandafter\def\csname r@ax-tg-qasper-bm25-high-v\endcsname{diff.}
\expandafter\def\csname r@ax-tg-qasper-bm25-low\endcsname{$-$0.1 [$-$3.2, +3.0]}
\expandafter\def\csname r@ax-tg-qasper-bm25-low-ci\endcsname{[$-$3.2, +3.0]}
\expandafter\def\csname r@ax-tg-qasper-bm25-low-ci95\endcsname{[$-$3.2, +3.0]}
\expandafter\def\csname r@ax-tg-qasper-bm25-low-d\endcsname{$-$0.1}
\expandafter\def\csname r@ax-tg-qasper-bm25-low-p\endcsname{--}
\expandafter\def\csname r@ax-tg-qasper-bm25-low-v\endcsname{n.d.}
\expandafter\def\csname r@ax-tg-qasper-bm25-mid\endcsname{+11.6 [+7.6, +16.0]}
\expandafter\def\csname r@ax-tg-qasper-bm25-mid-ci\endcsname{[+7.6, +16.0]}
\expandafter\def\csname r@ax-tg-qasper-bm25-mid-ci95\endcsname{[+7.6, +16.0]}
\expandafter\def\csname r@ax-tg-qasper-bm25-mid-d\endcsname{+11.6}
\expandafter\def\csname r@ax-tg-qasper-bm25-mid-p\endcsname{--}
\expandafter\def\csname r@ax-tg-qasper-bm25-mid-v\endcsname{diff.}
\expandafter\def\csname r@ax-tg-qasper-gold\endcsname{1.6}
\expandafter\def\csname r@ax-tg-qasper-hq3-c\endcsname{+9.8 [+4.5, +14.9]}
\expandafter\def\csname r@ax-tg-qasper-hq3-c-ci\endcsname{[+4.5, +14.9]}
\expandafter\def\csname r@ax-tg-qasper-hq3-c-ci95\endcsname{[+4.5, +14.9]}
\expandafter\def\csname r@ax-tg-qasper-hq3-c-d\endcsname{+9.8}
\expandafter\def\csname r@ax-tg-qasper-hq3-c-p\endcsname{--}
\expandafter\def\csname r@ax-tg-qasper-hq3-c-v\endcsname{diff.}
\expandafter\def\csname r@ax-tg-qasper-hq3-high\endcsname{+9.1 [+6.0, +12.3]}
\expandafter\def\csname r@ax-tg-qasper-hq3-high-ci\endcsname{[+6.0, +12.3]}
\expandafter\def\csname r@ax-tg-qasper-hq3-high-ci95\endcsname{[+6.0, +12.3]}
\expandafter\def\csname r@ax-tg-qasper-hq3-high-d\endcsname{+9.1}
\expandafter\def\csname r@ax-tg-qasper-hq3-high-p\endcsname{--}
\expandafter\def\csname r@ax-tg-qasper-hq3-high-v\endcsname{diff.}
\expandafter\def\csname r@ax-tg-qasper-hq3-low\endcsname{$-$0.7 [$-$4.7, +3.4]}
\expandafter\def\csname r@ax-tg-qasper-hq3-low-ci\endcsname{[$-$4.7, +3.4]}
\expandafter\def\csname r@ax-tg-qasper-hq3-low-ci95\endcsname{[$-$4.7, +3.4]}
\expandafter\def\csname r@ax-tg-qasper-hq3-low-d\endcsname{$-$0.7}
\expandafter\def\csname r@ax-tg-qasper-hq3-low-p\endcsname{--}
\expandafter\def\csname r@ax-tg-qasper-hq3-low-v\endcsname{n.d.}
\expandafter\def\csname r@ax-tg-qasper-hq3-mid\endcsname{+5.4 [+0.3, +10.1]}
\expandafter\def\csname r@ax-tg-qasper-hq3-mid-ci\endcsname{[+0.3, +10.1]}
\expandafter\def\csname r@ax-tg-qasper-hq3-mid-ci95\endcsname{[+0.3, +10.1]}
\expandafter\def\csname r@ax-tg-qasper-hq3-mid-d\endcsname{+5.4}
\expandafter\def\csname r@ax-tg-qasper-hq3-mid-p\endcsname{--}
\expandafter\def\csname r@ax-tg-qasper-hq3-mid-v\endcsname{diff.}
\expandafter\def\csname r@ax-tg-qasper-hyb-c\endcsname{+7.7 [+2.6, +13.2]}
\expandafter\def\csname r@ax-tg-qasper-hyb-c-ci\endcsname{[+2.6, +13.2]}
\expandafter\def\csname r@ax-tg-qasper-hyb-c-ci95\endcsname{[+2.6, +13.2]}
\expandafter\def\csname r@ax-tg-qasper-hyb-c-d\endcsname{+7.7}
\expandafter\def\csname r@ax-tg-qasper-hyb-c-p\endcsname{--}
\expandafter\def\csname r@ax-tg-qasper-hyb-c-v\endcsname{diff.}
\expandafter\def\csname r@ax-tg-qasper-hyb-high\endcsname{+8.6 [+4.9, +12.6]}
\expandafter\def\csname r@ax-tg-qasper-hyb-high-ci\endcsname{[+4.9, +12.6]}
\expandafter\def\csname r@ax-tg-qasper-hyb-high-ci95\endcsname{[+4.9, +12.6]}
\expandafter\def\csname r@ax-tg-qasper-hyb-high-d\endcsname{+8.6}
\expandafter\def\csname r@ax-tg-qasper-hyb-high-p\endcsname{--}
\expandafter\def\csname r@ax-tg-qasper-hyb-high-v\endcsname{diff.}
\expandafter\def\csname r@ax-tg-qasper-hyb-low\endcsname{+0.9 [$-$3.3, +4.7]}
\expandafter\def\csname r@ax-tg-qasper-hyb-low-ci\endcsname{[$-$3.3, +4.7]}
\expandafter\def\csname r@ax-tg-qasper-hyb-low-ci95\endcsname{[$-$3.3, +4.7]}
\expandafter\def\csname r@ax-tg-qasper-hyb-low-d\endcsname{+0.9}
\expandafter\def\csname r@ax-tg-qasper-hyb-low-p\endcsname{--}
\expandafter\def\csname r@ax-tg-qasper-hyb-low-v\endcsname{n.d.}
\expandafter\def\csname r@ax-tg-qasper-hyb-mid\endcsname{+7.0 [+2.1, +12.1]}
\expandafter\def\csname r@ax-tg-qasper-hyb-mid-ci\endcsname{[+2.1, +12.1]}
\expandafter\def\csname r@ax-tg-qasper-hyb-mid-ci95\endcsname{[+2.1, +12.1]}
\expandafter\def\csname r@ax-tg-qasper-hyb-mid-d\endcsname{+7.0}
\expandafter\def\csname r@ax-tg-qasper-hyb-mid-p\endcsname{--}
\expandafter\def\csname r@ax-tg-qasper-hyb-mid-v\endcsname{diff.}
\expandafter\def\csname r@ax-tg-qasper-mxbai-c\endcsname{+12.3 [+6.9, +17.9]}
\expandafter\def\csname r@ax-tg-qasper-mxbai-c-ci\endcsname{[+6.9, +17.9]}
\expandafter\def\csname r@ax-tg-qasper-mxbai-c-ci95\endcsname{[+6.9, +17.9]}
\expandafter\def\csname r@ax-tg-qasper-mxbai-c-d\endcsname{+12.3}
\expandafter\def\csname r@ax-tg-qasper-mxbai-c-p\endcsname{--}
\expandafter\def\csname r@ax-tg-qasper-mxbai-c-v\endcsname{diff.}
\expandafter\def\csname r@ax-tg-qasper-mxbai-high\endcsname{+5.7 [+2.3, +9.3]}
\expandafter\def\csname r@ax-tg-qasper-mxbai-high-ci\endcsname{[+2.3, +9.3]}
\expandafter\def\csname r@ax-tg-qasper-mxbai-high-ci95\endcsname{[+2.3, +9.3]}
\expandafter\def\csname r@ax-tg-qasper-mxbai-high-d\endcsname{+5.7}
\expandafter\def\csname r@ax-tg-qasper-mxbai-high-p\endcsname{--}
\expandafter\def\csname r@ax-tg-qasper-mxbai-high-v\endcsname{diff.}
\expandafter\def\csname r@ax-tg-qasper-mxbai-low\endcsname{$-$6.6 [$-$10.8, $-$2.3]}
\expandafter\def\csname r@ax-tg-qasper-mxbai-low-ci\endcsname{[$-$10.8, $-$2.3]}
\expandafter\def\csname r@ax-tg-qasper-mxbai-low-ci95\endcsname{[$-$10.8, $-$2.3]}
\expandafter\def\csname r@ax-tg-qasper-mxbai-low-d\endcsname{$-$6.6}
\expandafter\def\csname r@ax-tg-qasper-mxbai-low-p\endcsname{--}
\expandafter\def\csname r@ax-tg-qasper-mxbai-low-v\endcsname{diff.}
\expandafter\def\csname r@ax-tg-qasper-mxbai-mid\endcsname{+3.0 [$-$1.1, +7.3]}
\expandafter\def\csname r@ax-tg-qasper-mxbai-mid-ci\endcsname{[$-$1.1, +7.3]}
\expandafter\def\csname r@ax-tg-qasper-mxbai-mid-ci95\endcsname{[$-$1.1, +7.3]}
\expandafter\def\csname r@ax-tg-qasper-mxbai-mid-d\endcsname{+3.0}
\expandafter\def\csname r@ax-tg-qasper-mxbai-mid-p\endcsname{--}
\expandafter\def\csname r@ax-tg-qasper-mxbai-mid-v\endcsname{n.d.}
\expandafter\def\csname r@ax-tg-qasper-nomic-c\endcsname{+7.8 [+1.5, +14.0]}
\expandafter\def\csname r@ax-tg-qasper-nomic-c-ci\endcsname{[+1.5, +14.0]}
\expandafter\def\csname r@ax-tg-qasper-nomic-c-ci95\endcsname{[+1.5, +14.0]}
\expandafter\def\csname r@ax-tg-qasper-nomic-c-d\endcsname{+7.8}
\expandafter\def\csname r@ax-tg-qasper-nomic-c-p\endcsname{--}
\expandafter\def\csname r@ax-tg-qasper-nomic-c-v\endcsname{diff.}
\expandafter\def\csname r@ax-tg-qasper-nomic-high\endcsname{+5.6 [+2.3, +9.0]}
\expandafter\def\csname r@ax-tg-qasper-nomic-high-ci\endcsname{[+2.3, +9.0]}
\expandafter\def\csname r@ax-tg-qasper-nomic-high-ci95\endcsname{[+2.3, +9.0]}
\expandafter\def\csname r@ax-tg-qasper-nomic-high-d\endcsname{+5.6}
\expandafter\def\csname r@ax-tg-qasper-nomic-high-p\endcsname{--}
\expandafter\def\csname r@ax-tg-qasper-nomic-high-v\endcsname{diff.}
\expandafter\def\csname r@ax-tg-qasper-nomic-low\endcsname{$-$2.3 [$-$7.5, +2.6]}
\expandafter\def\csname r@ax-tg-qasper-nomic-low-ci\endcsname{[$-$7.5, +2.6]}
\expandafter\def\csname r@ax-tg-qasper-nomic-low-ci95\endcsname{[$-$7.5, +2.6]}
\expandafter\def\csname r@ax-tg-qasper-nomic-low-d\endcsname{$-$2.3}
\expandafter\def\csname r@ax-tg-qasper-nomic-low-p\endcsname{--}
\expandafter\def\csname r@ax-tg-qasper-nomic-low-v\endcsname{n.d.}
\expandafter\def\csname r@ax-tg-qasper-nomic-mid\endcsname{$-$0.7 [$-$5.4, +4.0]}
\expandafter\def\csname r@ax-tg-qasper-nomic-mid-ci\endcsname{[$-$5.4, +4.0]}
\expandafter\def\csname r@ax-tg-qasper-nomic-mid-ci95\endcsname{[$-$5.4, +4.0]}
\expandafter\def\csname r@ax-tg-qasper-nomic-mid-d\endcsname{$-$0.7}
\expandafter\def\csname r@ax-tg-qasper-nomic-mid-p\endcsname{--}
\expandafter\def\csname r@ax-tg-qasper-nomic-mid-v\endcsname{n.d.}
\expandafter\def\csname r@ax-tg-qasper-other\endcsname{0.7}
\expandafter\def\csname r@ax-tg-qasper-q3-c\endcsname{+6.2 [+0.6, +11.9]}
\expandafter\def\csname r@ax-tg-qasper-q3-c-ci\endcsname{[+0.6, +11.9]}
\expandafter\def\csname r@ax-tg-qasper-q3-c-ci95\endcsname{[+0.6, +11.9]}
\expandafter\def\csname r@ax-tg-qasper-q3-c-d\endcsname{+6.2}
\expandafter\def\csname r@ax-tg-qasper-q3-c-p\endcsname{--}
\expandafter\def\csname r@ax-tg-qasper-q3-c-v\endcsname{diff.}
\expandafter\def\csname r@ax-tg-qasper-q3-high\endcsname{+4.2 [+1.2, +7.3]}
\expandafter\def\csname r@ax-tg-qasper-q3-high-ci\endcsname{[+1.2, +7.3]}
\expandafter\def\csname r@ax-tg-qasper-q3-high-ci95\endcsname{[+1.2, +7.3]}
\expandafter\def\csname r@ax-tg-qasper-q3-high-d\endcsname{+4.2}
\expandafter\def\csname r@ax-tg-qasper-q3-high-p\endcsname{--}
\expandafter\def\csname r@ax-tg-qasper-q3-high-v\endcsname{diff.}
\expandafter\def\csname r@ax-tg-qasper-q3-low\endcsname{$-$2.0 [$-$6.9, +2.8]}
\expandafter\def\csname r@ax-tg-qasper-q3-low-ci\endcsname{[$-$6.9, +2.8]}
\expandafter\def\csname r@ax-tg-qasper-q3-low-ci95\endcsname{[$-$6.9, +2.8]}
\expandafter\def\csname r@ax-tg-qasper-q3-low-d\endcsname{$-$2.0}
\expandafter\def\csname r@ax-tg-qasper-q3-low-p\endcsname{--}
\expandafter\def\csname r@ax-tg-qasper-q3-low-v\endcsname{n.d.}
\expandafter\def\csname r@ax-tg-qasper-q3-mid\endcsname{+2.3 [$-$2.0, +6.5]}
\expandafter\def\csname r@ax-tg-qasper-q3-mid-ci\endcsname{[$-$2.0, +6.5]}
\expandafter\def\csname r@ax-tg-qasper-q3-mid-ci95\endcsname{[$-$2.0, +6.5]}
\expandafter\def\csname r@ax-tg-qasper-q3-mid-d\endcsname{+2.3}
\expandafter\def\csname r@ax-tg-qasper-q3-mid-p\endcsname{--}
\expandafter\def\csname r@ax-tg-qasper-q3-mid-v\endcsname{n.d.}
\expandafter\def\csname r@ax-tg-qasper-rr-c\endcsname{+6.6 [+1.4, +12.2]}
\expandafter\def\csname r@ax-tg-qasper-rr-c-ci\endcsname{[+1.4, +12.2]}
\expandafter\def\csname r@ax-tg-qasper-rr-c-ci95\endcsname{[+1.4, +12.2]}
\expandafter\def\csname r@ax-tg-qasper-rr-c-d\endcsname{+6.6}
\expandafter\def\csname r@ax-tg-qasper-rr-c-p\endcsname{--}
\expandafter\def\csname r@ax-tg-qasper-rr-c-v\endcsname{diff.}
\expandafter\def\csname r@ax-tg-qasper-rr-high\endcsname{+1.8 [$-$1.8, +5.4]}
\expandafter\def\csname r@ax-tg-qasper-rr-high-ci\endcsname{[$-$1.8, +5.4]}
\expandafter\def\csname r@ax-tg-qasper-rr-high-ci95\endcsname{[$-$1.8, +5.4]}
\expandafter\def\csname r@ax-tg-qasper-rr-high-d\endcsname{+1.8}
\expandafter\def\csname r@ax-tg-qasper-rr-high-p\endcsname{--}
\expandafter\def\csname r@ax-tg-qasper-rr-high-v\endcsname{n.d.}
\expandafter\def\csname r@ax-tg-qasper-rr-low\endcsname{$-$4.8 [$-$8.8, $-$1.0]}
\expandafter\def\csname r@ax-tg-qasper-rr-low-ci\endcsname{[$-$8.8, $-$1.0]}
\expandafter\def\csname r@ax-tg-qasper-rr-low-ci95\endcsname{[$-$8.8, $-$1.0]}
\expandafter\def\csname r@ax-tg-qasper-rr-low-d\endcsname{$-$4.8}
\expandafter\def\csname r@ax-tg-qasper-rr-low-p\endcsname{--}
\expandafter\def\csname r@ax-tg-qasper-rr-low-v\endcsname{diff.}
\expandafter\def\csname r@ax-tg-qasper-rr-mid\endcsname{+4.2 [+0.9, +7.4]}
\expandafter\def\csname r@ax-tg-qasper-rr-mid-ci\endcsname{[+0.9, +7.4]}
\expandafter\def\csname r@ax-tg-qasper-rr-mid-ci95\endcsname{[+0.9, +7.4]}
\expandafter\def\csname r@ax-tg-qasper-rr-mid-d\endcsname{+4.2}
\expandafter\def\csname r@ax-tg-qasper-rr-mid-p\endcsname{--}
\expandafter\def\csname r@ax-tg-qasper-rr-mid-v\endcsname{diff.}
\expandafter\def\csname r@ax-tok-fs-CR\endcsname{8,860}
\expandafter\def\csname r@ax-tok-fs-E\endcsname{1,188}
\expandafter\def\csname r@ax-tok-fs-E-strong\endcsname{1,486}
\expandafter\def\csname r@ax-tok-qasper-CR\endcsname{5,945}
\expandafter\def\csname r@ax-tok-qasper-CR-strong\endcsname{6,381}
\expandafter\def\csname r@ax-tok-qasper-E\endcsname{1,205}
\expandafter\def\csname r@ax-tok-qasper-E-strong\endcsname{1,558}
\expandafter\def\csname r@ax-wtl-fs-bm25-loss\endcsname{33.2}
\expandafter\def\csname r@ax-wtl-fs-bm25-tie\endcsname{24.3}
\expandafter\def\csname r@ax-wtl-fs-bm25-win\endcsname{42.6}
\expandafter\def\csname r@ax-wtl-fs-hq3-loss\endcsname{35.7}
\expandafter\def\csname r@ax-wtl-fs-hq3-tie\endcsname{17.4}
\expandafter\def\csname r@ax-wtl-fs-hq3-win\endcsname{46.8}
\expandafter\def\csname r@ax-wtl-fs-hyb-loss\endcsname{37.9}
\expandafter\def\csname r@ax-wtl-fs-hyb-tie\endcsname{9.4}
\expandafter\def\csname r@ax-wtl-fs-hyb-win\endcsname{52.8}
\expandafter\def\csname r@ax-wtl-fs-jina-loss\endcsname{48.1}
\expandafter\def\csname r@ax-wtl-fs-jina-tie\endcsname{9.4}
\expandafter\def\csname r@ax-wtl-fs-jina-win\endcsname{42.6}
\expandafter\def\csname r@ax-wtl-fs-mxbai-loss\endcsname{41.3}
\expandafter\def\csname r@ax-wtl-fs-mxbai-tie\endcsname{11.9}
\expandafter\def\csname r@ax-wtl-fs-mxbai-win\endcsname{46.8}
\expandafter\def\csname r@ax-wtl-fs-nomic-loss\endcsname{44.3}
\expandafter\def\csname r@ax-wtl-fs-nomic-tie\endcsname{8.1}
\expandafter\def\csname r@ax-wtl-fs-nomic-win\endcsname{47.7}
\expandafter\def\csname r@ax-wtl-fs-q3-loss\endcsname{44.3}
\expandafter\def\csname r@ax-wtl-fs-q3-tie\endcsname{9.4}
\expandafter\def\csname r@ax-wtl-fs-q3-win\endcsname{46.4}
\expandafter\def\csname r@ax-wtl-fs-rr-loss\endcsname{44.3}
\expandafter\def\csname r@ax-wtl-fs-rr-tie\endcsname{9.4}
\expandafter\def\csname r@ax-wtl-fs-rr-win\endcsname{46.4}
\expandafter\def\csname r@ax-wtl-qasper-bm25-loss\endcsname{5.7}
\expandafter\def\csname r@ax-wtl-qasper-bm25-tie\endcsname{75.8}
\expandafter\def\csname r@ax-wtl-qasper-bm25-win\endcsname{18.5}
\expandafter\def\csname r@ax-wtl-qasper-hq3-loss\endcsname{10.2}
\expandafter\def\csname r@ax-wtl-qasper-hq3-tie\endcsname{73.8}
\expandafter\def\csname r@ax-wtl-qasper-hq3-win\endcsname{16.0}
\expandafter\def\csname r@ax-wtl-qasper-hyb-loss\endcsname{11.1}
\expandafter\def\csname r@ax-wtl-qasper-hyb-tie\endcsname{71.2}
\expandafter\def\csname r@ax-wtl-qasper-hyb-win\endcsname{17.7}
\expandafter\def\csname r@ax-wtl-qasper-jina-loss\endcsname{14.6}
\expandafter\def\csname r@ax-wtl-qasper-jina-tie\endcsname{68.5}
\expandafter\def\csname r@ax-wtl-qasper-jina-win\endcsname{16.9}
\expandafter\def\csname r@ax-wtl-qasper-mxbai-loss\endcsname{13.2}
\expandafter\def\csname r@ax-wtl-qasper-mxbai-tie\endcsname{72.7}
\expandafter\def\csname r@ax-wtl-qasper-mxbai-win\endcsname{14.1}
\expandafter\def\csname r@ax-wtl-qasper-nomic-loss\endcsname{14.3}
\expandafter\def\csname r@ax-wtl-qasper-nomic-tie\endcsname{70.2}
\expandafter\def\csname r@ax-wtl-qasper-nomic-win\endcsname{15.5}
\expandafter\def\csname r@ax-wtl-qasper-q3-loss\endcsname{11.1}
\expandafter\def\csname r@ax-wtl-qasper-q3-tie\endcsname{75.5}
\expandafter\def\csname r@ax-wtl-qasper-q3-win\endcsname{13.4}
\expandafter\def\csname r@ax-wtl-qasper-rr-loss\endcsname{12.3}
\expandafter\def\csname r@ax-wtl-qasper-rr-tie\endcsname{76.1}
\expandafter\def\csname r@ax-wtl-qasper-rr-win\endcsname{11.6}
\expandafter\def\csname r@base-M-TP-fs\endcsname{+4.4 [+2.2, +6.8]}
\expandafter\def\csname r@base-M-TP-fs-ci\endcsname{[+2.2, +6.8]}
\expandafter\def\csname r@base-M-TP-fs-ci95\endcsname{[+2.2, +6.8]}
\expandafter\def\csname r@base-M-TP-fs-d\endcsname{+4.4}
\expandafter\def\csname r@base-M-TP-fs-p\endcsname{--}
\expandafter\def\csname r@base-M-TP-fs-v\endcsname{diff.}
\expandafter\def\csname r@base-M-TP-qasper\endcsname{$-$5.6 [$-$8.0, $-$3.4]}
\expandafter\def\csname r@base-M-TP-qasper-ci\endcsname{[$-$8.0, $-$3.4]}
\expandafter\def\csname r@base-M-TP-qasper-ci95\endcsname{[$-$8.0, $-$3.4]}
\expandafter\def\csname r@base-M-TP-qasper-d\endcsname{$-$5.6}
\expandafter\def\csname r@base-M-TP-qasper-p\endcsname{--}
\expandafter\def\csname r@base-M-TP-qasper-v\endcsname{diff.}
\expandafter\def\csname r@base-M-fs\endcsname{+0.3 [$-$1.0, +1.6]}
\expandafter\def\csname r@base-M-fs-ci\endcsname{[$-$1.0, +1.6]}
\expandafter\def\csname r@base-M-fs-ci95\endcsname{[$-$1.0, +1.6]}
\expandafter\def\csname r@base-M-fs-d\endcsname{+0.3}
\expandafter\def\csname r@base-M-fs-p\endcsname{0.001}
\expandafter\def\csname r@base-M-fs-pperm\endcsname{1.000}
\expandafter\def\csname r@base-M-fs-v\endcsname{equiv.}
\expandafter\def\csname r@base-M-noRK-fs\endcsname{+0.5 [$-$0.2, +1.3]}
\expandafter\def\csname r@base-M-noRK-fs-ci\endcsname{[$-$0.2, +1.3]}
\expandafter\def\csname r@base-M-noRK-fs-ci95\endcsname{[$-$0.2, +1.3]}
\expandafter\def\csname r@base-M-noRK-fs-d\endcsname{+0.5}
\expandafter\def\csname r@base-M-noRK-fs-p\endcsname{--}
\expandafter\def\csname r@base-M-noRK-fs-v\endcsname{n.d.}
\expandafter\def\csname r@base-M-noRK-qasper\endcsname{$-$0.9 [$-$2.1, +0.1]}
\expandafter\def\csname r@base-M-noRK-qasper-ci\endcsname{[$-$2.1, +0.1]}
\expandafter\def\csname r@base-M-noRK-qasper-ci95\endcsname{[$-$2.1, +0.1]}
\expandafter\def\csname r@base-M-noRK-qasper-d\endcsname{$-$0.9}
\expandafter\def\csname r@base-M-noRK-qasper-p\endcsname{--}
\expandafter\def\csname r@base-M-noRK-qasper-v\endcsname{n.d.}
\expandafter\def\csname r@base-M-qasper\endcsname{$-$2.2 [$-$3.8, $-$0.7]}
\expandafter\def\csname r@base-M-qasper-ci\endcsname{[$-$3.8, $-$0.7]}
\expandafter\def\csname r@base-M-qasper-ci95\endcsname{[$-$3.8, $-$0.7]}
\expandafter\def\csname r@base-M-qasper-d\endcsname{$-$2.2}
\expandafter\def\csname r@base-M-qasper-p\endcsname{0.006}
\expandafter\def\csname r@base-M-qasper-pperm\endcsname{0.054}
\expandafter\def\csname r@base-M-qasper-v\endcsname{equiv.}
\expandafter\def\csname r@cost-E-vs-TP-in-fs\endcsname{13}
\expandafter\def\csname r@cost-E-vs-TP-in-qasper\endcsname{10}
\expandafter\def\csname r@cost-dict-in-fs\endcsname{19}
\expandafter\def\csname r@cost-dict-in-qasper\endcsname{13}
\expandafter\def\csname r@cost-tp-in-fs\endcsname{3.2}
\expandafter\def\csname r@cost-tp-in-qasper\endcsname{2.2}
\expandafter\def\csname r@crratio-local-fs\endcsname{8.7}
\expandafter\def\csname r@crratio-local-qasper\endcsname{5.8}
\expandafter\def\csname r@crratio-strong-qasper\endcsname{5.8}
\expandafter\def\csname r@ctl-neg\endcsname{6.8}
\expandafter\def\csname r@ctl-pos\endcsname{97.6}
\expandafter\def\csname r@dial-M-TP-E-noRK-fs\endcsname{+4.4 [+2.2, +6.8]}
\expandafter\def\csname r@dial-M-TP-E-noRK-fs-ci\endcsname{[+2.2, +6.8]}
\expandafter\def\csname r@dial-M-TP-E-noRK-fs-ci95\endcsname{[+2.2, +6.8]}
\expandafter\def\csname r@dial-M-TP-E-noRK-fs-d\endcsname{+4.4}
\expandafter\def\csname r@dial-M-TP-E-noRK-fs-p\endcsname{--}
\expandafter\def\csname r@dial-M-TP-E-noRK-fs-rec\endcsname{+1.4 [+0.7, +2.3]}
\expandafter\def\csname r@dial-M-TP-E-noRK-fs-rec-ci\endcsname{[+0.7, +2.3]}
\expandafter\def\csname r@dial-M-TP-E-noRK-fs-rec-ci95\endcsname{[+0.7, +2.3]}
\expandafter\def\csname r@dial-M-TP-E-noRK-fs-rec-d\endcsname{+1.4}
\expandafter\def\csname r@dial-M-TP-E-noRK-fs-rec-p\endcsname{--}
\expandafter\def\csname r@dial-M-TP-E-noRK-fs-rec-v\endcsname{diff.}
\expandafter\def\csname r@dial-M-TP-E-noRK-fs-v\endcsname{diff.}
\expandafter\def\csname r@dial-M-TP-E-noRK-qasper\endcsname{$-$5.6 [$-$8.0, $-$3.4]}
\expandafter\def\csname r@dial-M-TP-E-noRK-qasper-ci\endcsname{[$-$8.0, $-$3.4]}
\expandafter\def\csname r@dial-M-TP-E-noRK-qasper-ci95\endcsname{[$-$8.0, $-$3.4]}
\expandafter\def\csname r@dial-M-TP-E-noRK-qasper-d\endcsname{$-$5.6}
\expandafter\def\csname r@dial-M-TP-E-noRK-qasper-p\endcsname{--}
\expandafter\def\csname r@dial-M-TP-E-noRK-qasper-v\endcsname{diff.}
\expandafter\def\csname r@dial-M-TP-RM-TP-fs\endcsname{+2.3 [+0.6, +4.2]}
\expandafter\def\csname r@dial-M-TP-RM-TP-fs-ci\endcsname{[+0.6, +4.2]}
\expandafter\def\csname r@dial-M-TP-RM-TP-fs-ci95\endcsname{[+0.6, +4.2]}
\expandafter\def\csname r@dial-M-TP-RM-TP-fs-d\endcsname{+2.3}
\expandafter\def\csname r@dial-M-TP-RM-TP-fs-p\endcsname{--}
\expandafter\def\csname r@dial-M-TP-RM-TP-fs-rec\endcsname{+0.8 [+0.1, +1.7]}
\expandafter\def\csname r@dial-M-TP-RM-TP-fs-rec-ci\endcsname{[+0.1, +1.7]}
\expandafter\def\csname r@dial-M-TP-RM-TP-fs-rec-ci95\endcsname{[+0.1, +1.7]}
\expandafter\def\csname r@dial-M-TP-RM-TP-fs-rec-d\endcsname{+0.8}
\expandafter\def\csname r@dial-M-TP-RM-TP-fs-rec-p\endcsname{--}
\expandafter\def\csname r@dial-M-TP-RM-TP-fs-rec-v\endcsname{diff.}
\expandafter\def\csname r@dial-M-TP-RM-TP-fs-v\endcsname{diff.}
\expandafter\def\csname r@dial-M-TP-RM-TP-qasper\endcsname{+2.2 [+0.2, +4.1]}
\expandafter\def\csname r@dial-M-TP-RM-TP-qasper-ci\endcsname{[+0.2, +4.1]}
\expandafter\def\csname r@dial-M-TP-RM-TP-qasper-ci95\endcsname{[+0.2, +4.1]}
\expandafter\def\csname r@dial-M-TP-RM-TP-qasper-d\endcsname{+2.2}
\expandafter\def\csname r@dial-M-TP-RM-TP-qasper-p\endcsname{--}
\expandafter\def\csname r@dial-M-TP-RM-TP-qasper-v\endcsname{diff.}
\expandafter\def\csname r@dial-M-TP-SM-TP-fs\endcsname{+1.9 [$-$0.3, +4.1]}
\expandafter\def\csname r@dial-M-TP-SM-TP-fs-ci\endcsname{[$-$0.3, +4.1]}
\expandafter\def\csname r@dial-M-TP-SM-TP-fs-ci95\endcsname{[$-$0.3, +4.1]}
\expandafter\def\csname r@dial-M-TP-SM-TP-fs-d\endcsname{+1.9}
\expandafter\def\csname r@dial-M-TP-SM-TP-fs-p\endcsname{--}
\expandafter\def\csname r@dial-M-TP-SM-TP-fs-rec\endcsname{+0.5 [$-$0.7, +1.3]}
\expandafter\def\csname r@dial-M-TP-SM-TP-fs-rec-ci\endcsname{[$-$0.7, +1.3]}
\expandafter\def\csname r@dial-M-TP-SM-TP-fs-rec-ci95\endcsname{[$-$0.7, +1.3]}
\expandafter\def\csname r@dial-M-TP-SM-TP-fs-rec-d\endcsname{+0.5}
\expandafter\def\csname r@dial-M-TP-SM-TP-fs-rec-p\endcsname{--}
\expandafter\def\csname r@dial-M-TP-SM-TP-fs-rec-v\endcsname{n.d.}
\expandafter\def\csname r@dial-M-TP-SM-TP-fs-v\endcsname{n.d.}
\expandafter\def\csname r@dial-M-TP-SM-TP-qasper\endcsname{$-$0.0 [$-$2.6, +2.4]}
\expandafter\def\csname r@dial-M-TP-SM-TP-qasper-ci\endcsname{[$-$2.6, +2.4]}
\expandafter\def\csname r@dial-M-TP-SM-TP-qasper-ci95\endcsname{[$-$2.6, +2.4]}
\expandafter\def\csname r@dial-M-TP-SM-TP-qasper-d\endcsname{$-$0.0}
\expandafter\def\csname r@dial-M-TP-SM-TP-qasper-p\endcsname{--}
\expandafter\def\csname r@dial-M-TP-SM-TP-qasper-v\endcsname{n.d.}
\expandafter\def\csname r@dial-RM-TP-E-noRK-fs\endcsname{+2.1 [+0.3, +3.8]}
\expandafter\def\csname r@dial-RM-TP-E-noRK-fs-ci\endcsname{[+0.3, +3.8]}
\expandafter\def\csname r@dial-RM-TP-E-noRK-fs-ci95\endcsname{[+0.3, +3.8]}
\expandafter\def\csname r@dial-RM-TP-E-noRK-fs-d\endcsname{+2.1}
\expandafter\def\csname r@dial-RM-TP-E-noRK-fs-p\endcsname{--}
\expandafter\def\csname r@dial-RM-TP-E-noRK-fs-rec\endcsname{+0.6 [+0.1, +1.2]}
\expandafter\def\csname r@dial-RM-TP-E-noRK-fs-rec-ci\endcsname{[+0.1, +1.2]}
\expandafter\def\csname r@dial-RM-TP-E-noRK-fs-rec-ci95\endcsname{[+0.1, +1.2]}
\expandafter\def\csname r@dial-RM-TP-E-noRK-fs-rec-d\endcsname{+0.6}
\expandafter\def\csname r@dial-RM-TP-E-noRK-fs-rec-p\endcsname{--}
\expandafter\def\csname r@dial-RM-TP-E-noRK-fs-rec-v\endcsname{diff.}
\expandafter\def\csname r@dial-RM-TP-E-noRK-fs-v\endcsname{diff.}
\expandafter\def\csname r@dial-RM-TP-E-noRK-qasper\endcsname{$-$7.8 [$-$9.9, $-$5.9]}
\expandafter\def\csname r@dial-RM-TP-E-noRK-qasper-ci\endcsname{[$-$9.9, $-$5.9]}
\expandafter\def\csname r@dial-RM-TP-E-noRK-qasper-ci95\endcsname{[$-$9.9, $-$5.9]}
\expandafter\def\csname r@dial-RM-TP-E-noRK-qasper-d\endcsname{$-$7.8}
\expandafter\def\csname r@dial-RM-TP-E-noRK-qasper-p\endcsname{--}
\expandafter\def\csname r@dial-RM-TP-E-noRK-qasper-v\endcsname{diff.}
\expandafter\def\csname r@dial-SM-TP-E-noRK-fs\endcsname{+2.5 [+0.5, +4.5]}
\expandafter\def\csname r@dial-SM-TP-E-noRK-fs-ci\endcsname{[+0.5, +4.5]}
\expandafter\def\csname r@dial-SM-TP-E-noRK-fs-ci95\endcsname{[+0.5, +4.5]}
\expandafter\def\csname r@dial-SM-TP-E-noRK-fs-d\endcsname{+2.5}
\expandafter\def\csname r@dial-SM-TP-E-noRK-fs-p\endcsname{--}
\expandafter\def\csname r@dial-SM-TP-E-noRK-fs-rec\endcsname{+0.9 [+0.2, +1.9]}
\expandafter\def\csname r@dial-SM-TP-E-noRK-fs-rec-ci\endcsname{[+0.2, +1.9]}
\expandafter\def\csname r@dial-SM-TP-E-noRK-fs-rec-ci95\endcsname{[+0.2, +1.9]}
\expandafter\def\csname r@dial-SM-TP-E-noRK-fs-rec-d\endcsname{+0.9}
\expandafter\def\csname r@dial-SM-TP-E-noRK-fs-rec-p\endcsname{--}
\expandafter\def\csname r@dial-SM-TP-E-noRK-fs-rec-v\endcsname{diff.}
\expandafter\def\csname r@dial-SM-TP-E-noRK-fs-v\endcsname{diff.}
\expandafter\def\csname r@dial-SM-TP-E-noRK-qasper\endcsname{$-$5.6 [$-$8.2, $-$3.1]}
\expandafter\def\csname r@dial-SM-TP-E-noRK-qasper-ci\endcsname{[$-$8.2, $-$3.1]}
\expandafter\def\csname r@dial-SM-TP-E-noRK-qasper-ci95\endcsname{[$-$8.2, $-$3.1]}
\expandafter\def\csname r@dial-SM-TP-E-noRK-qasper-d\endcsname{$-$5.6}
\expandafter\def\csname r@dial-SM-TP-E-noRK-qasper-p\endcsname{--}
\expandafter\def\csname r@dial-SM-TP-E-noRK-qasper-v\endcsname{diff.}
\expandafter\def\csname r@dial-short\endcsname{44}
\expandafter\def\csname r@f1-qasper-CR\endcsname{38.8}
\expandafter\def\csname r@f1-qasper-CR-strong\endcsname{39.0}
\expandafter\def\csname r@f1-qasper-E\endcsname{39.0}
\expandafter\def\csname r@f1-qasper-E-strong\endcsname{39.1}
\expandafter\def\csname r@f1-qasper-F256t\endcsname{34.2}
\expandafter\def\csname r@f1-qasper-F512c\endcsname{37.8}
\expandafter\def\csname r@f1-qasper-S\endcsname{37.7}
\expandafter\def\csname r@f1-qasper-S+T\endcsname{37.6}
\expandafter\def\csname r@hq3H1-fs\endcsname{+1.0 [$-$1.0, +2.9]}
\expandafter\def\csname r@hq3H1-fs-ci\endcsname{[$-$1.0, +2.9]}
\expandafter\def\csname r@hq3H1-fs-ci95\endcsname{[$-$1.0, +2.9]}
\expandafter\def\csname r@hq3H1-fs-d\endcsname{+1.0}
\expandafter\def\csname r@hq3H1-fs-p\endcsname{--}
\expandafter\def\csname r@hq3H1-fs-v\endcsname{equiv.}
\expandafter\def\csname r@hq3H1-qasper\endcsname{+4.6 [+2.0, +7.1]}
\expandafter\def\csname r@hq3H1-qasper-ci\endcsname{[+2.0, +7.1]}
\expandafter\def\csname r@hq3H1-qasper-ci95\endcsname{[+2.0, +7.1]}
\expandafter\def\csname r@hq3H1-qasper-d\endcsname{+4.6}
\expandafter\def\csname r@hq3H1-qasper-p\endcsname{--}
\expandafter\def\csname r@hq3H1-qasper-v\endcsname{diff.}
\expandafter\def\csname r@judge-failed\endcsname{4}
\expandafter\def\csname r@keys-E-TP-fs\endcsname{13.3}
\expandafter\def\csname r@keys-E-TP-qasper\endcsname{15.3}
\expandafter\def\csname r@keys-E-fs\endcsname{16.2}
\expandafter\def\csname r@keys-E-noRK-fs\endcsname{17.7}
\expandafter\def\csname r@keys-E-noRK-qasper\endcsname{22.6}
\expandafter\def\csname r@keys-E-qasper\endcsname{20.2}
\expandafter\def\csname r@lcE-fs\endcsname{$-$0.9 [$-$5.3, +3.2]}
\expandafter\def\csname r@lcE-fs-ci\endcsname{[$-$5.3, +3.2]}
\expandafter\def\csname r@lcE-fs-ci95\endcsname{[$-$5.3, +3.2]}
\expandafter\def\csname r@lcE-fs-d\endcsname{$-$0.9}
\expandafter\def\csname r@lcE-fs-p\endcsname{--}
\expandafter\def\csname r@lcE-fs-v\endcsname{n.d.}
\expandafter\def\csname r@lcE-qasper\endcsname{+13.6 [+10.2, +17.0]}
\expandafter\def\csname r@lcE-qasper-ci\endcsname{[+10.2, +17.0]}
\expandafter\def\csname r@lcE-qasper-ci95\endcsname{[+10.2, +17.0]}
\expandafter\def\csname r@lcE-qasper-d\endcsname{+13.6}
\expandafter\def\csname r@lcE-qasper-p\endcsname{--}
\expandafter\def\csname r@lcE-qasper-v\endcsname{diff.}
\expandafter\def\csname r@lcS-fs\endcsname{$-$0.5 [$-$4.7, +3.8]}
\expandafter\def\csname r@lcS-fs-ci\endcsname{[$-$4.7, +3.8]}
\expandafter\def\csname r@lcS-fs-ci95\endcsname{[$-$4.7, +3.8]}
\expandafter\def\csname r@lcS-fs-d\endcsname{$-$0.5}
\expandafter\def\csname r@lcS-fs-p\endcsname{--}
\expandafter\def\csname r@lcS-fs-v\endcsname{n.d.}
\expandafter\def\csname r@lcS-qasper\endcsname{$-$11.4 [$-$14.4, $-$8.1]}
\expandafter\def\csname r@lcS-qasper-ci\endcsname{[$-$14.4, $-$8.1]}
\expandafter\def\csname r@lcS-qasper-ci95\endcsname{[$-$14.4, $-$8.1]}
\expandafter\def\csname r@lcS-qasper-d\endcsname{$-$11.4}
\expandafter\def\csname r@lcS-qasper-p\endcsname{--}
\expandafter\def\csname r@lcS-qasper-v\endcsname{diff.}
\expandafter\def\csname r@lcsim-fs-late\endcsname{0.94}
\expandafter\def\csname r@lcsim-fs-n\endcsname{359}
\expandafter\def\csname r@lcsim-fs-plain\endcsname{0.56}
\expandafter\def\csname r@lcsim-qasper-late\endcsname{0.94}
\expandafter\def\csname r@lcsim-qasper-n\endcsname{300}
\expandafter\def\csname r@lcsim-qasper-plain\endcsname{0.45}
\expandafter\def\csname r@len-enr-median\endcsname{179}
\expandafter\def\csname r@len-enr-over512\endcsname{0.5}
\expandafter\def\csname r@len-merged-median\endcsname{193}
\expandafter\def\csname r@len-merged-over512\endcsname{3.8}
\expandafter\def\csname r@links-all-fs\endcsname{94}
\expandafter\def\csname r@links-all-qasper\endcsname{97}
\expandafter\def\csname r@links-ret-fs\endcsname{99}
\expandafter\def\csname r@links-ret-qasper\endcsname{98}
\expandafter\def\csname r@m-fs-CR\endcsname{29.0}
\expandafter\def\csname r@m-fs-E\endcsname{30.8}
\expandafter\def\csname r@m-fs-E(meta+key)\endcsname{30.3}
\expandafter\def\csname r@m-fs-E+AX\endcsname{33.5}
\expandafter\def\csname r@m-fs-E+KX\endcsname{32.0}
\expandafter\def\csname r@m-fs-E+SX\endcsname{31.5}
\expandafter\def\csname r@m-fs-E-noRK\endcsname{29.4}
\expandafter\def\csname r@m-fs-E-strong\endcsname{29.8}
\expandafter\def\csname r@m-fs-F256t\endcsname{29.5}
\expandafter\def\csname r@m-fs-F512c\endcsname{23.6}
\expandafter\def\csname r@m-fs-FL\endcsname{25.1}
\expandafter\def\csname r@m-fs-M\endcsname{31.0}
\expandafter\def\csname r@m-fs-M-TP\endcsname{33.8}
\expandafter\def\csname r@m-fs-M-noRK\endcsname{29.9}
\expandafter\def\csname r@m-fs-PP\endcsname{28.7}
\expandafter\def\csname r@m-fs-RM\endcsname{30.6}
\expandafter\def\csname r@m-fs-S\endcsname{26.7}
\expandafter\def\csname r@m-fs-S+T\endcsname{28.0}
\expandafter\def\csname r@m-fs-SM\endcsname{30.6}
\expandafter\def\csname r@m-fs-bm25-CR\endcsname{23.0}
\expandafter\def\csname r@m-fs-bm25-E\endcsname{25.1}
\expandafter\def\csname r@m-fs-bm25-E-strong\endcsname{24.9}
\expandafter\def\csname r@m-fs-bm25-F256t\endcsname{23.8}
\expandafter\def\csname r@m-fs-bm25-F512c\endcsname{18.8}
\expandafter\def\csname r@m-fs-bm25-FL\endcsname{21.1}
\expandafter\def\csname r@m-fs-bm25-PP\endcsname{23.9}
\expandafter\def\csname r@m-fs-bm25-S\endcsname{22.0}
\expandafter\def\csname r@m-fs-bm25-S+T\endcsname{22.7}
\expandafter\def\csname r@m-fs-hybrid+rerank-CR\endcsname{34.0}
\expandafter\def\csname r@m-fs-hybrid+rerank-E\endcsname{34.9}
\expandafter\def\csname r@m-fs-hybrid+rerank-E-strong\endcsname{35.9}
\expandafter\def\csname r@m-fs-hybrid+rerank-F256t\endcsname{35.1}
\expandafter\def\csname r@m-fs-hybrid+rerank-F512c\endcsname{29.3}
\expandafter\def\csname r@m-fs-hybrid+rerank-FL\endcsname{31.8}
\expandafter\def\csname r@m-fs-hybrid+rerank-PP\endcsname{36.2}
\expandafter\def\csname r@m-fs-hybrid+rerank-S\endcsname{31.2}
\expandafter\def\csname r@m-fs-hybrid+rerank-S+T\endcsname{34.1}
\expandafter\def\csname r@m-fs-hybrid-CR\endcsname{29.0}
\expandafter\def\csname r@m-fs-hybrid-E\endcsname{30.8}
\expandafter\def\csname r@m-fs-hybrid-E-strong\endcsname{29.8}
\expandafter\def\csname r@m-fs-hybrid-F256t\endcsname{29.5}
\expandafter\def\csname r@m-fs-hybrid-F512c\endcsname{23.6}
\expandafter\def\csname r@m-fs-hybrid-FL\endcsname{25.1}
\expandafter\def\csname r@m-fs-hybrid-PP\endcsname{28.7}
\expandafter\def\csname r@m-fs-hybrid-S\endcsname{26.7}
\expandafter\def\csname r@m-fs-hybrid-S+T\endcsname{28.0}
\expandafter\def\csname r@m-fs-hybrid-qwen3-CR\endcsname{32.9}
\expandafter\def\csname r@m-fs-hybrid-qwen3-E\endcsname{33.0}
\expandafter\def\csname r@m-fs-hybrid-qwen3-E-strong\endcsname{33.3}
\expandafter\def\csname r@m-fs-hybrid-qwen3-F256t\endcsname{34.6}
\expandafter\def\csname r@m-fs-hybrid-qwen3-F512c\endcsname{28.2}
\expandafter\def\csname r@m-fs-hybrid-qwen3-FL\endcsname{30.2}
\expandafter\def\csname r@m-fs-hybrid-qwen3-PP\endcsname{32.6}
\expandafter\def\csname r@m-fs-hybrid-qwen3-S\endcsname{31.1}
\expandafter\def\csname r@m-fs-hybrid-qwen3-S+T\endcsname{32.0}
\expandafter\def\csname r@m-fs-jina-CR\endcsname{33.7}
\expandafter\def\csname r@m-fs-jina-E\endcsname{32.2}
\expandafter\def\csname r@m-fs-jina-LC-S\endcsname{33.2}
\expandafter\def\csname r@m-fs-jina-S\endcsname{33.7}
\expandafter\def\csname r@m-fs-jina-S+T\endcsname{33.6}
\expandafter\def\csname r@m-fs-mxbai-CR\endcsname{31.6}
\expandafter\def\csname r@m-fs-mxbai-E\endcsname{32.2}
\expandafter\def\csname r@m-fs-mxbai-E-strong\endcsname{31.5}
\expandafter\def\csname r@m-fs-mxbai-F256t\endcsname{30.8}
\expandafter\def\csname r@m-fs-mxbai-F512c\endcsname{27.2}
\expandafter\def\csname r@m-fs-mxbai-FL\endcsname{28.5}
\expandafter\def\csname r@m-fs-mxbai-PP\endcsname{32.8}
\expandafter\def\csname r@m-fs-mxbai-S\endcsname{30.3}
\expandafter\def\csname r@m-fs-mxbai-S+T\endcsname{32.2}
\expandafter\def\csname r@m-fs-nomic-CR\endcsname{27.2}
\expandafter\def\csname r@m-fs-nomic-E\endcsname{29.5}
\expandafter\def\csname r@m-fs-nomic-E-strong\endcsname{29.1}
\expandafter\def\csname r@m-fs-nomic-F256t\endcsname{27.8}
\expandafter\def\csname r@m-fs-nomic-F512c\endcsname{22.4}
\expandafter\def\csname r@m-fs-nomic-FL\endcsname{22.7}
\expandafter\def\csname r@m-fs-nomic-PP\endcsname{27.5}
\expandafter\def\csname r@m-fs-nomic-S\endcsname{24.2}
\expandafter\def\csname r@m-fs-nomic-S+T\endcsname{26.9}
\expandafter\def\csname r@m-fs-qwen3-CR\endcsname{35.4}
\expandafter\def\csname r@m-fs-qwen3-E\endcsname{34.8}
\expandafter\def\csname r@m-fs-qwen3-E-strong\endcsname{35.7}
\expandafter\def\csname r@m-fs-qwen3-F256t\endcsname{34.5}
\expandafter\def\csname r@m-fs-qwen3-F512c\endcsname{29.4}
\expandafter\def\csname r@m-fs-qwen3-FL\endcsname{31.8}
\expandafter\def\csname r@m-fs-qwen3-PP\endcsname{34.5}
\expandafter\def\csname r@m-fs-qwen3-S\endcsname{31.9}
\expandafter\def\csname r@m-fs-qwen3-S+T\endcsname{34.6}
\expandafter\def\csname r@m-qasper-CR\endcsname{46.1}
\expandafter\def\csname r@m-qasper-CR-strong\endcsname{47.7}
\expandafter\def\csname r@m-qasper-E\endcsname{48.1}
\expandafter\def\csname r@m-qasper-E(meta+key)\endcsname{48.2}
\expandafter\def\csname r@m-qasper-E+AX\endcsname{40.3}
\expandafter\def\csname r@m-qasper-E+KX\endcsname{38.2}
\expandafter\def\csname r@m-qasper-E+SX\endcsname{44.3}
\expandafter\def\csname r@m-qasper-E-noRK\endcsname{47.5}
\expandafter\def\csname r@m-qasper-E-strong\endcsname{49.3}
\expandafter\def\csname r@m-qasper-F256t\endcsname{35.0}
\expandafter\def\csname r@m-qasper-F512c\endcsname{35.0}
\expandafter\def\csname r@m-qasper-FL\endcsname{34.3}
\expandafter\def\csname r@m-qasper-M\endcsname{45.9}
\expandafter\def\csname r@m-qasper-M-TP\endcsname{41.9}
\expandafter\def\csname r@m-qasper-M-noRK\endcsname{46.6}
\expandafter\def\csname r@m-qasper-PF\endcsname{48.3}
\expandafter\def\csname r@m-qasper-PP\endcsname{37.2}
\expandafter\def\csname r@m-qasper-RM\endcsname{44.1}
\expandafter\def\csname r@m-qasper-S\endcsname{42.5}
\expandafter\def\csname r@m-qasper-S+T\endcsname{42.7}
\expandafter\def\csname r@m-qasper-SM\endcsname{46.0}
\expandafter\def\csname r@m-qasper-bm25-CR\endcsname{33.6}
\expandafter\def\csname r@m-qasper-bm25-CR-strong\endcsname{33.7}
\expandafter\def\csname r@m-qasper-bm25-E\endcsname{38.6}
\expandafter\def\csname r@m-qasper-bm25-E-strong\endcsname{39.9}
\expandafter\def\csname r@m-qasper-bm25-F256t\endcsname{24.1}
\expandafter\def\csname r@m-qasper-bm25-F512c\endcsname{26.8}
\expandafter\def\csname r@m-qasper-bm25-FL\endcsname{23.8}
\expandafter\def\csname r@m-qasper-bm25-PP\endcsname{26.8}
\expandafter\def\csname r@m-qasper-bm25-S\endcsname{29.7}
\expandafter\def\csname r@m-qasper-bm25-S+T\endcsname{29.9}
\expandafter\def\csname r@m-qasper-hybrid+rerank-CR\endcsname{54.5}
\expandafter\def\csname r@m-qasper-hybrid+rerank-CR-strong\endcsname{57.0}
\expandafter\def\csname r@m-qasper-hybrid+rerank-E\endcsname{54.9}
\expandafter\def\csname r@m-qasper-hybrid+rerank-E-strong\endcsname{57.0}
\expandafter\def\csname r@m-qasper-hybrid+rerank-F256t\endcsname{43.6}
\expandafter\def\csname r@m-qasper-hybrid+rerank-F512c\endcsname{44.0}
\expandafter\def\csname r@m-qasper-hybrid+rerank-FL\endcsname{42.7}
\expandafter\def\csname r@m-qasper-hybrid+rerank-PP\endcsname{47.3}
\expandafter\def\csname r@m-qasper-hybrid+rerank-S\endcsname{53.0}
\expandafter\def\csname r@m-qasper-hybrid+rerank-S+T\endcsname{54.5}
\expandafter\def\csname r@m-qasper-hybrid-CR\endcsname{46.1}
\expandafter\def\csname r@m-qasper-hybrid-CR-strong\endcsname{47.7}
\expandafter\def\csname r@m-qasper-hybrid-E\endcsname{48.1}
\expandafter\def\csname r@m-qasper-hybrid-E-strong\endcsname{49.3}
\expandafter\def\csname r@m-qasper-hybrid-F256t\endcsname{35.0}
\expandafter\def\csname r@m-qasper-hybrid-F512c\endcsname{35.0}
\expandafter\def\csname r@m-qasper-hybrid-FL\endcsname{34.3}
\expandafter\def\csname r@m-qasper-hybrid-PP\endcsname{37.2}
\expandafter\def\csname r@m-qasper-hybrid-S\endcsname{42.5}
\expandafter\def\csname r@m-qasper-hybrid-S+T\endcsname{42.7}
\expandafter\def\csname r@m-qasper-hybrid-qwen3-CR\endcsname{47.7}
\expandafter\def\csname r@m-qasper-hybrid-qwen3-CR-strong\endcsname{48.4}
\expandafter\def\csname r@m-qasper-hybrid-qwen3-E\endcsname{49.7}
\expandafter\def\csname r@m-qasper-hybrid-qwen3-E-strong\endcsname{51.4}
\expandafter\def\csname r@m-qasper-hybrid-qwen3-F256t\endcsname{38.3}
\expandafter\def\csname r@m-qasper-hybrid-qwen3-F512c\endcsname{36.9}
\expandafter\def\csname r@m-qasper-hybrid-qwen3-FL\endcsname{36.1}
\expandafter\def\csname r@m-qasper-hybrid-qwen3-PP\endcsname{39.7}
\expandafter\def\csname r@m-qasper-hybrid-qwen3-S\endcsname{44.0}
\expandafter\def\csname r@m-qasper-hybrid-qwen3-S+T\endcsname{45.2}
\expandafter\def\csname r@m-qasper-jina-CR\endcsname{50.7}
\expandafter\def\csname r@m-qasper-jina-E\endcsname{48.7}
\expandafter\def\csname r@m-qasper-jina-LC-S\endcsname{35.1}
\expandafter\def\csname r@m-qasper-jina-S\endcsname{46.4}
\expandafter\def\csname r@m-qasper-jina-S+T\endcsname{45.9}
\expandafter\def\csname r@m-qasper-mxbai-CR\endcsname{46.5}
\expandafter\def\csname r@m-qasper-mxbai-CR-strong\endcsname{45.7}
\expandafter\def\csname r@m-qasper-mxbai-E\endcsname{47.9}
\expandafter\def\csname r@m-qasper-mxbai-E-strong\endcsname{49.4}
\expandafter\def\csname r@m-qasper-mxbai-F256t\endcsname{35.5}
\expandafter\def\csname r@m-qasper-mxbai-F512c\endcsname{36.4}
\expandafter\def\csname r@m-qasper-mxbai-FL\endcsname{35.7}
\expandafter\def\csname r@m-qasper-mxbai-PP\endcsname{37.9}
\expandafter\def\csname r@m-qasper-mxbai-S\endcsname{44.4}
\expandafter\def\csname r@m-qasper-mxbai-S+T\endcsname{47.2}
\expandafter\def\csname r@m-qasper-nomic-CR\endcsname{49.9}
\expandafter\def\csname r@m-qasper-nomic-CR-strong\endcsname{51.2}
\expandafter\def\csname r@m-qasper-nomic-E\endcsname{48.6}
\expandafter\def\csname r@m-qasper-nomic-E-strong\endcsname{51.4}
\expandafter\def\csname r@m-qasper-nomic-F256t\endcsname{37.5}
\expandafter\def\csname r@m-qasper-nomic-F512c\endcsname{38.1}
\expandafter\def\csname r@m-qasper-nomic-FL\endcsname{38.4}
\expandafter\def\csname r@m-qasper-nomic-PP\endcsname{39.7}
\expandafter\def\csname r@m-qasper-nomic-S\endcsname{47.9}
\expandafter\def\csname r@m-qasper-nomic-S+T\endcsname{47.8}
\expandafter\def\csname r@m-qasper-qwen3-CR\endcsname{55.7}
\expandafter\def\csname r@m-qasper-qwen3-CR-strong\endcsname{56.1}
\expandafter\def\csname r@m-qasper-qwen3-E\endcsname{55.1}
\expandafter\def\csname r@m-qasper-qwen3-E-strong\endcsname{54.6}
\expandafter\def\csname r@m-qasper-qwen3-F256t\endcsname{44.6}
\expandafter\def\csname r@m-qasper-qwen3-F512c\endcsname{43.2}
\expandafter\def\csname r@m-qasper-qwen3-FL\endcsname{42.2}
\expandafter\def\csname r@m-qasper-qwen3-PP\endcsname{48.1}
\expandafter\def\csname r@m-qasper-qwen3-S\endcsname{52.0}
\expandafter\def\csname r@m-qasper-qwen3-S+T\endcsname{53.6}
\expandafter\def\csname r@merges-E-TP-fs\endcsname{1,724}
\expandafter\def\csname r@merges-E-TP-qasper\endcsname{2,029}
\expandafter\def\csname r@merges-E-fs\endcsname{853}
\expandafter\def\csname r@merges-E-noRK-fs\endcsname{328}
\expandafter\def\csname r@merges-E-noRK-qasper\endcsname{390}
\expandafter\def\csname r@merges-E-qasper\endcsname{995}
\expandafter\def\csname r@nug-CR\endcsname{42.4}
\expandafter\def\csname r@nug-CR-SpT\endcsname{$-$1.3 [$-$5.2, +2.7]}
\expandafter\def\csname r@nug-CR-SpT-ci\endcsname{[$-$5.2, +2.7]}
\expandafter\def\csname r@nug-CR-SpT-ci95\endcsname{[$-$5.2, +2.7]}
\expandafter\def\csname r@nug-CR-SpT-d\endcsname{$-$1.3}
\expandafter\def\csname r@nug-CR-SpT-p\endcsname{--}
\expandafter\def\csname r@nug-CR-SpT-v\endcsname{n.d.}
\expandafter\def\csname r@nug-E\endcsname{44.2}
\expandafter\def\csname r@nug-E-CR\endcsname{+1.8 [$-$1.7, +5.3]}
\expandafter\def\csname r@nug-E-CR-ci\endcsname{[$-$1.7, +5.3]}
\expandafter\def\csname r@nug-E-CR-ci95\endcsname{[$-$1.7, +5.3]}
\expandafter\def\csname r@nug-E-CR-d\endcsname{+1.8}
\expandafter\def\csname r@nug-E-CR-p\endcsname{--}
\expandafter\def\csname r@nug-E-CR-v\endcsname{equiv.}
\expandafter\def\csname r@nug-E-SpT\endcsname{+0.5 [$-$3.3, +4.4]}
\expandafter\def\csname r@nug-E-SpT-ci\endcsname{[$-$3.3, +4.4]}
\expandafter\def\csname r@nug-E-SpT-ci95\endcsname{[$-$3.3, +4.4]}
\expandafter\def\csname r@nug-E-SpT-d\endcsname{+0.5}
\expandafter\def\csname r@nug-E-SpT-p\endcsname{--}
\expandafter\def\csname r@nug-E-SpT-v\endcsname{equiv.}
\expandafter\def\csname r@nug-E-strong\endcsname{45.4}
\expandafter\def\csname r@nug-E-strong-E\endcsname{+1.3 [$-$2.3, +5.0]}
\expandafter\def\csname r@nug-E-strong-E-ci\endcsname{[$-$2.3, +5.0]}
\expandafter\def\csname r@nug-E-strong-E-ci95\endcsname{[$-$2.3, +5.0]}
\expandafter\def\csname r@nug-E-strong-E-d\endcsname{+1.3}
\expandafter\def\csname r@nug-E-strong-E-p\endcsname{--}
\expandafter\def\csname r@nug-E-strong-E-v\endcsname{n.d.}
\expandafter\def\csname r@nug-F256t\endcsname{41.0}
\expandafter\def\csname r@nug-F512c\endcsname{41.0}
\expandafter\def\csname r@nug-S\endcsname{42.4}
\expandafter\def\csname r@nug-S+T\endcsname{43.7}
\expandafter\def\csname r@nug-S-F256t\endcsname{+1.5 [$-$2.7, +5.7]}
\expandafter\def\csname r@nug-S-F256t-ci\endcsname{[$-$2.7, +5.7]}
\expandafter\def\csname r@nug-S-F256t-ci95\endcsname{[$-$2.7, +5.7]}
\expandafter\def\csname r@nug-S-F256t-d\endcsname{+1.5}
\expandafter\def\csname r@nug-S-F256t-p\endcsname{--}
\expandafter\def\csname r@nug-S-F256t-v\endcsname{n.d.}
\expandafter\def\csname r@nug-S-F512c\endcsname{+1.4 [$-$2.9, +5.8]}
\expandafter\def\csname r@nug-S-F512c-ci\endcsname{[$-$2.9, +5.8]}
\expandafter\def\csname r@nug-S-F512c-ci95\endcsname{[$-$2.9, +5.8]}
\expandafter\def\csname r@nug-S-F512c-d\endcsname{+1.4}
\expandafter\def\csname r@nug-S-F512c-p\endcsname{--}
\expandafter\def\csname r@nug-S-F512c-v\endcsname{n.d.}
\expandafter\def\csname r@pf-calls-ratio\endcsname{4.0}
\expandafter\def\csname r@pf-in-ratio\endcsname{1.60}
\expandafter\def\csname r@pf-out-ratio\endcsname{0.77}
\expandafter\def\csname r@q3H1-fs\endcsname{+0.3 [$-$1.4, +2.0]}
\expandafter\def\csname r@q3H1-fs-ci\endcsname{[$-$1.4, +2.0]}
\expandafter\def\csname r@q3H1-fs-ci95\endcsname{[$-$1.4, +2.0]}
\expandafter\def\csname r@q3H1-fs-d\endcsname{+0.3}
\expandafter\def\csname r@q3H1-fs-p\endcsname{--}
\expandafter\def\csname r@q3H1-fs-v\endcsname{equiv.}
\expandafter\def\csname r@q3H1-qasper\endcsname{+1.5 [$-$1.0, +3.9]}
\expandafter\def\csname r@q3H1-qasper-ci\endcsname{[$-$1.0, +3.9]}
\expandafter\def\csname r@q3H1-qasper-ci95\endcsname{[$-$1.0, +3.9]}
\expandafter\def\csname r@q3H1-qasper-d\endcsname{+1.5}
\expandafter\def\csname r@q3H1-qasper-p\endcsname{--}
\expandafter\def\csname r@q3H1-qasper-v\endcsname{equiv.}
\expandafter\def\csname r@reuse-E-TP-fs\endcsname{28.6}
\expandafter\def\csname r@reuse-E-TP-qasper\endcsname{36.3}
\expandafter\def\csname r@reuse-E-fs\endcsname{13.2}
\expandafter\def\csname r@reuse-E-noRK-fs\endcsname{5.1}
\expandafter\def\csname r@reuse-E-noRK-qasper\endcsname{6.1}
\expandafter\def\csname r@reuse-E-qasper\endcsname{16.2}
\expandafter\def\csname r@rrH1-fs\endcsname{+0.8 [$-$1.4, +3.0]}
\expandafter\def\csname r@rrH1-fs-ci\endcsname{[$-$1.4, +3.0]}
\expandafter\def\csname r@rrH1-fs-ci95\endcsname{[$-$1.4, +3.0]}
\expandafter\def\csname r@rrH1-fs-d\endcsname{+0.8}
\expandafter\def\csname r@rrH1-fs-p\endcsname{--}
\expandafter\def\csname r@rrH1-fs-v\endcsname{equiv.}
\expandafter\def\csname r@rrH1-qasper\endcsname{+0.4 [$-$1.7, +2.5]}
\expandafter\def\csname r@rrH1-qasper-ci\endcsname{[$-$1.7, +2.5]}
\expandafter\def\csname r@rrH1-qasper-ci95\endcsname{[$-$1.7, +2.5]}
\expandafter\def\csname r@rrH1-qasper-d\endcsname{+0.4}
\expandafter\def\csname r@rrH1-qasper-p\endcsname{--}
\expandafter\def\csname r@rrH1-qasper-v\endcsname{equiv.}
\expandafter\def\csname r@rrH2-fs\endcsname{+0.9 [$-$1.4, +3.5]}
\expandafter\def\csname r@rrH2-fs-ci\endcsname{[$-$1.4, +3.5]}
\expandafter\def\csname r@rrH2-fs-ci95\endcsname{[$-$1.4, +3.5]}
\expandafter\def\csname r@rrH2-fs-d\endcsname{+0.9}
\expandafter\def\csname r@rrH2-fs-p\endcsname{--}
\expandafter\def\csname r@rrH2-fs-v\endcsname{equiv.}
\expandafter\def\csname r@rrH2-qasper\endcsname{+0.3 [$-$1.9, +2.5]}
\expandafter\def\csname r@rrH2-qasper-ci\endcsname{[$-$1.9, +2.5]}
\expandafter\def\csname r@rrH2-qasper-ci95\endcsname{[$-$1.9, +2.5]}
\expandafter\def\csname r@rrH2-qasper-d\endcsname{+0.3}
\expandafter\def\csname r@rrH2-qasper-p\endcsname{--}
\expandafter\def\csname r@rrH2-qasper-v\endcsname{equiv.}
\expandafter\def\csname r@scale-E\endcsname{44.2}
\expandafter\def\csname r@scale-E-S+T\endcsname{$-$1.8 [$-$10.4, +6.2]}
\expandafter\def\csname r@scale-E-S+T-ci\endcsname{[$-$10.4, +6.2]}
\expandafter\def\csname r@scale-E-S+T-ci95\endcsname{[$-$10.4, +6.2]}
\expandafter\def\csname r@scale-E-S+T-d\endcsname{$-$1.8}
\expandafter\def\csname r@scale-E-S+T-p\endcsname{--}
\expandafter\def\csname r@scale-E-S+T-v\endcsname{n.d.}
\expandafter\def\csname r@scale-E-qwen235b\endcsname{53.5}
\expandafter\def\csname r@scale-E-qwen235b-E\endcsname{+9.3 [$-$0.1, +18.2]}
\expandafter\def\csname r@scale-E-qwen235b-E-ci\endcsname{[$-$0.1, +18.2]}
\expandafter\def\csname r@scale-E-qwen235b-E-ci95\endcsname{[$-$0.1, +18.2]}
\expandafter\def\csname r@scale-E-qwen235b-E-d\endcsname{+9.3}
\expandafter\def\csname r@scale-E-qwen235b-E-p\endcsname{--}
\expandafter\def\csname r@scale-E-qwen235b-E-strong\endcsname{+8.7 [$-$1.6, +20.8]}
\expandafter\def\csname r@scale-E-qwen235b-E-strong-ci\endcsname{[$-$1.6, +20.8]}
\expandafter\def\csname r@scale-E-qwen235b-E-strong-ci95\endcsname{[$-$1.6, +20.8]}
\expandafter\def\csname r@scale-E-qwen235b-E-strong-d\endcsname{+8.7}
\expandafter\def\csname r@scale-E-qwen235b-E-strong-p\endcsname{--}
\expandafter\def\csname r@scale-E-qwen235b-E-strong-v\endcsname{n.d.}
\expandafter\def\csname r@scale-E-qwen235b-E-v\endcsname{n.d.}
\expandafter\def\csname r@scale-E-qwen235b-S+T\endcsname{+7.5 [$-$0.0, +15.3]}
\expandafter\def\csname r@scale-E-qwen235b-S+T-ci\endcsname{[$-$0.0, +15.3]}
\expandafter\def\csname r@scale-E-qwen235b-S+T-ci95\endcsname{[$-$0.0, +15.3]}
\expandafter\def\csname r@scale-E-qwen235b-S+T-d\endcsname{+7.5}
\expandafter\def\csname r@scale-E-qwen235b-S+T-p\endcsname{--}
\expandafter\def\csname r@scale-E-qwen235b-S+T-v\endcsname{n.d.}
\expandafter\def\csname r@scale-E-strong\endcsname{44.8}
\expandafter\def\csname r@scale-E-strong-E\endcsname{+0.6 [$-$10.7, +8.5]}
\expandafter\def\csname r@scale-E-strong-E-ci\endcsname{[$-$10.7, +8.5]}
\expandafter\def\csname r@scale-E-strong-E-ci95\endcsname{[$-$10.7, +8.5]}
\expandafter\def\csname r@scale-E-strong-E-d\endcsname{+0.6}
\expandafter\def\csname r@scale-E-strong-E-p\endcsname{--}
\expandafter\def\csname r@scale-E-strong-E-v\endcsname{n.d.}
\expandafter\def\csname r@scale-S+T\endcsname{46.0}
\expandafter\def\csname r@scale-n\endcsname{23}
\expandafter\def\csname r@spend\endcsname{3.71}
\expandafter\def\csname r@tok-local-cr-fs-in\endcsname{62.1M}
\expandafter\def\csname r@tok-local-cr-fs-outpercall\endcsname{48}
\expandafter\def\csname r@tok-local-cr-fs-percall\endcsname{8,813}
\expandafter\def\csname r@tok-local-cr-qasper-in\endcsname{42.5M}
\expandafter\def\csname r@tok-local-cr-qasper-outpercall\endcsname{60}
\expandafter\def\csname r@tok-local-cr-qasper-percall\endcsname{5,885}
\expandafter\def\csname r@tok-local-enr-fs-in\endcsname{7.2M}
\expandafter\def\csname r@tok-local-enr-fs-outpercall\endcsname{172}
\expandafter\def\csname r@tok-local-enr-fs-percall\endcsname{1,016}
\expandafter\def\csname r@tok-local-enr-qasper-in\endcsname{7.3M}
\expandafter\def\csname r@tok-local-enr-qasper-outpercall\endcsname{190}
\expandafter\def\csname r@tok-local-enr-qasper-percall\endcsname{1,015}
\expandafter\def\csname r@tok-strong-cr-qasper-in\endcsname{45.2M}
\expandafter\def\csname r@tok-strong-cr-qasper-outpercall\endcsname{118}
\expandafter\def\csname r@tok-strong-cr-qasper-percall\endcsname{6,263}
\expandafter\def\csname r@tok-strong-enr-fs-in\endcsname{7.6M}
\expandafter\def\csname r@tok-strong-enr-fs-outpercall\endcsname{413}
\expandafter\def\csname r@tok-strong-enr-fs-percall\endcsname{1,073}
\expandafter\def\csname r@tok-strong-enr-qasper-in\endcsname{7.8M}
\expandafter\def\csname r@tok-strong-enr-qasper-outpercall\endcsname{476}
\expandafter\def\csname r@tok-strong-enr-qasper-percall\endcsname{1,081}
\expandafter\def\csname r@tp-failed-fs\endcsname{10}
\expandafter\def\csname r@tp-failed-qasper\endcsname{1}
\expandafter\def\csname r@usd-cr-qasper\endcsname{1.82}
\expandafter\def\csname r@usd-enr-fs\endcsname{0.78}
\expandafter\def\csname r@usd-enr-qasper\endcsname{0.87}
\expandafter\def\csname r@usdpercall-cr-qasper\endcsname{252}
\expandafter\def\csname r@usdpercall-enr-fs\endcsname{110}
\expandafter\def\csname r@usdpercall-enr-qasper\endcsname{121}
\makeatother

